Learning with Muscles: Benefits for Data-Efficiency and Robustness in Anthropomorphic Tasks

Humans are able to outperform robots in terms of robustness, versatility, and learning of new tasks in a wide variety of movements. We hypothesize that highly nonlinear muscle dynamics play a large role in providing inherent stability, which is favorable to learning. While recent advances have been made in applying modern learning techniques to muscle-actuated systems both in simulation as well as in robotics, so far, no detailed analysis has been performed to show the benefits of muscles when learning from scratch. Our study closes this gap and showcases the potential of muscle actuators for core robotics challenges in terms of data-efficiency, hyperparameter sensitivity, and robustness.

==> figures/arm26_reaching_hyperparameter_sigmaanalysis_c005_onlyaxis.tex <==
\begin{axis}[%
name =ax3,
scaled y ticks=base 10:\Factor,
at={(ax2.south east)},
xlabel near ticks, ylabel near ticks,
xshift=1.2cm,
width=0.647\figW,
height=\figH,
scale only axis,
xmin=0,
xmax=100,
xtick={  0,  20,  40,  60,  80, 100},
xlabel style={font=\color{white!15!black}},
xlabel={generations},
ymode=log,
ymin=280,
ymax=2500,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={cost},
axis background/.style={fill=white},
title={c = 0.05 s},
legend style={at={(1.03,0.5)}, anchor=west, legend cell align=left, align=left, draw=white!15!black}
]

\addplot[area legend, draw=none, fill=mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	983.408809246568\\
2	963.68014721135\\
3	948.581305801999\\
4	929.518771103599\\
5	915.257457279405\\
6	894.299328386004\\
7	865.098436781494\\
8	848.560520634739\\
9	823.813869877298\\
10	796.101475555287\\
11	767.292597180797\\
12	747.779910120003\\
13	727.342730494041\\
14	690.008901823186\\
15	671.336726074325\\
16	635.453313124292\\
17	619.394504165648\\
18	587.202257779995\\
19	572.453264382456\\
20	557.845860756486\\
21	529.703802592844\\
22	519.245975463718\\
23	497.018088606702\\
24	465.717013717401\\
25	446.923045597944\\
26	420.286651413607\\
27	407.726846361541\\
28	386.536495829086\\
29	371.830885519474\\
30	354.169923695433\\
31	338.860850451809\\
32	332.131179739378\\
33	329.297859313405\\
34	326.36100522812\\
35	326.954378095597\\
36	327.027979121566\\
37	323.0890958591\\
38	323.0890958591\\
39	322.448495293344\\
40	322.760282730235\\
41	321.704707549839\\
42	319.033565995314\\
43	319.033565995314\\
44	319.033565995314\\
45	317.881590525082\\
46	316.039371575143\\
47	316.039371575143\\
48	316.209989486683\\
49	316.209989486683\\
50	316.209989486683\\
51	316.209989486683\\
52	315.109008767046\\
53	314.817093980282\\
54	314.817093980282\\
55	314.446168895118\\
56	314.364096367651\\
57	314.580192303856\\
58	311.373577920061\\
59	309.903601368996\\
60	310.511090476109\\
61	310.131154468234\\
62	310.086349174439\\
63	309.120341642475\\
64	305.811435116366\\
65	305.811435116366\\
66	305.683577912636\\
67	304.482533114574\\
68	304.482533114574\\
69	304.482533114574\\
70	304.482533114574\\
71	304.482533114574\\
72	304.482533114574\\
73	304.482533114574\\
74	305.569551079389\\
75	305.569551079389\\
76	305.687580795526\\
77	305.687580795526\\
78	305.687580795526\\
79	306.06519464192\\
80	306.06519464192\\
81	306.06519464192\\
82	304.896294512179\\
83	305.128176916027\\
84	305.128176916027\\
85	305.337590662223\\
86	305.337590662223\\
87	305.337590662223\\
88	305.337590662223\\
89	305.337590662223\\
90	305.337590662223\\
91	305.337590662223\\
92	305.454781052982\\
93	305.40940485951\\
94	305.27137386499\\
95	305.27137386499\\
96	304.809611296021\\
97	304.809611296021\\
98	304.809928783123\\
99	304.7831970641\\
100	304.549754572925\\
100	315.463491151597\\
99	315.573354962036\\
98	315.588039513949\\
97	315.589707078044\\
96	315.589707078044\\
95	315.716906671908\\
94	315.716906671908\\
93	315.756626321648\\
92	316.665479049276\\
91	318.042661016249\\
90	318.042661016249\\
89	318.042661016249\\
88	318.042661016249\\
87	318.042661016249\\
86	318.042661016249\\
85	318.042661016249\\
84	320.378358868779\\
83	320.378358868779\\
82	323.273915508578\\
81	323.644701742594\\
80	323.644701742594\\
79	323.644701742594\\
78	326.730922290144\\
77	326.730922290144\\
76	326.730922290144\\
75	327.277983849319\\
74	327.277983849319\\
73	331.657546904387\\
72	331.657546904387\\
71	331.657546904387\\
70	331.657546904387\\
69	331.657546904387\\
68	331.657546904387\\
67	331.657546904387\\
66	332.313509261391\\
65	332.409903012913\\
64	332.409903012913\\
63	333.328321556851\\
62	334.005711373698\\
61	334.047737014641\\
60	334.53302246705\\
59	338.130746128307\\
58	341.769045478456\\
57	342.974027017539\\
56	346.955507770261\\
55	348.058039974397\\
54	350.0794006766\\
53	350.0794006766\\
52	350.06411184368\\
51	350.610107590153\\
50	350.610107590153\\
49	350.610107590153\\
48	350.610107590153\\
47	352.719152241662\\
46	352.719152241662\\
45	352.650893289839\\
44	355.833156596519\\
43	355.833156596519\\
42	355.833156596519\\
41	355.783552228516\\
40	355.83937315658\\
39	365.556687079539\\
38	365.599963436183\\
37	365.599963436183\\
36	377.063771547892\\
35	377.403201468668\\
34	380.016405489559\\
33	385.237453037843\\
32	389.352043210099\\
31	397.908934169274\\
30	404.587637857353\\
29	434.893668174185\\
28	462.028178068858\\
27	485.111275393491\\
26	505.072588617434\\
25	532.900330050372\\
24	582.660704213071\\
23	599.272885156631\\
22	622.89959852275\\
21	651.19039072197\\
20	672.018991988861\\
19	704.308496612997\\
18	724.328647104833\\
17	776.132048478483\\
16	815.831695455343\\
15	849.060993267786\\
14	864.655124811764\\
13	883.268506630806\\
12	916.663516245262\\
11	930.528179423127\\
10	954.064318680108\\
9	971.748660456978\\
8	981.647803113023\\
7	1016.88304445214\\
6	1035.46661890878\\
5	1047.54568895479\\
4	1068.10669887765\\
3	1081.98570487579\\
2	1105.6549538673\\
1	1124.79990721244\\
}--cycle;
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	1054\\
2	1035\\
3	1015\\
4	999\\
5	981\\
6	965\\
7	941\\
8	915\\
9	898\\
10	875\\
11	849\\
12	832\\
13	805\\
14	777\\
15	760\\
16	726\\
17	698\\
18	656\\
19	638\\
20	615\\
21	590\\
22	571\\
23	548\\
24	524\\
25	490\\
26	463\\
27	446\\
28	424\\
29	403\\
30	379\\
31	368\\
32	361\\
33	357\\
34	353\\
35	352\\
36	352\\
37	344\\
38	344\\
39	344\\
40	339\\
41	339\\
42	337\\
43	337\\
44	337\\
45	335\\
46	334\\
47	334\\
48	333\\
49	333\\
50	333\\
51	333\\
52	333\\
53	332\\
54	332\\
55	331\\
56	331\\
57	329\\
58	327\\
59	324\\
60	323\\
61	322\\
62	322\\
63	321\\
64	319\\
65	319\\
66	319\\
67	318\\
68	318\\
69	318\\
70	318\\
71	318\\
72	318\\
73	318\\
74	316\\
75	316\\
76	316\\
77	316\\
78	316\\
79	315\\
80	315\\
81	315\\
82	314\\
83	313\\
84	313\\
85	312\\
86	312\\
87	312\\
88	312\\
89	312\\
90	312\\
91	312\\
92	311\\
93	311\\
94	310\\
95	310\\
96	310\\
97	310\\
98	310\\
99	310\\
100	310\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.05}$}


\addplot[area legend, draw=none, fill=red!50!mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	942.431299442678\\
2	927.713091846125\\
3	892.786465190705\\
4	853.683648900448\\
5	812.478200541257\\
6	771.238077972228\\
7	722.802316950293\\
8	698.881722902924\\
9	653.955776695597\\
10	632.141629677727\\
11	588.225797290225\\
12	573.410142702837\\
13	551.407240595421\\
14	537.938711435625\\
15	491.118144958107\\
16	457.797891071158\\
17	441.186673434634\\
18	430.781836804113\\
19	408.884474469483\\
20	401.456876344459\\
21	385.664905545617\\
22	379.179863791793\\
23	366.333020483523\\
24	365.790300880162\\
25	355.823719061216\\
26	343.484671786849\\
27	343.016738999502\\
28	335.872524829867\\
29	334.283253690994\\
30	333.504987626602\\
31	334.156297850529\\
32	333.601123949253\\
33	332.827105817262\\
34	330.867621795974\\
35	325.857500840199\\
36	325.406824148163\\
37	325.442334358907\\
38	325.442334358907\\
39	323.738697447779\\
40	322.915385909587\\
41	323.273543139044\\
42	321.822290223521\\
43	320.066699936302\\
44	320.066699936302\\
45	320.066699936302\\
46	320.066699936302\\
47	318.965650191582\\
48	318.104889179373\\
49	316.720297188465\\
50	317.208980093678\\
51	317.208980093678\\
52	317.255917685927\\
53	316.727780069971\\
54	314.528922176991\\
55	314.528922176991\\
56	314.528922176991\\
57	314.528922176991\\
58	314.333573372499\\
59	313.325420573022\\
60	313.325420573022\\
61	313.238736282799\\
62	312.88430023448\\
63	312.673970208639\\
64	311.55843721972\\
65	311.383049298606\\
66	311.339996888447\\
67	310.297033175766\\
68	310.210868967769\\
69	308.765307574444\\
70	308.734937613629\\
71	307.377290247213\\
72	307.20686429437\\
73	306.913204796255\\
74	306.324955938443\\
75	305.597744920062\\
76	305.597744920062\\
77	305.597744920062\\
78	305.597744920062\\
79	305.597744920062\\
80	305.597744920062\\
81	305.597744920062\\
82	305.597744920062\\
83	305.597744920062\\
84	305.923979536661\\
85	306.53234340802\\
86	306.53234340802\\
87	306.53234340802\\
88	306.53234340802\\
89	306.783416932641\\
90	305.850551316725\\
91	305.850551316725\\
92	304.9229346747\\
93	304.9229346747\\
94	304.9229346747\\
95	304.9229346747\\
96	304.9229346747\\
97	304.9229346747\\
98	304.9229346747\\
99	304.9229346747\\
100	305.248604957861\\
100	310.258648519348\\
99	312.735731237883\\
98	312.735731237883\\
97	312.735731237883\\
96	312.735731237883\\
95	312.735731237883\\
94	312.735731237883\\
93	312.735731237883\\
92	312.735731237883\\
91	312.620835578519\\
90	312.620835578519\\
89	312.715020203457\\
88	316.922596667516\\
87	316.922596667516\\
86	316.922596667516\\
85	316.922596667516\\
84	318.88683613086\\
83	319.917552706627\\
82	319.917552706627\\
81	319.917552706627\\
80	319.917552706627\\
79	319.917552706627\\
78	319.917552706627\\
77	319.917552706627\\
76	319.917552706627\\
75	319.917552706627\\
74	320.297295250766\\
73	320.372324633716\\
72	320.743326401487\\
71	321.048334293176\\
70	321.254645961618\\
69	321.30767432993\\
68	322.301785524288\\
67	322.316671179219\\
66	322.712537620942\\
65	322.835341774372\\
64	323.740209823694\\
63	326.259154207594\\
62	326.371545866962\\
61	327.064510096684\\
60	327.59329569222\\
59	327.59329569222\\
58	327.47049887881\\
57	327.454385629825\\
56	327.454385629825\\
55	327.454385629825\\
54	327.454385629825\\
53	330.578464712271\\
52	331.348600035016\\
51	333.099288839973\\
50	333.099288839973\\
49	339.743556737644\\
48	339.814463381243\\
47	339.957422350552\\
46	340.323758899342\\
45	340.323758899342\\
44	340.323758899342\\
43	340.323758899342\\
42	342.819381032663\\
41	347.246916425374\\
40	352.953981823128\\
39	356.018709355916\\
38	356.778567149528\\
37	356.778567149528\\
36	357.463170462926\\
35	361.58365920976\\
34	365.05886960934\\
33	364.634260783572\\
32	367.541015862391\\
31	375.669922841693\\
30	379.365649538742\\
29	379.225317394158\\
28	381.968608714062\\
27	392.204534735965\\
26	393.623949381945\\
25	395.007668389393\\
24	407.004181620804\\
23	409.394444677417\\
22	416.635143085337\\
21	420.804638980179\\
20	444.246271922813\\
19	457.514064585288\\
18	494.49564361158\\
17	522.822724489755\\
16	544.744638372065\\
15	564.656007865392\\
14	607.141291697953\\
13	635.436308883413\\
12	676.499471940444\\
11	722.502709170342\\
10	753.235797093225\\
9	805.817020747737\\
8	840.584221491553\\
7	873.366927079373\\
6	920.526147564248\\
5	963.896273679546\\
4	984.580476235741\\
3	1028.41579143717\\
2	1059.022624154\\
1	1072.56530525092\\
}--cycle;
\addplot [color=red!50!mycolor1]
  table[row sep=crcr]{%
1	1007\\
2	993\\
3	961\\
4	919\\
5	888\\
6	846\\
7	798\\
8	770\\
9	730\\
10	693\\
11	655\\
12	625\\
13	593\\
14	573\\
15	528\\
16	501\\
17	482\\
18	463\\
19	433\\
20	423\\
21	403\\
22	398\\
23	388\\
24	386\\
25	375\\
26	369\\
27	368\\
28	359\\
29	357\\
30	356\\
31	355\\
32	351\\
33	349\\
34	348\\
35	344\\
36	341\\
37	341\\
38	341\\
39	340\\
40	338\\
41	335\\
42	332\\
43	330\\
44	330\\
45	330\\
46	330\\
47	329\\
48	329\\
49	328\\
50	325\\
51	325\\
52	324\\
53	324\\
54	321\\
55	321\\
56	321\\
57	321\\
58	321\\
59	320\\
60	320\\
61	320\\
62	320\\
63	319\\
64	318\\
65	317\\
66	317\\
67	316\\
68	316\\
69	315\\
70	315\\
71	314\\
72	314\\
73	314\\
74	313\\
75	313\\
76	313\\
77	313\\
78	313\\
79	313\\
80	313\\
81	313\\
82	313\\
83	313\\
84	312\\
85	312\\
86	312\\
87	312\\
88	312\\
89	310\\
90	309\\
91	309\\
92	309\\
93	309\\
94	309\\
95	309\\
96	309\\
97	309\\
98	309\\
99	309\\
100	308\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.1}$}


\addplot[area legend, draw=none, fill=red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	891.813524513513\\
2	819.409843551937\\
3	766.927512436109\\
4	681.790680263488\\
5	649.033795495181\\
6	592.132559512566\\
7	484.435877900163\\
8	472.088364883036\\
9	443.342397611295\\
10	426.391575269901\\
11	402.090747821125\\
12	385.924804431583\\
13	372.144984684559\\
14	359.458853051741\\
15	354.447215788007\\
16	347.479898170432\\
17	346.02794573735\\
18	336.158708629221\\
19	334.376507703783\\
20	329.870870084657\\
21	330.012487688409\\
22	329.471144850914\\
23	329.471144850914\\
24	328.405149708682\\
25	326.029065632327\\
26	323.784277314758\\
27	322.755013130461\\
28	321.875611921904\\
29	322.473074096898\\
30	321.665435072793\\
31	321.896634485784\\
32	321.621919715792\\
33	320.982561993955\\
34	320.982561993955\\
35	319.493867874908\\
36	318.652385910739\\
37	318.808018437192\\
38	318.808018437192\\
39	320.76094240268\\
40	319.860838462048\\
41	319.912091285084\\
42	320.07549917476\\
43	320.07549917476\\
44	320.07549917476\\
45	318.08163196237\\
46	318.08163196237\\
47	317.770448196243\\
48	317.291240761116\\
49	317.291240761116\\
50	316.171163054462\\
51	316.171163054462\\
52	316.171163054462\\
53	316.890828061565\\
54	315.960066347777\\
55	315.710672576696\\
56	315.710672576696\\
57	313.161472150081\\
58	312.509780109113\\
59	312.080489574408\\
60	311.585451287641\\
61	311.682414500046\\
62	311.682414500046\\
63	311.682414500046\\
64	310.544425483001\\
65	310.544425483001\\
66	310.246696193509\\
67	309.74268026204\\
68	309.74268026204\\
69	309.74268026204\\
70	309.739933175232\\
71	308.618275932413\\
72	308.618275932413\\
73	306.975277029445\\
74	306.975277029445\\
75	306.173589656686\\
76	306.562741648895\\
77	305.664372923498\\
78	305.664372923498\\
79	305.664372923498\\
80	305.640874469217\\
81	305.77782594072\\
82	305.77782594072\\
83	305.77782594072\\
84	305.880275684867\\
85	305.880275684867\\
86	305.579299824209\\
87	305.051837259119\\
88	304.551919087331\\
89	304.583425846264\\
90	304.583425846264\\
91	304.583425846264\\
92	304.583425846264\\
93	304.573778178\\
94	304.411291306328\\
95	304.411291306328\\
96	304.411291306328\\
97	304.411291306328\\
98	304.411291306328\\
99	304.411291306328\\
100	304.257610128137\\
100	309.523233804604\\
99	310.392556236287\\
98	310.392556236287\\
97	310.392556236287\\
96	310.392556236287\\
95	310.392556236287\\
94	310.392556236287\\
93	311.409361324253\\
92	311.578967880502\\
91	311.578967880502\\
90	311.578967880502\\
89	311.578967880502\\
88	312.35798113371\\
87	312.478676873282\\
86	312.807456768638\\
85	314.563128518639\\
84	314.563128518639\\
83	315.513123869668\\
82	315.513123869668\\
81	315.513123869668\\
80	316.308225496201\\
79	316.367888818264\\
78	316.367888818264\\
77	316.367888818264\\
76	316.177295979946\\
75	317.782385189032\\
74	318.633615309913\\
73	318.633615309913\\
72	321.168133906284\\
71	321.168133906284\\
70	321.714134862103\\
69	321.714234646203\\
68	321.714234646203\\
67	321.714234646203\\
66	322.348366315542\\
65	322.308677800564\\
64	322.308677800564\\
63	322.366906446803\\
62	322.366906446803\\
61	322.366906446803\\
60	323.3095213827\\
59	324.402983224711\\
58	329.43727699767\\
57	329.566591977709\\
56	329.539424948941\\
55	329.539424948941\\
54	329.555785881415\\
53	329.717094672125\\
52	332.929442762828\\
51	332.929442762828\\
50	332.929442762828\\
49	334.766872048467\\
48	334.766872048467\\
47	334.864782639788\\
46	334.953214384808\\
45	334.953214384808\\
44	339.141598778996\\
43	339.141598778996\\
42	339.141598778996\\
41	340.317282215621\\
40	340.486070378614\\
39	340.691905353095\\
38	346.90083866664\\
37	346.90083866664\\
36	347.386392996367\\
35	348.179239330056\\
34	351.944118040282\\
33	351.944118040282\\
32	353.560847305629\\
31	356.711858038168\\
30	360.366751381295\\
29	360.566123651921\\
28	366.714319688962\\
27	366.70049718591\\
26	366.845950420562\\
25	367.044018866555\\
24	369.097458938452\\
23	369.538389581555\\
22	369.538389581555\\
21	369.828437691072\\
20	372.882659133978\\
19	372.752109694634\\
18	381.884984204696\\
17	404.386836655814\\
16	414.595925807957\\
15	426.023966372821\\
14	441.544066109695\\
13	451.289982961733\\
12	462.47911059179\\
11	497.017208028262\\
10	535.203306088386\\
9	564.393761209783\\
8	570.317601196132\\
7	652.606919628772\\
6	673.567520911265\\
5	709.307959696982\\
4	798.762127891694\\
3	871.949668402133\\
2	957.603899121031\\
1	1021.93461883201\\
}--cycle;
\addplot [color=red]
  table[row sep=crcr]{%
1	957\\
2	889\\
3	819\\
4	740\\
5	679\\
6	633\\
7	569\\
8	521\\
9	504\\
10	481\\
11	450\\
12	424\\
13	412\\
14	401\\
15	390\\
16	381\\
17	375\\
18	359\\
19	354\\
20	351\\
21	350\\
22	350\\
23	350\\
24	349\\
25	347\\
26	345\\
27	345\\
28	344\\
29	342\\
30	341\\
31	339\\
32	338\\
33	336\\
34	336\\
35	334\\
36	333\\
37	333\\
38	333\\
39	331\\
40	330\\
41	330\\
42	330\\
43	330\\
44	330\\
45	327\\
46	327\\
47	326\\
48	326\\
49	326\\
50	325\\
51	325\\
52	325\\
53	323\\
54	323\\
55	323\\
56	323\\
57	321\\
58	321\\
59	318\\
60	317\\
61	317\\
62	317\\
63	317\\
64	316\\
65	316\\
66	316\\
67	316\\
68	316\\
69	316\\
70	316\\
71	315\\
72	315\\
73	313\\
74	313\\
75	312\\
76	311\\
77	311\\
78	311\\
79	311\\
80	311\\
81	311\\
82	311\\
83	311\\
84	310\\
85	310\\
86	309\\
87	309\\
88	308\\
89	308\\
90	308\\
91	308\\
92	308\\
93	308\\
94	307\\
95	307\\
96	307\\
97	307\\
98	307\\
99	307\\
100	307\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.2}$}


\addplot[area legend, draw=none, fill=mycolor2, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	776.178801942436\\
2	713.671739229807\\
3	675.862282591752\\
4	672.876915187539\\
5	616.092362886695\\
6	605.675150670455\\
7	545.979190509929\\
8	544.848889522189\\
9	544.848889522189\\
10	530.305637878101\\
11	520.746560652419\\
12	505.811105058077\\
13	492.626376292945\\
14	479.407172106701\\
15	473.232148899699\\
16	473.232148899699\\
17	473.232148899699\\
18	472.060097047995\\
19	469.538127674204\\
20	468.821285152509\\
21	468.821285152509\\
22	444.814916694802\\
23	444.814916694802\\
24	432.525481424807\\
25	431.429069669373\\
26	431.429069669373\\
27	431.429069669373\\
28	431.429069669373\\
29	434.612387995196\\
30	434.612387995196\\
31	429.41482129197\\
32	429.41482129197\\
33	420.365060094548\\
34	404.729213625595\\
35	404.729213625595\\
36	404.729213625595\\
37	391.152311720303\\
38	386.878580501394\\
39	381.266794920632\\
40	381.266794920632\\
41	373.639606578808\\
42	373.639606578808\\
43	375.93254589739\\
44	375.93254589739\\
45	373.196128099068\\
46	377.650261544166\\
47	377.650261544166\\
48	377.650261544166\\
49	366.567193093926\\
50	361.827300468157\\
51	361.827300468157\\
52	361.827300468157\\
53	361.827300468157\\
54	351.630069918473\\
55	351.630069918473\\
56	351.428266092671\\
57	351.428266092671\\
58	351.080590362171\\
59	349.438779050036\\
60	352.058859047714\\
61	352.058859047714\\
62	347.996180851597\\
63	347.996180851597\\
64	347.996180851597\\
65	347.996180851597\\
66	344.347363662508\\
67	343.437717057087\\
68	343.437717057087\\
69	340.301091896175\\
70	340.301091896175\\
71	338.609569218502\\
72	333.186272057411\\
73	333.186272057411\\
74	332.108195937957\\
75	332.108195937957\\
76	331.948743641375\\
77	331.948743641375\\
78	331.260559971989\\
79	331.260559971989\\
80	329.760049343707\\
81	323.603019917034\\
82	323.603019917034\\
83	319.70878057296\\
84	319.70878057296\\
85	319.70878057296\\
86	319.70878057296\\
87	319.455792197287\\
88	319.216567198886\\
89	317.191034942806\\
90	316.089637195954\\
91	316.089637195954\\
92	316.089637195954\\
93	316.089637195954\\
94	316.548034759115\\
95	316.541047063797\\
96	316.59359958545\\
97	316.59359958545\\
98	315.508170716684\\
99	315.508170716684\\
100	315.369714721369\\
100	339.145520433183\\
99	339.879311943088\\
98	339.879311943088\\
97	344.719421739338\\
96	344.719421739338\\
95	345.888194421472\\
94	346.555364815161\\
93	356.132200317301\\
92	356.132200317301\\
91	356.132200317301\\
90	356.132200317301\\
89	363.774213227071\\
88	363.920216677986\\
87	364.207310188279\\
86	368.016806202858\\
85	368.016806202858\\
84	368.016806202858\\
83	368.016806202858\\
82	375.706548237292\\
81	375.706548237292\\
80	375.159716900708\\
79	379.871072409119\\
78	379.871072409119\\
77	389.399181217212\\
76	389.399181217212\\
75	389.777449902353\\
74	389.777449902353\\
73	389.725207096321\\
72	389.725207096321\\
71	389.262681127554\\
70	389.081722271072\\
69	389.081722271072\\
68	388.969349328043\\
67	388.969349328043\\
66	388.835728532265\\
65	389.508239247504\\
64	389.508239247504\\
63	389.508239247504\\
62	389.508239247504\\
61	389.431730493861\\
60	389.431730493861\\
59	402.743701029881\\
58	409.160040409893\\
57	424.073712963552\\
56	424.073712963552\\
55	424.059411637485\\
54	424.059411637485\\
53	426.525925091326\\
52	426.525925091326\\
51	426.525925091326\\
50	426.525925091326\\
49	429.643944971919\\
48	427.324126317941\\
47	427.324126317941\\
46	427.324126317941\\
45	445.802590610007\\
44	453.1827877133\\
43	453.1827877133\\
42	463.14330512504\\
41	463.14330512504\\
40	465.579389319528\\
39	465.579389319528\\
38	465.062284153744\\
37	467.906024023518\\
36	468.228744341721\\
35	468.228744341721\\
34	468.228744341721\\
33	471.915988582009\\
32	482.44054062918\\
31	482.44054062918\\
30	491.709051978394\\
29	491.709051978394\\
28	512.429945749832\\
27	512.429945749832\\
26	512.429945749832\\
25	512.429945749832\\
24	512.664984151057\\
23	524.718462031073\\
22	524.718462031073\\
21	520.094669321163\\
20	520.094669321163\\
19	525.016984836057\\
18	524.910860246815\\
17	524.916854890951\\
16	524.916854890951\\
15	524.916854890951\\
14	546.547598651659\\
13	578.962891156017\\
12	595.50650006122\\
11	615.286759632804\\
10	617.807569796087\\
9	646.025311246803\\
8	646.025311246803\\
7	665.129595522678\\
6	713.663440166059\\
5	716.314031382121\\
4	800.183610857953\\
3	835.231386160426\\
2	843.473449337223\\
1	907.649831754755\\
}--cycle;
\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	842\\
2	779\\
3	756\\
4	737\\
5	666\\
6	660\\
7	606\\
8	595\\
9	595\\
10	574\\
11	568\\
12	551\\
13	536\\
14	513\\
15	499\\
16	499\\
17	499\\
18	498\\
19	497\\
20	494\\
21	494\\
22	485\\
23	485\\
24	473\\
25	472\\
26	472\\
27	472\\
28	472\\
29	463\\
30	463\\
31	456\\
32	456\\
33	446\\
34	436\\
35	436\\
36	436\\
37	430\\
38	426\\
39	423\\
40	423\\
41	418\\
42	418\\
43	415\\
44	415\\
45	409\\
46	402\\
47	402\\
48	402\\
49	398\\
50	394\\
51	394\\
52	394\\
53	394\\
54	388\\
55	388\\
56	388\\
57	388\\
58	380\\
59	376\\
60	371\\
61	371\\
62	369\\
63	369\\
64	369\\
65	369\\
66	367\\
67	366\\
68	366\\
69	365\\
70	365\\
71	364\\
72	361\\
73	361\\
74	361\\
75	361\\
76	361\\
77	361\\
78	356\\
79	356\\
80	352\\
81	350\\
82	350\\
83	344\\
84	344\\
85	344\\
86	344\\
87	342\\
88	342\\
89	340\\
90	336\\
91	336\\
92	336\\
93	336\\
94	332\\
95	331\\
96	331\\
97	331\\
98	328\\
99	328\\
100	327\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.5}$}


\addplot[area legend, draw=none, fill=mycolor3, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	800.417856969901\\
2	672.080702487746\\
3	672.323227533077\\
4	605.284785849053\\
5	608.08838250569\\
6	580.261770642392\\
7	579.401753173239\\
8	579.547056865069\\
9	562.014483011524\\
10	561.735954686617\\
11	561.735954686617\\
12	552.939521937521\\
13	552.939521937521\\
14	552.939521937521\\
15	552.939521937521\\
16	552.939521937521\\
17	552.939521937521\\
18	548.840026070659\\
19	548.840026070659\\
20	548.840026070659\\
21	548.840026070659\\
22	548.840026070659\\
23	548.840026070659\\
24	548.755700860798\\
25	548.755700860798\\
26	548.755700860798\\
27	548.755700860798\\
28	548.755700860798\\
29	548.755700860798\\
30	548.755700860798\\
31	530.367029045622\\
32	530.367029045622\\
33	523.213929154763\\
34	523.213929154763\\
35	523.431318391119\\
36	523.431318391119\\
37	523.172170904657\\
38	513.601191280676\\
39	513.601191280676\\
40	513.601191280676\\
41	513.601191280676\\
42	510.900111676553\\
43	510.900111676553\\
44	501.649103912945\\
45	497.375446432261\\
46	497.375446432261\\
47	493.444490303567\\
48	493.444490303567\\
49	493.444490303567\\
50	493.444490303567\\
51	493.444490303567\\
52	493.444490303567\\
53	494.331718002986\\
54	494.331718002986\\
55	490.161411259495\\
56	490.161411259495\\
57	490.161411259495\\
58	490.161411259495\\
59	490.161411259495\\
60	490.161411259495\\
61	486.109614859138\\
62	474.395241838082\\
63	474.395241838082\\
64	473.900101078087\\
65	473.900101078087\\
66	473.900101078087\\
67	473.900101078087\\
68	473.900101078087\\
69	473.900101078087\\
70	468.983232077348\\
71	468.983232077348\\
72	463.850927842373\\
73	461.147908455771\\
74	454.21934279136\\
75	454.21934279136\\
76	454.21934279136\\
77	441.765316456131\\
78	441.10335514349\\
79	433.964362578351\\
80	422.887249119\\
81	406.274074513797\\
82	406.274074513797\\
83	406.274074513797\\
84	405.437646181628\\
85	400.298856459237\\
86	395.360257994246\\
87	392.283951270446\\
88	392.283951270446\\
89	392.283951270446\\
90	392.283951270446\\
91	392.283951270446\\
92	390.122553487204\\
93	390.122553487204\\
94	384.093887740401\\
95	384.093887740401\\
96	384.093887740401\\
97	363.495008080629\\
98	363.495008080629\\
99	363.495008080629\\
100	363.495008080629\\
100	496.778280636392\\
99	496.778280636392\\
98	496.778280636392\\
97	496.778280636392\\
96	500.889349749743\\
95	500.889349749743\\
94	500.889349749743\\
93	502.351870232256\\
92	502.351870232256\\
91	503.197827126201\\
90	503.197827126201\\
89	503.197827126201\\
88	503.197827126201\\
87	503.197827126201\\
86	504.735968581336\\
85	513.896719444131\\
84	517.168292406474\\
83	519.935509917189\\
82	519.935509917189\\
81	519.935509917189\\
80	522.024087615562\\
79	524.15480262086\\
78	529.51528931197\\
77	530.458207956975\\
76	527.617502192791\\
75	527.617502192791\\
74	527.617502192791\\
73	528.833092232088\\
72	529.876601589016\\
71	534.619952568042\\
70	534.619952568042\\
69	533.649101937419\\
68	533.649101937419\\
67	533.649101937419\\
66	533.649101937419\\
65	533.649101937419\\
64	533.649101937419\\
63	533.562024062053\\
62	533.562024062053\\
61	532.571620536925\\
60	533.269643292925\\
59	533.269643292925\\
58	533.269643292925\\
57	533.269643292925\\
56	533.269643292925\\
55	533.269643292925\\
54	538.457304774454\\
53	538.457304774454\\
52	542.480477901711\\
51	542.480477901711\\
50	542.480477901711\\
49	542.480477901711\\
48	542.480477901711\\
47	542.480477901711\\
46	546.673272503588\\
45	546.673272503588\\
44	549.464695675724\\
43	547.502996644345\\
42	547.502996644345\\
41	559.56021355634\\
40	559.56021355634\\
39	559.56021355634\\
38	559.56021355634\\
37	571.28834085641\\
36	573.74334962555\\
35	573.74334962555\\
34	580.327153897479\\
33	580.327153897479\\
32	589.82113487056\\
31	589.82113487056\\
30	584.54991726794\\
29	584.54991726794\\
28	584.54991726794\\
27	584.54991726794\\
26	584.54991726794\\
25	584.54991726794\\
24	584.54991726794\\
23	585.530408087539\\
22	585.530408087539\\
21	585.530408087539\\
20	585.530408087539\\
19	585.530408087539\\
18	585.530408087539\\
17	627.168334788253\\
16	627.168334788253\\
15	627.168334788253\\
14	627.168334788253\\
13	627.168334788253\\
12	627.168334788253\\
11	640.225498547354\\
10	640.225498547354\\
9	649.929081499374\\
8	668.526736671013\\
7	678.808425121207\\
6	694.503560127868\\
5	737.509439948426\\
4	749.791168645935\\
3	823.339889377515\\
2	846.442999572572\\
1	899.846441242712\\
}--cycle;
\addplot [color=mycolor3]
  table[row sep=crcr]{%
1	850\\
2	759\\
3	748\\
4	678\\
5	673\\
6	637\\
7	629\\
8	624\\
9	606\\
10	601\\
11	601\\
12	590\\
13	590\\
14	590\\
15	590\\
16	590\\
17	590\\
18	567\\
19	567\\
20	567\\
21	567\\
22	567\\
23	567\\
24	567\\
25	567\\
26	567\\
27	567\\
28	567\\
29	567\\
30	567\\
31	560\\
32	560\\
33	552\\
34	552\\
35	549\\
36	549\\
37	547\\
38	537\\
39	537\\
40	537\\
41	537\\
42	529\\
43	529\\
44	526\\
45	522\\
46	522\\
47	518\\
48	518\\
49	518\\
50	518\\
51	518\\
52	518\\
53	516\\
54	516\\
55	512\\
56	512\\
57	512\\
58	512\\
59	512\\
60	512\\
61	509\\
62	504\\
63	504\\
64	504\\
65	504\\
66	504\\
67	504\\
68	504\\
69	504\\
70	502\\
71	502\\
72	497\\
73	495\\
74	491\\
75	491\\
76	491\\
77	486\\
78	485\\
79	479\\
80	472\\
81	463\\
82	463\\
83	463\\
84	461\\
85	457\\
86	450\\
87	448\\
88	448\\
89	448\\
90	448\\
91	448\\
92	446\\
93	446\\
94	442\\
95	442\\
96	442\\
97	430\\
98	430\\
99	430\\
100	430\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.7}$}


\addplot[area legend, draw=none, fill=blue, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	5032.28040320084\\
2	4983.41552154718\\
3	4007.97476992585\\
4	3722.93111829836\\
5	3042.01689621005\\
6	2732.57931467022\\
7	2676.96826337124\\
8	2461.70242957567\\
9	2363.00726939588\\
10	2305.1816383237\\
11	1991.58264022913\\
12	1973.22276126954\\
13	1756.35993489771\\
14	1800.20090490457\\
15	1706.33263471041\\
16	1646.15995692229\\
17	1505.07641206342\\
18	1388.74455805244\\
19	1421.72250962331\\
20	1388.81764169892\\
21	1206.69813734123\\
22	1120.35032160357\\
23	1108.78543621908\\
24	1102.56003500371\\
25	915.097193722725\\
26	907.306037533226\\
27	946.78832331602\\
28	797.524317340605\\
29	773.797252673957\\
30	775.891610617625\\
31	775.891610617625\\
32	739.36721813202\\
33	748.999717970998\\
34	725.220834644576\\
35	725.220834644576\\
36	726.872792042312\\
37	723.690287706517\\
38	722.928039524979\\
39	755.506660077652\\
40	769.018978905761\\
41	700.586772146479\\
42	716.978226851962\\
43	735.43547841906\\
44	716.781267835165\\
45	723.713156696358\\
46	726.553721308808\\
47	741.934410477295\\
48	740.575356346204\\
49	751.286724300225\\
50	747.107885872919\\
51	751.095485840795\\
52	746.466605240673\\
53	758.470960097676\\
54	758.470960097676\\
55	763.723260414346\\
56	752.530045082842\\
57	750.574650623501\\
58	747.84997518325\\
59	749.674045662523\\
60	740.464332979313\\
61	736.141575803429\\
62	711.918503356736\\
63	711.918503356736\\
64	711.918503356736\\
65	698.464025431301\\
66	698.464025431301\\
67	692.973228614113\\
68	686.587550896599\\
69	683.52339942784\\
70	684.132544972858\\
71	647.206415079608\\
72	644.281218851191\\
73	647.312017176939\\
74	647.312017176939\\
75	648.080066470104\\
76	648.080066470104\\
77	646.158897817314\\
78	642.256072948572\\
79	602.540317035291\\
80	555.526815789894\\
81	555.526815789894\\
82	544.437980677054\\
83	544.437980677054\\
84	530.82456553618\\
85	530.82456553618\\
86	525.821481117942\\
87	525.821481117942\\
88	525.821481117942\\
89	527.2342426634\\
90	527.2342426634\\
91	527.969131933106\\
92	525.559965364878\\
93	525.559965364878\\
94	525.559965364878\\
95	496.728424449097\\
96	496.51729785869\\
97	497.08341749055\\
98	497.08341749055\\
99	497.08341749055\\
100	492.220392787996\\
100	961.215331473906\\
99	962.228902221763\\
98	962.228902221763\\
97	962.228902221763\\
96	967.057327808374\\
95	972.61806345396\\
94	987.129594593699\\
93	987.129594593699\\
92	987.129594593699\\
91	986.820853245908\\
90	999.514879744509\\
89	999.514879744509\\
88	1015.29629895765\\
87	1015.29629895765\\
86	1015.29629895765\\
85	1014.73889571487\\
84	1014.73889571487\\
83	1023.38620113216\\
82	1023.38620113216\\
81	1033.57104399646\\
80	1033.57104399646\\
79	1042.533094152\\
78	1071.97044840017\\
77	1079.28872505131\\
76	1103.74177758343\\
75	1103.74177758343\\
74	1156.08741715821\\
73	1156.08741715821\\
72	1186.5985045672\\
71	1216.66757439539\\
70	1228.3366995166\\
69	1240.25988704425\\
68	1239.88436311617\\
67	1244.1544921328\\
66	1244.7404010059\\
65	1244.7404010059\\
64	1251.03952990031\\
63	1251.03952990031\\
62	1251.03952990031\\
61	1264.32048775863\\
60	1263.63159654561\\
59	1262.24094553864\\
58	1415.21429684311\\
57	1433.0959784826\\
56	1457.31632653835\\
55	1462.14337909972\\
54	1491.6232364994\\
53	1491.6232364994\\
52	1595.71370307422\\
51	1619.98887039907\\
50	1637.69878024589\\
49	1670.90751980017\\
48	1793.69660382338\\
47	1799.99275282556\\
46	1910.70845452427\\
45	2000.51869975122\\
44	2074.25696918758\\
43	2573.4168540206\\
42	2784.25985604298\\
41	3054.50808168586\\
40	3091.74322389932\\
39	3200.59979009016\\
38	3430.89565559493\\
37	3440.95296392164\\
36	3504.55099830269\\
35	3568.95579586199\\
34	3568.95579586199\\
33	3622.63648102809\\
32	3883.49375328884\\
31	3887.0347673737\\
30	3887.0347673737\\
29	3905.07468569901\\
28	3989.30948208676\\
27	4012.19605560734\\
26	4697.08356211693\\
25	4829.10576303623\\
24	5281.66904976004\\
23	5281.88902836637\\
22	5286.57359792404\\
21	5288.08751273845\\
20	5389.23874045549\\
19	5408.5295814454\\
18	5598.58307432658\\
17	5595.23281345446\\
16	5631.66523037093\\
15	5630.24226935945\\
14	5630.69303016084\\
13	5842.42040458256\\
12	5896.58328667912\\
11	5897.69121012702\\
10	5980.12224089119\\
9	5980.45370188815\\
8	6241.0120853557\\
7	6245.71457323994\\
6	6489.10931621061\\
5	7266.98253536845\\
4	7678.57827770961\\
3	9051.52496428257\\
2	10240.5318914656\\
1	11402.2590070127\\
}--cycle;
\addplot [color=blue]
  table[row sep=crcr]{%
1	8217\\
2	7612\\
3	6530\\
4	5701\\
5	5154\\
6	4611\\
7	4461\\
8	4351\\
9	4172\\
10	4143\\
11	3945\\
12	3935\\
13	3799\\
14	3715\\
15	3668\\
16	3639\\
17	3550\\
18	3494\\
19	3415\\
20	3389\\
21	3247\\
22	3203\\
23	3195\\
24	3192\\
25	2872\\
26	2802\\
27	2479\\
28	2393\\
29	2339\\
30	2331\\
31	2331\\
32	2311\\
33	2186\\
34	2147\\
35	2147\\
36	2116\\
37	2082\\
38	2077\\
39	1978\\
40	1930\\
41	1878\\
42	1751\\
43	1654\\
44	1396\\
45	1362\\
46	1319\\
47	1271\\
48	1267\\
49	1211\\
50	1192\\
51	1186\\
52	1171\\
53	1125\\
54	1125\\
55	1113\\
56	1105\\
57	1092\\
58	1082\\
59	1006\\
60	1002\\
61	1000\\
62	981\\
63	981\\
64	981\\
65	972\\
66	972\\
67	969\\
68	963\\
69	962\\
70	956\\
71	932\\
72	915\\
73	902\\
74	902\\
75	876\\
76	876\\
77	863\\
78	857\\
79	823\\
80	795\\
81	795\\
82	784\\
83	784\\
84	773\\
85	773\\
86	771\\
87	771\\
88	771\\
89	763\\
90	763\\
91	757\\
92	756\\
93	756\\
94	756\\
95	735\\
96	732\\
97	730\\
98	730\\
99	730\\
100	727\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.05}$}


\addplot[area legend, draw=none, fill=mycolor4, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	5746.48095652576\\
2	3956.30025093671\\
3	3404.48663667791\\
4	3158.53112241048\\
5	2890.78760596591\\
6	2482.77626599247\\
7	2480.15960442528\\
8	2448.02851915756\\
9	2272.84378125441\\
10	2227.70194447431\\
11	1948.98368640154\\
12	1929.79505353681\\
13	1929.79505353681\\
14	1810.64148335669\\
15	1578.99215432534\\
16	1554.06044010273\\
17	1559.23733503174\\
18	1504.05995241501\\
19	1302.34311058614\\
20	1294.75936359682\\
21	1293.97722956165\\
22	1283.74344277472\\
23	1251.95444732432\\
24	1291.33176110835\\
25	1291.33176110835\\
26	1228.47384462404\\
27	1192.12297028848\\
28	1112.50826955766\\
29	990.076063312886\\
30	990.076063312886\\
31	990.076063312886\\
32	990.076063312886\\
33	990.076063312886\\
34	992.132266118096\\
35	993.668535551294\\
36	987.358116816971\\
37	989.773354912653\\
38	965.871014128431\\
39	965.871014128431\\
40	965.871014128431\\
41	965.871014128431\\
42	965.0812737234\\
43	963.53419200373\\
44	947.92332492348\\
45	947.92332492348\\
46	937.958572453425\\
47	937.958572453425\\
48	937.958572453425\\
49	934.134555087941\\
50	875.077908429547\\
51	875.077908429547\\
52	794.540309276063\\
53	794.586977234122\\
54	794.586977234122\\
55	787.534081438816\\
56	785.786339218315\\
57	765.997816607402\\
58	786.344419589404\\
59	786.344419589404\\
60	786.344419589404\\
61	785.543928809743\\
62	785.543928809743\\
63	785.333313111157\\
64	783.240326091349\\
65	775.544141679683\\
66	775.544141679683\\
67	743.281771116611\\
68	740.462194550358\\
69	739.994960031629\\
70	724.44169951345\\
71	724.44169951345\\
72	719.812164602752\\
73	719.540299432322\\
74	715.75870789972\\
75	715.75870789972\\
76	715.75870789972\\
77	711.13944491556\\
78	711.13944491556\\
79	708.43114749986\\
80	681.375520527688\\
81	686.121713524405\\
82	686.121713524405\\
83	668.338003697083\\
84	668.338003697083\\
85	667.811188645805\\
86	666.871588887393\\
87	666.871588887393\\
88	655.705996496645\\
89	656.85808581381\\
90	657.581864814224\\
91	657.520357000238\\
92	648.611751389616\\
93	630.426843552715\\
94	633.274331924298\\
95	633.274331924298\\
96	626.498283460329\\
97	608.217456491841\\
98	591.038839736904\\
99	588.746100446418\\
100	584.411680862521\\
100	785.009750470754\\
99	784.809806238338\\
98	784.753107367592\\
97	807.843925704039\\
96	810.940822120712\\
95	812.746289343874\\
94	812.746289343874\\
93	824.005565891872\\
92	849.995244252501\\
91	914.344035512805\\
90	915.010137317715\\
89	921.190898433797\\
88	929.528068611545\\
87	960.784187766286\\
86	960.784187766286\\
85	989.006239666322\\
84	993.425031038423\\
83	993.425031038423\\
82	997.786454596566\\
81	997.786454596566\\
80	1024.11477580101\\
79	1044.55206684489\\
78	1085.72130523653\\
77	1085.72130523653\\
76	1090.40832696076\\
75	1090.40832696076\\
74	1090.40832696076\\
73	1103.92965474078\\
72	1105.22508569526\\
71	1104.67405581161\\
70	1104.67405581161\\
69	1103.1929025287\\
68	1103.1583276247\\
67	1124.05925024409\\
66	1127.73290910216\\
65	1127.73290910216\\
64	1130.84070480091\\
63	1130.82735723888\\
62	1130.80786768001\\
61	1130.80786768001\\
60	1143.03662460589\\
59	1143.03662460589\\
58	1143.03662460589\\
57	1235.79866555808\\
56	1235.76697967603\\
55	1242.15665750586\\
54	1328.97027860268\\
53	1328.97027860268\\
52	1331.98578942902\\
51	1339.06328021512\\
50	1339.06328021512\\
49	1347.48993889452\\
48	1348.59338759097\\
47	1348.59338759097\\
46	1348.59338759097\\
45	1352.20997695426\\
44	1352.20997695426\\
43	1360.8719236104\\
42	1362.00799040174\\
41	1380.4461279546\\
40	1380.4461279546\\
39	1380.4461279546\\
38	1380.4461279546\\
37	1408.59710805221\\
36	1465.89985308063\\
35	1476.25143734111\\
34	1562.94547508774\\
33	1576.48920972436\\
32	1576.48920972436\\
31	1576.48920972436\\
30	1576.48920972436\\
29	1576.48920972436\\
28	1616.77425399389\\
27	1709.77469661033\\
26	1878.90165589381\\
25	1922.67409168238\\
24	1922.67409168238\\
23	2225.49456252037\\
22	2264.17002015532\\
21	2283.15006322976\\
20	2392.81097232991\\
19	2397.79731851328\\
18	2515.13743714695\\
17	2866.12231360036\\
16	2976.65742890072\\
15	3001.75741100996\\
14	3544.40660023582\\
13	3616.67817289903\\
12	3616.67817289903\\
11	4262.6832811168\\
10	4557.68910271143\\
9	4578.86536727355\\
8	4703.98510602787\\
7	4747.38204617347\\
6	5428.07820944332\\
5	6574.27924033891\\
4	6773.14336607283\\
3	6778.34745707971\\
2	7714.00661971796\\
1	8926.92417775687\\
}--cycle;
\addplot [color=mycolor4]
  table[row sep=crcr]{%
1	7337\\
2	5835\\
3	5091\\
4	4966\\
5	4733\\
6	3955\\
7	3614\\
8	3576\\
9	3426\\
10	3393\\
11	3106\\
12	2773\\
13	2773\\
14	2678\\
15	2290\\
16	2265\\
17	2213\\
18	2010\\
19	1850\\
20	1844\\
21	1789\\
22	1774\\
23	1739\\
24	1607\\
25	1607\\
26	1554\\
27	1451\\
28	1365\\
29	1283\\
30	1283\\
31	1283\\
32	1283\\
33	1283\\
34	1278\\
35	1235\\
36	1227\\
37	1199\\
38	1173\\
39	1173\\
40	1173\\
41	1173\\
42	1164\\
43	1162\\
44	1150\\
45	1150\\
46	1143\\
47	1143\\
48	1143\\
49	1141\\
50	1107\\
51	1107\\
52	1063\\
53	1062\\
54	1062\\
55	1015\\
56	1011\\
57	1001\\
58	965\\
59	965\\
60	965\\
61	958\\
62	958\\
63	958\\
64	957\\
65	952\\
66	952\\
67	934\\
68	922\\
69	922\\
70	915\\
71	915\\
72	913\\
73	912\\
74	903\\
75	903\\
76	903\\
77	898\\
78	898\\
79	876\\
80	853\\
81	842\\
82	842\\
83	831\\
84	831\\
85	828\\
86	814\\
87	814\\
88	793\\
89	789\\
90	786\\
91	786\\
92	749\\
93	727\\
94	723\\
95	723\\
96	719\\
97	708\\
98	688\\
99	687\\
100	685\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.1}$}


\addplot[area legend, draw=none, fill=mycolor5, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	5170.03227375288\\
2	3643.14937266689\\
3	3013.88527938524\\
4	2783.06302901892\\
5	2549.27558055067\\
6	2205.76574250587\\
7	1736.53564003158\\
8	2025.07266339973\\
9	1933.88406465493\\
10	1862.31313228524\\
11	1813.45295146484\\
12	1535.58352075129\\
13	1419.20393942324\\
14	1302.38076622633\\
15	1260.28962879832\\
16	1216.52422340768\\
17	1216.52422340768\\
18	1140.17085108422\\
19	1026.54299533562\\
20	1026.54299533562\\
21	989.444818262883\\
22	964.4433972427\\
23	1011.36789330552\\
24	1028.30328882717\\
25	995.364425543746\\
26	995.364425543746\\
27	861.221345909889\\
28	823.945474588184\\
29	782.86172469087\\
30	782.86172469087\\
31	672.346402142427\\
32	680.882151120109\\
33	668.05050271671\\
34	647.775849970312\\
35	661.863514329305\\
36	673.36497392303\\
37	650.899122928831\\
38	566.681462789805\\
39	565.824814884483\\
40	565.824814884483\\
41	581.248166400597\\
42	589.111342550479\\
43	568.737250729501\\
44	581.285834479515\\
45	624.045399513396\\
46	605.210537505279\\
47	605.210537505279\\
48	605.210537505279\\
49	575.082734050564\\
50	575.082734050564\\
51	522.021632429589\\
52	494.714663446711\\
53	492.470394688581\\
54	487.464935565014\\
55	450.039038431918\\
56	438.747085867178\\
57	433.1179991205\\
58	422.485130389727\\
59	417.929148202331\\
60	431.177789871439\\
61	458.839303277193\\
62	458.839303277193\\
63	460.71701090311\\
64	460.71701090311\\
65	463.58723210839\\
66	516.538182005144\\
67	475.511449975345\\
68	475.511449975345\\
69	475.511449975345\\
70	416.417408383608\\
71	403.575941395932\\
72	399.111668085704\\
73	384.812067099911\\
74	417.763251132279\\
75	408.163147211992\\
76	408.163147211992\\
77	393.830605810589\\
78	413.536109632479\\
79	413.536109632479\\
80	413.536109632479\\
81	408.284445260311\\
82	389.082529534418\\
83	388.288298937817\\
84	417.8818916726\\
85	417.8818916726\\
86	417.636749850663\\
87	397.310580403872\\
88	397.192368692042\\
89	393.936863880994\\
90	413.376581858168\\
91	413.376581858168\\
92	405.190150470063\\
93	433.503949282877\\
94	433.503949282877\\
95	430.256629385682\\
96	430.256629385682\\
97	430.247981309142\\
98	424.62876209212\\
99	416.460492542109\\
100	431.15899699201\\
100	1197.84165586544\\
99	1257.97137573982\\
98	1260.58849430647\\
97	1262.54808321891\\
96	1262.55085180562\\
95	1262.55085180562\\
94	1263.61816175387\\
93	1263.61816175387\\
92	1390.56130791087\\
91	1393.21489136149\\
90	1393.21489136149\\
89	1451.54191816615\\
88	1452.71548167627\\
87	1452.75223077959\\
86	1459.81164653627\\
85	1459.90206577437\\
84	1459.90206577437\\
83	1549.50567257604\\
82	1549.7937327662\\
81	1556.50279462597\\
80	1558.54644637074\\
79	1558.54644637074\\
78	1558.54644637074\\
77	1644.4319506761\\
76	1650.38071209823\\
75	1650.38071209823\\
74	1653.82364503072\\
73	1752.97187263258\\
72	1757.42776226991\\
71	1759.15794742782\\
70	1764.57193898686\\
69	1785.45032960566\\
68	1785.45032960566\\
67	1785.45032960566\\
66	1796.39057309957\\
65	1971.64672289783\\
64	1980.26674830263\\
63	1980.26674830263\\
62	1985.90591930752\\
61	1985.90591930752\\
60	2090.36077908667\\
59	2130.15679684688\\
58	2131.78529674959\\
57	2136.09402329121\\
56	2137.85312466122\\
55	2142.7685853537\\
54	2153.76840739466\\
53	2155.19037026667\\
52	2155.95160872277\\
51	2165.13087277362\\
50	2181.52532096602\\
49	2181.52532096602\\
48	2192.40522106257\\
47	2192.40522106257\\
46	2192.40522106257\\
45	2200.65619943934\\
44	2486.53412169753\\
43	2527.30643768789\\
42	2577.68449966283\\
41	2601.3313908603\\
40	2647.7088956018\\
39	2647.7088956018\\
38	2648.05186856348\\
37	2675.28029988324\\
36	2683.6543589496\\
35	2718.2407792816\\
34	2774.1504087651\\
33	2782.95884486911\\
32	2786.4183029955\\
31	2812.11423213712\\
30	2853.46061567132\\
29	2853.46061567132\\
28	2867.26835056141\\
27	2881.38937961344\\
26	2918.27442389441\\
25	2918.27442389441\\
24	2932.83070250423\\
23	2983.93259459486\\
22	3125.42726114772\\
21	3134.70195505357\\
20	3150.21711913398\\
19	3150.21711913398\\
18	3210.1664588243\\
17	3225.86509212053\\
16	3225.86509212053\\
15	3233.50488148559\\
14	3244.18632076094\\
13	3315.37838555635\\
12	3395.02896668288\\
11	3502.76422321806\\
10	3911.99422186422\\
9	3948.92765822696\\
8	3999.63463916276\\
7	4993.00451050724\\
6	5242.57856212147\\
5	5319.98328006031\\
4	5374.79535934662\\
3	5486.10505602762\\
2	5970.80733529359\\
1	7826.03005114544\\
}--cycle;
\addplot [color=mycolor5]
  table[row sep=crcr]{%
1	6498\\
2	4807\\
3	4250\\
4	4079\\
5	3935\\
6	3724\\
7	3365\\
8	3012\\
9	2941\\
10	2887\\
11	2658\\
12	2465\\
13	2367\\
14	2273\\
15	2247\\
16	2221\\
17	2221\\
18	2175\\
19	2088\\
20	2088\\
21	2062\\
22	2045\\
23	1998\\
24	1981\\
25	1957\\
26	1957\\
27	1871\\
28	1846\\
29	1818\\
30	1818\\
31	1742\\
32	1734\\
33	1726\\
34	1711\\
35	1690\\
36	1679\\
37	1663\\
38	1607\\
39	1607\\
40	1607\\
41	1591\\
42	1583\\
43	1548\\
44	1534\\
45	1412\\
46	1399\\
47	1399\\
48	1399\\
49	1378\\
50	1378\\
51	1344\\
52	1325\\
53	1324\\
54	1321\\
55	1296\\
56	1288\\
57	1285\\
58	1277\\
59	1274\\
60	1261\\
61	1222\\
62	1222\\
63	1220\\
64	1220\\
65	1218\\
66	1156\\
67	1130\\
68	1130\\
69	1130\\
70	1090\\
71	1081\\
72	1078\\
73	1069\\
74	1036\\
75	1029\\
76	1029\\
77	1019\\
78	986\\
79	986\\
80	986\\
81	982\\
82	969\\
83	969\\
84	939\\
85	939\\
86	939\\
87	925\\
88	925\\
89	923\\
90	903\\
91	903\\
92	898\\
93	849\\
94	849\\
95	846\\
96	846\\
97	846\\
98	843\\
99	837\\
100	815\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.2}$}


\addplot[area legend, draw=none, fill=mycolor6, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	3982.26244981736\\
2	3451.73674915169\\
3	3254.12321054569\\
4	3103.49447266683\\
5	2943.24821639861\\
6	2872.82246130382\\
7	2481.21473575911\\
8	2433.86635120258\\
9	2259.98428911061\\
10	2259.98428911061\\
11	2060.82257246376\\
12	2068.99351804662\\
13	2058.10452707527\\
14	1949.99893357497\\
15	1986.75692592812\\
16	1962.4993005091\\
17	1939.42983040767\\
18	1790.29674839426\\
19	1622.20253600069\\
20	1622.20253600069\\
21	1610.86595159914\\
22	1586.12425301169\\
23	1506.53137022763\\
24	1506.53137022763\\
25	1391.95473042241\\
26	1364.83631532303\\
27	1391.92725812808\\
28	1386.50623592407\\
29	1296.09701468073\\
30	1252.98550435093\\
31	1252.98550435093\\
32	1196.00180513194\\
33	1165.42631209102\\
34	1175.61420426624\\
35	1106.64458812375\\
36	1045.89090705776\\
37	1045.89090705776\\
38	990.366924536073\\
39	990.366924536073\\
40	964.957226937759\\
41	964.957226937759\\
42	964.957226937759\\
43	948.17378342998\\
44	948.17378342998\\
45	943.744927767915\\
46	951.586325063291\\
47	851.04200602225\\
48	833.811938660335\\
49	860.631649773383\\
50	860.631649773383\\
51	860.631649773383\\
52	836.019095685888\\
53	835.823424265065\\
54	835.823424265065\\
55	844.897612184827\\
56	848.841187527851\\
57	848.841187527851\\
58	848.841187527851\\
59	825.388305138377\\
60	764.31965125998\\
61	774.959184074575\\
62	769.498487082263\\
63	769.498487082263\\
64	769.498487082263\\
65	770.54128387233\\
66	763.611488599405\\
67	759.501626024203\\
68	759.077399956621\\
69	755.850548396647\\
70	755.850548396647\\
71	755.850548396647\\
72	756.432755694086\\
73	747.917049197545\\
74	747.596576869402\\
75	747.596576869402\\
76	744.994504786302\\
77	742.118261936829\\
78	739.689381340163\\
79	737.622523468709\\
80	737.229954588812\\
81	721.464841110054\\
82	708.241551104745\\
83	708.241551104745\\
84	708.241551104745\\
85	699.383762117052\\
86	696.69729366459\\
87	696.69729366459\\
88	683.817872919025\\
89	673.255289105591\\
90	657.927714425383\\
91	655.037035945047\\
92	646.508704568939\\
93	638.113161323236\\
94	631.99042183128\\
95	631.99042183128\\
96	636.138003955456\\
97	631.109117999222\\
98	622.244419751776\\
99	616.592266298718\\
100	610.701944712142\\
100	664.11781451631\\
99	674.567591710442\\
98	679.008057047012\\
97	677.893691125573\\
96	680.448698748541\\
95	709.958876275655\\
94	709.958876275655\\
93	710.091651113594\\
92	722.624760183242\\
91	737.083846663445\\
90	739.664426243027\\
89	739.137386073187\\
88	768.534813441101\\
87	772.947328282493\\
86	772.947328282493\\
85	773.462341129869\\
84	782.588736782321\\
83	782.588736782321\\
82	782.588736782321\\
81	783.980588916132\\
80	810.225867792534\\
79	811.161358113588\\
78	819.393160080367\\
77	826.504990291053\\
76	827.629816121563\\
75	829.204492621018\\
74	829.204492621018\\
73	830.816263512099\\
72	856.065762362182\\
71	863.656741645824\\
70	863.656741645824\\
69	863.656741645824\\
68	870.28033883986\\
67	871.733007943317\\
66	887.075187052114\\
65	938.698909812338\\
64	944.838265611576\\
63	944.838265611576\\
62	944.838265611576\\
61	951.280640579504\\
60	1001.11237442044\\
59	1000.58379442517\\
58	1026.16483678125\\
57	1026.16483678125\\
56	1026.16483678125\\
55	1039.41668829149\\
54	1086.06304548937\\
53	1086.06304548937\\
52	1111.31883663379\\
51	1120.12730878286\\
50	1120.12730878286\\
49	1120.12730878286\\
48	1207.90016408279\\
47	1230.2275145078\\
46	1245.49242193682\\
45	1270.35310027854\\
44	1271.20751401726\\
43	1271.20751401726\\
42	1302.05207246793\\
41	1302.05207246793\\
40	1302.05207246793\\
39	1321.01788292005\\
38	1321.01788292005\\
37	1356.14854031723\\
36	1356.14854031723\\
35	1394.08591115456\\
34	1380.06403682144\\
33	1498.48229733787\\
32	1557.28858869063\\
31	1622.33231802466\\
30	1622.33231802466\\
29	1678.76928106141\\
28	1729.98011133468\\
27	1734.97590157797\\
26	1931.86894409935\\
25	1961.12942684655\\
24	2000.564713923\\
23	2000.564713923\\
22	2050.51993382379\\
21	2110.58745446605\\
20	2133.69855513713\\
19	2133.69855513713\\
18	2092.86035247036\\
17	2121.3597669631\\
16	2131.24779657908\\
15	2209.83273044458\\
14	2508.92718291413\\
13	2645.46114089384\\
12	2643.05044801122\\
11	2824.48930216756\\
10	3142.92803154194\\
9	3142.92803154194\\
8	3260.51775528838\\
7	3318.78269910982\\
6	3442.81225957486\\
5	3451.92802464889\\
4	4253.90771336182\\
3	5365.55507120655\\
2	5609.39495502756\\
1	6752.35691263179\\
}--cycle;
\addplot [color=mycolor6]
  table[row sep=crcr]{%
1	5367\\
2	4531\\
3	4310\\
4	3679\\
5	3198\\
6	3158\\
7	2900\\
8	2847\\
9	2701\\
10	2701\\
11	2443\\
12	2356\\
13	2352\\
14	2229\\
15	2098\\
16	2047\\
17	2030\\
18	1942\\
19	1878\\
20	1878\\
21	1861\\
22	1818\\
23	1754\\
24	1754\\
25	1677\\
26	1648\\
27	1563\\
28	1558\\
29	1487\\
30	1438\\
31	1438\\
32	1377\\
33	1332\\
34	1278\\
35	1250\\
36	1201\\
37	1201\\
38	1156\\
39	1156\\
40	1134\\
41	1134\\
42	1134\\
43	1110\\
44	1110\\
45	1107\\
46	1099\\
47	1041\\
48	1021\\
49	990\\
50	990\\
51	990\\
52	974\\
53	961\\
54	961\\
55	942\\
56	938\\
57	938\\
58	938\\
59	913\\
60	883\\
61	863\\
62	857\\
63	857\\
64	857\\
65	855\\
66	825\\
67	816\\
68	815\\
69	810\\
70	810\\
71	810\\
72	806\\
73	789\\
74	788\\
75	788\\
76	786\\
77	784\\
78	780\\
79	774\\
80	774\\
81	753\\
82	745\\
83	745\\
84	745\\
85	736\\
86	735\\
87	735\\
88	726\\
89	706\\
90	699\\
91	696\\
92	685\\
93	674\\
94	671\\
95	671\\
96	658\\
97	655\\
98	651\\
99	646\\
100	637\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.5}$}


\addplot[area legend, draw=none, fill=mycolor7, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	5082.81175515935\\
2	4055.27975911248\\
3	3068.5323125499\\
4	3015.24968781448\\
5	3015.24968781448\\
6	3015.24968781448\\
7	2724.68193141728\\
8	2672.01696813761\\
9	2672.01696813761\\
10	2553.33837983798\\
11	2553.33837983798\\
12	2553.33837983798\\
13	2553.33837983798\\
14	2553.33837983798\\
15	2465.47418318117\\
16	2456.59670049739\\
17	2105.37115154177\\
18	2039.39207410757\\
19	2039.39207410757\\
20	2039.39207410757\\
21	2039.39207410757\\
22	1952.74837141132\\
23	1949.90277739389\\
24	1949.90277739389\\
25	1949.90277739389\\
26	1949.90277739389\\
27	1949.90277739389\\
28	1949.90277739389\\
29	1949.90277739389\\
30	1782.28262831904\\
31	1782.28262831904\\
32	1775.64498103657\\
33	1775.64498103657\\
34	1775.64498103657\\
35	1775.64498103657\\
36	1774.5743583764\\
37	1774.5743583764\\
38	1663.61588681183\\
39	1627.72709287808\\
40	1490.48021787494\\
41	1391.23915454571\\
42	1391.23915454571\\
43	1359.12516598273\\
44	1359.12516598273\\
45	1295.70141473634\\
46	1240.79034108102\\
47	1240.79034108102\\
48	1240.79034108102\\
49	1181.94996785118\\
50	1135.25075088001\\
51	1135.25075088001\\
52	1074.19612064463\\
53	1074.19612064463\\
54	1039.75969122595\\
55	1039.75969122595\\
56	1039.75969122595\\
57	1039.75969122595\\
58	1039.75969122595\\
59	1039.75969122595\\
60	1032.59417063858\\
61	997.435567243278\\
62	995.795339398861\\
63	995.795339398861\\
64	995.795339398861\\
65	987.774311368881\\
66	971.38626876887\\
67	954.86579397669\\
68	944.353187176986\\
69	938.889691259745\\
70	860.706277196179\\
71	860.285090149403\\
72	854.372797941329\\
73	838.018929688897\\
74	838.018929688897\\
75	785.518657629668\\
76	785.518657629668\\
77	774.008419673167\\
78	766.247363267722\\
79	766.247363267722\\
80	749.196427104072\\
81	749.196427104072\\
82	749.196427104072\\
83	685.826268013938\\
84	685.826268013938\\
85	677.415318651831\\
86	666.575696884269\\
87	655.557174896233\\
88	611.020149871376\\
89	611.020149871376\\
90	611.020149871376\\
91	570.356730015718\\
92	568.155397151872\\
93	568.155397151872\\
94	567.938003323501\\
95	567.938003323501\\
96	567.938003323501\\
97	567.938003323501\\
98	567.938003323501\\
99	567.79595007498\\
100	567.79595007498\\
100	1867.67193961219\\
99	1867.67193961219\\
98	1867.68834871305\\
97	1867.68834871305\\
96	1867.68834871305\\
95	1867.68834871305\\
94	1867.68834871305\\
93	1867.71116666493\\
92	1867.71116666493\\
91	1867.94686617123\\
90	1879.40069500928\\
89	1879.40069500928\\
88	1879.40069500928\\
87	2018.97087013924\\
86	2029.39629990377\\
85	2032.26962835751\\
84	2032.63432799334\\
83	2032.63432799334\\
82	2056.73630624806\\
81	2056.73630624806\\
80	2056.73630624806\\
79	2061.75616085603\\
78	2061.75616085603\\
77	2061.46487819039\\
76	2061.14466891837\\
75	2061.14466891837\\
74	2063.07062610291\\
73	2063.07062610291\\
72	2062.47796312692\\
71	2062.90473022103\\
70	2062.93736738668\\
69	2114.77459577527\\
68	2114.83495705803\\
67	2126.43945171541\\
66	2148.94352977846\\
65	2179.15366882405\\
64	2198.6648313712\\
63	2198.6648313712\\
62	2198.6648313712\\
61	2203.22414869415\\
60	2202.92804806426\\
59	2458.94501847906\\
58	2458.94501847906\\
57	2458.94501847906\\
56	2458.94501847906\\
55	2458.94501847906\\
54	2458.94501847906\\
53	2454.65614372744\\
52	2454.65614372744\\
51	2455.63558452699\\
50	2455.63558452699\\
49	2459.89923281958\\
48	2449.89278431457\\
47	2449.89278431457\\
46	2449.89278431457\\
45	2442.20969504462\\
44	2436.02153329627\\
43	2436.02153329627\\
42	2434.34540296095\\
41	2434.34540296095\\
40	2435.99393493873\\
39	2429.95234004433\\
38	2429.11902556038\\
37	2570.03133875341\\
36	2570.03133875341\\
35	2569.92131902348\\
34	2569.92131902348\\
33	2569.92131902348\\
32	2569.92131902348\\
31	2592.67906765827\\
30	2592.67906765827\\
29	2613.30923463839\\
28	2613.30923463839\\
27	2613.30923463839\\
26	2613.30923463839\\
25	2613.30923463839\\
24	2613.30923463839\\
23	2613.30923463839\\
22	2614.10781325793\\
21	2691.64730910467\\
20	2691.64730910467\\
19	2691.64730910467\\
18	2691.64730910467\\
17	2670.63652480551\\
16	2624.00699290703\\
15	2630.39596060566\\
14	2896.46595250112\\
13	2896.46595250112\\
12	2896.46595250112\\
11	2896.46595250112\\
10	2896.46595250112\\
9	3719.86477720372\\
8	3719.86477720372\\
7	3756.58837504695\\
6	4061.49938689107\\
5	4061.49938689107\\
4	4061.49938689107\\
3	4726.21617389984\\
2	5198.84310432623\\
1	8030.69282526226\\
}--cycle;
\addplot [color=mycolor7]
  table[row sep=crcr]{%
1	6557\\
2	4627\\
3	3897\\
4	3538\\
5	3538\\
6	3538\\
7	3241\\
8	3196\\
9	3196\\
10	2725\\
11	2725\\
12	2725\\
13	2725\\
14	2725\\
15	2548\\
16	2540\\
17	2388\\
18	2366\\
19	2366\\
20	2366\\
21	2366\\
22	2283\\
23	2282\\
24	2282\\
25	2282\\
26	2282\\
27	2282\\
28	2282\\
29	2282\\
30	2187\\
31	2187\\
32	2173\\
33	2173\\
34	2173\\
35	2173\\
36	2172\\
37	2172\\
38	2046\\
39	2029\\
40	1963\\
41	1913\\
42	1913\\
43	1898\\
44	1898\\
45	1869\\
46	1845\\
47	1845\\
48	1845\\
49	1821\\
50	1795\\
51	1795\\
52	1764\\
53	1764\\
54	1749\\
55	1749\\
56	1749\\
57	1749\\
58	1749\\
59	1749\\
60	1618\\
61	1600\\
62	1597\\
63	1597\\
64	1597\\
65	1583\\
66	1560\\
67	1541\\
68	1530\\
69	1527\\
70	1462\\
71	1462\\
72	1458\\
73	1451\\
74	1451\\
75	1423\\
76	1423\\
77	1418\\
78	1414\\
79	1414\\
80	1403\\
81	1403\\
82	1403\\
83	1359\\
84	1359\\
85	1355\\
86	1348\\
87	1337\\
88	1245\\
89	1245\\
90	1245\\
91	1219\\
92	1218\\
93	1218\\
94	1218\\
95	1218\\
96	1218\\
97	1218\\
98	1218\\
99	1218\\
100	1218\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.7}$}

\legend{}
\end{axis}


==> figures/arm26_reaching_hyperparameter_sigmaanalysis_c015_onlyaxis.tex <==
\begin{axis}[%
name =ax2,
scaled y ticks=base 10:\Factor,
at={(ax1.south east)},
xlabel near ticks, ylabel near ticks,
xshift=1.2cm,
width=0.647\figW,
height=\figH,
scale only axis,
xmin=0,
xmax=100,
xtick={  0,  20,  40,  60,  80, 100},
xlabel style={font=\color{white!15!black}},
xlabel={generations},
ymode=log,
ymin=280,
ymax=2500,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={cost},
axis background/.style={fill=white},
title={c = 0.15 s},
legend style={at={(1.03,0.5)}, anchor=west, legend cell align=left, align=left, draw=white!15!black}
]

\addplot[area legend, draw=none, fill=mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	778.101048833769\\
2	718.547288674323\\
3	680.968795144266\\
4	630.005863003624\\
5	602.529734852083\\
6	553.450618850634\\
7	527.170704708651\\
8	489.096928317016\\
9	467.626979349717\\
10	419.821478449191\\
11	411.926033980843\\
12	387.025689906637\\
13	381.960956665551\\
14	383.450109258817\\
15	373.174402610915\\
16	366.363916920037\\
17	361.49758228121\\
18	344.392487959534\\
19	339.377289376658\\
20	339.377289376658\\
21	325.740055524343\\
22	330.46804410454\\
23	320.563966181166\\
24	317.584773891573\\
25	315.395763751817\\
26	314.431374908226\\
27	310.656866446326\\
28	313.639097806286\\
29	313.639097806286\\
30	313.639097806286\\
31	314.384378975853\\
32	312.729567657712\\
33	312.57121135163\\
34	312.57121135163\\
35	312.57121135163\\
36	312.51108228968\\
37	311.140171583532\\
38	311.140171583532\\
39	311.140171583532\\
40	311.140171583532\\
41	310.197032416145\\
42	309.223873583057\\
43	306.236803093673\\
44	306.236803093673\\
45	306.236803093673\\
46	306.236803093673\\
47	305.883765667238\\
48	305.663154700722\\
49	305.663154700722\\
50	304.46819231443\\
51	304.79369557135\\
52	304.802852127371\\
53	304.802852127371\\
54	304.142199915585\\
55	303.94454597547\\
56	302.833159462753\\
57	302.68410171532\\
58	302.463664055866\\
59	301.868910056268\\
60	301.138676828621\\
61	301.136920571518\\
62	301.127174331955\\
63	301.127174331955\\
64	299.791560315441\\
65	298.899574653297\\
66	298.612142305591\\
67	298.612142305591\\
68	298.285754047744\\
69	298.285754047744\\
70	297.926122897797\\
71	297.926122897797\\
72	297.908236447304\\
73	297.657957319836\\
74	297.197118286449\\
75	297.149484152631\\
76	297.856430012959\\
77	297.856430012959\\
78	297.254249647114\\
79	296.852835309131\\
80	296.852835309131\\
81	296.852835309131\\
82	296.852835309131\\
83	296.774238127827\\
84	296.500260885767\\
85	296.377254437614\\
86	296.377254437614\\
87	295.641111707491\\
88	295.597234467381\\
89	295.392008359461\\
90	295.276991913741\\
91	295.21706730151\\
92	295.047681760061\\
93	295.68761303743\\
94	295.68761303743\\
95	295.178125391993\\
96	295.178125391993\\
97	295.095224826455\\
98	295.04617049397\\
99	295.446007968851\\
100	295.430361828267\\
100	298.353350412997\\
99	298.36022034127\\
98	299.574107984775\\
97	300.269819214768\\
96	300.304493048224\\
95	300.304493048224\\
94	300.659026960589\\
93	300.659026960589\\
92	303.534716288731\\
91	303.55836242684\\
90	303.570706676296\\
89	303.665247741014\\
88	303.700860328603\\
87	303.709468397295\\
86	304.252357652401\\
85	304.252357652401\\
84	304.26139172882\\
83	304.955908613055\\
82	304.960277551999\\
81	304.960277551999\\
80	304.960277551999\\
79	304.960277551999\\
78	305.162894731814\\
77	305.546021274703\\
76	305.546021274703\\
75	308.675328413075\\
74	308.722771615658\\
73	308.975007552913\\
72	309.100411116753\\
71	309.128600976582\\
70	309.128600976582\\
69	309.168131051349\\
68	309.168131051349\\
67	309.597166431891\\
66	309.597166431891\\
65	309.587295428893\\
64	311.626719154322\\
63	315.835049854235\\
62	315.835049854235\\
61	315.834297068085\\
60	315.834887662194\\
59	316.017626696139\\
58	315.976748868062\\
57	315.969281669982\\
56	316.355165863141\\
55	316.911629001632\\
54	319.133283144948\\
53	319.077633286183\\
52	319.077633286183\\
51	319.228354017577\\
50	321.658361230706\\
49	322.217030422378\\
48	322.217030422378\\
47	322.393891337147\\
46	322.765558626376\\
45	322.765558626376\\
44	322.765558626376\\
43	322.765558626376\\
42	323.72403243383\\
41	326.518104097597\\
40	329.650690377703\\
39	329.650690377703\\
38	329.650690377703\\
37	329.650690377703\\
36	331.651928963783\\
35	331.866771465955\\
34	331.866771465955\\
33	331.866771465955\\
32	332.696601033725\\
31	332.194239717604\\
30	339.883010375027\\
29	339.883010375027\\
28	339.883010375027\\
27	351.194630397967\\
26	351.080356171693\\
25	351.14541605335\\
24	351.530719975563\\
23	353.118035011665\\
22	381.470919256701\\
21	405.867425668191\\
20	413.57256459389\\
19	413.57256459389\\
18	416.080191748683\\
17	436.473170756586\\
16	439.561612022001\\
15	454.795541645998\\
14	465.976677986475\\
13	471.601288032546\\
12	526.731895406584\\
11	564.063313259295\\
10	640.446785143921\\
9	710.020656662019\\
8	745.122278410809\\
7	833.457963290909\\
6	887.044959211137\\
5	955.468535834571\\
4	1010.99772452003\\
3	1046.5978579264\\
2	1108.48983563155\\
1	1147.32710049761\\
}--cycle;
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	963\\
2	914\\
3	864\\
4	821\\
5	779\\
6	720\\
7	680\\
8	617\\
9	589\\
10	530\\
11	488\\
12	457\\
13	427\\
14	425\\
15	414\\
16	403\\
17	399\\
18	380\\
19	376\\
20	376\\
21	366\\
22	356\\
23	337\\
24	335\\
25	333\\
26	333\\
27	331\\
28	327\\
29	327\\
30	327\\
31	323\\
32	323\\
33	322\\
34	322\\
35	322\\
36	322\\
37	320\\
38	320\\
39	320\\
40	320\\
41	318\\
42	316\\
43	315\\
44	315\\
45	315\\
46	315\\
47	314\\
48	314\\
49	314\\
50	313\\
51	312\\
52	312\\
53	312\\
54	312\\
55	310\\
56	310\\
57	309\\
58	309\\
59	309\\
60	308\\
61	308\\
62	308\\
63	308\\
64	306\\
65	304\\
66	304\\
67	304\\
68	304\\
69	304\\
70	304\\
71	304\\
72	304\\
73	303\\
74	303\\
75	303\\
76	302\\
77	302\\
78	301\\
79	301\\
80	301\\
81	301\\
82	301\\
83	301\\
84	300\\
85	300\\
86	300\\
87	300\\
88	300\\
89	300\\
90	299\\
91	299\\
92	299\\
93	298\\
94	298\\
95	298\\
96	298\\
97	298\\
98	297\\
99	297\\
100	297\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.05}$}


\addplot[area legend, draw=none, fill=red!50!mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	657.797722076001\\
2	620.140960710903\\
3	568.187128487284\\
4	528.325036380342\\
5	501.92965968414\\
6	471.600927471901\\
7	401.501180712657\\
8	393.809226731129\\
9	391.694357732241\\
10	368.186922393593\\
11	352.420539176814\\
12	344.274937047082\\
13	344.282772383675\\
14	338.255452286316\\
15	330.914878815981\\
16	326.294269821234\\
17	325.169971574022\\
18	323.046093819843\\
19	320.557295423224\\
20	315.752955940678\\
21	315.49968456325\\
22	314.468064556269\\
23	310.895587685061\\
24	310.895587685061\\
25	311.086244140923\\
26	310.995470137032\\
27	310.063165586762\\
28	308.168244363432\\
29	307.274647037016\\
30	306.354773075509\\
31	306.972473663397\\
32	306.972473663397\\
33	306.462535741288\\
34	305.575422249569\\
35	305.575422249569\\
36	305.575422249569\\
37	304.842930877496\\
38	304.497474529507\\
39	304.497474529507\\
40	305.612555022763\\
41	304.290165546201\\
42	304.070062124327\\
43	304.070062124327\\
44	301.228516927286\\
45	301.029131743546\\
46	299.752130417099\\
47	299.752130417099\\
48	299.752130417099\\
49	299.750778006297\\
50	299.749256566117\\
51	299.749256566117\\
52	299.749256566117\\
53	299.749256566117\\
54	299.749256566117\\
55	298.836175465047\\
56	298.742226981954\\
57	298.742226981954\\
58	298.737788009747\\
59	298.737788009747\\
60	298.356351369039\\
61	298.057041029626\\
62	298.106192945083\\
63	297.888064289046\\
64	298.122277548865\\
65	297.857594669301\\
66	296.988367811644\\
67	296.988367811644\\
68	297.18233518066\\
69	297.18233518066\\
70	297.401571616439\\
71	297.391417599633\\
72	296.570704672994\\
73	296.865439460578\\
74	296.901932494826\\
75	297.055392895914\\
76	296.877773851361\\
77	296.877773851361\\
78	296.911397553388\\
79	296.947345068191\\
80	296.677426207848\\
81	296.410345900206\\
82	296.410345900206\\
83	296.44117843722\\
84	296.350605996593\\
85	296.345362196205\\
86	296.241878831988\\
87	295.638212119382\\
88	295.643936137529\\
89	295.629111689484\\
90	295.199465047314\\
91	295.193469338846\\
92	295.193469338846\\
93	295.229741074041\\
94	295.23238511998\\
95	295.23238511998\\
96	294.951327288427\\
97	294.951327288427\\
98	294.889080546128\\
99	294.848050320998\\
100	294.806926103928\\
100	296.01152431478\\
99	296.138307356781\\
98	296.143492604303\\
97	296.403259417758\\
96	296.403259417758\\
95	296.446745511762\\
94	296.446745511762\\
93	296.570243642407\\
92	296.869528018339\\
91	296.869528018339\\
90	296.874579278754\\
89	297.520993372125\\
88	297.559533294045\\
87	297.599469158167\\
86	298.012551925998\\
85	298.0124620835\\
84	298.660655880135\\
83	298.655546922399\\
82	298.782029755146\\
81	298.782029755146\\
80	298.801511349776\\
79	298.966635699071\\
78	299.114693587413\\
77	299.244543944158\\
76	299.244543944158\\
75	299.569638895056\\
74	300.182057233765\\
73	300.565343822733\\
72	301.860619134913\\
71	302.704903737618\\
70	302.713069024009\\
69	303.586941890239\\
68	303.586941890239\\
67	304.287034676646\\
66	304.287034676646\\
65	304.465672320307\\
64	304.609789819751\\
63	305.410978680123\\
62	305.439922302322\\
61	305.602169346629\\
60	305.673675418512\\
59	306.388389551442\\
58	306.388389551442\\
57	306.405558379235\\
56	306.405558379235\\
55	307.281611506238\\
54	307.668585024528\\
53	307.668585024528\\
52	307.668585024528\\
51	307.668585024528\\
50	307.668585024528\\
49	308.155621264362\\
48	308.156636977729\\
47	308.156636977729\\
46	308.156636977729\\
45	308.867012580208\\
44	309.297646898281\\
43	308.726355657731\\
42	308.726355657731\\
41	308.725380874995\\
40	308.765041216164\\
39	314.595499639329\\
38	314.595499639329\\
37	314.640284323161\\
36	316.588418607733\\
35	316.588418607733\\
34	316.588418607733\\
33	317.174049994862\\
32	318.074121937804\\
31	318.074121937804\\
30	320.560324381383\\
29	321.708184977624\\
28	321.90445912514\\
27	324.435393373698\\
26	327.963655566677\\
25	329.622274543507\\
24	332.126717270001\\
23	332.126717270001\\
22	331.500825963183\\
21	333.440274986173\\
20	334.697777611008\\
19	341.023097300855\\
18	348.040286555503\\
17	357.10696560839\\
16	357.512973340018\\
15	359.562190550665\\
14	360.941661467378\\
13	362.214318295988\\
12	385.422484498313\\
11	415.788094384871\\
10	469.720139511076\\
9	498.943337035919\\
8	586.722127992102\\
7	638.854288684408\\
6	729.422384778684\\
5	784.38402497442\\
4	830.477115325733\\
3	947.278409391687\\
2	1021.47141154903\\
1	1087.4206066384\\
}--cycle;
\addplot [color=red!50!mycolor1]
  table[row sep=crcr]{%
1	873\\
2	821\\
3	758\\
4	679\\
5	643\\
6	601\\
7	520\\
8	490\\
9	445\\
10	419\\
11	384\\
12	365\\
13	353\\
14	350\\
15	345\\
16	342\\
17	341\\
18	336\\
19	331\\
20	325\\
21	324\\
22	323\\
23	322\\
24	322\\
25	320\\
26	319\\
27	317\\
28	315\\
29	314\\
30	313\\
31	313\\
32	313\\
33	312\\
34	311\\
35	311\\
36	311\\
37	310\\
38	310\\
39	310\\
40	307\\
41	307\\
42	306\\
43	306\\
44	305\\
45	305\\
46	304\\
47	304\\
48	304\\
49	304\\
50	304\\
51	304\\
52	304\\
53	304\\
54	304\\
55	303\\
56	303\\
57	303\\
58	303\\
59	303\\
60	302\\
61	302\\
62	302\\
63	302\\
64	301\\
65	301\\
66	301\\
67	301\\
68	300\\
69	300\\
70	300\\
71	300\\
72	299\\
73	299\\
74	299\\
75	298\\
76	298\\
77	298\\
78	298\\
79	298\\
80	298\\
81	298\\
82	298\\
83	298\\
84	298\\
85	297\\
86	297\\
87	297\\
88	297\\
89	297\\
90	296\\
91	296\\
92	296\\
93	296\\
94	296\\
95	296\\
96	296\\
97	296\\
98	296\\
99	295\\
100	295\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.1}$}


\addplot[area legend, draw=none, fill=red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	552.682241146824\\
2	532.195486728073\\
3	494.982852784691\\
4	458.861138435318\\
5	431.997275946587\\
6	408.396995591456\\
7	387.742175484299\\
8	370.309003353631\\
9	370.545132782615\\
10	362.592665080047\\
11	359.049052768056\\
12	340.88791327695\\
13	334.886017540123\\
14	332.314620106687\\
15	330.910297188282\\
16	330.910297188282\\
17	326.180634119869\\
18	321.805250128372\\
19	322.760608780375\\
20	317.313798359896\\
21	314.943710728092\\
22	314.435600535633\\
23	313.271744527597\\
24	312.58056132806\\
25	307.93361519106\\
26	307.892618440559\\
27	307.628295892923\\
28	307.628295892923\\
29	307.628295892923\\
30	305.829809290952\\
31	305.829809290952\\
32	306.427226186994\\
33	305.290178087892\\
34	302.86729123274\\
35	301.836009686807\\
36	301.358685655954\\
37	298.639750364164\\
38	297.088710303267\\
39	296.666613933378\\
40	296.666613933378\\
41	296.666613933378\\
42	296.666613933378\\
43	295.922884928342\\
44	295.922884928342\\
45	295.922884928342\\
46	298.904607297776\\
47	298.635085760101\\
48	298.635085760101\\
49	297.458750244978\\
50	297.409053523348\\
51	297.409053523348\\
52	297.274088662947\\
53	296.432088012206\\
54	295.895319641192\\
55	295.966679079473\\
56	295.82187808108\\
57	295.82187808108\\
58	295.82187808108\\
59	295.730491087913\\
60	295.930767620448\\
61	295.930767620448\\
62	295.021567464205\\
63	293.849212335177\\
64	293.849212335177\\
65	293.431147503788\\
66	293.431147503788\\
67	293.431147503788\\
68	292.870840882251\\
69	292.870840882251\\
70	292.870840882251\\
71	293.882471050094\\
72	293.762743690591\\
73	293.762743690591\\
74	293.614047478722\\
75	293.614047478722\\
76	293.614047478722\\
77	293.614047478722\\
78	293.583204800804\\
79	293.145118731767\\
80	293.0431027717\\
81	292.832716719971\\
82	293.03983837787\\
83	293.255007749399\\
84	293.255007749399\\
85	293.255007749399\\
86	292.908873796951\\
87	293.746636735984\\
88	293.399802072843\\
89	293.65941124007\\
90	293.65941124007\\
91	293.503528032247\\
92	293.521369224434\\
93	293.479526562105\\
94	293.479526562105\\
95	293.479526562105\\
96	293.378389847049\\
97	293.201098692096\\
98	293.201098692096\\
99	293.201098692096\\
100	293.208612584878\\
100	299.285750487676\\
99	299.343445420326\\
98	299.343445420326\\
97	299.343445420326\\
96	299.361803134541\\
95	299.431758787246\\
94	299.431758787246\\
93	299.431758787246\\
92	299.451103280379\\
91	299.506681995384\\
90	299.546107857017\\
89	299.546107857017\\
88	300.404192729822\\
87	300.601863677189\\
86	303.309530787653\\
85	303.449296759838\\
84	303.449296759838\\
83	303.449296759838\\
82	304.110987259452\\
81	304.975048644508\\
80	305.004153976787\\
79	305.026975227037\\
78	305.202122411977\\
77	305.206083655068\\
76	305.206083655068\\
75	305.206083655068\\
74	305.206083655068\\
73	305.255049799549\\
72	305.255049799549\\
71	305.301043688151\\
70	308.377474589691\\
69	308.377474589691\\
68	308.377474589691\\
67	308.656411476383\\
66	308.656411476383\\
65	308.656411476383\\
64	308.839302789658\\
63	308.839302789658\\
62	309.322895227011\\
61	309.792279942395\\
60	309.792279942395\\
59	311.9418471586\\
58	314.941545698064\\
57	314.941545698064\\
56	314.941545698064\\
55	315.000080653988\\
54	316.474834998047\\
53	316.809738331155\\
52	316.917644447434\\
51	317.016328129872\\
50	317.016328129872\\
49	317.022703541049\\
48	317.356134907148\\
47	317.356134907148\\
46	317.411298747907\\
45	328.602764805711\\
44	328.602764805711\\
43	328.602764805711\\
42	328.924306078856\\
41	328.924306078856\\
40	328.924306078856\\
39	328.924306078856\\
38	329.205093740657\\
37	329.71848713306\\
36	330.532495137564\\
35	330.741080513088\\
34	331.161791898278\\
33	331.855676971329\\
32	332.147620707169\\
31	337.038802431629\\
30	337.038802431629\\
29	337.885464925427\\
28	337.885464925427\\
27	337.885464925427\\
26	338.151817382729\\
25	338.196639034067\\
24	340.154745016621\\
23	340.538991652407\\
22	341.603028507782\\
21	341.537554335023\\
20	345.757949292655\\
19	345.255106311983\\
18	349.063446075038\\
17	351.276562073804\\
16	353.493318791377\\
15	353.493318791377\\
14	359.717515949388\\
13	362.380356689992\\
12	368.414944249113\\
11	374.885869760552\\
10	392.274111948794\\
9	399.382479588957\\
8	448.306287795917\\
7	494.469893338674\\
6	560.959781508393\\
5	628.047365255794\\
4	681.189497337559\\
3	760.867271863049\\
2	842.521082164984\\
1	927.149794195054\\
}--cycle;
\addplot [color=red]
  table[row sep=crcr]{%
1	740\\
2	687\\
3	628\\
4	570\\
5	530\\
6	485\\
7	441\\
8	409\\
9	385\\
10	377\\
11	367\\
12	355\\
13	349\\
14	346\\
15	342\\
16	342\\
17	339\\
18	335\\
19	334\\
20	332\\
21	328\\
22	328\\
23	327\\
24	326\\
25	323\\
26	323\\
27	323\\
28	323\\
29	323\\
30	321\\
31	321\\
32	319\\
33	319\\
34	317\\
35	316\\
36	316\\
37	314\\
38	313\\
39	313\\
40	313\\
41	313\\
42	313\\
43	312\\
44	312\\
45	312\\
46	308\\
47	308\\
48	308\\
49	307\\
50	307\\
51	307\\
52	307\\
53	307\\
54	306\\
55	305\\
56	305\\
57	305\\
58	305\\
59	304\\
60	303\\
61	303\\
62	302\\
63	301\\
64	301\\
65	301\\
66	301\\
67	301\\
68	301\\
69	301\\
70	301\\
71	300\\
72	300\\
73	300\\
74	299\\
75	299\\
76	299\\
77	299\\
78	299\\
79	299\\
80	299\\
81	299\\
82	299\\
83	298\\
84	298\\
85	298\\
86	298\\
87	297\\
88	297\\
89	297\\
90	297\\
91	297\\
92	296\\
93	296\\
94	296\\
95	296\\
96	296\\
97	296\\
98	296\\
99	296\\
100	296\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.2}$}


\addplot[area legend, draw=none, fill=mycolor2, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	485.260438219598\\
2	445.014477324329\\
3	402.587607239574\\
4	400.865078730495\\
5	409.671232480042\\
6	372.349876197839\\
7	370.718427678177\\
8	361.959692631281\\
9	361.959692631281\\
10	344.178938244941\\
11	350.699235914973\\
12	346.817214492602\\
13	345.322057979861\\
14	345.322057979861\\
15	340.852162592647\\
16	340.852162592647\\
17	340.852162592647\\
18	339.127362332871\\
19	342.465078013264\\
20	342.465078013264\\
21	342.285289158232\\
22	338.529718042369\\
23	338.529718042369\\
24	338.529718042369\\
25	340.182120252352\\
26	340.182120252352\\
27	340.182120252352\\
28	325.239306075879\\
29	320.057244006094\\
30	317.87772261536\\
31	317.87772261536\\
32	315.52033224309\\
33	315.52033224309\\
34	312.591210016689\\
35	313.313356613948\\
36	315.401795902413\\
37	315.27454473159\\
38	311.141596430674\\
39	308.242932269894\\
40	308.242932269894\\
41	309.471048588421\\
42	308.372779540485\\
43	307.913556173953\\
44	307.913556173953\\
45	308.269945928367\\
46	308.269945928367\\
47	308.267930157601\\
48	308.267930157601\\
49	308.267930157601\\
50	303.155015201816\\
51	303.155015201816\\
52	302.92502446252\\
53	302.903935238734\\
54	302.903935238734\\
55	302.903935238734\\
56	302.839343565556\\
57	299.425159972798\\
58	298.395753053014\\
59	298.395753053014\\
60	298.395753053014\\
61	298.529952695655\\
62	298.604754598018\\
63	298.604754598018\\
64	298.549477362773\\
65	298.549477362773\\
66	298.549477362773\\
67	297.976089222531\\
68	297.976089222531\\
69	297.976089222531\\
70	297.520134555886\\
71	297.520134555886\\
72	297.579568763894\\
73	297.619386435062\\
74	297.619386435062\\
75	297.704612807902\\
76	297.746967848083\\
77	297.754870062575\\
78	297.754870062575\\
79	297.104808382197\\
80	297.179437033496\\
81	296.680446591353\\
82	296.680446591353\\
83	296.680446591353\\
84	296.587394972281\\
85	296.587394972281\\
86	296.567798505733\\
87	296.463245249814\\
88	296.187543981079\\
89	296.187543981079\\
90	296.220680490117\\
91	295.941885752216\\
92	295.856541475983\\
93	295.856541475983\\
94	295.856541475983\\
95	295.856541475983\\
96	295.674380842114\\
97	295.674380842114\\
98	295.49926481626\\
99	295.160784569992\\
100	295.160784569992\\
100	297.267876208005\\
99	297.267876208005\\
98	297.389879075381\\
97	297.566361543669\\
96	297.566361543669\\
95	297.826875800009\\
94	297.826875800009\\
93	297.826875800009\\
92	297.826875800009\\
91	298.272035349948\\
90	298.1947720145\\
89	299.008520545771\\
88	299.008520545771\\
87	299.034142109414\\
86	299.353785165675\\
85	299.350719006294\\
84	299.350719006294\\
83	299.533475981715\\
82	299.533475981715\\
81	299.533475981715\\
80	299.537331248538\\
79	300.175558053783\\
78	301.006847565711\\
77	301.006847565711\\
76	302.207084652533\\
75	302.755624135419\\
74	303.749387752585\\
73	303.749387752585\\
72	303.982853277692\\
71	304.291491112154\\
70	304.291491112154\\
69	304.671037290906\\
68	304.671037290906\\
67	304.671037290906\\
66	304.666696571143\\
65	304.666696571143\\
64	304.666696571143\\
63	305.645059605078\\
62	305.645059605078\\
61	306.347977372327\\
60	307.954111772376\\
59	307.954111772376\\
58	307.954111772376\\
57	308.246531709616\\
56	310.915302420123\\
55	311.535601574522\\
54	311.535601574522\\
53	311.535601574522\\
52	312.909639752579\\
51	313.916778557558\\
50	313.916778557558\\
49	315.203454775342\\
48	315.203454775342\\
47	315.203454775342\\
46	315.9204834785\\
45	315.9204834785\\
44	318.606173441909\\
43	318.606173441909\\
42	318.753140729288\\
41	325.962522957616\\
40	331.136664919911\\
39	331.136664919911\\
38	331.267267102804\\
37	332.812036547981\\
36	332.808557415651\\
35	339.764461313756\\
34	342.059850026259\\
33	343.14969583889\\
32	343.14969583889\\
31	343.282646339942\\
30	343.282646339942\\
29	344.916716573667\\
28	363.575871749461\\
27	364.092132334994\\
26	364.092132334994\\
25	364.092132334994\\
24	369.911410750732\\
23	369.911410750732\\
22	369.911410750732\\
21	373.905851257266\\
20	374.561189052529\\
19	374.561189052529\\
18	389.500755814199\\
17	389.462315217213\\
16	389.462315217213\\
15	389.462315217213\\
14	393.651651679157\\
13	393.651651679157\\
12	404.001927610133\\
11	403.788825868673\\
10	435.405243236803\\
9	444.158142208825\\
8	444.158142208825\\
7	443.524859213219\\
6	477.838633009574\\
5	499.5299672631\\
4	554.853999274549\\
3	556.772305816044\\
2	667.550951231157\\
1	707.164150076889\\
}--cycle;
\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	596\\
2	556\\
3	480\\
4	478\\
5	455\\
6	425\\
7	407\\
8	403\\
9	403\\
10	390\\
11	377\\
12	375\\
13	369\\
14	369\\
15	365\\
16	365\\
17	365\\
18	364\\
19	359\\
20	359\\
21	358\\
22	354\\
23	354\\
24	354\\
25	352\\
26	352\\
27	352\\
28	344\\
29	332\\
30	331\\
31	331\\
32	329\\
33	329\\
34	327\\
35	327\\
36	324\\
37	324\\
38	321\\
39	320\\
40	320\\
41	318\\
42	314\\
43	313\\
44	313\\
45	312\\
46	312\\
47	312\\
48	312\\
49	312\\
50	309\\
51	309\\
52	308\\
53	307\\
54	307\\
55	307\\
56	307\\
57	304\\
58	303\\
59	303\\
60	303\\
61	302\\
62	302\\
63	302\\
64	302\\
65	302\\
66	302\\
67	301\\
68	301\\
69	301\\
70	301\\
71	301\\
72	301\\
73	301\\
74	301\\
75	300\\
76	300\\
77	299\\
78	299\\
79	299\\
80	298\\
81	298\\
82	298\\
83	298\\
84	298\\
85	298\\
86	298\\
87	298\\
88	298\\
89	298\\
90	297\\
91	297\\
92	297\\
93	297\\
94	297\\
95	297\\
96	297\\
97	297\\
98	296\\
99	296\\
100	296\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.5}$}


\addplot[area legend, draw=none, fill=mycolor3, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	689.655347308703\\
2	593.688053050603\\
3	548.617294122159\\
4	468.349658122467\\
5	465.39131075111\\
6	416.009120348287\\
7	417.807580053622\\
8	413.259182664739\\
9	395.959629549251\\
10	392.406911281067\\
11	401.905121018074\\
12	401.905121018074\\
13	390.99527161324\\
14	390.99527161324\\
15	390.99527161324\\
16	379.665102877262\\
17	379.665102877262\\
18	379.665102877262\\
19	378.629901915463\\
20	366.903458417476\\
21	363.96745648523\\
22	360.307660680183\\
23	360.48740003124\\
24	351.992406494908\\
25	350.534709957685\\
26	350.534709957685\\
27	338.90637334312\\
28	338.90637334312\\
29	338.90637334312\\
30	338.657580001014\\
31	338.657580001014\\
32	337.659143614758\\
33	337.659143614758\\
34	336.331316739806\\
35	336.331316739806\\
36	336.331316739806\\
37	335.672533411975\\
38	334.654633667271\\
39	328.100326861916\\
40	328.100326861916\\
41	328.100326861916\\
42	323.312091796903\\
43	316.051455452586\\
44	310.56910138105\\
45	310.56910138105\\
46	308.602169351035\\
47	308.602169351035\\
48	308.602169351035\\
49	308.602169351035\\
50	308.260924797492\\
51	307.759956840058\\
52	307.759956840058\\
53	307.759956840058\\
54	307.078367590284\\
55	308.583296977472\\
56	308.144213430282\\
57	307.863512578294\\
58	313.561056140672\\
59	311.778371894903\\
60	310.954235000959\\
61	308.511772517701\\
62	309.034431607977\\
63	309.499596216558\\
64	308.469632730602\\
65	307.473915056677\\
66	306.030109986096\\
67	305.945786525385\\
68	305.945786525385\\
69	305.735195748305\\
70	305.604667942358\\
71	306.195267911289\\
72	305.48835103438\\
73	304.531553981078\\
74	302.758098167155\\
75	302.758098167155\\
76	303.421433363958\\
77	299.851656952353\\
78	301.35898891744\\
79	301.062624730895\\
80	300.656831761001\\
81	300.589966726626\\
82	299.782042128104\\
83	299.762894157462\\
84	299.762894157462\\
85	299.755918417859\\
86	299.452724749556\\
87	299.452724749556\\
88	298.681927735979\\
89	298.60194447643\\
90	298.523712596475\\
91	298.903350838652\\
92	298.494498420464\\
93	298.028493150565\\
94	297.962170961313\\
95	297.390170422964\\
96	296.824253806746\\
97	296.824253806746\\
98	296.824253806746\\
99	296.824253806746\\
100	296.013619232882\\
100	300.95978719422\\
99	301.589259468984\\
98	301.589259468984\\
97	301.589259468984\\
96	301.589259468984\\
95	301.71273752757\\
94	302.009769288708\\
93	302.057013463567\\
92	302.062341615884\\
91	302.40033315662\\
90	303.931409125744\\
89	304.04921251448\\
88	304.075130965499\\
87	304.592607374205\\
86	304.592607374205\\
85	305.41007022381\\
84	305.915358523353\\
83	305.915358523353\\
82	305.920346669101\\
81	305.990044231516\\
80	306.009796653357\\
79	306.156042443239\\
78	306.25390169443\\
77	312.037250713956\\
76	313.730198954016\\
75	315.953793969943\\
74	315.953793969943\\
73	318.618961284922\\
72	318.809138618948\\
71	318.918335777564\\
70	320.999320707874\\
69	321.00794350242\\
68	321.091126025671\\
67	321.091126025671\\
66	321.110640095459\\
65	321.371332883702\\
64	322.862045565008\\
63	323.131561085309\\
62	326.122591895022\\
61	327.848805689916\\
60	329.456060413857\\
59	334.1721124228\\
58	335.399491397812\\
57	354.722920454406\\
56	354.80673949548\\
55	356.253810155298\\
54	362.086617366184\\
53	362.512966100526\\
52	362.512966100526\\
51	362.512966100526\\
50	363.783980273058\\
49	363.838552449908\\
48	363.838552449908\\
47	363.838552449908\\
46	363.838552449908\\
45	366.27875006758\\
44	366.27875006758\\
43	369.804846610078\\
42	374.323790123846\\
41	377.597129118562\\
40	377.597129118562\\
39	377.597129118562\\
38	376.640299059273\\
37	376.562416343574\\
36	377.324794249133\\
35	377.324794249133\\
34	377.324794249133\\
33	378.199840514142\\
32	378.199840514142\\
31	380.820316782071\\
30	380.820316782071\\
29	382.106028782762\\
28	382.106028782762\\
27	382.106028782762\\
26	385.282109145576\\
25	385.282109145576\\
24	390.621388696304\\
23	389.033863666671\\
22	390.624957757958\\
21	419.152164340648\\
20	419.972786594077\\
19	423.215796244054\\
18	424.647740721704\\
17	424.647740721704\\
16	424.647740721704\\
15	428.124069432822\\
14	428.124069432822\\
13	428.124069432822\\
12	439.451184282169\\
11	439.451184282169\\
10	477.869140198812\\
9	500.914024114037\\
8	507.64021406923\\
7	509.645114153594\\
6	533.828167289916\\
5	587.774904057256\\
4	597.090200138921\\
3	609.780268096632\\
2	688.582951763186\\
1	817.671857385813\\
}--cycle;
\addplot [color=mycolor3]
  table[row sep=crcr]{%
1	754\\
2	641\\
3	579\\
4	533\\
5	527\\
6	475\\
7	464\\
8	460\\
9	448\\
10	435\\
11	421\\
12	421\\
13	410\\
14	410\\
15	410\\
16	402\\
17	402\\
18	402\\
19	401\\
20	393\\
21	392\\
22	375\\
23	375\\
24	371\\
25	368\\
26	368\\
27	361\\
28	361\\
29	361\\
30	360\\
31	360\\
32	358\\
33	358\\
34	357\\
35	357\\
36	357\\
37	356\\
38	356\\
39	353\\
40	353\\
41	353\\
42	349\\
43	343\\
44	338\\
45	338\\
46	336\\
47	336\\
48	336\\
49	336\\
50	336\\
51	335\\
52	335\\
53	335\\
54	335\\
55	332\\
56	331\\
57	331\\
58	324\\
59	323\\
60	320\\
61	318\\
62	318\\
63	316\\
64	316\\
65	314\\
66	314\\
67	314\\
68	314\\
69	313\\
70	313\\
71	313\\
72	312\\
73	312\\
74	309\\
75	309\\
76	309\\
77	306\\
78	304\\
79	304\\
80	303\\
81	303\\
82	303\\
83	303\\
84	303\\
85	303\\
86	302\\
87	302\\
88	301\\
89	301\\
90	301\\
91	301\\
92	300\\
93	300\\
94	300\\
95	300\\
96	299\\
97	299\\
98	299\\
99	299\\
100	298\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.7}$}


\addplot[area legend, draw=none, fill=blue, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	2508.98350670848\\
2	1772.44580957159\\
3	1486.01863104862\\
4	1007.33565013928\\
5	429.781710825477\\
6	42.3942935049399\\
7	1e-09\\
8	1e-09\\
9	1e-09\\
10	1e-09\\
11	1e-09\\
12	1e-09\\
13	1e-09\\
14	1e-09\\
15	1e-09\\
16	1e-09\\
17	1e-09\\
18	1e-09\\
19	1e-09\\
20	1e-09\\
21	1e-09\\
22	1e-09\\
23	1e-09\\
24	1e-09\\
25	1e-09\\
26	16.9383209653113\\
27	43.6867378895365\\
28	178.001855755732\\
29	325.647223094182\\
30	314.147071625827\\
31	297.061158522604\\
32	297.061158522604\\
33	337.75027532086\\
34	382.084846322653\\
35	381.00926859331\\
36	410.110650148942\\
37	403.866671349691\\
38	442.878282419142\\
39	439.90933559887\\
40	414.404490728851\\
41	408.36010799553\\
42	418.302734337943\\
43	396.451230543194\\
44	383.762113060786\\
45	383.762113060786\\
46	398.827894422311\\
47	398.051835997846\\
48	392.639612873365\\
49	392.639612873365\\
50	367.66641579249\\
51	364.77917055048\\
52	379.796628690914\\
53	372.905807118798\\
54	385.847888278873\\
55	385.847888278873\\
56	384.957988857316\\
57	384.957988857316\\
58	358.316800024066\\
59	357.040999314439\\
60	351.61759178355\\
61	328.127199298679\\
62	317.861241511923\\
63	316.20150994413\\
64	316.473817789117\\
65	310.693212029146\\
66	300.418163751851\\
67	303.229156200405\\
68	302.556102619522\\
69	307.375152303053\\
70	306.800597827904\\
71	295.12614434113\\
72	276.953969639387\\
73	276.953969639387\\
74	277.894895392628\\
75	281.557210102747\\
76	284.816440105218\\
77	284.816440105218\\
78	280.632974912277\\
79	281.168080674262\\
80	279.904551700417\\
81	279.904551700417\\
82	280.900597350494\\
83	276.321157574243\\
84	276.036791095995\\
85	276.036791095995\\
86	279.034734149456\\
87	279.034734149456\\
88	276.259956701335\\
89	277.758175585697\\
90	276.215535770344\\
91	281.275840522349\\
92	294.414736237191\\
93	293.857248613512\\
94	293.974322583577\\
95	293.364112241266\\
96	293.364112241266\\
97	293.257097647043\\
98	292.443333834995\\
99	290.503645920827\\
100	290.503645920827\\
100	322.854413309593\\
99	322.854413309593\\
98	323.167063821056\\
97	323.509259078097\\
96	328.323437670638\\
95	328.323437670638\\
94	328.358831728531\\
93	333.359908007609\\
92	333.552713826122\\
91	384.696255083147\\
90	401.228847465813\\
89	401.615963805598\\
88	406.173476971819\\
87	407.024820781738\\
86	407.024820781738\\
85	416.972842205774\\
84	416.972842205774\\
83	417.032531004446\\
82	419.034573596878\\
81	422.070395102694\\
80	422.070395102694\\
79	422.579379265842\\
78	429.047266627942\\
77	431.327541963441\\
76	431.327541963441\\
75	441.352081414528\\
74	452.569910329549\\
73	456.463953970593\\
72	456.463953970593\\
71	471.41024457469\\
70	481.022055961661\\
69	481.723219072525\\
68	514.21004488934\\
67	514.247798155693\\
66	524.769785911751\\
65	528.084312564543\\
64	533.058334681618\\
63	534.082406420734\\
62	534.120158409333\\
61	539.175211728565\\
60	550.388698240757\\
59	557.407146849122\\
58	559.709328449861\\
57	571.820938550984\\
56	571.820938550984\\
55	573.228550198559\\
54	573.228550198559\\
53	636.336736132964\\
52	644.174413181418\\
51	706.747130519055\\
50	707.608418923508\\
49	721.853328424731\\
48	721.853328424731\\
47	722.7324170314\\
46	723.447868664957\\
45	783.015925356086\\
44	783.015925356086\\
43	791.740860231987\\
42	793.521796898463\\
41	828.251620697376\\
40	829.441923922163\\
39	830.189378568962\\
38	831.877271948504\\
37	1003.07850704991\\
36	1005.98504393859\\
35	1106.44028472101\\
34	1126.59372148121\\
33	1288.05304934314\\
32	1415.0162734801\\
31	1415.0162734801\\
30	1418.5205086357\\
29	1423.11577387112\\
28	1897.99001419976\\
27	2307.30162149961\\
26	2548.61840251399\\
25	3376.89536637453\\
24	3948.16193730536\\
23	4371.96312613074\\
22	5566.47997522428\\
21	5633.57845146754\\
20	5764.66487983494\\
19	5776.77612942707\\
18	5779.718369266\\
17	5839.11343352442\\
16	5839.11343352442\\
15	5917.88485893273\\
14	5958.54231611366\\
13	5985.28235950644\\
12	5992.54440214593\\
11	6013.79942339453\\
10	6044.63496445845\\
9	6049.14496041793\\
8	6144.62649011973\\
7	6218.04011045767\\
6	6330.43115998311\\
5	6533.13335796326\\
4	6951.91093288277\\
3	7786.10996212916\\
2	8822.9686738946\\
1	9584.40670907969\\
}--cycle;
\addplot [color=blue]
  table[row sep=crcr]{%
1	6047\\
2	5298\\
3	4636\\
4	3980\\
5	3481\\
6	3186\\
7	2962\\
8	2827\\
9	2647\\
10	2638\\
11	2576\\
12	2534\\
13	2519\\
14	2510\\
15	2479\\
16	2453\\
17	2453\\
18	2433\\
19	2427\\
20	2406\\
21	2342\\
22	2311\\
23	1912\\
24	1765\\
25	1566\\
26	1283\\
27	1175\\
28	1038\\
29	874\\
30	866\\
31	856\\
32	856\\
33	813\\
34	754\\
35	744\\
36	708\\
37	703\\
38	637\\
39	635\\
40	622\\
41	618\\
42	606\\
43	594\\
44	583\\
45	583\\
46	561\\
47	560\\
48	557\\
49	557\\
50	538\\
51	536\\
52	512\\
53	505\\
54	480\\
55	480\\
56	478\\
57	478\\
58	459\\
59	457\\
60	451\\
61	434\\
62	426\\
63	425\\
64	425\\
65	419\\
66	413\\
67	409\\
68	408\\
69	395\\
70	394\\
71	383\\
72	367\\
73	367\\
74	365\\
75	361\\
76	358\\
77	358\\
78	355\\
79	352\\
80	351\\
81	351\\
82	350\\
83	347\\
84	347\\
85	347\\
86	343\\
87	343\\
88	341\\
89	340\\
90	339\\
91	333\\
92	314\\
93	314\\
94	311\\
95	311\\
96	311\\
97	308\\
98	308\\
99	307\\
100	307\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.05}$}


\addplot[area legend, draw=none, fill=mycolor4, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	599.853480828543\\
2	295.638438041201\\
3	1e-09\\
4	1e-09\\
5	1e-09\\
6	1e-09\\
7	1e-09\\
8	1e-09\\
9	1e-09\\
10	1e-09\\
11	1e-09\\
12	1e-09\\
13	1e-09\\
14	1e-09\\
15	1e-09\\
16	290.935931567767\\
17	377.0203379756\\
18	435.605103942321\\
19	502.562278795789\\
20	555.847500521305\\
21	555.847500521305\\
22	555.047207961567\\
23	610.369326926542\\
24	606.90561759187\\
25	598.623800447891\\
26	598.623800447891\\
27	597.271733236089\\
28	622.279180903948\\
29	622.376931327052\\
30	594.800568276171\\
31	591.201567395869\\
32	583.649094910527\\
33	582.697558380594\\
34	559.290719645321\\
35	557.912459951453\\
36	556.03831747728\\
37	469.646834544059\\
38	458.858240991822\\
39	457.416443276594\\
40	457.416443276594\\
41	456.639528620948\\
42	456.639528620948\\
43	452.965212120578\\
44	445.330952117514\\
45	445.330952117514\\
46	443.415636393881\\
47	436.743018226965\\
48	469.809111696597\\
49	457.67220162729\\
50	457.67220162729\\
51	457.67220162729\\
52	457.67220162729\\
53	448.239491600902\\
54	452.319042505081\\
55	416.417615408584\\
56	373.626781843014\\
57	350.127057656312\\
58	337.774783920889\\
59	337.488646966664\\
60	337.488646966664\\
61	336.860670907436\\
62	336.860670907436\\
63	336.860670907436\\
64	326.895563663312\\
65	325.401904242463\\
66	323.969826649957\\
67	323.969826649957\\
68	316.183127744939\\
69	316.183127744939\\
70	311.407119268324\\
71	304.293542428972\\
72	303.500308539831\\
73	303.500308539831\\
74	292.559723585172\\
75	292.559723585172\\
76	288.195052361888\\
77	288.195052361888\\
78	288.628904250565\\
79	285.859301797066\\
80	277.593459293724\\
81	277.040697389917\\
82	270.229991904625\\
83	269.333448680978\\
84	265.879585010188\\
85	274.219593302134\\
86	271.942380308863\\
87	270.484407180133\\
88	270.067338234468\\
89	268.322735641451\\
90	268.057579210915\\
91	270.162798077601\\
92	267.897690289179\\
93	279.204829951991\\
94	288.87017233011\\
95	285.889809539789\\
96	285.807450832768\\
97	286.298694376395\\
98	288.222397037447\\
99	288.124237023432\\
100	286.061103591375\\
100	316.376905032227\\
99	316.599526798087\\
98	316.852193973229\\
97	326.295176697892\\
96	331.980582707472\\
95	332.006159417036\\
94	334.48336527035\\
93	368.167674964903\\
92	403.233292645275\\
91	404.500027481528\\
90	412.272415965562\\
89	412.336850139078\\
88	412.843092462262\\
87	412.977037748436\\
86	413.347083222361\\
85	413.89192264744\\
84	440.436237811202\\
83	442.50896081415\\
82	444.824248546289\\
81	449.771058138422\\
80	449.883461629687\\
79	487.941995691752\\
78	489.079186191627\\
77	491.93155340965\\
76	491.93155340965\\
75	492.768038559013\\
74	492.768038559013\\
73	501.775114923318\\
72	501.775114923318\\
71	505.152376163159\\
70	506.594078898577\\
69	507.694139454987\\
68	507.694139454987\\
67	539.014174390998\\
66	539.014174390998\\
65	548.705112076823\\
64	552.051252494887\\
63	583.551314962766\\
62	583.551314962766\\
61	583.551314962766\\
60	583.693657010859\\
59	583.693657010859\\
58	584.143344552996\\
57	588.235621199152\\
56	629.650215002196\\
55	643.24695138635\\
54	647.302563203666\\
53	673.668393849338\\
52	675.037242057597\\
51	675.037242057597\\
50	675.037242057597\\
49	675.037242057597\\
48	684.921175512608\\
47	797.787356631649\\
46	800.033473506741\\
45	801.54239671151\\
44	801.54239671151\\
43	805.202622678335\\
42	836.865522514832\\
41	836.865522514832\\
40	837.903303321535\\
39	837.903303321535\\
38	838.033198799112\\
37	841.707334602154\\
36	924.648796173735\\
35	949.461043906511\\
34	951.608181772217\\
33	953.715286004869\\
32	954.159268692899\\
31	954.231365308337\\
30	958.051127636009\\
29	960.125895191901\\
28	961.745342609478\\
27	1124.94131329745\\
26	1128.85860337077\\
25	1128.85860337077\\
24	1131.12541957936\\
23	1131.88813676597\\
22	1339.05660486282\\
21	1340.22898526504\\
20	1340.22898526504\\
19	1539.80216621524\\
18	1750.79205237387\\
17	1995.97944060353\\
16	2272.74877501566\\
15	5014.3240273887\\
14	6019.8016708334\\
13	6019.8016708334\\
12	6027.91321508525\\
11	6047.60105981837\\
10	6047.60105981837\\
9	6047.60105981837\\
8	6066.12539666344\\
7	6223.35448036035\\
6	6299.12054079651\\
5	6330.30355468447\\
4	6343.72993714739\\
3	7000.71175952291\\
2	7579.5528681757\\
1	7992.79927287055\\
}--cycle;
\addplot [color=mycolor4]
  table[row sep=crcr]{%
1	4296\\
2	3938\\
3	3454\\
4	2908\\
5	2885\\
6	2815\\
7	2686\\
8	2631\\
9	2600\\
10	2600\\
11	2600\\
12	2561\\
13	2547\\
14	2547\\
15	2198\\
16	1282\\
17	1186\\
18	1093\\
19	1021\\
20	948\\
21	948\\
22	947\\
23	871\\
24	869\\
25	864\\
26	864\\
27	861\\
28	792\\
29	791\\
30	776\\
31	773\\
32	769\\
33	768\\
34	755\\
35	754\\
36	740\\
37	656\\
38	648\\
39	648\\
40	648\\
41	647\\
42	647\\
43	629\\
44	623\\
45	623\\
46	622\\
47	617\\
48	577\\
49	566\\
50	566\\
51	566\\
52	566\\
53	561\\
54	550\\
55	530\\
56	502\\
57	469\\
58	461\\
59	461\\
60	461\\
61	460\\
62	460\\
63	460\\
64	439\\
65	437\\
66	431\\
67	431\\
68	412\\
69	412\\
70	409\\
71	405\\
72	403\\
73	403\\
74	393\\
75	393\\
76	390\\
77	390\\
78	389\\
79	387\\
80	364\\
81	363\\
82	358\\
83	356\\
84	353\\
85	344\\
86	343\\
87	342\\
88	341\\
89	340\\
90	340\\
91	337\\
92	336\\
93	324\\
94	312\\
95	309\\
96	309\\
97	306\\
98	303\\
99	302\\
100	301\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.1}$}


\addplot[area legend, draw=none, fill=mycolor5, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	661.289616605163\\
2	977.246670931292\\
3	944.509069720273\\
4	797.088050841908\\
5	756.338211651292\\
6	756.338211651292\\
7	756.338211651292\\
8	713.338547394196\\
9	713.338547394196\\
10	732.614609950776\\
11	715.301703223654\\
12	715.301703223654\\
13	702.04431388911\\
14	684.770629381988\\
15	684.770629381988\\
16	685.317806528589\\
17	685.296116283732\\
18	662.233568320906\\
19	638.193654648692\\
20	633.014868592728\\
21	606.912306113397\\
22	584.742583739849\\
23	569.358785490491\\
24	566.87175227992\\
25	567.543842129013\\
26	567.543842129013\\
27	559.377762114584\\
28	554.973517325879\\
29	549.430901562195\\
30	545.424750257415\\
31	535.130794937847\\
32	528.045998842465\\
33	499.541660773917\\
34	489.238779114913\\
35	489.238779114913\\
36	493.922469729725\\
37	487.667479342535\\
38	486.397742459972\\
39	482.25104375025\\
40	479.047266542927\\
41	473.912832585759\\
42	489.806071925413\\
43	485.994712020022\\
44	469.405351037119\\
45	466.924573839571\\
46	461.895387821864\\
47	458.641032793744\\
48	452.323403061573\\
49	466.297711812363\\
50	450.639343158452\\
51	444.714664229167\\
52	439.839705700187\\
53	434.163446939647\\
54	389.77671703227\\
55	389.43363113756\\
56	389.744117920342\\
57	379.565692149799\\
58	342.279714205261\\
59	341.263581062384\\
60	329.105281336259\\
61	329.105281336259\\
62	324.465824693138\\
63	319.731088165226\\
64	321.711910102816\\
65	306.460308832485\\
66	304.988682722165\\
67	297.841720067647\\
68	298.091739237359\\
69	295.810940046274\\
70	295.964379056398\\
71	292.467723135313\\
72	291.961612840659\\
73	289.398128391543\\
74	288.918906132034\\
75	289.957864677694\\
76	287.262161123179\\
77	287.949082455263\\
78	288.004801819658\\
79	288.785248081413\\
80	287.699492653192\\
81	282.961945109615\\
82	281.889179708085\\
83	278.498393780664\\
84	278.57793028674\\
85	277.977567743912\\
86	275.1564070434\\
87	275.584023680347\\
88	273.586872250078\\
89	274.910214462076\\
90	274.910214462076\\
91	281.775586771367\\
92	279.425920195026\\
93	279.015757859746\\
94	278.635098154042\\
95	277.971443148872\\
96	277.969019823314\\
97	281.596297494516\\
98	284.819534000973\\
99	286.920146941799\\
100	286.580071340258\\
100	317.462913720376\\
99	317.556895364824\\
98	325.16357294226\\
97	348.676930738359\\
96	359.794350418751\\
95	359.795300566413\\
94	359.928093064211\\
93	360.067454042013\\
92	360.23173629622\\
91	369.587352887379\\
90	390.57323362271\\
89	390.57323362271\\
88	396.609671945447\\
87	397.406504780326\\
86	401.918404220232\\
85	403.077125648195\\
84	404.587142917951\\
83	404.830091701385\\
82	405.612187192105\\
81	406.030556139149\\
80	408.999185946104\\
79	417.602487608854\\
78	420.051272581233\\
77	420.225884117689\\
76	422.376279145479\\
75	423.226866337677\\
74	426.956258223376\\
73	427.02582965994\\
72	431.633091881714\\
71	431.988604231846\\
70	434.515388717464\\
69	436.130594478499\\
68	436.397404468093\\
67	437.183445970326\\
66	445.230281212171\\
65	445.91758916621\\
64	453.360502221058\\
63	469.048411168029\\
62	474.655871765328\\
61	481.322114569626\\
60	481.322114569626\\
59	503.941235621222\\
58	506.985183138122\\
57	534.127543197494\\
56	542.435333706015\\
55	546.133272723632\\
54	546.864736280153\\
53	553.79549207305\\
52	563.129994386468\\
51	568.262945993505\\
50	588.867367345949\\
49	588.071885361522\\
48	672.472730837903\\
47	682.582472158894\\
46	757.754189750951\\
45	759.435735920918\\
44	763.559698148652\\
43	765.370703547091\\
42	767.28504273211\\
41	820.234724090187\\
40	850.267694936585\\
39	850.415459155712\\
38	851.784669890548\\
37	856.111071147276\\
36	856.446090931515\\
35	871.217185250978\\
34	871.217185250978\\
33	873.995361148473\\
32	921.695713159492\\
31	921.763689415109\\
30	956.176790981338\\
29	966.964219813359\\
28	990.055513813827\\
27	990.368403938458\\
26	1003.38219992896\\
25	1003.38219992896\\
24	1005.76929383791\\
23	1006.05697110472\\
22	1010.57962817735\\
21	1010.65809201974\\
20	1022.35374868098\\
19	1022.91042944751\\
18	1026.62994856721\\
17	1034.13282897698\\
16	1034.15667088096\\
15	1075.64058534475\\
14	1075.64058534475\\
13	1075.75650922861\\
12	1094.62157339565\\
11	1094.62157339565\\
10	1322.2349201139\\
9	1505.05801564296\\
8	1505.05801564296\\
7	1596.18568083774\\
6	1596.18568083774\\
5	1596.18568083774\\
4	1615.70612566641\\
3	2324.15102345855\\
2	3680.9530728926\\
1	6491.36035484248\\
}--cycle;
\addplot [color=mycolor5]
  table[row sep=crcr]{%
1	3576\\
2	2329\\
3	1634\\
4	1206\\
5	1176\\
6	1176\\
7	1176\\
8	1109\\
9	1109\\
10	1027\\
11	905\\
12	905\\
13	889\\
14	880\\
15	880\\
16	860\\
17	860\\
18	844\\
19	831\\
20	828\\
21	809\\
22	798\\
23	788\\
24	786\\
25	785\\
26	785\\
27	775\\
28	773\\
29	758\\
30	751\\
31	728\\
32	725\\
33	687\\
34	680\\
35	680\\
36	675\\
37	672\\
38	669\\
39	666\\
40	665\\
41	647\\
42	629\\
43	626\\
44	616\\
45	613\\
46	610\\
47	571\\
48	562\\
49	527\\
50	520\\
51	506\\
52	501\\
53	494\\
54	468\\
55	468\\
56	466\\
57	457\\
58	425\\
59	423\\
60	405\\
61	405\\
62	400\\
63	394\\
64	388\\
65	376\\
66	375\\
67	368\\
68	367\\
69	366\\
70	365\\
71	362\\
72	362\\
73	358\\
74	358\\
75	357\\
76	355\\
77	354\\
78	354\\
79	353\\
80	348\\
81	344\\
82	344\\
83	342\\
84	342\\
85	341\\
86	339\\
87	336\\
88	335\\
89	333\\
90	333\\
91	326\\
92	320\\
93	320\\
94	319\\
95	319\\
96	319\\
97	315\\
98	305\\
99	302\\
100	302\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.2}$}


\addplot[area legend, draw=none, fill=mycolor6, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1539.33964108625\\
2	1238.47744926174\\
3	1256.67638090192\\
4	1114.29172452104\\
5	1066.75691875831\\
6	1066.75691875831\\
7	1066.0574378397\\
8	1032.14402228052\\
9	909.964053127863\\
10	832.059072747605\\
11	832.059072747605\\
12	832.059072747605\\
13	701.191809737287\\
14	701.191809737287\\
15	701.191809737287\\
16	701.191809737287\\
17	693.501363124321\\
18	666.841411374731\\
19	633.241141341979\\
20	639.919180623935\\
21	643.306005851664\\
22	670.387530684257\\
23	670.387530684257\\
24	670.387530684257\\
25	657.492169100254\\
26	657.492169100254\\
27	609.686206454106\\
28	605.52865482848\\
29	605.52865482848\\
30	603.20410081044\\
31	587.665434659474\\
32	567.072079692941\\
33	556.647126756754\\
34	539.207015158666\\
35	539.943311101062\\
36	522.740648330502\\
37	537.210180484308\\
38	537.210180484308\\
39	529.24283295823\\
40	491.052433024976\\
41	500.386173351339\\
42	500.386173351339\\
43	500.386173351339\\
44	499.022889494373\\
45	492.813686552851\\
46	479.739382532148\\
47	512.164492065296\\
48	510.166589044181\\
49	512.91600659567\\
50	512.775380233935\\
51	512.775380233935\\
52	508.854463822449\\
53	508.854463822449\\
54	508.854463822449\\
55	508.303138862179\\
56	509.126843303827\\
57	494.105833257054\\
58	494.105833257054\\
59	494.148130803504\\
60	444.671251913643\\
61	443.514191866588\\
62	442.239380967352\\
63	442.968252842781\\
64	441.272491616195\\
65	438.501790604142\\
66	438.942676849773\\
67	424.653309148873\\
68	422.443681597403\\
69	365.585464815118\\
70	365.535851985145\\
71	353.529117656946\\
72	352.5003487111\\
73	348.759251910178\\
74	348.393339394827\\
75	339.604051662486\\
76	339.604051662486\\
77	329.063050031282\\
78	329.063050031282\\
79	326.394102979992\\
80	324.591741367935\\
81	319.547760756068\\
82	308.783763697891\\
83	310.067182609843\\
84	304.819604373315\\
85	290.58712657093\\
86	290.965634255233\\
87	302.650745745992\\
88	296.954566666138\\
89	295.190852354474\\
90	292.238789184436\\
91	288.432502687707\\
92	288.432502687707\\
93	292.923872962937\\
94	292.923872962937\\
95	292.049565286063\\
96	292.049565286063\\
97	291.988256322216\\
98	291.988256322216\\
99	291.988256322216\\
100	292.770185749466\\
100	332.97522291967\\
99	335.713837276431\\
98	335.713837276431\\
97	335.713837276431\\
96	335.725747384082\\
95	335.725747384082\\
94	336.883748060327\\
93	336.883748060327\\
92	361.965050812435\\
91	361.965050812435\\
90	362.617648817301\\
89	363.202553971493\\
88	364.460481185827\\
87	366.491515012813\\
86	404.545835063827\\
85	407.755132716984\\
84	412.742813270634\\
83	419.902242146613\\
82	423.798773920122\\
81	430.505528013695\\
80	432.755520436696\\
79	434.219888143209\\
78	434.707509155204\\
77	434.707509155204\\
76	451.065906974887\\
75	451.065906974887\\
74	466.229071109492\\
73	466.388554275385\\
72	469.715509512888\\
71	476.066121973766\\
70	493.406903870476\\
69	494.715095649311\\
68	508.949595885612\\
67	518.403220724819\\
66	529.499313319278\\
65	535.932207077502\\
64	540.182953750364\\
63	545.169657399799\\
62	549.180247848972\\
61	551.900181173623\\
60	557.146139661725\\
59	556.36184704859\\
58	567.956025579715\\
57	567.956025579715\\
56	578.108873249376\\
55	581.060357316116\\
54	582.148971051615\\
53	582.148971051615\\
52	582.148971051615\\
51	588.47423373442\\
50	588.47423373442\\
49	609.954480562179\\
48	730.412225537835\\
47	730.515469114477\\
46	851.170547512981\\
45	854.408760794717\\
44	856.00863585638\\
43	877.245426525623\\
42	877.245426525623\\
41	877.245426525623\\
40	906.339081948972\\
39	916.829761544325\\
38	920.881709603515\\
37	920.881709603515\\
36	985.601629142738\\
35	997.934719343094\\
34	1000.17184899773\\
33	1005.73134594605\\
32	1012.31009746998\\
31	1037.02458322529\\
30	1050.77622208005\\
29	1052.61708651271\\
28	1052.61708651271\\
27	1053.30646950409\\
26	1088.37924710925\\
25	1088.37924710925\\
24	1096.85748765922\\
23	1096.85748765922\\
22	1096.85748765922\\
21	1188.49037178994\\
20	1305.42366433666\\
19	1328.15049895276\\
18	1363.38448767838\\
17	1376.76799765855\\
16	1376.82162585203\\
15	1376.82162585203\\
14	1376.82162585203\\
13	1376.82162585203\\
12	1387.50840027868\\
11	1387.50840027868\\
10	1387.50840027868\\
9	1475.30538200128\\
8	1484.54345755295\\
7	1511.26666303604\\
6	1511.11804008646\\
5	1511.11804008646\\
4	1678.15677509442\\
3	1656.19005093429\\
2	1844.83045807206\\
1	2759.79885549972\\
}--cycle;
\addplot [color=mycolor6]
  table[row sep=crcr]{%
1	2150\\
2	1542\\
3	1456\\
4	1396\\
5	1289\\
6	1289\\
7	1289\\
8	1258\\
9	1193\\
10	1110\\
11	1110\\
12	1110\\
13	1039\\
14	1039\\
15	1039\\
16	1039\\
17	1035\\
18	1015\\
19	981\\
20	973\\
21	916\\
22	884\\
23	884\\
24	884\\
25	873\\
26	873\\
27	831\\
28	829\\
29	829\\
30	827\\
31	812\\
32	790\\
33	781\\
34	770\\
35	769\\
36	754\\
37	729\\
38	729\\
39	723\\
40	699\\
41	689\\
42	689\\
43	689\\
44	678\\
45	674\\
46	665\\
47	621\\
48	620\\
49	561\\
50	551\\
51	551\\
52	546\\
53	546\\
54	546\\
55	545\\
56	544\\
57	531\\
58	531\\
59	525\\
60	501\\
61	498\\
62	496\\
63	494\\
64	491\\
65	487\\
66	484\\
67	472\\
68	466\\
69	430\\
70	429\\
71	415\\
72	411\\
73	408\\
74	407\\
75	395\\
76	395\\
77	382\\
78	382\\
79	380\\
80	379\\
81	375\\
82	366\\
83	365\\
84	359\\
85	349\\
86	348\\
87	335\\
88	331\\
89	329\\
90	327\\
91	325\\
92	325\\
93	315\\
94	315\\
95	314\\
96	314\\
97	314\\
98	314\\
99	314\\
100	313\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.5}$}


\addplot[area legend, draw=none, fill=mycolor7, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1777.28911745297\\
2	1416.10247051751\\
3	1416.10247051751\\
4	1363.64203087805\\
5	1101.88667650767\\
6	1101.88667650767\\
7	1101.88667650767\\
8	1101.88667650767\\
9	1051.86292611166\\
10	1051.86292611166\\
11	1051.86292611166\\
12	1051.86292611166\\
13	1051.86292611166\\
14	1008.78042477\\
15	1008.78042477\\
16	1008.78042477\\
17	1008.78042477\\
18	857.027919237047\\
19	857.027919237047\\
20	852.016462582213\\
21	852.016462582213\\
22	850.012148571157\\
23	850.012148571157\\
24	850.012148571157\\
25	849.594529115203\\
26	810.451198771846\\
27	810.451198771846\\
28	810.451198771846\\
29	781.415648634716\\
30	781.415648634716\\
31	773.539516051128\\
32	773.539516051128\\
33	753.868252816079\\
34	748.511500637598\\
35	710.566232301631\\
36	698.160535996126\\
37	697.377351900761\\
38	697.377351900761\\
39	683.450422912688\\
40	649.7348952428\\
41	633.402411415612\\
42	633.402411415612\\
43	630.579787886069\\
44	630.579787886069\\
45	611.17234479079\\
46	556.384919475065\\
47	545.66399896013\\
48	543.416142587108\\
49	536.352598738495\\
50	517.721781742283\\
51	512.562829967678\\
52	499.594900218568\\
53	491.865267215397\\
54	474.178303115178\\
55	464.265072465343\\
56	458.371349922037\\
57	458.371349922037\\
58	458.371349922037\\
59	454.213180465935\\
60	465.495988175354\\
61	462.433098837243\\
62	459.937273527481\\
63	459.937273527481\\
64	456.867358181428\\
65	445.801146073964\\
66	447.097382034293\\
67	446.211620727395\\
68	439.219415904334\\
69	439.219415904334\\
70	435.452258473358\\
71	432.872856259469\\
72	429.474217791181\\
73	424.803321341565\\
74	423.830951010552\\
75	423.830951010552\\
76	413.290576647843\\
77	409.05319443115\\
78	418.24667204026\\
79	400.084413403918\\
80	397.202545927681\\
81	389.628038595399\\
82	388.659322523502\\
83	389.803935893676\\
84	382.785084782676\\
85	362.189387157074\\
86	359.719591580073\\
87	351.144901095434\\
88	363.832098803462\\
89	332.042350231955\\
90	334.831857633076\\
91	334.831483304657\\
92	333.818264122132\\
93	328.914512988699\\
94	322.163058207139\\
95	322.104820602014\\
96	322.865938097148\\
97	313.362950112584\\
98	313.252118894316\\
99	311.508118126258\\
100	311.806498980865\\
100	525.338511826706\\
99	528.349158909132\\
98	528.874655749778\\
97	528.91002970577\\
96	533.049532725287\\
95	541.632272633756\\
94	541.62884393283\\
93	549.119782955774\\
92	580.843740227881\\
91	581.955063818553\\
90	582.012295382536\\
89	610.077800684124\\
88	623.377894838536\\
87	760.023894018957\\
86	834.614116713743\\
85	854.069182404918\\
84	861.534187643202\\
83	862.948306236791\\
82	873.367455067424\\
81	874.148190907579\\
80	877.985867106616\\
79	892.250572561921\\
78	902.684445617963\\
77	940.669360220277\\
76	942.768493010212\\
75	954.720222132585\\
74	954.720222132585\\
73	970.816843954447\\
72	975.062488762308\\
71	975.611585274086\\
70	976.252240726962\\
69	977.007279526246\\
68	977.007279526246\\
67	978.001633755288\\
66	978.262953194142\\
65	1068.04831639041\\
64	1069.78938322762\\
63	1070.37124282667\\
62	1070.37124282667\\
61	1070.878836247\\
60	1099.31618837467\\
59	1136.8500193033\\
58	1137.43556590555\\
57	1137.43556590555\\
56	1137.43556590555\\
55	1138.66434959331\\
54	1140.76212148877\\
53	1143.9765619077\\
52	1145.0866667897\\
51	1147.60419173872\\
50	1148.88402405535\\
49	1153.50750571623\\
48	1155.96317850204\\
47	1156.82622836264\\
46	1158.18911717511\\
45	1256.23111328244\\
44	1296.1008416598\\
43	1296.1008416598\\
42	1296.15885600089\\
41	1296.15885600089\\
40	1296.9087349117\\
39	1300.97600826197\\
38	1301.80837891351\\
37	1301.80837891351\\
36	1301.8466223485\\
35	1302.71580868651\\
34	1309.40086490566\\
33	1309.38948670299\\
32	1316.19066731723\\
31	1316.19066731723\\
30	1316.0309523964\\
29	1316.0309523964\\
28	1333.7347464149\\
27	1333.7347464149\\
26	1333.7347464149\\
25	1335.50427087315\\
24	1335.55625825763\\
23	1335.55625825763\\
22	1335.55625825763\\
21	1337.06075939047\\
20	1337.06075939047\\
19	1341.24278362979\\
18	1341.24278362979\\
17	1390.59383058479\\
16	1390.59383058479\\
15	1390.59383058479\\
14	1390.59383058479\\
13	1625.60022906434\\
12	1625.60022906434\\
11	1625.60022906434\\
10	1625.60022906434\\
9	1625.60022906434\\
8	1662.68554704435\\
7	1662.68554704435\\
6	1662.68554704435\\
5	1662.68554704435\\
4	1804.9850168649\\
3	1831.04082186412\\
2	1831.04082186412\\
1	2421.16510471306\\
}--cycle;
\addplot [color=mycolor7]
  table[row sep=crcr]{%
1	2099\\
2	1624\\
3	1624\\
4	1584\\
5	1382\\
6	1382\\
7	1382\\
8	1382\\
9	1339\\
10	1339\\
11	1339\\
12	1339\\
13	1339\\
14	1200\\
15	1200\\
16	1200\\
17	1200\\
18	1099\\
19	1099\\
20	1095\\
21	1095\\
22	1093\\
23	1093\\
24	1093\\
25	1093\\
26	1072\\
27	1072\\
28	1072\\
29	1049\\
30	1049\\
31	1045\\
32	1045\\
33	1032\\
34	1029\\
35	1007\\
36	1000\\
37	1000\\
38	1000\\
39	992\\
40	973\\
41	965\\
42	965\\
43	963\\
44	963\\
45	934\\
46	857\\
47	851\\
48	850\\
49	845\\
50	833\\
51	830\\
52	822\\
53	818\\
54	807\\
55	801\\
56	798\\
57	798\\
58	798\\
59	796\\
60	782\\
61	767\\
62	765\\
63	765\\
64	763\\
65	757\\
66	713\\
67	712\\
68	708\\
69	708\\
70	706\\
71	704\\
72	702\\
73	698\\
74	689\\
75	689\\
76	678\\
77	675\\
78	660\\
79	646\\
80	638\\
81	632\\
82	631\\
83	626\\
84	622\\
85	608\\
86	597\\
87	556\\
88	494\\
89	471\\
90	458\\
91	458\\
92	457\\
93	439\\
94	432\\
95	432\\
96	428\\
97	421\\
98	421\\
99	420\\
100	419\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.7}$}

\legend{}
\end{axis}


==> figures/arm26_reaching_hyperparameter_sigmaanalysis_c03_onlyaxis.tex <==
\begin{axis}[%
name =ax1,
scaled y ticks=base 10:\Factor,
xlabel near ticks, ylabel near ticks,
xshift=-1.0cm,
width=0.647\figW,
height=\figH,
at={(0\figW,0\figH)},
scale only axis,
xmin=0,
xmax=100,
xtick={  0,  20,  40,  60,  80, 100},
xlabel style={font=\color{white!15!black}},
xlabel={generations},
ymode=log,
ymin=280,
ymax=2500,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={cost},
axis background/.style={fill=white},
title={c = 0.3 s},
legend style={at={(1.03,0.5)}, anchor=west, legend cell align=left, align=left, draw=white!15!black}
]

\addplot[area legend, draw=none, fill=mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	610.080725726333\\
2	559.257296473224\\
3	520.882750239577\\
4	478.820467819373\\
5	388.230395069858\\
6	381.616374043357\\
7	376.203159650353\\
8	331.973050728223\\
9	342.890713439095\\
10	334.232198565178\\
11	326.863555620317\\
12	319.999711997991\\
13	323.715962444603\\
14	324.589177277104\\
15	324.589177277104\\
16	324.589177277104\\
17	324.157429937016\\
18	324.010332722175\\
19	322.680942997876\\
20	318.802256239238\\
21	318.802256239238\\
22	317.013292456386\\
23	315.31514445723\\
24	311.134316950911\\
25	311.134316950911\\
26	309.176410784935\\
27	306.735137624687\\
28	305.387281696289\\
29	303.03451983688\\
30	302.302097253956\\
31	302.668466311783\\
32	299.994806913134\\
33	299.994806913134\\
34	300.551527734446\\
35	301.050300476297\\
36	301.135737076246\\
37	301.236011198606\\
38	301.27541889656\\
39	301.400112418594\\
40	301.255260766896\\
41	301.255260766896\\
42	300.685390436115\\
43	300.305365203936\\
44	300.305365203936\\
45	299.445616680128\\
46	298.712168813696\\
47	298.712168813696\\
48	298.593461174171\\
49	297.601262225735\\
50	297.539297224312\\
51	297.082436272825\\
52	297.082436272825\\
53	297.082436272825\\
54	297.082436272825\\
55	297.082436272825\\
56	297.131614578768\\
57	297.131614578768\\
58	297.131614578768\\
59	297.131614578768\\
60	297.131614578768\\
61	296.916537322093\\
62	296.814388555559\\
63	296.81044323083\\
64	296.81044323083\\
65	296.324815276574\\
66	296.312753006003\\
67	296.374059713204\\
68	296.2092332334\\
69	296.209133778318\\
70	296.209133778318\\
71	296.276366082792\\
72	296.292761887271\\
73	296.200121445798\\
74	296.199757657216\\
75	296.192517384496\\
76	296.177280891925\\
77	296.177280891925\\
78	296.123963351698\\
79	296.12519984186\\
80	295.98411331925\\
81	295.98411331925\\
82	295.932596649031\\
83	295.932176322643\\
84	295.893581269188\\
85	295.88090293522\\
86	295.829061096107\\
87	295.805401168948\\
88	295.789260459508\\
89	295.725082862851\\
90	295.690677025299\\
91	295.6461216249\\
92	295.581273081773\\
93	295.51768975937\\
94	295.502644832136\\
95	295.503047920863\\
96	295.461731402526\\
97	295.410506393161\\
98	295.370629540324\\
99	295.395587166005\\
100	295.353401063779\\
100	296.87044562534\\
99	296.882421757491\\
98	296.960404659769\\
97	296.997836303198\\
96	297.077945192704\\
95	297.080120380834\\
94	297.091953685332\\
93	297.10267217837\\
92	297.125787382526\\
91	297.180562322514\\
90	297.191220035341\\
89	297.205965515668\\
88	297.516024844818\\
87	297.703391105297\\
86	297.702782285742\\
85	297.764989725855\\
84	297.784629540551\\
83	297.7837343534\\
82	297.783975827188\\
81	297.783146622542\\
80	297.783146622542\\
79	297.964734118342\\
78	298.002853308625\\
77	298.156406397813\\
76	298.156406397813\\
75	298.329609357716\\
74	298.421614887626\\
73	298.513984309725\\
72	298.506637668611\\
71	298.716197395805\\
70	299.144523595447\\
69	299.144523595447\\
68	299.144522543973\\
67	299.187687662668\\
66	299.732590603412\\
65	299.750125579175\\
64	299.958013632138\\
63	299.958013632138\\
62	300.683125361646\\
61	300.76800265768\\
60	301.027635337465\\
59	301.027635337465\\
58	301.027635337465\\
57	301.027635337465\\
56	301.027635337465\\
55	301.633713998557\\
54	301.633713998557\\
53	301.633713998557\\
52	301.633713998557\\
51	301.633713998557\\
50	301.71910072782\\
49	301.889836761252\\
48	301.941042934864\\
47	302.005185906115\\
46	302.005185906115\\
45	302.780391865923\\
44	303.107262272166\\
43	303.107262272166\\
42	303.111909724557\\
41	303.785628144574\\
40	303.785628144574\\
39	303.777325550524\\
38	304.570786975224\\
37	306.934225399573\\
36	307.381191816748\\
35	307.730527465405\\
34	311.082222443381\\
33	313.038782433248\\
32	313.038782433248\\
31	314.185400987419\\
30	315.488289081034\\
29	316.233338260775\\
28	316.160128922545\\
27	319.409879822912\\
26	321.946945162464\\
25	322.220488216554\\
24	322.220488216554\\
23	325.116541224163\\
22	335.446498486265\\
21	339.356384639927\\
20	339.356384639927\\
19	340.73398663949\\
18	341.130551054639\\
17	342.767547365755\\
16	343.217372974486\\
15	343.217372974486\\
14	343.217372974486\\
13	349.044782014441\\
12	366.092704047268\\
11	375.246476874377\\
10	374.881068703486\\
9	379.608694960475\\
8	442.974679831313\\
7	563.094234893714\\
6	586.235670501307\\
5	642.701444436561\\
4	813.600989772495\\
3	908.310096623366\\
2	993.039101755796\\
1	1077.74482141739\\
}--cycle;
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	844\\
2	776\\
3	715\\
4	646\\
5	515\\
6	484\\
7	470\\
8	387\\
9	361\\
10	355\\
11	351\\
12	343\\
13	336\\
14	334\\
15	334\\
16	334\\
17	333\\
18	333\\
19	332\\
20	329\\
21	329\\
22	326\\
23	320\\
24	317\\
25	317\\
26	316\\
27	313\\
28	311\\
29	310\\
30	309\\
31	308\\
32	307\\
33	307\\
34	306\\
35	304\\
36	304\\
37	304\\
38	303\\
39	303\\
40	303\\
41	303\\
42	302\\
43	302\\
44	302\\
45	301\\
46	300\\
47	300\\
48	300\\
49	300\\
50	300\\
51	299\\
52	299\\
53	299\\
54	299\\
55	299\\
56	299\\
57	299\\
58	299\\
59	299\\
60	299\\
61	299\\
62	299\\
63	298\\
64	298\\
65	298\\
66	298\\
67	298\\
68	298\\
69	298\\
70	298\\
71	297\\
72	297\\
73	297\\
74	297\\
75	297\\
76	297\\
77	297\\
78	297\\
79	297\\
80	297\\
81	297\\
82	297\\
83	297\\
84	297\\
85	297\\
86	297\\
87	297\\
88	297\\
89	296\\
90	296\\
91	296\\
92	296\\
93	296\\
94	296\\
95	296\\
96	296\\
97	296\\
98	296\\
99	296\\
100	296\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.05}$}


\addplot[area legend, draw=none, fill=red!50!mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	574.590636174493\\
2	504.482551239974\\
3	458.70557937696\\
4	412.330760226305\\
5	398.124873755798\\
6	364.368468127149\\
7	328.851416021858\\
8	327.794111282855\\
9	326.727953195728\\
10	331.726200886715\\
11	327.344674730927\\
12	326.673159800281\\
13	326.673159800281\\
14	313.619360548059\\
15	313.086857188722\\
16	310.61377553934\\
17	310.856325320687\\
18	310.116357957132\\
19	307.957383758578\\
20	307.803252887839\\
21	307.803252887839\\
22	306.594164649141\\
23	305.649406997739\\
24	305.14883579357\\
25	304.221496799892\\
26	304.221496799892\\
27	305.002377819107\\
28	304.54602386558\\
29	303.026581606118\\
30	303.317164501091\\
31	303.422119400888\\
32	303.012894040244\\
33	300.875561327285\\
34	300.165186336181\\
35	300.165186336181\\
36	300.091918602587\\
37	298.590633336832\\
38	298.590633336832\\
39	298.590633336832\\
40	298.590633336832\\
41	298.590633336832\\
42	298.604635930631\\
43	298.604635930631\\
44	298.604635930631\\
45	298.334123045413\\
46	298.333571304372\\
47	298.280368271115\\
48	298.280368271115\\
49	298.35779266451\\
50	298.167107653463\\
51	298.194209165001\\
52	297.590404390805\\
53	297.133827473878\\
54	297.180882322766\\
55	297.029490947571\\
56	296.589617892813\\
57	296.222025820482\\
58	296.079772884328\\
59	296.079772884328\\
60	295.917420624695\\
61	295.917420624695\\
62	295.903038158445\\
63	295.967875153182\\
64	295.965451565458\\
65	296.013756898799\\
66	295.984527292368\\
67	295.963882400963\\
68	296.128213389346\\
69	296.118700575655\\
70	296.118756867134\\
71	296.123181860633\\
72	295.998421531238\\
73	295.998421531238\\
74	295.993496165583\\
75	295.967122816138\\
76	295.921804294985\\
77	295.921804294985\\
78	295.921804294985\\
79	295.921526821156\\
80	295.921526821156\\
81	295.920213044568\\
82	295.901235052945\\
83	295.882129576275\\
84	295.863205432848\\
85	295.77624015162\\
86	295.77624015162\\
87	295.758670216226\\
88	295.730634900326\\
89	295.658309974363\\
90	295.631753174279\\
91	295.597906810601\\
92	295.613544352319\\
93	295.616955089257\\
94	295.615909935295\\
95	295.604479329906\\
96	295.563042250387\\
97	295.546894631966\\
98	295.522349096408\\
99	295.506536657252\\
100	295.506536657252\\
100	296.144637550393\\
99	296.144637550393\\
98	296.149433367371\\
97	296.18305166399\\
96	296.179967241419\\
95	296.261596283954\\
94	296.262915145364\\
93	296.263173690715\\
92	296.314348657191\\
91	296.422156253042\\
90	296.4809543039\\
89	296.515336978292\\
88	296.667163258091\\
87	296.663757717614\\
86	296.695481999996\\
85	296.695481999996\\
84	297.114392468841\\
83	297.110875779203\\
82	297.15706461902\\
81	297.182220578333\\
80	297.181987499288\\
79	297.181987499288\\
78	297.291552576785\\
77	297.291552576785\\
76	297.291552576785\\
75	297.309666588504\\
74	297.361170132629\\
73	297.910659493061\\
72	297.910659493061\\
71	297.921853310219\\
70	299.242977627121\\
69	299.317055374767\\
68	299.372265106167\\
67	300.510212722299\\
66	300.509426833982\\
65	300.570164476365\\
64	300.753441106708\\
63	300.758412293751\\
62	300.997188675399\\
61	301.024409954541\\
60	301.024409954541\\
59	301.166577385912\\
58	301.166577385912\\
57	301.375651801643\\
56	301.407157080866\\
55	301.364321217721\\
54	301.754347051692\\
53	301.973271713564\\
52	302.237869723555\\
51	302.576112757207\\
50	303.666332243144\\
49	303.644046740759\\
48	304.050063519826\\
47	304.050063519826\\
46	304.54467109203\\
45	304.707924261426\\
44	304.980622247648\\
43	304.980622247648\\
42	304.980622247648\\
41	305.484509684879\\
40	305.484509684879\\
39	305.484509684879\\
38	305.484509684879\\
37	305.484509684879\\
36	305.783399101254\\
35	305.921810432195\\
34	305.921810432195\\
33	306.451376543144\\
32	305.897403477023\\
31	305.968971101339\\
30	307.480703308149\\
29	308.59168335019\\
28	310.703451216571\\
27	310.705073452704\\
26	313.815765600946\\
25	313.815765600946\\
24	315.48409611199\\
23	322.666931218638\\
22	332.33238268832\\
21	332.773249345197\\
20	332.773249345197\\
19	332.85222213892\\
18	335.163661571831\\
17	335.480971139473\\
16	347.332621577132\\
15	355.385843731124\\
14	355.492928298716\\
13	360.462371119615\\
12	360.462371119615\\
11	364.217965255135\\
10	364.242639050921\\
9	425.447328347945\\
8	428.193626034796\\
7	458.091773023166\\
6	498.533226664248\\
5	598.3137171518\\
4	634.040390563704\\
3	722.329316913036\\
2	861.43770922437\\
1	999.852936397043\\
}--cycle;
\addplot [color=red!50!mycolor1]
  table[row sep=crcr]{%
1	787\\
2	683\\
3	591\\
4	523\\
5	498\\
6	431\\
7	393\\
8	378\\
9	376\\
10	348\\
11	346\\
12	344\\
13	344\\
14	335\\
15	334\\
16	329\\
17	323\\
18	323\\
19	320\\
20	320\\
21	320\\
22	319\\
23	314\\
24	310\\
25	309\\
26	309\\
27	308\\
28	308\\
29	306\\
30	305\\
31	305\\
32	304\\
33	304\\
34	303\\
35	303\\
36	303\\
37	302\\
38	302\\
39	302\\
40	302\\
41	302\\
42	302\\
43	302\\
44	302\\
45	302\\
46	301\\
47	301\\
48	301\\
49	301\\
50	301\\
51	300\\
52	300\\
53	300\\
54	299\\
55	299\\
56	299\\
57	299\\
58	299\\
59	299\\
60	298\\
61	298\\
62	298\\
63	298\\
64	298\\
65	298\\
66	298\\
67	298\\
68	298\\
69	298\\
70	298\\
71	297\\
72	297\\
73	297\\
74	297\\
75	297\\
76	297\\
77	297\\
78	297\\
79	297\\
80	297\\
81	297\\
82	297\\
83	296\\
84	296\\
85	296\\
86	296\\
87	296\\
88	296\\
89	296\\
90	296\\
91	296\\
92	296\\
93	296\\
94	296\\
95	296\\
96	296\\
97	296\\
98	296\\
99	296\\
100	296\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.1}$}


\addplot[area legend, draw=none, fill=red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	478.784964605733\\
2	405.471064872286\\
3	371.293077597947\\
4	334.211355718086\\
5	307.72086890057\\
6	314.992386608893\\
7	309.494558607774\\
8	314.80792297688\\
9	316.945715123061\\
10	320.254359515838\\
11	320.254359515838\\
12	321.522045810314\\
13	321.522045810314\\
14	321.593397134307\\
15	315.080002510151\\
16	315.440630126395\\
17	315.052452168554\\
18	315.768254645231\\
19	314.982019815006\\
20	312.292325636975\\
21	311.250962132487\\
22	311.20627700475\\
23	309.546729077254\\
24	307.864576436952\\
25	307.733989558666\\
26	307.738727936513\\
27	306.968471738838\\
28	306.903692317399\\
29	306.903692317399\\
30	302.720290737671\\
31	302.049444733298\\
32	301.098596324628\\
33	300.86232388654\\
34	300.896349498827\\
35	301.2500477729\\
36	299.493512580349\\
37	299.493512580349\\
38	299.058271870041\\
39	299.971851466504\\
40	299.27014701626\\
41	298.7326150187\\
42	298.688094535372\\
43	298.688094535372\\
44	298.872348590486\\
45	298.818975230423\\
46	298.663696096775\\
47	298.632724864559\\
48	298.30039004882\\
49	298.263747831709\\
50	298.054445519377\\
51	297.769434461424\\
52	297.645645914504\\
53	297.645645914504\\
54	297.798436488542\\
55	297.441368811099\\
56	297.474038740806\\
57	297.463196541043\\
58	297.075002375787\\
59	297.075002375787\\
60	297.091501870633\\
61	297.14738620463\\
62	297.063581419628\\
63	297.063581419628\\
64	297.066901738977\\
65	296.96040675893\\
66	296.905477221653\\
67	296.73239123112\\
68	296.679288939549\\
69	296.38193836614\\
70	296.38193836614\\
71	296.258263077049\\
72	296.258263077049\\
73	296.096515432179\\
74	296.064794076049\\
75	295.878982979178\\
76	295.878982979178\\
77	295.874079302839\\
78	295.807449262563\\
79	295.807449262563\\
80	295.829974509044\\
81	295.80705517866\\
82	295.748636480224\\
83	295.690104573764\\
84	295.620965874913\\
85	295.531053499314\\
86	295.507753271011\\
87	295.503806281136\\
88	295.490050992914\\
89	295.471324035258\\
90	295.469055603906\\
91	295.466708822964\\
92	295.322785658597\\
93	295.322785658597\\
94	295.319357104251\\
95	295.213290065541\\
96	295.225047984934\\
97	295.218750949224\\
98	295.241732960207\\
99	295.185141706945\\
100	295.207515905097\\
100	296.586373624062\\
99	296.744789154563\\
98	296.758481322761\\
97	296.830223682989\\
96	296.84529919263\\
95	296.881890366744\\
94	296.926320742229\\
93	296.927465114184\\
92	296.927465114184\\
91	297.046559951219\\
90	297.046520721542\\
89	297.144622496289\\
88	297.271015503229\\
87	297.271253964249\\
86	297.272554508571\\
85	297.274976148588\\
84	297.31587165495\\
83	297.37105387912\\
82	297.534131463404\\
81	297.528366169792\\
80	297.52850887704\\
79	297.702675576991\\
78	297.702675576991\\
77	297.744711387975\\
76	297.808055619363\\
75	297.808055619363\\
74	297.824411043288\\
73	297.82029600616\\
72	298.112071739658\\
71	298.112071739658\\
70	298.127744495144\\
69	298.127744495144\\
68	298.444783258253\\
67	298.51816438613\\
66	298.791119361473\\
65	298.864810448537\\
64	299.448562220308\\
63	299.486941558375\\
62	299.486941558375\\
61	299.466518094596\\
60	299.822723559806\\
59	299.932578654324\\
58	299.932578654324\\
57	300.324016439382\\
56	300.473936213258\\
55	300.758478320026\\
54	300.957036842652\\
53	301.79806761209\\
52	301.79806761209\\
51	301.883617082383\\
50	301.938875423132\\
49	302.019544363849\\
48	302.090969132876\\
47	302.124407350267\\
46	302.155450503061\\
45	302.430556773513\\
44	303.155189568671\\
43	304.468835760873\\
42	304.468835760873\\
41	304.925579773449\\
40	306.661043106797\\
39	306.864639193877\\
38	309.949401243958\\
37	310.070071099272\\
36	310.070071099272\\
35	310.768267538967\\
34	311.925858288884\\
33	312.392857328035\\
32	312.415955980691\\
31	313.335379799198\\
30	313.493741306611\\
29	315.426303195577\\
28	315.426303195577\\
27	317.791511387295\\
26	318.864199388826\\
25	319.057883109539\\
24	319.347361658081\\
23	321.478311072659\\
22	321.941704326059\\
21	322.468406608785\\
20	327.116203869101\\
19	328.277876371554\\
18	329.64644410863\\
17	332.763691791231\\
16	333.545560136616\\
15	341.132416208063\\
14	349.101152806001\\
13	349.792668213235\\
12	349.792668213235\\
11	363.250716867875\\
10	363.250716867875\\
9	395.456901363967\\
8	402.427850686458\\
7	434.902433668952\\
6	463.030045055925\\
5	504.219555150483\\
4	581.319239144814\\
3	636.122637822107\\
2	724.181215955365\\
1	875.388880002082\\
}--cycle;
\addplot [color=red]
  table[row sep=crcr]{%
1	677\\
2	565\\
3	504\\
4	458\\
5	406\\
6	389\\
7	372\\
8	359\\
9	356\\
10	342\\
11	342\\
12	336\\
13	336\\
14	335\\
15	328\\
16	324\\
17	324\\
18	323\\
19	322\\
20	320\\
21	317\\
22	317\\
23	316\\
24	314\\
25	313\\
26	313\\
27	312\\
28	311\\
29	311\\
30	308\\
31	308\\
32	307\\
33	307\\
34	306\\
35	306\\
36	305\\
37	305\\
38	305\\
39	303\\
40	303\\
41	302\\
42	302\\
43	302\\
44	301\\
45	301\\
46	300\\
47	300\\
48	300\\
49	300\\
50	300\\
51	300\\
52	300\\
53	300\\
54	299\\
55	299\\
56	299\\
57	299\\
58	299\\
59	299\\
60	298\\
61	298\\
62	298\\
63	298\\
64	298\\
65	298\\
66	298\\
67	298\\
68	298\\
69	297\\
70	297\\
71	297\\
72	297\\
73	297\\
74	297\\
75	297\\
76	297\\
77	297\\
78	297\\
79	297\\
80	297\\
81	297\\
82	297\\
83	297\\
84	296\\
85	296\\
86	296\\
87	296\\
88	296\\
89	296\\
90	296\\
91	296\\
92	296\\
93	296\\
94	296\\
95	296\\
96	296\\
97	296\\
98	296\\
99	296\\
100	296\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.2}$}


\addplot[area legend, draw=none, fill=mycolor2, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	440.880384858302\\
2	410.752588592428\\
3	353.215811261925\\
4	353.215811261925\\
5	346.465807572189\\
6	325.98720373934\\
7	325.98720373934\\
8	326.351543170665\\
9	322.714434434859\\
10	321.797038590862\\
11	316.596997811258\\
12	314.751469779706\\
13	310.102271278369\\
14	308.432411528166\\
15	308.432411528166\\
16	308.432411528166\\
17	309.142918770485\\
18	310.191176041378\\
19	310.191176041378\\
20	307.395353519551\\
21	306.443353087053\\
22	307.159189802365\\
23	304.987901595467\\
24	301.947036314267\\
25	300.039666984919\\
26	300.039666984919\\
27	300.670117219709\\
28	300.815670526351\\
29	300.815670526351\\
30	300.551227064412\\
31	300.336283501157\\
32	300.336283501157\\
33	300.336283501157\\
34	300.336283501157\\
35	300.336283501157\\
36	300.336283501157\\
37	300.034430551224\\
38	300.034430551224\\
39	300.034430551224\\
40	299.772980117173\\
41	299.772980117173\\
42	299.765417210216\\
43	299.563910286052\\
44	298.950123754916\\
45	298.950123754916\\
46	298.950123754916\\
47	297.897404309196\\
48	297.319053146285\\
49	297.336510187199\\
50	297.211598318053\\
51	297.178876950506\\
52	297.123528109215\\
53	296.974110752804\\
54	296.974110752804\\
55	297.037526683998\\
56	297.037526683998\\
57	297.01588374582\\
58	296.884830571919\\
59	296.88362586397\\
60	296.864463208863\\
61	296.717206208773\\
62	296.692271010581\\
63	296.525840876333\\
64	296.448173044543\\
65	296.448173044543\\
66	296.319518038293\\
67	296.319518038293\\
68	296.319518038293\\
69	296.319518038293\\
70	296.303947817225\\
71	296.303947817225\\
72	296.235051113069\\
73	296.086333446495\\
74	296.024735323272\\
75	295.9276750708\\
76	295.9276750708\\
77	295.894866089181\\
78	295.880134302369\\
79	295.81057841128\\
80	295.81057841128\\
81	295.800147309807\\
82	295.786434836542\\
83	295.750837513128\\
84	295.759746286468\\
85	295.71423312612\\
86	295.71423312612\\
87	295.624681433615\\
88	295.633833143323\\
89	295.634483876064\\
90	295.609834312176\\
91	295.565468971277\\
92	295.543578827746\\
93	295.543578827746\\
94	295.514057425512\\
95	295.484996006689\\
96	295.48402749903\\
97	295.486882189795\\
98	295.480231476633\\
99	295.480231476633\\
100	295.472439071108\\
100	295.818737145113\\
99	295.817311894906\\
98	295.817311894906\\
97	295.841713514383\\
96	295.905943842214\\
95	295.909031329182\\
94	295.92246423966\\
93	295.937170986756\\
92	295.937170986756\\
91	295.933040062725\\
90	296.120578896222\\
89	296.121507824209\\
88	296.222565376512\\
87	296.261257436637\\
86	296.305177241054\\
85	296.305177241054\\
84	296.528271715951\\
83	296.605944612213\\
82	296.626415194969\\
81	296.652959864406\\
80	296.745257460848\\
79	296.745257460848\\
78	296.756496143204\\
77	296.925201044799\\
76	296.929594712163\\
75	296.929594712163\\
74	296.952160383374\\
73	297.004207533998\\
72	297.185297927193\\
71	297.283354821545\\
70	297.283354821545\\
69	297.470894352798\\
68	297.470894352798\\
67	297.470894352798\\
66	297.470894352798\\
65	297.43611664023\\
64	297.43611664023\\
63	297.555173908989\\
62	297.509065455661\\
61	297.905281303661\\
60	298.380728987917\\
59	298.454209851409\\
58	298.46637777703\\
57	298.442538981863\\
56	298.646791500761\\
55	298.646791500761\\
54	299.165574525435\\
53	299.165574525435\\
52	299.369445144248\\
51	300.272538108846\\
50	300.333802333029\\
49	301.697647789468\\
48	301.799047895832\\
47	301.86965388416\\
46	301.956864979236\\
45	301.956864979236\\
44	301.956864979236\\
43	302.046154602219\\
42	302.065284782973\\
41	302.066831408835\\
40	302.066831408835\\
39	303.19801166423\\
38	303.19801166423\\
37	303.19801166423\\
36	303.24694625132\\
35	303.24694625132\\
34	303.24694625132\\
33	303.24694625132\\
32	303.24694625132\\
31	303.24694625132\\
30	304.943114444573\\
29	308.773431778368\\
28	308.773431778368\\
27	309.228397616204\\
26	311.175201467532\\
25	311.175201467532\\
24	318.373875074698\\
23	319.866989381276\\
22	321.565377393571\\
21	323.916143173755\\
20	324.193804108555\\
19	325.323271817311\\
18	325.323271817311\\
17	340.207822912717\\
16	342.535142015858\\
15	342.535142015858\\
14	342.535142015858\\
13	343.597913618077\\
12	344.343396391995\\
11	346.95765061288\\
10	348.842235862543\\
9	351.785394088166\\
8	356.872405444585\\
7	366.750347939384\\
6	366.750347939384\\
5	396.83344173172\\
4	433.268225216219\\
3	433.268225216219\\
2	501.006350769537\\
1	595.010127525404\\
}--cycle;
\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	518\\
2	456\\
3	393\\
4	393\\
5	372\\
6	346\\
7	346\\
8	342\\
9	337\\
10	335\\
11	332\\
12	330\\
13	327\\
14	325\\
15	325\\
16	325\\
17	325\\
18	318\\
19	318\\
20	316\\
21	315\\
22	314\\
23	312\\
24	310\\
25	306\\
26	306\\
27	305\\
28	305\\
29	305\\
30	303\\
31	302\\
32	302\\
33	302\\
34	302\\
35	302\\
36	302\\
37	302\\
38	302\\
39	302\\
40	301\\
41	301\\
42	301\\
43	301\\
44	300\\
45	300\\
46	300\\
47	300\\
48	300\\
49	300\\
50	299\\
51	299\\
52	298\\
53	298\\
54	298\\
55	298\\
56	298\\
57	298\\
58	298\\
59	298\\
60	298\\
61	297\\
62	297\\
63	297\\
64	297\\
65	297\\
66	297\\
67	297\\
68	297\\
69	297\\
70	297\\
71	297\\
72	297\\
73	297\\
74	296\\
75	296\\
76	296\\
77	296\\
78	296\\
79	296\\
80	296\\
81	296\\
82	296\\
83	296\\
84	296\\
85	296\\
86	296\\
87	296\\
88	296\\
89	296\\
90	296\\
91	296\\
92	296\\
93	296\\
94	296\\
95	296\\
96	296\\
97	296\\
98	296\\
99	296\\
100	296\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.5}$}


\addplot[area legend, draw=none, fill=mycolor3, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	424.209091812354\\
2	385.854861403863\\
3	388.378989002235\\
4	356.578338467151\\
5	356.578338467151\\
6	356.578338467151\\
7	363.624209443316\\
8	348.163911455242\\
9	348.163911455242\\
10	347.140027610186\\
11	347.140027610186\\
12	340.913346596959\\
13	342.842032770787\\
14	333.456448724994\\
15	329.671440944521\\
16	328.26878647854\\
17	322.768871894891\\
18	322.768871894891\\
19	322.768871894891\\
20	321.74380863981\\
21	319.536749572431\\
22	318.437246551281\\
23	318.111198166746\\
24	317.821921170461\\
25	313.966246594024\\
26	312.734349582798\\
27	312.734349582798\\
28	308.12054912292\\
29	306.858800086392\\
30	306.858800086392\\
31	306.676364458186\\
32	307.620492658136\\
33	305.564031629495\\
34	303.518994175049\\
35	303.34102415712\\
36	301.156212495486\\
37	300.776527923784\\
38	300.638970947066\\
39	301.809037311395\\
40	301.586757503405\\
41	301.356604042096\\
42	301.356604042096\\
43	301.356604042096\\
44	301.356604042096\\
45	301.356604042096\\
46	301.356604042096\\
47	300.494254850588\\
48	300.306230035745\\
49	299.941831952574\\
50	299.179179895808\\
51	299.179179895808\\
52	299.15165417468\\
53	299.481562517862\\
54	299.167329882398\\
55	298.895308849801\\
56	298.543407961176\\
57	298.560415422866\\
58	297.782341139522\\
59	297.210221312889\\
60	296.713964110145\\
61	296.665533512413\\
62	296.640961003316\\
63	296.283760715055\\
64	296.283760715055\\
65	296.86429045866\\
66	296.949400303922\\
67	296.949400303922\\
68	296.976108851566\\
69	296.658227394065\\
70	296.658227394065\\
71	296.647548747519\\
72	296.419606805924\\
73	296.3819765352\\
74	296.258816530866\\
75	296.002508019176\\
76	295.969202401674\\
77	295.969202401674\\
78	295.840036323747\\
79	295.883083529046\\
80	295.92207812703\\
81	295.873255527919\\
82	295.851099675353\\
83	295.81591342464\\
84	295.801954139206\\
85	295.801954139206\\
86	295.770899268893\\
87	295.871416732358\\
88	295.834814063449\\
89	295.865091095588\\
90	295.76038371583\\
91	295.709291823956\\
92	295.660284309977\\
93	295.642307728845\\
94	295.600015866424\\
95	295.584449571355\\
96	295.631211175505\\
97	295.658769729621\\
98	295.639343660521\\
99	295.6275340118\\
100	295.623020554947\\
100	296.743812807484\\
99	296.744333976475\\
98	296.745923812977\\
97	296.748855546021\\
96	297.01656720471\\
95	297.297937890565\\
94	297.300376099678\\
93	297.484725308558\\
92	297.487539235934\\
91	297.493802939672\\
90	297.523591121724\\
89	297.615723955734\\
88	298.19239098186\\
87	298.202202630927\\
86	298.646749227008\\
85	298.65564471329\\
84	298.65564471329\\
83	298.721772183956\\
82	298.74479841966\\
81	298.750362898857\\
80	298.752794792054\\
79	299.112189165887\\
78	299.513050606562\\
77	299.527886671762\\
76	299.527886671762\\
75	299.648560511777\\
74	299.673567382542\\
73	299.696015732459\\
72	299.705773613191\\
71	299.788515038929\\
70	300.767923862733\\
69	300.767923862733\\
68	300.769632275512\\
67	300.927376669941\\
66	300.927376669941\\
65	301.809946283686\\
64	304.179642709671\\
63	304.179642709671\\
62	304.945586183223\\
61	305.356046164378\\
60	305.497634962131\\
59	305.611311421065\\
58	306.884403192717\\
57	306.948561340244\\
56	307.014221639801\\
55	307.054526600844\\
54	307.102820898447\\
53	307.198961067337\\
52	308.418125965965\\
51	308.428778456016\\
50	308.428778456016\\
49	308.657148081397\\
48	309.952877818619\\
47	310.433689163799\\
46	311.308809916856\\
45	311.308809916856\\
44	311.308809916856\\
43	311.308809916856\\
42	311.308809916856\\
41	311.308809916856\\
40	311.382222092423\\
39	311.500647533729\\
38	317.327367088323\\
37	317.387246825038\\
36	325.403246803427\\
35	328.358122827696\\
34	328.387901448606\\
33	328.632370974356\\
32	329.305796546531\\
31	341.435945502282\\
30	341.502923465462\\
29	341.502923465462\\
28	342.118618989738\\
27	343.48726764311\\
26	343.48726764311\\
25	344.170070836283\\
24	343.764035955071\\
23	343.923812429082\\
22	344.135292026018\\
21	345.233100692602\\
20	351.979419700358\\
19	352.137449016844\\
18	352.137449016844\\
17	352.137449016844\\
16	351.698244139694\\
15	352.980572401079\\
14	357.307087671304\\
13	360.733620526586\\
12	381.703849426946\\
11	422.313936020997\\
10	422.313936020997\\
9	424.870902047458\\
8	424.870902047458\\
7	437.294573328321\\
6	466.644135850336\\
5	466.644135850336\\
4	466.644135850336\\
3	481.745579656083\\
2	543.661067974226\\
1	649.363254972089\\
}--cycle;
\addplot [color=mycolor3]
  table[row sep=crcr]{%
1	537\\
2	465\\
3	435\\
4	412\\
5	412\\
6	412\\
7	400\\
8	387\\
9	387\\
10	385\\
11	385\\
12	361\\
13	352\\
14	345\\
15	341\\
16	340\\
17	337\\
18	337\\
19	337\\
20	337\\
21	332\\
22	331\\
23	331\\
24	331\\
25	329\\
26	328\\
27	328\\
28	325\\
29	324\\
30	324\\
31	324\\
32	318\\
33	317\\
34	316\\
35	316\\
36	313\\
37	309\\
38	309\\
39	307\\
40	306\\
41	306\\
42	306\\
43	306\\
44	306\\
45	306\\
46	306\\
47	305\\
48	305\\
49	304\\
50	304\\
51	304\\
52	304\\
53	303\\
54	303\\
55	303\\
56	303\\
57	303\\
58	302\\
59	301\\
60	301\\
61	301\\
62	301\\
63	300\\
64	300\\
65	299\\
66	299\\
67	299\\
68	299\\
69	299\\
70	299\\
71	298\\
72	298\\
73	298\\
74	298\\
75	298\\
76	298\\
77	298\\
78	298\\
79	297\\
80	297\\
81	297\\
82	297\\
83	297\\
84	297\\
85	297\\
86	297\\
87	297\\
88	297\\
89	297\\
90	297\\
91	297\\
92	297\\
93	297\\
94	296\\
95	296\\
96	296\\
97	296\\
98	296\\
99	296\\
100	296\\
};
\addlegendentry{$\text{muscles, }\sigma\text{ = 0.7}$}


\addplot[area legend, draw=none, fill=blue, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1486.29866766228\\
2	1237.04784163398\\
3	921.664254907592\\
4	921.228739626176\\
5	844.224399960841\\
6	676.418537718795\\
7	606.511568923339\\
8	625.050178324099\\
9	437.893721388338\\
10	458.303216542483\\
11	499.36774498596\\
12	499.36774498596\\
13	490.11587011374\\
14	493.396608372521\\
15	482.845984746894\\
16	482.845984746894\\
17	490.505298350077\\
18	485.105765868267\\
19	487.003967100068\\
20	466.216786627253\\
21	466.216786627253\\
22	466.088908996226\\
23	466.088908996226\\
24	466.088908996226\\
25	459.699188315744\\
26	459.699188315744\\
27	457.389891131375\\
28	452.115406740434\\
29	439.67472812902\\
30	435.049939576593\\
31	435.041369453433\\
32	433.795008291412\\
33	421.457353112661\\
34	413.502932423109\\
35	413.502932423109\\
36	378.658796541772\\
37	372.39567532594\\
38	369.94546900188\\
39	369.94546900188\\
40	360.274548553219\\
41	358.929688527525\\
42	354.628559646979\\
43	349.75916441186\\
44	347.537886922596\\
45	355.210600713245\\
46	354.706058135111\\
47	361.453279749386\\
48	361.453279749386\\
49	361.453279749386\\
50	362.169728463792\\
51	364.311560340587\\
52	362.707928889271\\
53	361.997150364857\\
54	360.680039576514\\
55	360.100436244253\\
56	360.565681141837\\
57	360.381874607361\\
58	360.384114540212\\
59	359.564637870526\\
60	359.762798732182\\
61	359.385221263286\\
62	359.502425023374\\
63	359.634035378318\\
64	359.771759370387\\
65	359.708817762464\\
66	359.69713615926\\
67	359.876585508466\\
68	360.217447349478\\
69	360.054224392378\\
70	360.000355451914\\
71	360.132653244328\\
72	360.105770297336\\
73	360.044007238656\\
74	360.115617400202\\
75	360.011666650376\\
76	360.011666650376\\
77	359.941012429656\\
78	359.986880279142\\
79	359.976326418257\\
80	359.975871797668\\
81	359.975871797668\\
82	359.995152557831\\
83	359.995152557831\\
84	359.993198402265\\
85	359.981893219532\\
86	359.982938227363\\
87	359.982938227363\\
88	359.982938227363\\
89	359.999343183456\\
90	359.99918371073\\
91	360.006522489289\\
92	360.006522489289\\
93	360.006522489289\\
94	360.008069703984\\
95	360.008069703984\\
96	360.008069703984\\
97	360.008069703984\\
98	360.008001350738\\
99	360.00474661807\\
100	359.998804085519\\
100	448.80000227642\\
99	448.857293029129\\
98	448.857621972876\\
97	448.857628883929\\
96	448.857628883929\\
95	448.857628883929\\
94	448.857628883929\\
93	448.872872922577\\
92	448.872872922577\\
91	448.872872922577\\
90	448.944864008432\\
89	448.944880132968\\
88	449.105998345015\\
87	449.105998345015\\
86	449.105998345015\\
85	449.116646707839\\
84	449.241506073277\\
83	449.241703152772\\
82	449.241703152772\\
81	449.459274617846\\
80	449.459274617846\\
79	449.459320422938\\
78	449.460386776243\\
77	449.897167594373\\
76	450.0556242309\\
75	450.0556242309\\
74	450.066327726257\\
73	450.744237523594\\
72	451.282390599322\\
71	451.416710026794\\
70	452.534662291136\\
69	452.647199885884\\
68	452.717738506802\\
67	455.517491097429\\
66	457.338077879504\\
65	457.62484455643\\
64	457.768982577169\\
63	459.97786194421\\
62	461.499857102495\\
61	464.159750484218\\
60	464.954447067822\\
59	466.996592942355\\
58	467.928227490078\\
57	468.672274147225\\
56	468.691427795856\\
55	472.104123975494\\
54	473.097653741748\\
53	473.284854928615\\
52	474.278528974514\\
51	474.870269008373\\
50	491.869531723932\\
49	500.289479810366\\
48	500.289479810366\\
47	500.289479810366\\
46	536.39160500374\\
45	536.44328456618\\
44	563.886156292602\\
43	573.21303367881\\
42	574.557231052345\\
41	576.694728639923\\
40	576.807091671256\\
39	578.43003649826\\
38	578.43003649826\\
37	579.361410754698\\
36	581.533544924601\\
35	612.160469491839\\
34	612.160469491839\\
33	616.805969776963\\
32	626.56316604679\\
31	627.786095509834\\
30	627.79494988521\\
29	627.484166348087\\
28	636.962566139188\\
27	649.713513149165\\
26	659.740378993718\\
25	659.740378993718\\
24	675.158949790327\\
23	675.158949790327\\
22	675.158949790327\\
21	680.074455468129\\
20	680.074455468129\\
19	675.696180478889\\
18	690.611535502531\\
17	753.585683864031\\
16	780.706663293693\\
15	780.706663293693\\
14	781.280245048575\\
13	792.319972523722\\
12	817.520485290294\\
11	817.520485290294\\
10	963.140401544898\\
9	1029.45599901274\\
8	1134.8208229802\\
7	1263.63684170926\\
6	1297.715104444\\
5	1447.1811160799\\
4	1687.5080274347\\
3	1841.72078762697\\
2	2379.0227415859\\
1	2751.25996521179\\
}--cycle;
\addplot [color=blue]
  table[row sep=crcr]{%
1	2119\\
2	1808\\
3	1382\\
4	1304\\
5	1146\\
6	987\\
7	935\\
8	880\\
9	734\\
10	711\\
11	658\\
12	658\\
13	641\\
14	637\\
15	632\\
16	632\\
17	622\\
18	588\\
19	581\\
20	573\\
21	573\\
22	571\\
23	571\\
24	571\\
25	560\\
26	560\\
27	554\\
28	545\\
29	534\\
30	531\\
31	531\\
32	530\\
33	519\\
34	513\\
35	513\\
36	480\\
37	476\\
38	474\\
39	474\\
40	469\\
41	468\\
42	465\\
43	461\\
44	456\\
45	446\\
46	446\\
47	431\\
48	431\\
49	431\\
50	427\\
51	420\\
52	418\\
53	418\\
54	417\\
55	416\\
56	415\\
57	415\\
58	414\\
59	413\\
60	412\\
61	412\\
62	411\\
63	410\\
64	409\\
65	409\\
66	409\\
67	408\\
68	406\\
69	406\\
70	406\\
71	406\\
72	406\\
73	405\\
74	405\\
75	405\\
76	405\\
77	405\\
78	405\\
79	405\\
80	405\\
81	405\\
82	405\\
83	405\\
84	405\\
85	405\\
86	405\\
87	405\\
88	405\\
89	404\\
90	404\\
91	404\\
92	404\\
93	404\\
94	404\\
95	404\\
96	404\\
97	404\\
98	404\\
99	404\\
100	404\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.05}$}


\addplot[area legend, draw=none, fill=mycolor4, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1105.4300358003\\
2	1012.50568610285\\
3	723.050700225884\\
4	664.824553909692\\
5	577.844122042644\\
6	624.276905277525\\
7	616.051175613504\\
8	634.035878643123\\
9	634.035878643123\\
10	606.559183618427\\
11	606.559183618427\\
12	608.323043334369\\
13	603.889414222595\\
14	612.453347718784\\
15	612.453347718784\\
16	570.126665468166\\
17	559.334881732407\\
18	552.128547237413\\
19	549.338802846146\\
20	493.720574225866\\
21	480.908184588012\\
22	480.584912601675\\
23	474.393647629349\\
24	464.792503574289\\
25	466.668837601548\\
26	458.699464015059\\
27	460.538652163947\\
28	466.910742710675\\
29	453.296603460256\\
30	431.105474179125\\
31	432.058206717147\\
32	430.036984067653\\
33	409.932265079408\\
34	400.73295045679\\
35	381.979149957707\\
36	379.813077504848\\
37	377.43317888439\\
38	367.81930685578\\
39	363.626889091953\\
40	363.303732316622\\
41	363.303732316622\\
42	361.007945580887\\
43	367.135911694038\\
44	368.253116040071\\
45	367.608888693649\\
46	370.508746598937\\
47	369.039891108776\\
48	368.21419590836\\
49	369.69354271724\\
50	366.108577327354\\
51	365.385268274802\\
52	365.237183347076\\
53	366.009671659701\\
54	367.122479308969\\
55	368.903017755013\\
56	368.731850486535\\
57	368.639645688488\\
58	368.628232309984\\
59	369.233836824136\\
60	368.67884983383\\
61	368.559218982762\\
62	368.237207812444\\
63	368.409821528684\\
64	368.490884119099\\
65	368.439829040411\\
66	368.491112286196\\
67	368.352935622716\\
68	368.247698141632\\
69	368.26667440527\\
70	368.240744150961\\
71	368.254204127993\\
72	368.186651203908\\
73	368.179519657045\\
74	368.132152775105\\
75	368.127379057449\\
76	368.127099783874\\
77	368.123340410328\\
78	368.179798148195\\
79	368.170596719609\\
80	368.166113808613\\
81	368.162499184646\\
82	368.16729659929\\
83	368.16729659929\\
84	368.16729659929\\
85	368.165235453812\\
86	368.165235453812\\
87	368.1692494935\\
88	368.169162494317\\
89	368.159688223211\\
90	368.159273348956\\
91	368.159151068186\\
92	368.159151068186\\
93	368.143814433274\\
94	368.143633524576\\
95	368.143621242358\\
96	368.143621242358\\
97	368.143591562959\\
98	368.143591562959\\
99	368.143591562959\\
100	368.143513845215\\
100	368.170172351876\\
99	368.170700879096\\
98	368.170700879096\\
97	368.170700879096\\
96	368.170867058161\\
95	368.170867058161\\
94	368.170940991504\\
93	368.172166234564\\
92	368.171953438726\\
91	368.171953438726\\
90	368.174086956174\\
89	368.174730448367\\
88	368.173277625431\\
87	368.173291108158\\
86	368.19510445378\\
85	368.19510445378\\
84	368.197999234802\\
83	368.197999234802\\
82	368.197999234802\\
81	368.221281254119\\
80	368.222132391588\\
79	368.230687116709\\
78	368.233957513072\\
77	368.413666048567\\
76	368.415327193943\\
75	368.415405548564\\
74	368.416471906934\\
73	368.456424220263\\
72	368.621430884962\\
71	368.713378982989\\
70	368.771675057784\\
69	368.841380741636\\
68	369.516999859005\\
67	369.647509120423\\
66	369.701645113004\\
65	369.98744527492\\
64	370.0262727611\\
63	370.507808531372\\
62	371.816145927456\\
61	371.996506060581\\
60	372.070052404203\\
59	372.427275828216\\
58	375.317931117119\\
57	375.322266365544\\
56	375.396036781664\\
55	375.469271689239\\
54	382.467033497312\\
53	387.634535955748\\
52	390.920330869338\\
51	391.369442963044\\
50	391.583630233338\\
49	394.128321606031\\
48	399.221410813474\\
47	399.313015912533\\
46	399.820103517845\\
45	412.670984566891\\
44	416.901852055489\\
43	425.947095113949\\
42	444.443361235639\\
41	445.308104049248\\
40	445.308104049248\\
39	445.371272982401\\
38	449.393836931363\\
37	465.673193694159\\
36	476.212321713426\\
35	476.513021606946\\
34	484.564826788103\\
33	491.579745065218\\
32	516.411106140525\\
31	557.115665155568\\
30	574.632837330797\\
29	573.734887974133\\
28	573.210524229623\\
27	597.169360879243\\
26	603.588219312861\\
25	618.342799124536\\
24	628.354494882848\\
23	633.155972340802\\
22	639.004625831026\\
21	641.552956656679\\
20	656.120193238318\\
19	663.474104913829\\
18	671.908795096615\\
17	685.284213716197\\
16	691.751678504512\\
15	689.064804307218\\
14	689.064804307218\\
13	716.98569404258\\
12	727.375810151267\\
11	747.581833530455\\
10	747.581833530455\\
9	810.953123569672\\
8	810.953123569672\\
7	870.071221660919\\
6	874.608915539239\\
5	1019.9683225533\\
4	1152.18621426173\\
3	1389.65259166914\\
2	1800.0612240824\\
1	2122.05631171696\\
}--cycle;
\addplot [color=mycolor4]
  table[row sep=crcr]{%
1	1614\\
2	1406\\
3	1056\\
4	909\\
5	799\\
6	749\\
7	743\\
8	722\\
9	722\\
10	677\\
11	677\\
12	668\\
13	660\\
14	651\\
15	651\\
16	631\\
17	622\\
18	612\\
19	606\\
20	575\\
21	561\\
22	560\\
23	554\\
24	547\\
25	543\\
26	531\\
27	529\\
28	520\\
29	514\\
30	503\\
31	495\\
32	473\\
33	451\\
34	443\\
35	429\\
36	428\\
37	422\\
38	409\\
39	404\\
40	404\\
41	404\\
42	403\\
43	397\\
44	393\\
45	390\\
46	385\\
47	384\\
48	384\\
49	382\\
50	379\\
51	378\\
52	378\\
53	377\\
54	375\\
55	372\\
56	372\\
57	372\\
58	372\\
59	371\\
60	370\\
61	370\\
62	370\\
63	369\\
64	369\\
65	369\\
66	369\\
67	369\\
68	369\\
69	369\\
70	369\\
71	368\\
72	368\\
73	368\\
74	368\\
75	368\\
76	368\\
77	368\\
78	368\\
79	368\\
80	368\\
81	368\\
82	368\\
83	368\\
84	368\\
85	368\\
86	368\\
87	368\\
88	368\\
89	368\\
90	368\\
91	368\\
92	368\\
93	368\\
94	368\\
95	368\\
96	368\\
97	368\\
98	368\\
99	368\\
100	368\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.1}$}


\addplot[area legend, draw=none, fill=mycolor5, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1083.94164841792\\
2	794.545435134731\\
3	704.192255409083\\
4	701.134326487207\\
5	694.808452919495\\
6	652.209499657079\\
7	648.888903551531\\
8	656.45155232808\\
9	656.920038632598\\
10	649.40664047447\\
11	649.40664047447\\
12	645.434130799015\\
13	645.434130799015\\
14	645.699902211598\\
15	645.542333450434\\
16	645.542333450434\\
17	636.415999106652\\
18	637.603189663503\\
19	637.778933691178\\
20	636.635836780502\\
21	614.495885603808\\
22	614.107635046692\\
23	572.580531743537\\
24	555.324258364133\\
25	536.071943719922\\
26	536.071943719922\\
27	535.336137312279\\
28	526.774258154144\\
29	514.285240413715\\
30	502.249790877919\\
31	502.249790877919\\
32	500.236038119568\\
33	479.344870023028\\
34	454.021923366868\\
35	455.237778680672\\
36	451.012544814158\\
37	450.710770075302\\
38	449.941725825424\\
39	450.413910826878\\
40	447.926388059455\\
41	434.272252263923\\
42	427.015894526178\\
43	426.387885160478\\
44	432.339144158234\\
45	432.029235590877\\
46	429.779197357935\\
47	424.231140827622\\
48	423.969410390353\\
49	423.969410390353\\
50	423.914239015292\\
51	421.37221510034\\
52	418.876497373984\\
53	416.192693428237\\
54	410.405103097919\\
55	409.966573650248\\
56	407.441313763792\\
57	402.385715395574\\
58	395.372603645508\\
59	394.961683309964\\
60	394.547491419885\\
61	394.336376450156\\
62	388.698095262638\\
63	388.50793500901\\
64	388.482677424752\\
65	388.478373721849\\
66	388.393843902907\\
67	388.318082207792\\
68	388.318082207792\\
69	388.231559875928\\
70	386.9228618396\\
71	385.966217080338\\
72	385.935400238512\\
73	385.895337634896\\
74	384.393837711543\\
75	381.68983822879\\
76	381.68743000909\\
77	381.575900482241\\
78	381.561644666656\\
79	381.519729874943\\
80	380.613914828196\\
81	380.02435361736\\
82	379.308840419949\\
83	379.011322748535\\
84	378.999782004617\\
85	378.999085191276\\
86	378.649916635589\\
87	378.581360010999\\
88	378.581360010999\\
89	378.484445050155\\
90	378.479237041359\\
91	378.478819593061\\
92	378.408931554198\\
93	378.391918974319\\
94	378.284118355776\\
95	378.186739329333\\
96	378.186739329333\\
97	378.178320436045\\
98	378.178320436045\\
99	378.172674021632\\
100	378.155784640731\\
100	466.869762461439\\
99	466.868974866717\\
98	466.902174999279\\
97	466.902174999279\\
96	466.931627562019\\
95	466.931627562019\\
94	466.921870728478\\
93	466.930828323438\\
92	466.936404268747\\
91	466.929550821431\\
90	466.929507280735\\
89	466.982290626576\\
88	467.023049044693\\
87	467.023049044693\\
86	467.016439061075\\
85	466.983549807674\\
84	466.990458006029\\
83	467.109115724308\\
82	467.252465621823\\
81	467.191270294799\\
80	467.145337579885\\
79	467.083068623541\\
78	467.077432366927\\
77	467.223219271684\\
76	467.320123743087\\
75	467.345179076365\\
74	467.428115916062\\
73	467.821871928179\\
72	467.87042884477\\
71	467.865112595187\\
70	468.378195083874\\
69	468.40740774632\\
68	468.488377925865\\
67	468.488377925865\\
66	469.182100103753\\
65	470.163152307302\\
64	470.189892572444\\
63	470.47930675546\\
62	473.47906893478\\
61	473.732402600548\\
60	476.420549491272\\
59	476.327097226378\\
58	476.489479051228\\
57	479.35959615439\\
56	483.19165356278\\
55	486.747300965976\\
54	490.473817954474\\
53	502.652926565333\\
52	502.582830860023\\
51	508.298520830002\\
50	507.748011685474\\
49	507.942358863781\\
48	507.942358863781\\
47	508.798787017036\\
46	516.896462757442\\
45	516.285607989744\\
44	516.202348079164\\
43	556.935876311467\\
42	557.649180713919\\
41	558.043721890984\\
40	565.202346335247\\
39	567.859633281839\\
38	570.436632407033\\
37	570.326255688148\\
36	570.771422077133\\
35	616.422455480104\\
34	627.572379348708\\
33	638.816652783296\\
32	646.677998694583\\
31	650.74489237834\\
30	650.74489237834\\
29	653.579133632443\\
28	650.968912436178\\
27	670.113057525592\\
26	669.954442762706\\
25	669.954442762706\\
24	678.720269805939\\
23	673.437200496022\\
22	663.06998283479\\
21	667.775571933131\\
20	678.25224407229\\
19	690.962253191531\\
18	692.343556652675\\
17	699.187313669683\\
16	702.860691206039\\
15	702.860691206039\\
14	709.895225790493\\
13	712.652724679152\\
12	712.652724679152\\
11	714.091371662041\\
10	714.091371662041\\
9	724.854655488439\\
8	741.628495624467\\
7	811.155073642865\\
6	820.179777899462\\
5	826.308457721423\\
4	1021.05984776962\\
3	1062.36690407385\\
2	1628.79830806761\\
1	2046.4385193762\\
}--cycle;
\addplot [color=mycolor5]
  table[row sep=crcr]{%
1	1565\\
2	1212\\
3	883\\
4	861\\
5	761\\
6	736\\
7	730\\
8	699\\
9	691\\
10	682\\
11	682\\
12	679\\
13	679\\
14	678\\
15	674\\
16	674\\
17	668\\
18	665\\
19	664\\
20	657\\
21	641\\
22	639\\
23	623\\
24	617\\
25	603\\
26	603\\
27	603\\
28	589\\
29	584\\
30	576\\
31	576\\
32	573\\
33	559\\
34	541\\
35	536\\
36	511\\
37	511\\
38	510\\
39	509\\
40	507\\
41	496\\
42	492\\
43	492\\
44	474\\
45	474\\
46	473\\
47	467\\
48	466\\
49	466\\
50	466\\
51	465\\
52	461\\
53	459\\
54	450\\
55	448\\
56	445\\
57	441\\
58	436\\
59	436\\
60	435\\
61	434\\
62	431\\
63	429\\
64	429\\
65	429\\
66	429\\
67	428\\
68	428\\
69	428\\
70	428\\
71	427\\
72	427\\
73	427\\
74	426\\
75	425\\
76	425\\
77	424\\
78	424\\
79	424\\
80	424\\
81	424\\
82	423\\
83	423\\
84	423\\
85	423\\
86	423\\
87	423\\
88	423\\
89	423\\
90	423\\
91	423\\
92	423\\
93	423\\
94	423\\
95	423\\
96	423\\
97	423\\
98	423\\
99	423\\
100	423\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.2}$}


\addplot[area legend, draw=none, fill=mycolor6, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1333.96003293744\\
2	1019.2183990149\\
3	770.145200374987\\
4	783.821772963042\\
5	783.821772963042\\
6	725.176478256393\\
7	708.789106093025\\
8	708.789106093025\\
9	726.522075471952\\
10	728.424782489573\\
11	716.257799599123\\
12	709.087036548222\\
13	703.681650404158\\
14	702.023540698138\\
15	691.271906365867\\
16	689.70655585921\\
17	668.838646124298\\
18	668.838646124298\\
19	665.401091936027\\
20	663.377384645464\\
21	663.377384645464\\
22	658.301033610452\\
23	610.739023441802\\
24	608.910803938118\\
25	606.149600381993\\
26	600.304318501504\\
27	594.851187069116\\
28	594.851187069116\\
29	593.102757020306\\
30	552.629068856484\\
31	550.641224841725\\
32	543.792484738753\\
33	532.972597382329\\
34	532.830403451436\\
35	528.169434098781\\
36	505.130668672304\\
37	501.516504674584\\
38	501.516504674584\\
39	503.450560560249\\
40	493.315401559783\\
41	489.469039911631\\
42	483.749845457166\\
43	483.749845457166\\
44	484.291552855957\\
45	476.86985254135\\
46	453.176475316798\\
47	452.611086852732\\
48	436.794798722423\\
49	431.165666011113\\
50	410.65405720809\\
51	410.507790426603\\
52	401.282794749172\\
53	401.303171962328\\
54	392.403617906335\\
55	389.884750299448\\
56	389.238035390619\\
57	388.398201568955\\
58	388.379714151937\\
59	388.2764304751\\
60	388.161988556344\\
61	385.441670417142\\
62	384.433459715354\\
63	383.403708131861\\
64	381.821087567903\\
65	381.725056383067\\
66	381.576091145809\\
67	381.398443159984\\
68	381.225500705217\\
69	380.77891488357\\
70	380.478695339866\\
71	380.198363862388\\
72	379.96341588789\\
73	379.95816724871\\
74	379.462581544029\\
75	379.031094789009\\
76	379.031094789009\\
77	379.020411485991\\
78	378.971825452257\\
79	378.971825452257\\
80	378.938300364929\\
81	378.711480246441\\
82	378.679650853065\\
83	378.506498597172\\
84	378.479748173019\\
85	378.328962956243\\
86	378.316119754908\\
87	378.298348574024\\
88	378.292289891757\\
89	378.272141999184\\
90	378.214958788898\\
91	378.199412236124\\
92	378.156365242282\\
93	378.156365242282\\
94	378.156365242282\\
95	378.153219050851\\
96	378.152193847297\\
97	378.152193847297\\
98	378.152193847297\\
99	378.148527528476\\
100	378.143822623605\\
100	466.891860163122\\
99	466.906058451346\\
98	466.905688147729\\
97	466.905688147729\\
96	466.905688147729\\
95	466.905584547909\\
94	466.90752714415\\
93	466.90752714415\\
92	466.90752714415\\
91	466.96921649861\\
90	466.967641075342\\
89	466.989034290078\\
88	467.006233356774\\
87	467.020737521566\\
86	467.018932268999\\
85	467.017629623176\\
84	467.002565739354\\
83	466.999917848545\\
82	466.982215118657\\
81	466.978985641847\\
80	466.956240972471\\
79	466.967294309461\\
78	466.967294309461\\
77	467.451914920375\\
76	467.555736488215\\
75	467.555736488215\\
74	467.513791544583\\
73	467.635334582627\\
72	467.688758113684\\
71	467.732298018685\\
70	467.729698339728\\
69	468.044975729728\\
68	468.665585431061\\
67	468.969011341332\\
66	469.076306512484\\
65	469.061644053128\\
64	470.328267241073\\
63	470.323907709421\\
62	470.416248965988\\
61	470.31526808873\\
60	474.286525225952\\
59	476.278427211474\\
58	476.841980533485\\
57	476.949256876321\\
56	476.838238603861\\
55	482.307353247625\\
54	483.253474393141\\
53	482.81209314332\\
52	486.081119800288\\
51	485.463766279113\\
50	488.041030625396\\
49	488.451917531373\\
48	501.727950170636\\
47	506.268640359641\\
46	507.333351413766\\
45	549.538699337456\\
44	555.285578903145\\
43	560.943349939263\\
42	560.943349939263\\
41	565.397613373331\\
40	570.062661911195\\
39	575.146009028874\\
38	592.240337526627\\
37	592.240337526627\\
36	600.437912998498\\
35	612.580910151984\\
34	619.835889022087\\
33	620.51354940472\\
32	629.24956912334\\
31	643.974755327084\\
30	649.432201490309\\
29	647.840087776325\\
28	659.281280853053\\
27	659.281280853053\\
26	668.148652795996\\
25	674.37431658325\\
24	679.036967538006\\
23	689.447144134698\\
22	688.502696012781\\
21	690.026117974541\\
20	690.026117974541\\
19	697.405845968659\\
18	718.367808347192\\
17	718.367808347192\\
16	735.503942365475\\
15	739.930074487114\\
14	773.290434733968\\
13	778.047254740299\\
12	808.829445611791\\
11	813.755687750052\\
10	816.567031315072\\
9	853.446785992319\\
8	955.361513010394\\
7	955.361513010394\\
6	971.494406935115\\
5	1112.96335950799\\
4	1112.96335950799\\
3	1214.59152443583\\
2	1553.28904697728\\
1	1804.07879310806\\
}--cycle;
\addplot [color=mycolor6]
  table[row sep=crcr]{%
1	1569\\
2	1286\\
3	992\\
4	948\\
5	948\\
6	848\\
7	832\\
8	832\\
9	790\\
10	772\\
11	765\\
12	759\\
13	741\\
14	738\\
15	716\\
16	713\\
17	694\\
18	694\\
19	681\\
20	677\\
21	677\\
22	673\\
23	650\\
24	644\\
25	640\\
26	634\\
27	627\\
28	627\\
29	620\\
30	601\\
31	597\\
32	587\\
33	577\\
34	576\\
35	570\\
36	553\\
37	547\\
38	547\\
39	539\\
40	532\\
41	527\\
42	522\\
43	522\\
44	520\\
45	513\\
46	480\\
47	479\\
48	469\\
49	460\\
50	449\\
51	448\\
52	444\\
53	442\\
54	438\\
55	436\\
56	433\\
57	433\\
58	433\\
59	432\\
60	431\\
61	428\\
62	427\\
63	427\\
64	426\\
65	425\\
66	425\\
67	425\\
68	425\\
69	424\\
70	424\\
71	424\\
72	424\\
73	424\\
74	423\\
75	423\\
76	423\\
77	423\\
78	423\\
79	423\\
80	423\\
81	423\\
82	423\\
83	423\\
84	423\\
85	423\\
86	423\\
87	423\\
88	423\\
89	423\\
90	423\\
91	423\\
92	423\\
93	423\\
94	423\\
95	423\\
96	423\\
97	423\\
98	423\\
99	423\\
100	423\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.5}$}


\addplot[area legend, draw=none, fill=mycolor7, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1063.45563248907\\
2	842.602350387893\\
3	801.301593840768\\
4	815.801265464571\\
5	814.924141159664\\
6	819.509711541214\\
7	825.903093997114\\
8	796.203239877182\\
9	763.944270116316\\
10	679.799355853753\\
11	679.799355853753\\
12	655.370333088955\\
13	674.902711002286\\
14	672.320965880952\\
15	671.89881012501\\
16	671.89881012501\\
17	677.731030634613\\
18	677.731030634613\\
19	677.731030634613\\
20	656.484230628184\\
21	656.484230628184\\
22	654.213575882034\\
23	644.283462234822\\
24	636.452403559243\\
25	636.452403559243\\
26	636.101939858865\\
27	629.669027478605\\
28	633.100683158182\\
29	630.410987207088\\
30	624.716518336205\\
31	623.625411583066\\
32	617.49899808503\\
33	614.274482784444\\
34	583.935791619306\\
35	538.002552141463\\
36	537.75192927984\\
37	537.75192927984\\
38	512.375528701069\\
39	507.70734254202\\
40	505.724080531462\\
41	505.623878850374\\
42	505.042267604199\\
43	504.699113549792\\
44	474.639479826539\\
45	466.8327553506\\
46	468.024505274006\\
47	468.024505274006\\
48	468.091196277804\\
49	463.281652681785\\
50	461.435429701874\\
51	456.663554367788\\
52	450.608814596253\\
53	435.309532498398\\
54	425.060193327588\\
55	424.514903667391\\
56	422.60204537617\\
57	413.026906000061\\
58	412.984785131983\\
59	407.716929586642\\
60	407.531689908394\\
61	402.740379332446\\
62	396.697154818366\\
63	396.135719827823\\
64	395.877835433749\\
65	395.402765201282\\
66	390.929509646787\\
67	390.036847617362\\
68	389.111503474013\\
69	388.84014248403\\
70	388.390404216143\\
71	386.331273705994\\
72	386.060717553602\\
73	384.994147161503\\
74	384.842198304423\\
75	383.826435780315\\
76	383.782159727519\\
77	383.276465675148\\
78	383.005408334487\\
79	382.306946262902\\
80	382.095900614762\\
81	381.458602167868\\
82	381.444418304366\\
83	381.154706150394\\
84	381.148893019641\\
85	380.921191473102\\
86	380.712027843904\\
87	380.607282559193\\
88	379.993431685278\\
89	379.902335801433\\
90	379.393627090227\\
91	379.31562842226\\
92	379.244067394083\\
93	379.235210527909\\
94	378.916226813839\\
95	378.907871242118\\
96	378.859095555129\\
97	378.744245618358\\
98	378.744245618358\\
99	378.640530299106\\
100	378.610111983591\\
100	474.738793352202\\
99	474.902066193754\\
98	474.892483016944\\
97	474.892483016944\\
96	474.881999990349\\
95	474.979317748434\\
94	475.002814398622\\
93	475.105150343996\\
92	475.10437266989\\
91	475.139976376214\\
90	475.280603559606\\
89	475.260039734222\\
88	475.707351933575\\
87	475.719430369205\\
86	475.84401084157\\
85	475.827733490972\\
84	475.968642772527\\
83	475.99657251634\\
82	476.099149597609\\
81	476.176610898784\\
80	476.118641998715\\
79	476.369264439691\\
78	476.903134697287\\
77	476.970644491264\\
76	477.445221783603\\
75	477.532679981353\\
74	477.716609948125\\
73	477.743368463155\\
72	478.571219938817\\
71	479.086192558462\\
70	479.462614352669\\
69	479.448136875083\\
68	479.804265965208\\
67	480.089206117133\\
66	480.077893406194\\
65	479.584564876592\\
64	481.439835496529\\
63	483.631038923155\\
62	488.023350476119\\
61	489.020596675454\\
60	489.374880662514\\
59	491.452758379552\\
58	492.843848974305\\
57	493.113409787043\\
56	492.418052490982\\
55	492.574471272438\\
54	540.796711831796\\
53	546.548171638447\\
52	558.390599392293\\
51	576.922206826049\\
50	579.171493159095\\
49	579.489852928482\\
48	602.615484277102\\
47	603.461936086545\\
46	603.461936086545\\
45	620.058396307612\\
44	625.563602088532\\
43	630.403176989005\\
42	631.079094480651\\
41	631.046462195007\\
40	631.251895223844\\
39	645.886579454296\\
38	659.371930325726\\
37	666.755161357331\\
36	666.755161357331\\
35	673.646416871291\\
34	672.584713971984\\
33	700.81624996677\\
32	701.092090851452\\
31	708.916441874834\\
30	725.109657212747\\
29	727.332649193557\\
28	728.497829364139\\
27	739.031975146394\\
26	744.754877734188\\
25	744.88853779798\\
24	744.88853779798\\
23	750.094914467612\\
22	758.994207097588\\
21	762.342494835217\\
20	762.342494835217\\
19	773.725650489818\\
18	773.725650489818\\
17	773.725650489818\\
16	796.317970308512\\
15	796.317970308512\\
14	805.670446774248\\
13	807.616655251954\\
12	873.470396419145\\
11	897.928217929532\\
10	897.928217929532\\
9	937.245263747795\\
8	936.364475649056\\
7	970.081663960826\\
6	1120.24765052714\\
5	1135.53983723913\\
4	1136.17271253973\\
3	1310.40895160164\\
2	1351.30673128194\\
1	1514.51395122976\\
}--cycle;
\addplot [color=mycolor7]
  table[row sep=crcr]{%
1	1289\\
2	1097\\
3	1056\\
4	976\\
5	975\\
6	970\\
7	898\\
8	866\\
9	851\\
10	789\\
11	789\\
12	764\\
13	741\\
14	739\\
15	734\\
16	734\\
17	726\\
18	726\\
19	726\\
20	709\\
21	709\\
22	707\\
23	697\\
24	691\\
25	691\\
26	690\\
27	684\\
28	681\\
29	679\\
30	675\\
31	666\\
32	659\\
33	658\\
34	628\\
35	606\\
36	602\\
37	602\\
38	586\\
39	577\\
40	568\\
41	568\\
42	568\\
43	568\\
44	550\\
45	543\\
46	536\\
47	536\\
48	535\\
49	521\\
50	520\\
51	517\\
52	504\\
53	491\\
54	483\\
55	459\\
56	458\\
57	453\\
58	453\\
59	450\\
60	448\\
61	446\\
62	442\\
63	440\\
64	439\\
65	437\\
66	436\\
67	435\\
68	434\\
69	434\\
70	434\\
71	433\\
72	432\\
73	431\\
74	431\\
75	431\\
76	431\\
77	430\\
78	430\\
79	429\\
80	429\\
81	429\\
82	429\\
83	429\\
84	429\\
85	428\\
86	428\\
87	428\\
88	428\\
89	428\\
90	427\\
91	427\\
92	427\\
93	427\\
94	427\\
95	427\\
96	427\\
97	427\\
98	427\\
99	427\\
100	427\\
};
\addlegendentry{$\text{torques, }\sigma\text{ = 0.7}$}

\legend{}
\end{axis}


==> figures/arms_precision_random_onlyaxis.tex <==
\begin{axis}[
name =ax5,
scaled y ticks=base 10:\Factor,
at={(ax1.south west)},
xlabel near ticks, ylabel near ticks,
every y tick scale label/.style={at={(yticklabel* cs:1.03,0cm)},anchor=near yticklabel},
every x tick scale label/.style={at={(xticklabel* cs:1.05,-0.05cm)},anchor=near xticklabel},
title style={at={(0.5,0.93)}},
yshift=-3.5cm,
xshift=0.5cm,
height=\figH,
tick align=outside,
tick pos=left,
title={(e) precise point-reaching (RL)},
width=\figW,
x grid style={darkgray176},
xlabel={steps},
xmin=0, xmax=13500000,
xtick style={color=black},
y grid style={darkgray176},
ylabel={distance-return},
ymin=-984.547621707016, ymax=-264.929423938629,
ytick style={color=black}
]
\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.1]
(axis cs:100000,-842.078744585376)
--(axis cs:100000,-928.399331466097)
--(axis cs:200000,-924.253199635852)
--(axis cs:300000,-918.521306318757)
--(axis cs:400000,-909.361096424133)
--(axis cs:500000,-899.894924610639)
--(axis cs:600000,-889.489066470705)
--(axis cs:700000,-864.714021557915)
--(axis cs:800000,-840.85527455512)
--(axis cs:900000,-813.987429502855)
--(axis cs:1000000,-788.212721457616)
--(axis cs:1100000,-760.191498270846)
--(axis cs:1200000,-729.910512473897)
--(axis cs:1300000,-699.76238636936)
--(axis cs:1400000,-674.316293490071)
--(axis cs:1500000,-648.044486168908)
--(axis cs:1600000,-624.814985682082)
--(axis cs:1700000,-608.949731485994)
--(axis cs:1800000,-593.166760754121)
--(axis cs:1900000,-580.496145341388)
--(axis cs:2000000,-566.231169692722)
--(axis cs:2100000,-553.488101395032)
--(axis cs:2200000,-542.722819702763)
--(axis cs:2300000,-535.724534592159)
--(axis cs:2400000,-529.678463462295)
--(axis cs:2500000,-525.586361162678)
--(axis cs:2600000,-520.673467710639)
--(axis cs:2700000,-512.818789458595)
--(axis cs:2800000,-508.736014487481)
--(axis cs:2900000,-503.081933081235)
--(axis cs:3000000,-500.118303376233)
--(axis cs:3100000,-497.442276516773)
--(axis cs:3200000,-496.359638537372)
--(axis cs:3300000,-493.317096999673)
--(axis cs:3400000,-486.489444644476)
--(axis cs:3500000,-481.305309903257)
--(axis cs:3600000,-477.950252720189)
--(axis cs:3700000,-475.748748165091)
--(axis cs:3800000,-472.686022535988)
--(axis cs:3900000,-471.638441471314)
--(axis cs:4000000,-472.929335599948)
--(axis cs:4100000,-474.177434985525)
--(axis cs:4200000,-471.670578249111)
--(axis cs:4300000,-468.310596403142)
--(axis cs:4400000,-467.392155795325)
--(axis cs:4500000,-466.683172815402)
--(axis cs:4600000,-465.971716387832)
--(axis cs:4700000,-466.584656998859)
--(axis cs:4800000,-464.746301889886)
--(axis cs:4900000,-461.200696070421)
--(axis cs:5000000,-458.795291024682)
--(axis cs:5100000,-457.134995473599)
--(axis cs:5200000,-455.449886485324)
--(axis cs:5300000,-454.034398712104)
--(axis cs:5400000,-450.432992561043)
--(axis cs:5500000,-446.883579081438)
--(axis cs:5600000,-441.26285330529)
--(axis cs:5700000,-436.180729458866)
--(axis cs:5800000,-432.915844445373)
--(axis cs:5900000,-432.918314060709)
--(axis cs:6000000,-431.297154103717)
--(axis cs:6100000,-428.505137039863)
--(axis cs:6200000,-427.417549752931)
--(axis cs:6300000,-426.032648368006)
--(axis cs:6400000,-426.756612811242)
--(axis cs:6500000,-425.421139804923)
--(axis cs:6600000,-425.822729639966)
--(axis cs:6700000,-425.258295322717)
--(axis cs:6800000,-426.199077900197)
--(axis cs:6900000,-424.572476225383)
--(axis cs:7000000,-423.154475992143)
--(axis cs:7100000,-421.754936462861)
--(axis cs:7200000,-420.212761604328)
--(axis cs:7300000,-419.733583338169)
--(axis cs:7400000,-418.320308213104)
--(axis cs:7500000,-418.64319523498)
--(axis cs:7600000,-418.161959647342)
--(axis cs:7700000,-417.551290320056)
--(axis cs:7800000,-415.907164196277)
--(axis cs:7900000,-416.284137595614)
--(axis cs:8000000,-415.192272733402)
--(axis cs:8100000,-416.059893129519)
--(axis cs:8200000,-417.527066397242)
--(axis cs:8300000,-417.383533458894)
--(axis cs:8400000,-420.154127779058)
--(axis cs:8500000,-421.800590668141)
--(axis cs:8600000,-421.710500680373)
--(axis cs:8700000,-420.943455357467)
--(axis cs:8800000,-421.186899324352)
--(axis cs:8900000,-421.661663225019)
--(axis cs:9000000,-420.929236557276)
--(axis cs:9100000,-419.331244911794)
--(axis cs:9200000,-416.265472450167)
--(axis cs:9300000,-414.389002073603)
--(axis cs:9400000,-409.693118315861)
--(axis cs:9500000,-407.579513564091)
--(axis cs:9600000,-405.76780901905)
--(axis cs:9700000,-407.580142271883)
--(axis cs:9800000,-407.485830407793)
--(axis cs:9900000,-406.85737110689)
--(axis cs:10000000,-406.940937026902)
--(axis cs:10100000,-407.071128016353)
--(axis cs:10200000,-406.236531249251)
--(axis cs:10300000,-405.691858973323)
--(axis cs:10400000,-407.119881090627)
--(axis cs:10500000,-405.895858211714)
--(axis cs:10600000,-406.639427850285)
--(axis cs:10700000,-405.217501518123)
--(axis cs:10800000,-406.581614666001)
--(axis cs:10900000,-407.173787150793)
--(axis cs:11000000,-410.436174572995)
--(axis cs:11100000,-410.46574503251)
--(axis cs:11200000,-413.007140340751)
--(axis cs:11300000,-414.482543386813)
--(axis cs:11400000,-414.117241686779)
--(axis cs:11500000,-411.939554582861)
--(axis cs:11600000,-411.106621803333)
--(axis cs:11700000,-410.225654679442)
--(axis cs:11800000,-407.812163020438)
--(axis cs:11900000,-405.94933210285)
--(axis cs:12000000,-403.451679413806)
--(axis cs:12100000,-403.018244162061)
--(axis cs:12200000,-402.888472315914)
--(axis cs:12300000,-402.832006836015)
--(axis cs:12400000,-402.414585409021)
--(axis cs:12500000,-405.268291800407)
--(axis cs:12600000,-406.378590854292)
--(axis cs:12700000,-405.731705728965)
--(axis cs:12800000,-405.06463049259)
--(axis cs:12900000,-404.973242587456)
--(axis cs:13000000,-404.688439814705)
--(axis cs:13100000,-401.455363883454)
--(axis cs:13200000,-399.436104370867)
--(axis cs:13300000,-397.675095185355)
--(axis cs:13400000,-397.865135576919)
--(axis cs:13500000,-397.701046020869)
--(axis cs:13600000,-393.9683363391)
--(axis cs:13700000,-391.222525368433)
--(axis cs:13800000,-388.734389970154)
--(axis cs:13900000,-386.83907446489)
--(axis cs:14000000,-384.288231868885)
--(axis cs:14100000,-386.214894127984)
--(axis cs:14200000,-384.473501089609)
--(axis cs:14300000,-385.319359083341)
--(axis cs:14400000,-385.714227476948)
--(axis cs:14500000,-386.281779920215)
--(axis cs:14600000,-390.172423739937)
--(axis cs:14700000,-393.158775094639)
--(axis cs:14800000,-396.19641738752)
--(axis cs:14900000,-398.648565626688)
--(axis cs:15000000,-398.781372646638)
--(axis cs:15100000,-398.258984805322)
--(axis cs:15200000,-400.673798684697)
--(axis cs:15300000,-400.38561302341)
--(axis cs:15400000,-400.570752226369)
--(axis cs:15500000,-399.159643913828)
--(axis cs:15600000,-397.61662084209)
--(axis cs:15700000,-395.310465289036)
--(axis cs:15800000,-392.906470370269)
--(axis cs:15900000,-390.028788484108)
--(axis cs:16000000,-390.274918890205)
--(axis cs:16100000,-390.667708940687)
--(axis cs:16200000,-389.285653733365)
--(axis cs:16300000,-388.774233120993)
--(axis cs:16300000,-318.847172061993)
--(axis cs:16300000,-318.847172061993)
--(axis cs:16200000,-320.235909915103)
--(axis cs:16100000,-320.165164922046)
--(axis cs:16000000,-318.742973312392)
--(axis cs:15900000,-319.072426372596)
--(axis cs:15800000,-317.279741281543)
--(axis cs:15700000,-318.297102981553)
--(axis cs:15600000,-316.288226061691)
--(axis cs:15500000,-315.520955234221)
--(axis cs:15400000,-313.314009540944)
--(axis cs:15300000,-312.471829780171)
--(axis cs:15200000,-310.559147182012)
--(axis cs:15100000,-308.82249911934)
--(axis cs:15000000,-308.127387590758)
--(axis cs:14900000,-306.978734912378)
--(axis cs:14800000,-306.235620362988)
--(axis cs:14700000,-305.900775125135)
--(axis cs:14600000,-306.607171439298)
--(axis cs:14500000,-307.089126484737)
--(axis cs:14400000,-309.429227105246)
--(axis cs:14300000,-313.19304309133)
--(axis cs:14200000,-314.262440402759)
--(axis cs:14100000,-318.146740385206)
--(axis cs:14000000,-320.221177880374)
--(axis cs:13900000,-322.212005365116)
--(axis cs:13800000,-325.150451947525)
--(axis cs:13700000,-325.094488989685)
--(axis cs:13600000,-325.479768847645)
--(axis cs:13500000,-326.456748674975)
--(axis cs:13400000,-325.943012019003)
--(axis cs:13300000,-324.613949161355)
--(axis cs:13200000,-325.101883390903)
--(axis cs:13100000,-323.16035722762)
--(axis cs:13000000,-322.5282938488)
--(axis cs:12900000,-322.345394636955)
--(axis cs:12800000,-321.523464644564)
--(axis cs:12700000,-322.01953584038)
--(axis cs:12600000,-322.737466976583)
--(axis cs:12500000,-322.454837303422)
--(axis cs:12400000,-324.129146374235)
--(axis cs:12300000,-323.450590610551)
--(axis cs:12200000,-321.670934643849)
--(axis cs:12100000,-321.382437887234)
--(axis cs:12000000,-321.415717154875)
--(axis cs:11900000,-322.541892485554)
--(axis cs:11800000,-324.21638499087)
--(axis cs:11700000,-328.150318194921)
--(axis cs:11600000,-327.594328498479)
--(axis cs:11500000,-327.571968175866)
--(axis cs:11400000,-326.637423880699)
--(axis cs:11300000,-328.000476510131)
--(axis cs:11200000,-330.376774590988)
--(axis cs:11100000,-332.38452384896)
--(axis cs:11000000,-334.182132402295)
--(axis cs:10900000,-331.964189692574)
--(axis cs:10800000,-331.060620261837)
--(axis cs:10700000,-327.398917396597)
--(axis cs:10600000,-328.465748995852)
--(axis cs:10500000,-328.219987864745)
--(axis cs:10400000,-328.355556630015)
--(axis cs:10300000,-327.239486124423)
--(axis cs:10200000,-326.877943593769)
--(axis cs:10100000,-325.953682951515)
--(axis cs:10000000,-325.616012582567)
--(axis cs:9900000,-326.300292571786)
--(axis cs:9800000,-326.739184795563)
--(axis cs:9700000,-327.505925239731)
--(axis cs:9600000,-328.458599520042)
--(axis cs:9500000,-329.60923853891)
--(axis cs:9400000,-329.864439682861)
--(axis cs:9300000,-332.55468343586)
--(axis cs:9200000,-334.182915454497)
--(axis cs:9100000,-336.748864432555)
--(axis cs:9000000,-337.895770219201)
--(axis cs:8900000,-338.802842811794)
--(axis cs:8800000,-339.721474912768)
--(axis cs:8700000,-341.096821669201)
--(axis cs:8600000,-341.277494000901)
--(axis cs:8500000,-343.539080561753)
--(axis cs:8400000,-345.91998939134)
--(axis cs:8300000,-348.458144882311)
--(axis cs:8200000,-348.903923872861)
--(axis cs:8100000,-348.858086759994)
--(axis cs:8000000,-351.960543519158)
--(axis cs:7900000,-353.224402949765)
--(axis cs:7800000,-353.974216305262)
--(axis cs:7700000,-356.028793976235)
--(axis cs:7600000,-359.371372934079)
--(axis cs:7500000,-359.700892517745)
--(axis cs:7400000,-358.965471766969)
--(axis cs:7300000,-357.581363684602)
--(axis cs:7200000,-357.141537230125)
--(axis cs:7100000,-356.200100155923)
--(axis cs:7000000,-354.373883548458)
--(axis cs:6900000,-356.709026223683)
--(axis cs:6800000,-357.749461194579)
--(axis cs:6700000,-355.089438250849)
--(axis cs:6600000,-353.838190504179)
--(axis cs:6500000,-354.529918157281)
--(axis cs:6400000,-355.774889965152)
--(axis cs:6300000,-355.815132876262)
--(axis cs:6200000,-359.192231525018)
--(axis cs:6100000,-360.684815018134)
--(axis cs:6000000,-363.692632340316)
--(axis cs:5900000,-364.707620464274)
--(axis cs:5800000,-366.321221345692)
--(axis cs:5700000,-367.244357835887)
--(axis cs:5600000,-366.195731245453)
--(axis cs:5500000,-367.524766836199)
--(axis cs:5400000,-373.013049148018)
--(axis cs:5300000,-377.494332934533)
--(axis cs:5200000,-378.691113169878)
--(axis cs:5100000,-383.154078883304)
--(axis cs:5000000,-381.728696164204)
--(axis cs:4900000,-381.132001137358)
--(axis cs:4800000,-381.544435106869)
--(axis cs:4700000,-386.061500886012)
--(axis cs:4600000,-389.772294779704)
--(axis cs:4500000,-391.296651125565)
--(axis cs:4400000,-389.034898149218)
--(axis cs:4300000,-386.833368047789)
--(axis cs:4200000,-386.332457193097)
--(axis cs:4100000,-386.045844766238)
--(axis cs:4000000,-389.380710149472)
--(axis cs:3900000,-391.201915933534)
--(axis cs:3800000,-393.358445086104)
--(axis cs:3700000,-395.169330622236)
--(axis cs:3600000,-398.363286165574)
--(axis cs:3500000,-403.863517337558)
--(axis cs:3400000,-409.331320931862)
--(axis cs:3300000,-415.297371305487)
--(axis cs:3200000,-421.74370156166)
--(axis cs:3100000,-424.780858278977)
--(axis cs:3000000,-427.563019617279)
--(axis cs:2900000,-433.556214602182)
--(axis cs:2800000,-438.574469625691)
--(axis cs:2700000,-444.722606144675)
--(axis cs:2600000,-448.209554972699)
--(axis cs:2500000,-451.449648183271)
--(axis cs:2400000,-454.901038955423)
--(axis cs:2300000,-460.553220091162)
--(axis cs:2200000,-466.51764945677)
--(axis cs:2100000,-474.721125603606)
--(axis cs:2000000,-480.137691845723)
--(axis cs:1900000,-486.252834927572)
--(axis cs:1800000,-492.527974175381)
--(axis cs:1700000,-497.225809307892)
--(axis cs:1600000,-506.308048131752)
--(axis cs:1500000,-516.902664397297)
--(axis cs:1400000,-529.232161986317)
--(axis cs:1300000,-541.86819711752)
--(axis cs:1200000,-556.439349425445)
--(axis cs:1100000,-576.739960739125)
--(axis cs:1000000,-606.52644629696)
--(axis cs:900000,-633.85809962516)
--(axis cs:800000,-666.424959546841)
--(axis cs:700000,-700.587534284445)
--(axis cs:600000,-738.903867459901)
--(axis cs:500000,-755.831855896495)
--(axis cs:400000,-775.223537677258)
--(axis cs:300000,-797.459981996244)
--(axis cs:200000,-821.327234423086)
--(axis cs:100000,-842.078744585376)
--cycle;

\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.1]
(axis cs:100000,-742.362843748353)
--(axis cs:100000,-878.238837190504)
--(axis cs:200000,-877.518602751341)
--(axis cs:300000,-874.459805155482)
--(axis cs:400000,-872.729188604305)
--(axis cs:500000,-871.20403856565)
--(axis cs:600000,-868.887004073403)
--(axis cs:700000,-862.417631425612)
--(axis cs:800000,-859.101849571227)
--(axis cs:900000,-856.589835748335)
--(axis cs:1000000,-855.441381058696)
--(axis cs:1100000,-855.732456936582)
--(axis cs:1200000,-853.212876215542)
--(axis cs:1300000,-851.099516087513)
--(axis cs:1400000,-848.190258287321)
--(axis cs:1500000,-846.321975500461)
--(axis cs:1600000,-843.912527832945)
--(axis cs:1700000,-838.676708073548)
--(axis cs:1800000,-834.747963889947)
--(axis cs:1900000,-830.183433425839)
--(axis cs:2000000,-824.215402857863)
--(axis cs:2100000,-818.854396742398)
--(axis cs:2200000,-812.101460914331)
--(axis cs:2300000,-806.982349329623)
--(axis cs:2400000,-802.426563741913)
--(axis cs:2500000,-795.144420790832)
--(axis cs:2600000,-790.726797835201)
--(axis cs:2700000,-785.980094944686)
--(axis cs:2800000,-784.688909970783)
--(axis cs:2900000,-781.945587340285)
--(axis cs:3000000,-779.443753643985)
--(axis cs:3100000,-777.202822732354)
--(axis cs:3200000,-775.9082453861)
--(axis cs:3300000,-773.970847024413)
--(axis cs:3400000,-771.483016238869)
--(axis cs:3500000,-769.00621384848)
--(axis cs:3600000,-765.646926993934)
--(axis cs:3700000,-763.360272921565)
--(axis cs:3800000,-756.804222709283)
--(axis cs:3900000,-753.827107486865)
--(axis cs:4000000,-752.205437252459)
--(axis cs:4100000,-749.234029665723)
--(axis cs:4200000,-746.048664379232)
--(axis cs:4300000,-744.155314242985)
--(axis cs:4400000,-742.623696310384)
--(axis cs:4500000,-743.247472473733)
--(axis cs:4600000,-743.532450096476)
--(axis cs:4700000,-743.545856498432)
--(axis cs:4800000,-744.461144617149)
--(axis cs:4900000,-746.819584285437)
--(axis cs:5000000,-746.983683108242)
--(axis cs:5100000,-748.104558582819)
--(axis cs:5200000,-747.858939344193)
--(axis cs:5300000,-748.218403647174)
--(axis cs:5400000,-746.932589472127)
--(axis cs:5500000,-744.812738637979)
--(axis cs:5600000,-744.021476845227)
--(axis cs:5700000,-742.209527165159)
--(axis cs:5800000,-743.338483573831)
--(axis cs:5900000,-742.059751025182)
--(axis cs:6000000,-739.7925920866)
--(axis cs:6100000,-739.48717181829)
--(axis cs:6200000,-739.251681244326)
--(axis cs:6300000,-736.845872189664)
--(axis cs:6400000,-736.074417506157)
--(axis cs:6500000,-736.160179792523)
--(axis cs:6600000,-735.300937740323)
--(axis cs:6700000,-735.081586482502)
--(axis cs:6800000,-733.309303392558)
--(axis cs:6900000,-732.002326223251)
--(axis cs:7000000,-732.923953532425)
--(axis cs:7100000,-729.902545438727)
--(axis cs:7200000,-731.397228132565)
--(axis cs:7300000,-732.81204601887)
--(axis cs:7400000,-733.564495374928)
--(axis cs:7500000,-734.407930901426)
--(axis cs:7600000,-734.211907798039)
--(axis cs:7700000,-733.460137331163)
--(axis cs:7800000,-732.346205361428)
--(axis cs:7900000,-730.978238890095)
--(axis cs:8000000,-731.010205080138)
--(axis cs:8100000,-731.24876220413)
--(axis cs:8200000,-730.411012589353)
--(axis cs:8300000,-728.428782993904)
--(axis cs:8400000,-726.457210278687)
--(axis cs:8500000,-724.547782697837)
--(axis cs:8600000,-723.887794703054)
--(axis cs:8700000,-725.2106257842)
--(axis cs:8800000,-724.984521104363)
--(axis cs:8900000,-724.396702793684)
--(axis cs:9000000,-722.771851938422)
--(axis cs:9100000,-722.088401489522)
--(axis cs:9200000,-718.170767461594)
--(axis cs:9300000,-717.003945904728)
--(axis cs:9400000,-716.84930251304)
--(axis cs:9500000,-714.99108775197)
--(axis cs:9600000,-711.861893589914)
--(axis cs:9700000,-709.242904584816)
--(axis cs:9800000,-708.217707150403)
--(axis cs:9900000,-708.028455520421)
--(axis cs:10000000,-706.334409258593)
--(axis cs:10100000,-705.18278276308)
--(axis cs:10200000,-707.16955328091)
--(axis cs:10300000,-706.972930395026)
--(axis cs:10400000,-703.293169686294)
--(axis cs:10500000,-703.114525144781)
--(axis cs:10600000,-699.493744093816)
--(axis cs:10700000,-695.677840939442)
--(axis cs:10800000,-691.116718881897)
--(axis cs:10900000,-686.919194950624)
--(axis cs:11000000,-683.006196237902)
--(axis cs:11100000,-680.512052152678)
--(axis cs:11200000,-675.886717770449)
--(axis cs:11300000,-672.41213012183)
--(axis cs:11400000,-671.925288827668)
--(axis cs:11500000,-667.236375527717)
--(axis cs:11600000,-667.125748767867)
--(axis cs:11700000,-666.182793279289)
--(axis cs:11800000,-664.745176777481)
--(axis cs:11900000,-662.261942569206)
--(axis cs:12000000,-661.386438113483)
--(axis cs:12100000,-660.33785089909)
--(axis cs:12200000,-656.19589186178)
--(axis cs:12300000,-654.185278849895)
--(axis cs:12400000,-652.832022711455)
--(axis cs:12500000,-652.127900948462)
--(axis cs:12600000,-650.96933540122)
--(axis cs:12700000,-650.260747485965)
--(axis cs:12800000,-650.2632047291)
--(axis cs:12900000,-649.38745747453)
--(axis cs:13000000,-649.499118382919)
--(axis cs:13100000,-648.246757738288)
--(axis cs:13200000,-650.329614496493)
--(axis cs:13300000,-652.578420224094)
--(axis cs:13400000,-652.647510546134)
--(axis cs:13500000,-654.539231016054)
--(axis cs:13600000,-655.71293728494)
--(axis cs:13700000,-655.577928298233)
--(axis cs:13800000,-656.09134785362)
--(axis cs:13900000,-657.926405662493)
--(axis cs:14000000,-657.720825521147)
--(axis cs:14100000,-657.605379699922)
--(axis cs:14200000,-658.383524526318)
--(axis cs:14300000,-656.896341105705)
--(axis cs:14400000,-654.890000260248)
--(axis cs:14500000,-652.164224087151)
--(axis cs:14600000,-651.793567524594)
--(axis cs:14700000,-651.78262905319)
--(axis cs:14800000,-650.116390357828)
--(axis cs:14900000,-649.327276119998)
--(axis cs:14900000,-354.182831692074)
--(axis cs:14900000,-354.182831692074)
--(axis cs:14800000,-358.183059003394)
--(axis cs:14700000,-357.819566400294)
--(axis cs:14600000,-357.220473632449)
--(axis cs:14500000,-361.477447258466)
--(axis cs:14400000,-366.422242928159)
--(axis cs:14300000,-370.52082096061)
--(axis cs:14200000,-374.817463216609)
--(axis cs:14100000,-367.690731309753)
--(axis cs:14000000,-364.59964347451)
--(axis cs:13900000,-363.261244381514)
--(axis cs:13800000,-360.551641596775)
--(axis cs:13700000,-361.678091488363)
--(axis cs:13600000,-362.939822971504)
--(axis cs:13500000,-359.559225155356)
--(axis cs:13400000,-357.398450260219)
--(axis cs:13300000,-359.221265079134)
--(axis cs:13200000,-354.307433479763)
--(axis cs:13100000,-357.02579091626)
--(axis cs:13000000,-360.959661182603)
--(axis cs:12900000,-360.41081344194)
--(axis cs:12800000,-358.539938971261)
--(axis cs:12700000,-356.232806333861)
--(axis cs:12600000,-357.728704571052)
--(axis cs:12500000,-356.138391043606)
--(axis cs:12400000,-355.506135497401)
--(axis cs:12300000,-353.21053494786)
--(axis cs:12200000,-355.935861374191)
--(axis cs:12100000,-356.213070463208)
--(axis cs:12000000,-359.609851497337)
--(axis cs:11900000,-360.744538677487)
--(axis cs:11800000,-363.978495105226)
--(axis cs:11700000,-362.949893537548)
--(axis cs:11600000,-363.616618176217)
--(axis cs:11500000,-368.476597626343)
--(axis cs:11400000,-374.300432269069)
--(axis cs:11300000,-375.485070862955)
--(axis cs:11200000,-377.227338312813)
--(axis cs:11100000,-379.885569883277)
--(axis cs:11000000,-381.248541640327)
--(axis cs:10900000,-384.997644023563)
--(axis cs:10800000,-388.480006759464)
--(axis cs:10700000,-395.079970675684)
--(axis cs:10600000,-392.912827654611)
--(axis cs:10500000,-391.318448659012)
--(axis cs:10400000,-389.250866682051)
--(axis cs:10300000,-388.950798891763)
--(axis cs:10200000,-387.711211378818)
--(axis cs:10100000,-385.832748685089)
--(axis cs:10000000,-385.827289977613)
--(axis cs:9900000,-387.562609958075)
--(axis cs:9800000,-389.131716801147)
--(axis cs:9700000,-391.448802934136)
--(axis cs:9600000,-398.831108492621)
--(axis cs:9500000,-402.688121520806)
--(axis cs:9400000,-403.482900647016)
--(axis cs:9300000,-405.454377235459)
--(axis cs:9200000,-406.945392372587)
--(axis cs:9100000,-409.089381077706)
--(axis cs:9000000,-412.004971512373)
--(axis cs:8900000,-412.805266176402)
--(axis cs:8800000,-408.479331200708)
--(axis cs:8700000,-407.612264999519)
--(axis cs:8600000,-404.461710252187)
--(axis cs:8500000,-402.284712171651)
--(axis cs:8400000,-405.919160831309)
--(axis cs:8300000,-406.152472408405)
--(axis cs:8200000,-410.204527801257)
--(axis cs:8100000,-415.179089481411)
--(axis cs:8000000,-412.748765930053)
--(axis cs:7900000,-415.172572586613)
--(axis cs:7800000,-419.169356735321)
--(axis cs:7700000,-418.374605540871)
--(axis cs:7600000,-415.322374145828)
--(axis cs:7500000,-417.46988295509)
--(axis cs:7400000,-415.748576237021)
--(axis cs:7300000,-415.756793577683)
--(axis cs:7200000,-415.900797795702)
--(axis cs:7100000,-415.846092869704)
--(axis cs:7000000,-419.281391427625)
--(axis cs:6900000,-415.601375044033)
--(axis cs:6800000,-419.58821625309)
--(axis cs:6700000,-423.606372928259)
--(axis cs:6600000,-427.071976400881)
--(axis cs:6500000,-427.743594079605)
--(axis cs:6400000,-428.255047028066)
--(axis cs:6300000,-429.275973032835)
--(axis cs:6200000,-430.43637437293)
--(axis cs:6100000,-432.73753846384)
--(axis cs:6000000,-433.826773259789)
--(axis cs:5900000,-439.626895673573)
--(axis cs:5800000,-440.337841525851)
--(axis cs:5700000,-440.494408233173)
--(axis cs:5600000,-449.001140881142)
--(axis cs:5500000,-454.269195601161)
--(axis cs:5400000,-457.070590275292)
--(axis cs:5300000,-460.984024308308)
--(axis cs:5200000,-464.536635667478)
--(axis cs:5100000,-466.000934880544)
--(axis cs:5000000,-467.983467306685)
--(axis cs:4900000,-469.997612692468)
--(axis cs:4800000,-470.809167434198)
--(axis cs:4700000,-474.852145826609)
--(axis cs:4600000,-472.869816850726)
--(axis cs:4500000,-474.682234580593)
--(axis cs:4400000,-479.986472370165)
--(axis cs:4300000,-484.346911858217)
--(axis cs:4200000,-487.183138721686)
--(axis cs:4100000,-490.043080454293)
--(axis cs:4000000,-496.037204046908)
--(axis cs:3900000,-499.889842887125)
--(axis cs:3800000,-503.780241228085)
--(axis cs:3700000,-506.963016233884)
--(axis cs:3600000,-512.24258629493)
--(axis cs:3500000,-514.911368283954)
--(axis cs:3400000,-517.695087729675)
--(axis cs:3300000,-520.986737756042)
--(axis cs:3200000,-523.985634251448)
--(axis cs:3100000,-525.397239647441)
--(axis cs:3000000,-527.504912030684)
--(axis cs:2900000,-532.111850657005)
--(axis cs:2800000,-540.234019665116)
--(axis cs:2700000,-546.756022447411)
--(axis cs:2600000,-553.593682281703)
--(axis cs:2500000,-560.752791830269)
--(axis cs:2400000,-568.409852632319)
--(axis cs:2300000,-574.593040419657)
--(axis cs:2200000,-581.360573682256)
--(axis cs:2100000,-590.628086836266)
--(axis cs:2000000,-593.596253885511)
--(axis cs:1900000,-599.121617933695)
--(axis cs:1800000,-601.90910939657)
--(axis cs:1700000,-609.606494902185)
--(axis cs:1600000,-616.004349351991)
--(axis cs:1500000,-622.45925024726)
--(axis cs:1400000,-627.362071475513)
--(axis cs:1300000,-634.870154603126)
--(axis cs:1200000,-640.100364584404)
--(axis cs:1100000,-648.324425437747)
--(axis cs:1000000,-660.214365734753)
--(axis cs:900000,-670.189036283192)
--(axis cs:800000,-681.816278278769)
--(axis cs:700000,-690.954467356663)
--(axis cs:600000,-705.306569088089)
--(axis cs:500000,-710.189391855012)
--(axis cs:400000,-716.729340204572)
--(axis cs:300000,-722.951090249833)
--(axis cs:200000,-733.391812408179)
--(axis cs:100000,-742.362843748353)
--cycle;

\addplot [semithick, darkorange]
table {%
100000 -885.239038025737
200000 -872.790217029469
300000 -857.9906441575
400000 -842.292317050695
500000 -827.863390253567
600000 -814.196466965303
700000 -782.65077792118
800000 -753.64011705098
900000 -723.922764564007
1000000 -697.369583877288
1100000 -668.465729504985
1200000 -643.174930949671
1300000 -620.81529174344
1400000 -601.774227738194
1500000 -582.473575283103
1600000 -565.561516906917
1700000 -553.087770396943
1800000 -542.847367464751
1900000 -533.37449013448
2000000 -523.184430769222
2100000 -514.104613499319
2200000 -504.620234579767
2300000 -498.13887734166
2400000 -492.289751208859
2500000 -488.518004672974
2600000 -484.441511341669
2700000 -478.770697801635
2800000 -473.655242056586
2900000 -468.319073841708
3000000 -463.840661496756
3100000 -461.111567397875
3200000 -459.051670049516
3300000 -454.30723415258
3400000 -447.910382788169
3500000 -442.584413620407
3600000 -438.156769442881
3700000 -435.459039393663
3800000 -433.022233811046
3900000 -431.420178702424
4000000 -431.15502287471
4100000 -430.111639875881
4200000 -429.001517721104
4300000 -427.571982225465
4400000 -428.213526972271
4500000 -428.989911970484
4600000 -427.872005583768
4700000 -426.323078942435
4800000 -423.145368498377
4900000 -421.166348603889
5000000 -420.261993594443
5100000 -420.144537178452
5200000 -417.070499827601
5300000 -415.764365823319
5400000 -411.72302085453
5500000 -407.204172958819
5600000 -403.729292275372
5700000 -401.712543647376
5800000 -399.618532895533
5900000 -398.812967262491
6000000 -397.494893222017
6100000 -394.594976028999
6200000 -393.304890638975
6300000 -390.923890622134
6400000 -391.265751388197
6500000 -389.975528981102
6600000 -389.830460072073
6700000 -390.173866786783
6800000 -391.974269547388
6900000 -390.640751224533
7000000 -388.764179770301
7100000 -388.977518309392
7200000 -388.677149417226
7300000 -388.657473511385
7400000 -388.642889990037
7500000 -389.172043876362
7600000 -388.76666629071
7700000 -386.790042148146
7800000 -384.940690250769
7900000 -384.754270272689
8000000 -383.57640812628
8100000 -382.458989944756
8200000 -383.215495135051
8300000 -382.920839170602
8400000 -383.037058585199
8500000 -382.669835614947
8600000 -381.493997340637
8700000 -381.020138513334
8800000 -380.45418711856
8900000 -380.232253018406
9000000 -379.412503388238
9100000 -378.040054672174
9200000 -375.224193952332
9300000 -373.471842754732
9400000 -369.778778999361
9500000 -368.5943760515
9600000 -367.113204269546
9700000 -367.543033755807
9800000 -367.112507601678
9900000 -366.578831839338
10000000 -366.278474804734
10100000 -366.512405483934
10200000 -366.55723742151
10300000 -366.465672548873
10400000 -367.737718860321
10500000 -367.057923038229
10600000 -367.552588423068
10700000 -366.30820945736
10800000 -368.821117463919
10900000 -369.568988421683
11000000 -372.309153487645
11100000 -371.425134440735
11200000 -371.69195746587
11300000 -371.241509948472
11400000 -370.377332783739
11500000 -369.755761379364
11600000 -369.350475150906
11700000 -369.187986437182
11800000 -366.014274005654
11900000 -364.245612294202
12000000 -362.43369828434
12100000 -362.200341024647
12200000 -362.279703479881
12300000 -363.141298723283
12400000 -363.271865891628
12500000 -363.861564551915
12600000 -364.558028915438
12700000 -363.875620784673
12800000 -363.294047568577
12900000 -363.659318612206
13000000 -363.608366831752
13100000 -362.307860555537
13200000 -362.268993880885
13300000 -361.144522173355
13400000 -361.904073797961
13500000 -362.078897347922
13600000 -359.724052593373
13700000 -358.158507179059
13800000 -356.942420958839
13900000 -354.525539915003
14000000 -352.25470487463
14100000 -352.180817256595
14200000 -349.367970746184
14300000 -349.256201087336
14400000 -347.571727291097
14500000 -346.685453202476
14600000 -348.389797589618
14700000 -349.529775109887
14800000 -351.216018875254
14900000 -352.813650269533
15000000 -353.454380118698
15100000 -353.540741962331
15200000 -355.616472933354
15300000 -356.428721401791
15400000 -356.942380883656
15500000 -357.340299574025
15600000 -356.952423451891
15700000 -356.803784135294
15800000 -355.093105825906
15900000 -354.550607428352
16000000 -354.508946101298
16100000 -355.416436931367
16200000 -354.760781824234
16300000 -353.810702591493
};
\addplot [semithick, steelblue]
table {%
100000 -810.300840469429
200000 -805.45520757976
300000 -798.705447702657
400000 -794.729264404438
500000 -790.696715210331
600000 -787.096786580746
700000 -776.686049391138
800000 -770.459063924998
900000 -763.389436015764
1000000 -757.827873396724
1100000 -752.028441187165
1200000 -746.656620399973
1300000 -742.984835345319
1400000 -737.776164881417
1500000 -734.390612873861
1600000 -729.958438592468
1700000 -724.141601487867
1800000 -718.328536643258
1900000 -714.652525679767
2000000 -708.905828371687
2100000 -704.741241789332
2200000 -696.731017298294
2300000 -690.78769487464
2400000 -685.418208187116
2500000 -677.948606310551
2600000 -672.160240058452
2700000 -666.368058696049
2800000 -662.46146481795
2900000 -657.028718998645
3000000 -653.474332837335
3100000 -651.300031189897
3200000 -649.946939818774
3300000 -647.478792390227
3400000 -644.589051984272
3500000 -641.958791066217
3600000 -638.944756644432
3700000 -635.161644577725
3800000 -630.292231968684
3900000 -626.858475186995
4000000 -624.121320649683
4100000 -619.638555060008
4200000 -616.615901550459
4300000 -614.251113050601
4400000 -611.305084340274
4500000 -608.964853527163
4600000 -608.201133473601
4700000 -609.199001162521
4800000 -607.635156025674
4900000 -608.408598488953
5000000 -607.483575207463
5100000 -607.052746731682
5200000 -606.197787505835
5300000 -604.601213977741
5400000 -602.00158987371
5500000 -599.54096711957
5600000 -596.511308863184
5700000 -591.351967699166
5800000 -591.838162549841
5900000 -590.843323349378
6000000 -586.809682673195
6100000 -586.112355141065
6200000 -584.844027808628
6300000 -583.060922611249
6400000 -582.164732267112
6500000 -581.951886936064
6600000 -581.186457070602
6700000 -579.34397970538
6800000 -576.448759822824
6900000 -573.801850633642
7000000 -576.102672480025
7100000 -572.874319154216
7200000 -573.649012964134
7300000 -574.284419798276
7400000 -574.656535805974
7500000 -575.938906928258
7600000 -574.767140971933
7700000 -575.917371436017
7800000 -575.757781048375
7900000 -573.075405738354
8000000 -571.879485505096
8100000 -573.213925842771
8200000 -570.307770195305
8300000 -567.290627701155
8400000 -566.188185554998
8500000 -563.416247434744
8600000 -564.17475247762
8700000 -566.411445391859
8800000 -566.731926152536
8900000 -568.600984485043
9000000 -567.388411725398
9100000 -565.588891283614
9200000 -562.55807991709
9300000 -561.229161570094
9400000 -560.166101580028
9500000 -558.839604636388
9600000 -555.346501041268
9700000 -550.345853759476
9800000 -548.674711975775
9900000 -547.795532739248
10000000 -546.080849618103
10100000 -545.507765724084
10200000 -547.440382329864
10300000 -547.961864643395
10400000 -546.272018184172
10500000 -547.216486901896
10600000 -546.203285874214
10700000 -545.378905807563
10800000 -539.798362820681
10900000 -535.958419487093
11000000 -532.127368939114
11100000 -530.198811017977
11200000 -526.557028041631
11300000 -523.948600492392
11400000 -523.112860548369
11500000 -517.85648657703
11600000 -515.371183472042
11700000 -514.566343408419
11800000 -514.361835941353
11900000 -511.503240623346
12000000 -510.49814480541
12100000 -508.275460681149
12200000 -506.065876617985
12300000 -503.697906898877
12400000 -504.169079104428
12500000 -504.133145996034
12600000 -504.349019986136
12700000 -503.246776909913
12800000 -504.401571850181
12900000 -504.899135458235
13000000 -505.229389782761
13100000 -502.636274327274
13200000 -502.318523988128
13300000 -505.899842651614
13400000 -505.022980403176
13500000 -507.049228085705
13600000 -509.326380128222
13700000 -508.628009893298
13800000 -508.321494725198
13900000 -510.593825022004
14000000 -511.160234497828
14100000 -512.648055504837
14200000 -516.600493871463
14300000 -513.708581033157
14400000 -510.656121594203
14500000 -506.820835672809
14600000 -504.507020578522
14700000 -504.801097726742
14800000 -504.149724680611
14900000 -501.755053906036
};


\legend{}
\end{axis}


==> figures/arms_speed_random_onlyaxis.tex <==
\begin{axis}[
name =ax6,
at={(ax5.south east)},
xlabel near ticks, ylabel near ticks,
every y tick scale label/.style={at={(yticklabel* cs:1.03,0cm)},anchor=near yticklabel},
title style={at={(0.5,0.93)}},
every x tick scale label/.style={at={(xticklabel* cs:1.05,-0.05cm)},anchor=near xticklabel},
xshift=1.2cm,
height=\figH,
tick align=outside,
tick pos=left,
title={(f) fast point-reaching (RL)},
width=\figW,
x grid style={darkgray176},
xlabel={steps},
xmin=0, xmax=13500000,
xtick style={color=black},
y grid style={darkgray176},
ylabel={success rate},
ymin=-0.01, ymax=1.01,
ytick style={color=black}
]
\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.1]
(axis cs:100000,0.201258226654789)
--(axis cs:100000,-0.0469725123690745)
--(axis cs:200000,-0.0571471259739246)
--(axis cs:300000,-0.0522499840840786)
--(axis cs:400000,-0.0377963985703348)
--(axis cs:500000,-0.0218414290173717)
--(axis cs:600000,0.00448580833210138)
--(axis cs:700000,0.0541894699409294)
--(axis cs:800000,0.104911045044027)
--(axis cs:900000,0.161629818757389)
--(axis cs:1000000,0.220079499069045)
--(axis cs:1100000,0.289356051997882)
--(axis cs:1200000,0.354770155601875)
--(axis cs:1300000,0.412706286469163)
--(axis cs:1400000,0.466945676549054)
--(axis cs:1500000,0.521870946380589)
--(axis cs:1600000,0.55337726952564)
--(axis cs:1700000,0.563189208479936)
--(axis cs:1800000,0.612467633376838)
--(axis cs:1900000,0.64203468831498)
--(axis cs:2000000,0.686385270722192)
--(axis cs:2100000,0.712086142689998)
--(axis cs:2200000,0.752546215996132)
--(axis cs:2300000,0.796896798403345)
--(axis cs:2400000,0.831391695831177)
--(axis cs:2500000,0.865886593259009)
--(axis cs:2600000,0.90530933317653)
--(axis cs:2700000,0.945793732613407)
--(axis cs:2800000,0.945793732613407)
--(axis cs:2900000,0.965505102572168)
--(axis cs:3000000,0.970432945061859)
--(axis cs:3100000,0.985216472530929)
--(axis cs:3200000,0.99014431502062)
--(axis cs:3300000,0.99014431502062)
--(axis cs:3400000,0.99507215751031)
--(axis cs:3500000,0.99507215751031)
--(axis cs:3600000,1)
--(axis cs:3700000,1)
--(axis cs:3800000,1)
--(axis cs:3900000,1)
--(axis cs:4000000,1)
--(axis cs:4100000,1)
--(axis cs:4200000,1)
--(axis cs:4300000,1)
--(axis cs:4400000,1)
--(axis cs:4500000,1)
--(axis cs:4600000,1)
--(axis cs:4700000,1)
--(axis cs:4800000,1)
--(axis cs:4900000,1)
--(axis cs:5000000,1)
--(axis cs:5100000,1)
--(axis cs:5200000,1)
--(axis cs:5300000,1)
--(axis cs:5400000,1)
--(axis cs:5500000,1)
--(axis cs:5600000,1)
--(axis cs:5700000,1)
--(axis cs:5800000,1)
--(axis cs:5900000,1)
--(axis cs:6000000,1)
--(axis cs:6100000,1)
--(axis cs:6200000,1)
--(axis cs:6300000,1)
--(axis cs:6400000,1)
--(axis cs:6500000,1)
--(axis cs:6600000,1)
--(axis cs:6700000,1)
--(axis cs:6800000,1)
--(axis cs:6900000,1)
--(axis cs:7000000,1)
--(axis cs:7100000,1)
--(axis cs:7200000,1)
--(axis cs:7300000,1)
--(axis cs:7400000,1)
--(axis cs:7500000,1)
--(axis cs:7600000,1)
--(axis cs:7700000,1)
--(axis cs:7800000,1)
--(axis cs:7900000,1)
--(axis cs:8000000,1)
--(axis cs:8100000,1)
--(axis cs:8200000,1)
--(axis cs:8300000,1)
--(axis cs:8400000,1)
--(axis cs:8500000,1)
--(axis cs:8600000,1)
--(axis cs:8700000,1)
--(axis cs:8800000,1)
--(axis cs:8900000,1)
--(axis cs:9000000,1)
--(axis cs:9100000,1)
--(axis cs:9200000,1)
--(axis cs:9300000,1)
--(axis cs:9400000,1)
--(axis cs:9500000,1)
--(axis cs:9600000,1)
--(axis cs:9700000,1)
--(axis cs:9800000,1)
--(axis cs:9900000,1)
--(axis cs:10000000,1)
--(axis cs:10100000,1)
--(axis cs:10200000,1)
--(axis cs:10300000,1)
--(axis cs:10400000,1)
--(axis cs:10500000,1)
--(axis cs:10600000,1)
--(axis cs:10700000,1)
--(axis cs:10800000,1)
--(axis cs:10900000,1)
--(axis cs:11000000,1)
--(axis cs:11100000,1)
--(axis cs:11200000,1)
--(axis cs:11300000,1)
--(axis cs:11400000,1)
--(axis cs:11500000,1)
--(axis cs:11600000,1)
--(axis cs:11700000,1)
--(axis cs:11800000,1)
--(axis cs:11900000,1)
--(axis cs:12000000,1)
--(axis cs:12100000,1)
--(axis cs:12200000,1)
--(axis cs:12300000,1)
--(axis cs:12400000,1)
--(axis cs:12500000,1)
--(axis cs:12600000,1)
--(axis cs:12700000,1)
--(axis cs:12800000,1)
--(axis cs:12900000,1)
--(axis cs:13000000,1)
--(axis cs:13100000,1)
--(axis cs:13200000,1)
--(axis cs:13300000,1)
--(axis cs:13400000,1)
--(axis cs:13500000,1)
--(axis cs:13600000,1)
--(axis cs:13700000,1)
--(axis cs:13800000,1)
--(axis cs:13900000,1)
--(axis cs:14000000,1)
--(axis cs:14100000,1)
--(axis cs:14200000,1)
--(axis cs:14300000,1)
--(axis cs:14300000,1)
--(axis cs:14300000,1)
--(axis cs:14200000,1)
--(axis cs:14100000,1)
--(axis cs:14000000,1)
--(axis cs:13900000,1)
--(axis cs:13800000,1)
--(axis cs:13700000,1)
--(axis cs:13600000,1)
--(axis cs:13500000,1)
--(axis cs:13400000,1)
--(axis cs:13300000,1)
--(axis cs:13200000,1)
--(axis cs:13100000,1)
--(axis cs:13000000,1)
--(axis cs:12900000,1)
--(axis cs:12800000,1)
--(axis cs:12700000,1)
--(axis cs:12600000,1)
--(axis cs:12500000,1)
--(axis cs:12400000,1)
--(axis cs:12300000,1)
--(axis cs:12200000,1)
--(axis cs:12100000,1)
--(axis cs:12000000,1)
--(axis cs:11900000,1)
--(axis cs:11800000,1)
--(axis cs:11700000,1)
--(axis cs:11600000,1)
--(axis cs:11500000,1)
--(axis cs:11400000,1)
--(axis cs:11300000,1)
--(axis cs:11200000,1)
--(axis cs:11100000,1)
--(axis cs:11000000,1)
--(axis cs:10900000,1)
--(axis cs:10800000,1)
--(axis cs:10700000,1)
--(axis cs:10600000,1)
--(axis cs:10500000,1)
--(axis cs:10400000,1)
--(axis cs:10300000,1)
--(axis cs:10200000,1)
--(axis cs:10100000,1)
--(axis cs:10000000,1)
--(axis cs:9900000,1)
--(axis cs:9800000,1)
--(axis cs:9700000,1)
--(axis cs:9600000,1)
--(axis cs:9500000,1)
--(axis cs:9400000,1)
--(axis cs:9300000,1)
--(axis cs:9200000,1)
--(axis cs:9100000,1)
--(axis cs:9000000,1)
--(axis cs:8900000,1)
--(axis cs:8800000,1)
--(axis cs:8700000,1)
--(axis cs:8600000,1)
--(axis cs:8500000,1)
--(axis cs:8400000,1)
--(axis cs:8300000,1)
--(axis cs:8200000,1)
--(axis cs:8100000,1)
--(axis cs:8000000,1)
--(axis cs:7900000,1)
--(axis cs:7800000,1)
--(axis cs:7700000,1)
--(axis cs:7600000,1)
--(axis cs:7500000,1)
--(axis cs:7400000,1)
--(axis cs:7300000,1)
--(axis cs:7200000,1)
--(axis cs:7100000,1)
--(axis cs:7000000,1)
--(axis cs:6900000,1)
--(axis cs:6800000,1)
--(axis cs:6700000,1)
--(axis cs:6600000,1)
--(axis cs:6500000,1)
--(axis cs:6400000,1)
--(axis cs:6300000,1)
--(axis cs:6200000,1)
--(axis cs:6100000,1)
--(axis cs:6000000,1)
--(axis cs:5900000,1)
--(axis cs:5800000,1)
--(axis cs:5700000,1)
--(axis cs:5600000,1)
--(axis cs:5500000,1)
--(axis cs:5400000,1)
--(axis cs:5300000,1)
--(axis cs:5200000,1)
--(axis cs:5100000,1)
--(axis cs:5000000,1)
--(axis cs:4900000,1)
--(axis cs:4800000,1)
--(axis cs:4700000,1)
--(axis cs:4600000,1)
--(axis cs:4500000,1)
--(axis cs:4400000,1)
--(axis cs:4300000,1)
--(axis cs:4200000,1)
--(axis cs:4100000,1)
--(axis cs:4000000,1)
--(axis cs:3900000,1)
--(axis cs:3800000,1)
--(axis cs:3700000,1)
--(axis cs:3600000,1)
--(axis cs:3500000,1.00207069963255)
--(axis cs:3400000,1.00207069963255)
--(axis cs:3300000,1.00414139926509)
--(axis cs:3200000,1.00414139926509)
--(axis cs:3100000,1.00621209889764)
--(axis cs:3000000,1.01242419779528)
--(axis cs:2900000,1.01449489742783)
--(axis cs:2800000,1.02277769595802)
--(axis cs:2700000,1.02277769595802)
--(axis cs:2600000,1.03754780968061)
--(axis cs:2500000,1.05411340674099)
--(axis cs:2400000,1.06860830416882)
--(axis cs:2300000,1.08310320159666)
--(axis cs:2200000,1.10173949828958)
--(axis cs:2100000,1.11648528588143)
--(axis cs:2000000,1.12504330070638)
--(axis cs:1900000,1.14367959739931)
--(axis cs:1800000,1.15610379519459)
--(axis cs:1700000,1.17681079152006)
--(axis cs:1600000,1.18090844476007)
--(axis cs:1500000,1.17241476790513)
--(axis cs:1400000,1.15591146630809)
--(axis cs:1300000,1.13015085638798)
--(axis cs:1200000,1.09094413011241)
--(axis cs:1100000,1.05064394800212)
--(axis cs:1000000,0.98563478664524)
--(axis cs:900000,0.892655895528325)
--(axis cs:800000,0.795088954955973)
--(axis cs:700000,0.674381958630499)
--(axis cs:600000,0.555514191667899)
--(axis cs:500000,0.494857302033245)
--(axis cs:400000,0.434224969998906)
--(axis cs:300000,0.366535698369793)
--(axis cs:200000,0.295242364069163)
--(axis cs:100000,0.201258226654789)
--cycle;

\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.1]
(axis cs:100000,0.910951983289414)
--(axis cs:100000,0.137048016710586)
--(axis cs:200000,0.152445378019119)
--(axis cs:300000,0.175615111504607)
--(axis cs:400000,0.207574233131124)
--(axis cs:500000,0.220813167457139)
--(axis cs:600000,0.235456532293416)
--(axis cs:700000,0.274529982368218)
--(axis cs:800000,0.295714746777949)
--(axis cs:900000,0.307371434880609)
--(axis cs:1000000,0.32062514485972)
--(axis cs:1100000,0.336438696385672)
--(axis cs:1200000,0.3476008872865)
--(axis cs:1300000,0.347666767921404)
--(axis cs:1400000,0.336001310711483)
--(axis cs:1500000,0.335482997305846)
--(axis cs:1600000,0.331692583102507)
--(axis cs:1700000,0.333511263056433)
--(axis cs:1800000,0.330012429131821)
--(axis cs:1900000,0.342512904219929)
--(axis cs:2000000,0.353783343727486)
--(axis cs:2100000,0.371924575646239)
--(axis cs:2200000,0.391421797982091)
--(axis cs:2300000,0.408978901515831)
--(axis cs:2400000,0.419572739854766)
--(axis cs:2500000,0.436434722284217)
--(axis cs:2600000,0.448235923295762)
--(axis cs:2700000,0.457112291656839)
--(axis cs:2800000,0.469720608872094)
--(axis cs:2900000,0.477165262830146)
--(axis cs:3000000,0.479458473083794)
--(axis cs:3100000,0.476517453566026)
--(axis cs:3200000,0.479818845171768)
--(axis cs:3300000,0.483384527950383)
--(axis cs:3400000,0.492086339666068)
--(axis cs:3500000,0.496053544396121)
--(axis cs:3600000,0.500658656572412)
--(axis cs:3700000,0.499670751858444)
--(axis cs:3800000,0.509914483408265)
--(axis cs:3900000,0.514983102376816)
--(axis cs:4000000,0.523014850914447)
--(axis cs:4100000,0.52111281437746)
--(axis cs:4200000,0.519797908739154)
--(axis cs:4300000,0.521752013636743)
--(axis cs:4400000,0.528650210838127)
--(axis cs:4500000,0.530615194785067)
--(axis cs:4600000,0.537208021461833)
--(axis cs:4700000,0.54475192829951)
--(axis cs:4800000,0.54761390788643)
--(axis cs:4900000,0.545300207234661)
--(axis cs:5000000,0.543032344729298)
--(axis cs:5100000,0.556695682617844)
--(axis cs:5200000,0.551956938094187)
--(axis cs:5300000,0.553956938094187)
--(axis cs:5400000,0.554702442422532)
--(axis cs:5500000,0.549879365614181)
--(axis cs:5600000,0.545625038844196)
--(axis cs:5700000,0.53547134226345)
--(axis cs:5800000,0.530219612988428)
--(axis cs:5900000,0.525288749077576)
--(axis cs:6000000,0.515012034783141)
--(axis cs:6100000,0.490398684666507)
--(axis cs:6200000,0.491227392003138)
--(axis cs:6300000,0.488223900609395)
--(axis cs:6400000,0.465391263238866)
--(axis cs:6500000,0.471199425383139)
--(axis cs:6600000,0.464329702915313)
--(axis cs:6700000,0.466983318064151)
--(axis cs:6800000,0.467164745900097)
--(axis cs:6900000,0.471134233766914)
--(axis cs:7000000,0.481724989025839)
--(axis cs:7100000,0.487400477571043)
--(axis cs:7200000,0.486480398394148)
--(axis cs:7300000,0.478526638626654)
--(axis cs:7400000,0.490059670657724)
--(axis cs:7500000,0.491444619255158)
--(axis cs:7600000,0.494635261249715)
--(axis cs:7700000,0.502817699486164)
--(axis cs:7800000,0.505934179384367)
--(axis cs:7900000,0.499343424125443)
--(axis cs:8000000,0.506213280129202)
--(axis cs:8100000,0.513345373391516)
--(axis cs:8200000,0.506809284455146)
--(axis cs:8300000,0.514435829538307)
--(axis cs:8400000,0.520935363744522)
--(axis cs:8500000,0.515931048868324)
--(axis cs:8600000,0.524198911373687)
--(axis cs:8700000,0.521540921138959)
--(axis cs:8800000,0.527293621080277)
--(axis cs:8900000,0.529012694182512)
--(axis cs:9000000,0.518173350311936)
--(axis cs:9100000,0.521763584958529)
--(axis cs:9200000,0.536724569566774)
--(axis cs:9300000,0.542633049526497)
--(axis cs:9400000,0.546348773674327)
--(axis cs:9500000,0.548986383317317)
--(axis cs:9600000,0.541063073909627)
--(axis cs:9700000,0.545106012741789)
--(axis cs:9800000,0.54510601274179)
--(axis cs:9900000,0.554315672123002)
--(axis cs:10000000,0.565971119025329)
--(axis cs:10100000,0.567671486606862)
--(axis cs:10200000,0.566554330544422)
--(axis cs:10300000,0.566554330544422)
--(axis cs:10400000,0.568419871671982)
--(axis cs:10500000,0.570120239253515)
--(axis cs:10600000,0.581775686155842)
--(axis cs:10700000,0.577441709127989)
--(axis cs:10800000,0.577777671048283)
--(axis cs:10900000,0.579528355685373)
--(axis cs:11000000,0.577595096591181)
--(axis cs:11100000,0.57520222610429)
--(axis cs:11200000,0.567908989746809)
--(axis cs:11300000,0.56367674338604)
--(axis cs:11400000,0.564492846417791)
--(axis cs:11500000,0.564492846417791)
--(axis cs:11600000,0.564492846417791)
--(axis cs:11700000,0.568160485793968)
--(axis cs:11800000,0.562742161780702)
--(axis cs:11900000,0.555112963502927)
--(axis cs:12000000,0.545390775694791)
--(axis cs:12100000,0.547783646181683)
--(axis cs:12200000,0.549994520446191)
--(axis cs:12300000,0.549994520446191)
--(axis cs:12400000,0.544946171053671)
--(axis cs:12500000,0.544946171053671)
--(axis cs:12600000,0.537930549866507)
--(axis cs:12700000,0.53426291049033)
--(axis cs:12800000,0.539345272583303)
--(axis cs:12900000,0.547755665003224)
--(axis cs:13000000,0.556063130094563)
--(axis cs:13100000,0.552395490718386)
--(axis cs:13200000,0.552395490718386)
--(axis cs:13300000,0.552395490718386)
--(axis cs:13400000,0.552715377901007)
--(axis cs:13500000,0.550989777402367)
--(axis cs:13600000,0.554010633012939)
--(axis cs:13700000,0.558038440493703)
--(axis cs:13700000,1.17529489283963)
--(axis cs:13700000,1.17529489283963)
--(axis cs:13600000,1.17456079555849)
--(axis cs:13500000,1.17401022259763)
--(axis cs:13400000,1.17395128876566)
--(axis cs:13300000,1.17360450928161)
--(axis cs:13200000,1.17360450928161)
--(axis cs:13100000,1.17360450928161)
--(axis cs:13000000,1.17393686990544)
--(axis cs:12900000,1.17424433499678)
--(axis cs:12800000,1.1726547274167)
--(axis cs:12700000,1.17173708950967)
--(axis cs:12600000,1.17206945013349)
--(axis cs:12500000,1.17505382894633)
--(axis cs:12400000,1.17505382894633)
--(axis cs:12300000,1.17800547955381)
--(axis cs:12200000,1.17800547955381)
--(axis cs:12100000,1.17821635381832)
--(axis cs:12000000,1.17660922430521)
--(axis cs:11900000,1.17688703649707)
--(axis cs:11800000,1.1772578382193)
--(axis cs:11700000,1.17783951420603)
--(axis cs:11600000,1.17750715358221)
--(axis cs:11500000,1.17750715358221)
--(axis cs:11400000,1.17750715358221)
--(axis cs:11300000,1.17632325661396)
--(axis cs:11200000,1.17809101025319)
--(axis cs:11100000,1.17879777389571)
--(axis cs:11000000,1.18040490340882)
--(axis cs:10900000,1.18247164431463)
--(axis cs:10800000,1.18222232895172)
--(axis cs:10700000,1.18255829087201)
--(axis cs:10600000,1.18222431384416)
--(axis cs:10500000,1.17987976074649)
--(axis cs:10400000,1.17958012832802)
--(axis cs:10300000,1.17744566945558)
--(axis cs:10200000,1.17744566945558)
--(axis cs:10100000,1.17832851339314)
--(axis cs:10000000,1.17802888097467)
--(axis cs:9900000,1.175684327877)
--(axis cs:9800000,1.17089398725821)
--(axis cs:9700000,1.17089398725821)
--(axis cs:9600000,1.16893692609037)
--(axis cs:9500000,1.16701361668268)
--(axis cs:9400000,1.16565122632567)
--(axis cs:9300000,1.1633669504735)
--(axis cs:9200000,1.15927543043323)
--(axis cs:9100000,1.15623641504147)
--(axis cs:9000000,1.15382664968806)
--(axis cs:8900000,1.15498730581749)
--(axis cs:8800000,1.16070637891972)
--(axis cs:8700000,1.15845907886104)
--(axis cs:8600000,1.15980108862631)
--(axis cs:8500000,1.15806895113168)
--(axis cs:8400000,1.15906463625548)
--(axis cs:8300000,1.15956417046169)
--(axis cs:8200000,1.15919071554485)
--(axis cs:8100000,1.15665462660848)
--(axis cs:8000000,1.1557867198708)
--(axis cs:7900000,1.15265657587456)
--(axis cs:7800000,1.15006582061563)
--(axis cs:7700000,1.14918230051384)
--(axis cs:7600000,1.14536473875028)
--(axis cs:7500000,1.14455538074484)
--(axis cs:7400000,1.14394032934228)
--(axis cs:7300000,1.13947336137335)
--(axis cs:7200000,1.13951960160585)
--(axis cs:7100000,1.14059952242896)
--(axis cs:7000000,1.14427501097416)
--(axis cs:6900000,1.14286576623309)
--(axis cs:6800000,1.1448352540999)
--(axis cs:6700000,1.14101668193585)
--(axis cs:6600000,1.14567029708469)
--(axis cs:6500000,1.14680057461686)
--(axis cs:6400000,1.14460873676113)
--(axis cs:6300000,1.15177609939061)
--(axis cs:6200000,1.15277260799686)
--(axis cs:6100000,1.14960131533349)
--(axis cs:6000000,1.14898796521686)
--(axis cs:5900000,1.14871125092242)
--(axis cs:5800000,1.14578038701157)
--(axis cs:5700000,1.14852865773655)
--(axis cs:5600000,1.1463749611558)
--(axis cs:5500000,1.14812063438582)
--(axis cs:5400000,1.14729755757747)
--(axis cs:5300000,1.14604306190581)
--(axis cs:5200000,1.14404306190581)
--(axis cs:5100000,1.14730431738216)
--(axis cs:5000000,1.1449676552707)
--(axis cs:4900000,1.14469979276534)
--(axis cs:4800000,1.14438609211357)
--(axis cs:4700000,1.14324807170049)
--(axis cs:4600000,1.14479197853817)
--(axis cs:4500000,1.13938480521493)
--(axis cs:4400000,1.13934978916187)
--(axis cs:4300000,1.13624798636326)
--(axis cs:4200000,1.13620209126085)
--(axis cs:4100000,1.13088718562254)
--(axis cs:4000000,1.12898514908555)
--(axis cs:3900000,1.12901689762318)
--(axis cs:3800000,1.12608551659173)
--(axis cs:3700000,1.12232924814156)
--(axis cs:3600000,1.11734134342759)
--(axis cs:3500000,1.11594645560388)
--(axis cs:3400000,1.11391366033393)
--(axis cs:3300000,1.11261547204962)
--(axis cs:3200000,1.10618115482823)
--(axis cs:3100000,1.11148254643397)
--(axis cs:3000000,1.11054152691621)
--(axis cs:2900000,1.11083473716985)
--(axis cs:2800000,1.10827939112791)
--(axis cs:2700000,1.10688770834316)
--(axis cs:2600000,1.10176407670424)
--(axis cs:2500000,1.10156527771578)
--(axis cs:2400000,1.10042726014523)
--(axis cs:2300000,1.09502109848417)
--(axis cs:2200000,1.09657820201791)
--(axis cs:2100000,1.09207542435376)
--(axis cs:2000000,1.09421665627251)
--(axis cs:1900000,1.08948709578007)
--(axis cs:1800000,1.09398757086818)
--(axis cs:1700000,1.09448873694357)
--(axis cs:1600000,1.10430741689749)
--(axis cs:1500000,1.10851700269415)
--(axis cs:1400000,1.10799868928852)
--(axis cs:1300000,1.1143332320786)
--(axis cs:1200000,1.1123991127135)
--(axis cs:1100000,1.11356130361433)
--(axis cs:1000000,1.10137485514028)
--(axis cs:900000,1.09462856511939)
--(axis cs:800000,1.08628525322205)
--(axis cs:700000,1.05747001763178)
--(axis cs:600000,1.00854346770658)
--(axis cs:500000,0.994742388098416)
--(axis cs:400000,0.982425766868876)
--(axis cs:300000,0.961527745638251)
--(axis cs:200000,0.944221288647548)
--(axis cs:100000,0.910951983289414)
--cycle;

\addplot [semithick, darkorange]
table {%
100000 0.0771428571428572
200000 0.119047619047619
300000 0.157142857142857
400000 0.198214285714286
500000 0.236507936507937
600000 0.28
700000 0.364285714285714
800000 0.45
900000 0.527142857142857
1000000 0.602857142857143
1100000 0.67
1200000 0.722857142857143
1300000 0.771428571428571
1400000 0.811428571428571
1500000 0.847142857142857
1600000 0.867142857142857
1700000 0.87
1800000 0.884285714285714
1900000 0.892857142857143
2000000 0.905714285714285
2100000 0.914285714285714
2200000 0.927142857142857
2300000 0.94
2400000 0.95
2500000 0.96
2600000 0.971428571428571
2700000 0.984285714285714
2800000 0.984285714285714
2900000 0.99
3000000 0.991428571428571
3100000 0.995714285714286
3200000 0.997142857142857
3300000 0.997142857142857
3400000 0.998571428571429
3500000 0.998571428571429
3600000 1
3700000 1
3800000 1
3900000 1
4000000 1
4100000 1
4200000 1
4300000 1
4400000 1
4500000 1
4600000 1
4700000 1
4800000 1
4900000 1
5000000 1
5100000 1
5200000 1
5300000 1
5400000 1
5500000 1
5600000 1
5700000 1
5800000 1
5900000 1
6000000 1
6100000 1
6200000 1
6300000 1
6400000 1
6500000 1
6600000 1
6700000 1
6800000 1
6900000 1
7000000 1
7100000 1
7200000 1
7300000 1
7400000 1
7500000 1
7600000 1
7700000 1
7800000 1
7900000 1
8000000 1
8100000 1
8200000 1
8300000 1
8400000 1
8500000 1
8600000 1
8700000 1
8800000 1
8900000 1
9000000 1
9100000 1
9200000 1
9300000 1
9400000 1
9500000 1
9600000 1
9700000 1
9800000 1
9900000 1
10000000 1
10100000 1
10200000 1
10300000 1
10400000 1
10500000 1
10600000 1
10700000 1
10800000 1
10900000 1
11000000 1
11100000 1
11200000 1
11300000 1
11400000 1
11500000 1
11600000 1
11700000 1
11800000 1
11900000 1
12000000 1
12100000 1
12200000 1
12300000 1
12400000 1
12500000 1
12600000 1
12700000 1
12800000 1
12900000 1
13000000 1
13100000 1
13200000 1
13300000 1
13400000 1
13500000 1
13600000 1
13700000 1
13800000 1
13900000 1
14000000 1
14100000 1
14200000 1
14300000 1
};
\addplot [semithick, steelblue]
table {%
100000 0.524
200000 0.548333333333333
300000 0.568571428571429
400000 0.595
500000 0.607777777777778
600000 0.622
700000 0.666
800000 0.691
900000 0.701
1000000 0.711
1100000 0.725
1200000 0.73
1300000 0.731
1400000 0.722
1500000 0.722
1600000 0.718
1700000 0.714
1800000 0.712
1900000 0.716
2000000 0.724
2100000 0.732
2200000 0.744
2300000 0.752
2400000 0.76
2500000 0.769
2600000 0.775
2700000 0.782
2800000 0.789
2900000 0.794
3000000 0.795
3100000 0.794
3200000 0.793
3300000 0.798
3400000 0.803
3500000 0.806
3600000 0.809
3700000 0.811
3800000 0.818
3900000 0.822
4000000 0.826
4100000 0.826
4200000 0.828
4300000 0.829
4400000 0.834
4500000 0.835
4600000 0.841
4700000 0.844
4800000 0.846
4900000 0.845
5000000 0.844
5100000 0.852
5200000 0.848
5300000 0.85
5400000 0.851
5500000 0.849
5600000 0.846
5700000 0.842
5800000 0.838
5900000 0.837
6000000 0.832
6100000 0.82
6200000 0.822
6300000 0.82
6400000 0.805
6500000 0.809
6600000 0.805
6700000 0.804
6800000 0.806
6900000 0.807
7000000 0.813
7100000 0.814
7200000 0.813
7300000 0.809
7400000 0.817
7500000 0.818
7600000 0.82
7700000 0.826
7800000 0.828
7900000 0.826
8000000 0.831
8100000 0.835
8200000 0.833
8300000 0.837
8400000 0.84
8500000 0.837
8600000 0.842
8700000 0.84
8800000 0.844
8900000 0.842
9000000 0.836
9100000 0.839
9200000 0.848
9300000 0.853
9400000 0.856
9500000 0.858
9600000 0.855
9700000 0.858
9800000 0.858
9900000 0.865
10000000 0.872
10100000 0.873
10200000 0.872
10300000 0.872
10400000 0.874
10500000 0.875
10600000 0.882
10700000 0.88
10800000 0.88
10900000 0.881
11000000 0.879
11100000 0.877
11200000 0.873
11300000 0.87
11400000 0.871
11500000 0.871
11600000 0.871
11700000 0.873
11800000 0.87
11900000 0.866
12000000 0.861
12100000 0.863
12200000 0.864
12300000 0.864
12400000 0.86
12500000 0.86
12600000 0.855
12700000 0.853
12800000 0.856
12900000 0.861
13000000 0.865
13100000 0.863
13200000 0.863
13300000 0.863
13400000 0.863333333333333
13500000 0.8625
13600000 0.864285714285714
13700000 0.866666666666667
};
\legend{}
\end{axis}


==> figures/bipeds_hopping_onlyaxis.tex <==
\begin{axis}[
name =ax7,
scaled y ticks=base 10:\Factor,
at={(ax6.south east)},
xlabel near ticks, ylabel near ticks,
every y tick scale label/.style={at={(yticklabel* cs:1.03,0cm)},anchor=near yticklabel},
title style={at={(0.5,0.93)}},
every x tick scale label/.style={at={(xticklabel* cs:1.05,-0.05cm)},anchor=near xticklabel},
xshift=1.2cm,
height=\figH,
tick align=outside,
tick pos=left,
title={(g) hopping (RL)},
width=\figW,
x grid style={darkgray176},
xlabel={steps},
xmin=0, xmax=16000000,
xtick style={color=black},
y grid style={darkgray176},
ylabel={hop-return},
ymin=-1104.80038773498, ymax=8514.39021934421,
ytick style={color=black}
]
\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.1]
(axis cs:100000,847.557701639823)
--(axis cs:100000,312.701749511756)
--(axis cs:200000,377.108574402011)
--(axis cs:300000,420.66608908833)
--(axis cs:400000,483.977479535774)
--(axis cs:500000,518.787591683952)
--(axis cs:600000,553.187676884155)
--(axis cs:700000,655.899019944217)
--(axis cs:800000,725.363911541657)
--(axis cs:900000,760.513071614821)
--(axis cs:1000000,793.60786785263)
--(axis cs:1100000,807.08118941718)
--(axis cs:1200000,809.957482325671)
--(axis cs:1300000,850.063045090551)
--(axis cs:1400000,886.392802689847)
--(axis cs:1500000,897.294641168774)
--(axis cs:1600000,925.042803695031)
--(axis cs:1700000,931.986802456423)
--(axis cs:1800000,958.737546299846)
--(axis cs:1900000,996.181546572211)
--(axis cs:2000000,1032.84684546696)
--(axis cs:2100000,1055.50694277429)
--(axis cs:2200000,1108.03977534875)
--(axis cs:2300000,1152.45212976929)
--(axis cs:2400000,1172.14889781371)
--(axis cs:2500000,1216.24725192395)
--(axis cs:2600000,1265.09975751854)
--(axis cs:2700000,1303.24011922992)
--(axis cs:2800000,1362.22479244443)
--(axis cs:2900000,1402.77291564614)
--(axis cs:3000000,1436.88343901475)
--(axis cs:3100000,1495.54162692752)
--(axis cs:3200000,1530.39110791944)
--(axis cs:3300000,1544.78948706613)
--(axis cs:3400000,1544.49448061851)
--(axis cs:3500000,1585.03017309847)
--(axis cs:3600000,1585.88666326425)
--(axis cs:3700000,1586.5190468548)
--(axis cs:3800000,1568.43546115371)
--(axis cs:3900000,1570.52489982505)
--(axis cs:4000000,1572.13647545663)
--(axis cs:4100000,1591.6649845257)
--(axis cs:4200000,1618.48781534403)
--(axis cs:4300000,1640.87531640528)
--(axis cs:4400000,1701.50339114008)
--(axis cs:4500000,1674.81848428047)
--(axis cs:4600000,1692.96405889368)
--(axis cs:4700000,1692.41938987759)
--(axis cs:4800000,1706.76675636638)
--(axis cs:4900000,1722.13983075222)
--(axis cs:5000000,1743.85465673742)
--(axis cs:5100000,1754.56324147573)
--(axis cs:5200000,1759.40169736267)
--(axis cs:5300000,1746.9689632142)
--(axis cs:5400000,1694.22891226257)
--(axis cs:5500000,1740.67323645075)
--(axis cs:5600000,1766.4724257586)
--(axis cs:5700000,1798.17777247609)
--(axis cs:5800000,1831.43826040472)
--(axis cs:5900000,1890.10891707305)
--(axis cs:6000000,1924.09812318889)
--(axis cs:6100000,1972.91567474982)
--(axis cs:6200000,2022.68590761044)
--(axis cs:6300000,2081.14091192297)
--(axis cs:6400000,2175.96277417577)
--(axis cs:6500000,2231.52598529575)
--(axis cs:6600000,2236.89874221298)
--(axis cs:6700000,2246.38934852786)
--(axis cs:6800000,2250.3645230859)
--(axis cs:6900000,2234.52983482122)
--(axis cs:7000000,2240.11756102033)
--(axis cs:7100000,2261.41159815161)
--(axis cs:7200000,2249.66727759431)
--(axis cs:7300000,2228.85089518231)
--(axis cs:7400000,2193.97303127624)
--(axis cs:7500000,2126.67912554039)
--(axis cs:7600000,2138.53459891179)
--(axis cs:7700000,2132.62156288815)
--(axis cs:7800000,2144.37203498263)
--(axis cs:7900000,2171.34144710786)
--(axis cs:8000000,2174.72691647777)
--(axis cs:8100000,2138.95274176031)
--(axis cs:8200000,2113.70546904099)
--(axis cs:8300000,2112.61472138855)
--(axis cs:8400000,2100.22633733922)
--(axis cs:8500000,2127.85616737714)
--(axis cs:8600000,2087.96728106871)
--(axis cs:8700000,2129.02615987682)
--(axis cs:8800000,2119.69454778748)
--(axis cs:8900000,2136.25488275198)
--(axis cs:9000000,2191.48356496091)
--(axis cs:9100000,2230.21826423259)
--(axis cs:9200000,2266.39232885441)
--(axis cs:9300000,2286.43416764717)
--(axis cs:9400000,2332.01115641202)
--(axis cs:9500000,2351.66817439746)
--(axis cs:9600000,2369.48891831752)
--(axis cs:9700000,2350.72049537245)
--(axis cs:9800000,2361.15346132492)
--(axis cs:9900000,2353.82073369197)
--(axis cs:10000000,2299.66921844225)
--(axis cs:10100000,2284.27841506414)
--(axis cs:10200000,2274.67601231337)
--(axis cs:10300000,2276.5543236795)
--(axis cs:10400000,2211.90363671143)
--(axis cs:10500000,2183.1233083855)
--(axis cs:10600000,2175.52847742074)
--(axis cs:10700000,2178.71019830507)
--(axis cs:10800000,2180.27548652755)
--(axis cs:10900000,2145.94188866275)
--(axis cs:11000000,2155.10001676351)
--(axis cs:11100000,2136.86696295213)
--(axis cs:11200000,2111.16037268021)
--(axis cs:11300000,2083.72868029569)
--(axis cs:11400000,2147.77781357742)
--(axis cs:11500000,2169.07562822176)
--(axis cs:11600000,2217.77909643739)
--(axis cs:11700000,2199.46257977165)
--(axis cs:11800000,2186.47511482712)
--(axis cs:11900000,2184.15183718563)
--(axis cs:12000000,2148.51261743325)
--(axis cs:12100000,2162.30136104499)
--(axis cs:12200000,2192.82308237544)
--(axis cs:12300000,2202.00870380072)
--(axis cs:12400000,2191.56055121092)
--(axis cs:12500000,2161.53500792095)
--(axis cs:12600000,2143.20518739266)
--(axis cs:12700000,2148.74871109123)
--(axis cs:12800000,2185.33968723147)
--(axis cs:12900000,2193.87391058849)
--(axis cs:13000000,2234.9443781887)
--(axis cs:13100000,2218.62707950664)
--(axis cs:13200000,2141.21794840414)
--(axis cs:13300000,2153.10427493686)
--(axis cs:13400000,2135.37504203134)
--(axis cs:13500000,2157.68120792685)
--(axis cs:13600000,2132.94900329672)
--(axis cs:13700000,2115.93924386003)
--(axis cs:13800000,2065.03629288101)
--(axis cs:13900000,2050.68903199451)
--(axis cs:14000000,2003.27196234877)
--(axis cs:14100000,1989.72054445264)
--(axis cs:14200000,2080.98129657201)
--(axis cs:14300000,2057.15537312557)
--(axis cs:14400000,2054.64102995203)
--(axis cs:14500000,2061.52834271367)
--(axis cs:14600000,2116.66202250794)
--(axis cs:14700000,2164.81080388976)
--(axis cs:14800000,2173.9998342971)
--(axis cs:14900000,2189.51388246915)
--(axis cs:15000000,2232.58892707878)
--(axis cs:15100000,2263.91803140973)
--(axis cs:15200000,2265.38784931868)
--(axis cs:15300000,2313.01050350301)
--(axis cs:15400000,2321.39966594332)
--(axis cs:15500000,2348.49725695182)
--(axis cs:15600000,2355.27425775128)
--(axis cs:15700000,2366.59930188578)
--(axis cs:15800000,2371.22933109476)
--(axis cs:15900000,2369.47282184158)
--(axis cs:16000000,2358.08718347823)
--(axis cs:16100000,2364.34604685616)
--(axis cs:16200000,2331.16965873418)
--(axis cs:16300000,2284.12297745064)
--(axis cs:16400000,2281.31453842035)
--(axis cs:16500000,2260.53557884352)
--(axis cs:16600000,2249.21612857944)
--(axis cs:16700000,2233.18509931346)
--(axis cs:16800000,2273.97833283472)
--(axis cs:16900000,2267.72597097671)
--(axis cs:17000000,2279.93752693991)
--(axis cs:17100000,2254.58940174139)
--(axis cs:17200000,2266.29559624487)
--(axis cs:17300000,2281.23511733777)
--(axis cs:17400000,2274.03000864648)
--(axis cs:17500000,2244.58598075662)
--(axis cs:17600000,2202.15656400928)
--(axis cs:17700000,2164.52206003621)
--(axis cs:17800000,2147.28675277992)
--(axis cs:17900000,2170.73103316635)
--(axis cs:18000000,2175.80284337565)
--(axis cs:18100000,2173.31240134846)
--(axis cs:18200000,2141.88228903594)
--(axis cs:18300000,2153.755167295)
--(axis cs:18400000,2139.12928540302)
--(axis cs:18500000,2174.72644198079)
--(axis cs:18600000,2218.65905550452)
--(axis cs:18700000,2278.32755422372)
--(axis cs:18800000,2290.08217564621)
--(axis cs:18900000,2321.93977821553)
--(axis cs:19000000,2345.08827509932)
--(axis cs:19100000,2375.94761894336)
--(axis cs:19200000,2411.97878019333)
--(axis cs:19300000,2416.24636880505)
--(axis cs:19400000,2470.00382283399)
--(axis cs:19500000,2464.99491899327)
--(axis cs:19600000,2443.13202417677)
--(axis cs:19700000,2432.95170877588)
--(axis cs:19800000,2435.30800913714)
--(axis cs:19900000,2408.41268262587)
--(axis cs:20000000,2391.84179272255)
--(axis cs:20000000,3735.26053458107)
--(axis cs:20000000,3735.26053458107)
--(axis cs:19900000,3740.39041406229)
--(axis cs:19800000,3752.17051198008)
--(axis cs:19700000,3774.04733645851)
--(axis cs:19600000,3763.19411652262)
--(axis cs:19500000,3812.83304832902)
--(axis cs:19400000,3837.76549597037)
--(axis cs:19300000,3838.96695697173)
--(axis cs:19200000,3830.46352461395)
--(axis cs:19100000,3803.6736127416)
--(axis cs:19000000,3810.28908076675)
--(axis cs:18900000,3818.28529080652)
--(axis cs:18800000,3804.20765043912)
--(axis cs:18700000,3785.57217763313)
--(axis cs:18600000,3787.28224251848)
--(axis cs:18500000,3764.26333262764)
--(axis cs:18400000,3764.05198042839)
--(axis cs:18300000,3726.57171223076)
--(axis cs:18200000,3696.22881955262)
--(axis cs:18100000,3676.63413954501)
--(axis cs:18000000,3632.50955542935)
--(axis cs:17900000,3567.78796994378)
--(axis cs:17800000,3549.48159889908)
--(axis cs:17700000,3555.56959681964)
--(axis cs:17600000,3566.36590813626)
--(axis cs:17500000,3568.52936857144)
--(axis cs:17400000,3581.22606632411)
--(axis cs:17300000,3594.23280780284)
--(axis cs:17200000,3602.432687812)
--(axis cs:17100000,3633.12698882066)
--(axis cs:17000000,3661.52873049649)
--(axis cs:16900000,3714.28346507415)
--(axis cs:16800000,3705.85210877188)
--(axis cs:16700000,3695.43198483058)
--(axis cs:16600000,3707.72690188133)
--(axis cs:16500000,3735.31737239614)
--(axis cs:16400000,3743.29916295066)
--(axis cs:16300000,3772.6990361481)
--(axis cs:16200000,3782.17382350412)
--(axis cs:16100000,3764.58644588382)
--(axis cs:16000000,3744.95480447979)
--(axis cs:15900000,3739.95976375777)
--(axis cs:15800000,3757.28451780066)
--(axis cs:15700000,3739.44398004469)
--(axis cs:15600000,3709.100165368)
--(axis cs:15500000,3691.30898294604)
--(axis cs:15400000,3681.60975827714)
--(axis cs:15300000,3660.97733914978)
--(axis cs:15200000,3673.92585173501)
--(axis cs:15100000,3681.52703155481)
--(axis cs:15000000,3685.44428110084)
--(axis cs:14900000,3652.31816919485)
--(axis cs:14800000,3643.42328067193)
--(axis cs:14700000,3650.0782521664)
--(axis cs:14600000,3657.74935475697)
--(axis cs:14500000,3647.19799747855)
--(axis cs:14400000,3630.9835976366)
--(axis cs:14300000,3625.54151515446)
--(axis cs:14200000,3609.574282564)
--(axis cs:14100000,3604.64859730921)
--(axis cs:14000000,3611.79261127898)
--(axis cs:13900000,3632.20542077244)
--(axis cs:13800000,3654.52161005426)
--(axis cs:13700000,3652.57435730435)
--(axis cs:13600000,3641.27692990891)
--(axis cs:13500000,3620.65816209773)
--(axis cs:13400000,3605.41728318131)
--(axis cs:13300000,3588.85064364994)
--(axis cs:13200000,3560.11074249917)
--(axis cs:13100000,3535.29042172466)
--(axis cs:13000000,3526.78500225225)
--(axis cs:12900000,3534.1460283291)
--(axis cs:12800000,3507.73031711743)
--(axis cs:12700000,3494.35268671409)
--(axis cs:12600000,3507.85198842323)
--(axis cs:12500000,3533.07140837478)
--(axis cs:12400000,3576.32517885895)
--(axis cs:12300000,3605.19989861139)
--(axis cs:12200000,3614.18591838538)
--(axis cs:12100000,3607.60336734673)
--(axis cs:12000000,3622.41073025866)
--(axis cs:11900000,3641.69124079343)
--(axis cs:11800000,3649.75802448743)
--(axis cs:11700000,3676.31634283206)
--(axis cs:11600000,3675.22950381692)
--(axis cs:11500000,3662.45865862258)
--(axis cs:11400000,3640.13804874485)
--(axis cs:11300000,3632.8305466756)
--(axis cs:11200000,3665.37499820788)
--(axis cs:11100000,3702.85753738723)
--(axis cs:11000000,3676.75829345889)
--(axis cs:10900000,3629.71971625855)
--(axis cs:10800000,3635.93631421487)
--(axis cs:10700000,3623.26379049601)
--(axis cs:10600000,3628.80362384012)
--(axis cs:10500000,3632.22337056803)
--(axis cs:10400000,3632.845171731)
--(axis cs:10300000,3631.49133214199)
--(axis cs:10200000,3613.5554756669)
--(axis cs:10100000,3615.33977385138)
--(axis cs:10000000,3624.12242819282)
--(axis cs:9900000,3648.89799638575)
--(axis cs:9800000,3639.8585596372)
--(axis cs:9700000,3634.71573858528)
--(axis cs:9600000,3615.40985730793)
--(axis cs:9500000,3615.36524788177)
--(axis cs:9400000,3585.12356238866)
--(axis cs:9300000,3574.67300328968)
--(axis cs:9200000,3551.96284539624)
--(axis cs:9100000,3491.22109400553)
--(axis cs:9000000,3476.60036614164)
--(axis cs:8900000,3444.33607198208)
--(axis cs:8800000,3429.49922034562)
--(axis cs:8700000,3394.46444811015)
--(axis cs:8600000,3371.25051496498)
--(axis cs:8500000,3341.57484143775)
--(axis cs:8400000,3329.07484760365)
--(axis cs:8300000,3298.48846601405)
--(axis cs:8200000,3324.96559918741)
--(axis cs:8100000,3375.48675507183)
--(axis cs:8000000,3376.49522531462)
--(axis cs:7900000,3398.42827737078)
--(axis cs:7800000,3413.11246581166)
--(axis cs:7700000,3415.05966239415)
--(axis cs:7600000,3399.46334333753)
--(axis cs:7500000,3407.34107023144)
--(axis cs:7400000,3429.30151036194)
--(axis cs:7300000,3441.41000433382)
--(axis cs:7200000,3406.32755552127)
--(axis cs:7100000,3378.23567040881)
--(axis cs:7000000,3366.0118546953)
--(axis cs:6900000,3357.51742139425)
--(axis cs:6800000,3351.21800768349)
--(axis cs:6700000,3376.1916594858)
--(axis cs:6600000,3381.25839056066)
--(axis cs:6500000,3378.70716654885)
--(axis cs:6400000,3346.86329291917)
--(axis cs:6300000,3322.80086048087)
--(axis cs:6200000,3327.07136487176)
--(axis cs:6100000,3321.3858840832)
--(axis cs:6000000,3310.32341721226)
--(axis cs:5900000,3264.51987461486)
--(axis cs:5800000,3219.39844470417)
--(axis cs:5700000,3159.99191233662)
--(axis cs:5600000,3118.50387421511)
--(axis cs:5500000,3076.47693928784)
--(axis cs:5400000,3055.44822904125)
--(axis cs:5300000,3053.31337781342)
--(axis cs:5200000,3041.75253054193)
--(axis cs:5100000,3027.02719524784)
--(axis cs:5000000,3030.60098593085)
--(axis cs:4900000,3033.85453766751)
--(axis cs:4800000,3013.10702075972)
--(axis cs:4700000,3014.23700112093)
--(axis cs:4600000,2994.11089716727)
--(axis cs:4500000,2984.24839148552)
--(axis cs:4400000,2963.69154123827)
--(axis cs:4300000,2935.95386848271)
--(axis cs:4200000,2896.8471272568)
--(axis cs:4100000,2856.68276045257)
--(axis cs:4000000,2822.07065426274)
--(axis cs:3900000,2811.15373499294)
--(axis cs:3800000,2834.09611221916)
--(axis cs:3700000,2833.56785231684)
--(axis cs:3600000,2860.84812045906)
--(axis cs:3500000,2838.51199881016)
--(axis cs:3400000,2820.24339870641)
--(axis cs:3300000,2791.52811925949)
--(axis cs:3200000,2739.08930736323)
--(axis cs:3100000,2664.76119722121)
--(axis cs:3000000,2613.20092764297)
--(axis cs:2900000,2563.88614747345)
--(axis cs:2800000,2504.77512167721)
--(axis cs:2700000,2448.62848680753)
--(axis cs:2600000,2401.28517289384)
--(axis cs:2500000,2361.42215580448)
--(axis cs:2400000,2330.13317936184)
--(axis cs:2300000,2273.32379605872)
--(axis cs:2200000,2260.20052307247)
--(axis cs:2100000,2242.44593671225)
--(axis cs:2000000,2138.14612974607)
--(axis cs:1900000,2068.8932816166)
--(axis cs:1800000,1982.55807449398)
--(axis cs:1700000,1893.00233249394)
--(axis cs:1600000,1828.52636166302)
--(axis cs:1500000,1790.62042635464)
--(axis cs:1400000,1750.36451935771)
--(axis cs:1300000,1711.6163112826)
--(axis cs:1200000,1655.85333304351)
--(axis cs:1100000,1633.92411831388)
--(axis cs:1000000,1627.39445228924)
--(axis cs:900000,1575.19448528735)
--(axis cs:800000,1520.12808377148)
--(axis cs:700000,1434.64891693375)
--(axis cs:600000,1282.09757841231)
--(axis cs:500000,1216.13085600126)
--(axis cs:400000,1139.70036542226)
--(axis cs:300000,1068.97979708922)
--(axis cs:200000,973.694703987716)
--(axis cs:100000,847.557701639823)
--cycle;

\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.1]
(axis cs:100000,78.909357907448)
--(axis cs:100000,18.5040058123992)
--(axis cs:200000,18.8582802354978)
--(axis cs:300000,20.5929695729275)
--(axis cs:400000,20.9210793334036)
--(axis cs:500000,21.2810753194558)
--(axis cs:600000,22.4542365228175)
--(axis cs:700000,23.0861018283482)
--(axis cs:800000,24.5651132264086)
--(axis cs:900000,25.0089924076101)
--(axis cs:1000000,25.7582438674925)
--(axis cs:1100000,28.3403790966914)
--(axis cs:1200000,28.6347411136678)
--(axis cs:1300000,28.7699507132102)
--(axis cs:1400000,30.2401052849741)
--(axis cs:1500000,30.653618855429)
--(axis cs:1600000,27.1407215321835)
--(axis cs:1700000,26.3648542050976)
--(axis cs:1800000,28.0799501792431)
--(axis cs:1900000,32.056268039552)
--(axis cs:2000000,35.8460482396646)
--(axis cs:2100000,38.6933000939913)
--(axis cs:2200000,45.4631153105404)
--(axis cs:2300000,49.4033905863316)
--(axis cs:2400000,56.0097013708342)
--(axis cs:2500000,62.2119036423498)
--(axis cs:2600000,71.2094469695369)
--(axis cs:2700000,81.0561515090289)
--(axis cs:2800000,88.2675412704064)
--(axis cs:2900000,96.0291850877881)
--(axis cs:3000000,105.735874821992)
--(axis cs:3100000,113.962832620328)
--(axis cs:3200000,122.884143626292)
--(axis cs:3300000,135.814971050289)
--(axis cs:3400000,146.695347425526)
--(axis cs:3500000,165.079397613263)
--(axis cs:3600000,178.139755077545)
--(axis cs:3700000,192.057364742889)
--(axis cs:3800000,206.471331974519)
--(axis cs:3900000,217.920984465399)
--(axis cs:4000000,225.154795028021)
--(axis cs:4100000,240.670607587112)
--(axis cs:4200000,251.197639486538)
--(axis cs:4300000,264.091261740809)
--(axis cs:4400000,270.897850562621)
--(axis cs:4500000,271.476515879437)
--(axis cs:4600000,276.654095032939)
--(axis cs:4700000,286.926078933254)
--(axis cs:4800000,295.238765581367)
--(axis cs:4900000,298.309099837597)
--(axis cs:5000000,295.961142004266)
--(axis cs:5100000,290.30309020577)
--(axis cs:5200000,285.579009060745)
--(axis cs:5300000,280.656688845084)
--(axis cs:5400000,278.104381811931)
--(axis cs:5500000,259.552034930576)
--(axis cs:5600000,241.974634435922)
--(axis cs:5700000,203.252618891024)
--(axis cs:5800000,180.011599143558)
--(axis cs:5900000,159.643639753997)
--(axis cs:6000000,174.454526775291)
--(axis cs:6100000,162.557979674183)
--(axis cs:6200000,165.584115202354)
--(axis cs:6300000,172.55488286011)
--(axis cs:6400000,183.952621829352)
--(axis cs:6500000,216.619708429217)
--(axis cs:6600000,226.457206443146)
--(axis cs:6700000,249.372571320751)
--(axis cs:6800000,259.238046170371)
--(axis cs:6900000,279.350970979057)
--(axis cs:7000000,268.135769726482)
--(axis cs:7100000,278.086402884788)
--(axis cs:7200000,278.709674896629)
--(axis cs:7300000,278.013031514986)
--(axis cs:7400000,266.35705983929)
--(axis cs:7500000,248.179619958224)
--(axis cs:7600000,260.370632522132)
--(axis cs:7700000,270.730157495371)
--(axis cs:7800000,276.934601996311)
--(axis cs:7900000,278.555304531752)
--(axis cs:8000000,296.241075776104)
--(axis cs:8100000,309.762624412868)
--(axis cs:8200000,327.225967281143)
--(axis cs:8300000,334.095545676479)
--(axis cs:8400000,346.514611851)
--(axis cs:8500000,357.126692128045)
--(axis cs:8600000,357.922070002129)
--(axis cs:8700000,358.249723855213)
--(axis cs:8800000,365.698675801673)
--(axis cs:8900000,372.754507023032)
--(axis cs:9000000,377.857680014255)
--(axis cs:9100000,394.472025673481)
--(axis cs:9200000,401.69172926187)
--(axis cs:9300000,393.282727140785)
--(axis cs:9400000,413.091475267701)
--(axis cs:9500000,457.613412152782)
--(axis cs:9600000,488.607663599902)
--(axis cs:9700000,514.496480969975)
--(axis cs:9800000,542.085920535056)
--(axis cs:9900000,570.672620110021)
--(axis cs:10000000,612.055472601057)
--(axis cs:10100000,631.026774236755)
--(axis cs:10200000,647.266645601518)
--(axis cs:10300000,692.577669744242)
--(axis cs:10400000,709.460212964251)
--(axis cs:10500000,691.480961639809)
--(axis cs:10600000,701.336286295723)
--(axis cs:10700000,713.176748113035)
--(axis cs:10800000,743.194674063009)
--(axis cs:10900000,759.83590287825)
--(axis cs:11000000,759.62280119771)
--(axis cs:11100000,760.043951598545)
--(axis cs:11200000,763.955574103269)
--(axis cs:11300000,757.125558239177)
--(axis cs:11400000,755.61959533636)
--(axis cs:11500000,784.547688247065)
--(axis cs:11600000,788.542478453294)
--(axis cs:11700000,772.769644706757)
--(axis cs:11800000,757.353686414859)
--(axis cs:11900000,766.576723654634)
--(axis cs:12000000,758.175581231499)
--(axis cs:12100000,773.070466528014)
--(axis cs:12200000,783.012057538532)
--(axis cs:12300000,790.721459709835)
--(axis cs:12400000,818.772617465677)
--(axis cs:12500000,821.500869898999)
--(axis cs:12600000,846.98254116003)
--(axis cs:12700000,887.295142417526)
--(axis cs:12800000,878.885939784956)
--(axis cs:12900000,864.673212678287)
--(axis cs:13000000,879.996478149445)
--(axis cs:13100000,887.952525624693)
--(axis cs:13200000,877.847647308578)
--(axis cs:13300000,909.894746886032)
--(axis cs:13400000,889.840654254298)
--(axis cs:13500000,903.384977665305)
--(axis cs:13600000,895.335445869005)
--(axis cs:13700000,910.29817825948)
--(axis cs:13800000,935.830653183573)
--(axis cs:13900000,958.418318848063)
--(axis cs:14000000,934.319917411866)
--(axis cs:14100000,936.76019191928)
--(axis cs:14200000,967.497431535103)
--(axis cs:14300000,958.999989411986)
--(axis cs:14400000,980.375514406029)
--(axis cs:14500000,975.390162097113)
--(axis cs:14600000,982.37255278564)
--(axis cs:14700000,972.569256159892)
--(axis cs:14800000,987.596390580401)
--(axis cs:14900000,995.284798370792)
--(axis cs:15000000,1054.62970205761)
--(axis cs:15100000,1077.0553077074)
--(axis cs:15200000,1093.5306972606)
--(axis cs:15300000,1112.71226160224)
--(axis cs:15400000,1137.98070337603)
--(axis cs:15500000,1200.89474375412)
--(axis cs:15600000,1251.66550988808)
--(axis cs:15700000,1301.44999156348)
--(axis cs:15800000,1346.26400361095)
--(axis cs:15900000,1400.34379276959)
--(axis cs:16000000,1426.13129967836)
--(axis cs:16100000,1485.29035777195)
--(axis cs:16200000,1552.4754424006)
--(axis cs:16300000,1589.71264967404)
--(axis cs:16400000,1629.02660327085)
--(axis cs:16500000,1627.15046350005)
--(axis cs:16600000,1644.50887089877)
--(axis cs:16600000,6072.29413276565)
--(axis cs:16600000,6072.29413276565)
--(axis cs:16500000,6095.86173416073)
--(axis cs:16400000,6107.10552564344)
--(axis cs:16300000,6055.91963325397)
--(axis cs:16200000,6017.27809824303)
--(axis cs:16100000,5949.54274583677)
--(axis cs:16000000,5924.04390367852)
--(axis cs:15900000,5909.18597299532)
--(axis cs:15800000,5790.51294549368)
--(axis cs:15700000,5703.46018922679)
--(axis cs:15600000,5616.04145121824)
--(axis cs:15500000,5488.00395590348)
--(axis cs:15400000,5447.2204364081)
--(axis cs:15300000,5456.9436252013)
--(axis cs:15200000,5399.22698693757)
--(axis cs:15100000,5421.45731557237)
--(axis cs:15000000,5391.93281788843)
--(axis cs:14900000,5352.64274605415)
--(axis cs:14800000,5358.80890330294)
--(axis cs:14700000,5404.65571156005)
--(axis cs:14600000,5470.43006744271)
--(axis cs:14500000,5566.38155709315)
--(axis cs:14400000,5544.70919888921)
--(axis cs:14300000,5485.65987216922)
--(axis cs:14200000,5531.33291449168)
--(axis cs:14100000,5511.84319217472)
--(axis cs:14000000,5478.0313739264)
--(axis cs:13900000,5484.69795324785)
--(axis cs:13800000,5484.24326998446)
--(axis cs:13700000,5412.077934031)
--(axis cs:13600000,5327.70912474713)
--(axis cs:13500000,5285.25444791295)
--(axis cs:13400000,5227.54162810244)
--(axis cs:13300000,5181.70525820711)
--(axis cs:13200000,5146.81686256547)
--(axis cs:13100000,5123.51273422944)
--(axis cs:13000000,5133.70134716395)
--(axis cs:12900000,5103.83524286756)
--(axis cs:12800000,5056.79137930064)
--(axis cs:12700000,5061.27175217389)
--(axis cs:12600000,5061.45142583311)
--(axis cs:12500000,4988.83230630193)
--(axis cs:12400000,4955.83818313958)
--(axis cs:12300000,4936.27362262782)
--(axis cs:12200000,4856.2288861934)
--(axis cs:12100000,4773.11626804875)
--(axis cs:12000000,4643.53316634334)
--(axis cs:11900000,4551.96955808378)
--(axis cs:11800000,4484.513889977)
--(axis cs:11700000,4372.73010638004)
--(axis cs:11600000,4266.68331283245)
--(axis cs:11500000,4155.9157130515)
--(axis cs:11400000,4088.68255118678)
--(axis cs:11300000,4016.84227982884)
--(axis cs:11200000,3951.7736641406)
--(axis cs:11100000,3880.87334877999)
--(axis cs:11000000,3864.41603036606)
--(axis cs:10900000,3818.88347541399)
--(axis cs:10800000,3796.24925036236)
--(axis cs:10700000,3796.24816542058)
--(axis cs:10600000,3755.18412732096)
--(axis cs:10500000,3748.97583735023)
--(axis cs:10400000,3707.62337886754)
--(axis cs:10300000,3670.99784374216)
--(axis cs:10200000,3670.12907331058)
--(axis cs:10100000,3613.46040577481)
--(axis cs:10000000,3542.05806162733)
--(axis cs:9900000,3462.6207423862)
--(axis cs:9800000,3379.83682208812)
--(axis cs:9700000,3274.63078928554)
--(axis cs:9600000,3187.99035724487)
--(axis cs:9500000,3109.88541489918)
--(axis cs:9400000,3030.06615996667)
--(axis cs:9300000,2964.91974787899)
--(axis cs:9200000,2868.66625059461)
--(axis cs:9100000,2796.91091032251)
--(axis cs:9000000,2741.38233372994)
--(axis cs:8900000,2699.11550269765)
--(axis cs:8800000,2639.19646084205)
--(axis cs:8700000,2601.99134095219)
--(axis cs:8600000,2591.06215249722)
--(axis cs:8500000,2547.70146205633)
--(axis cs:8400000,2520.69632914346)
--(axis cs:8300000,2491.06153085557)
--(axis cs:8200000,2434.62346517424)
--(axis cs:8100000,2414.01930221707)
--(axis cs:8000000,2384.48154987757)
--(axis cs:7900000,2351.43059103887)
--(axis cs:7800000,2321.49010274386)
--(axis cs:7700000,2293.32928572245)
--(axis cs:7600000,2238.51784833639)
--(axis cs:7500000,2192.85591887481)
--(axis cs:7400000,2100.07640608655)
--(axis cs:7300000,2037.41775250309)
--(axis cs:7200000,1972.55454476996)
--(axis cs:7100000,1928.57518424252)
--(axis cs:7000000,1905.59042916822)
--(axis cs:6900000,1850.08690545156)
--(axis cs:6800000,1849.05960871762)
--(axis cs:6700000,1823.22721709233)
--(axis cs:6600000,1848.00657684209)
--(axis cs:6500000,1828.22578287487)
--(axis cs:6400000,1864.22776875243)
--(axis cs:6300000,1824.95753077506)
--(axis cs:6200000,1794.3730689446)
--(axis cs:6100000,1754.27159648747)
--(axis cs:6000000,1688.10558909089)
--(axis cs:5900000,1682.45841460298)
--(axis cs:5800000,1620.52285591896)
--(axis cs:5700000,1548.36945161244)
--(axis cs:5600000,1417.24965934807)
--(axis cs:5500000,1354.39459764687)
--(axis cs:5400000,1259.70197398285)
--(axis cs:5300000,1200.0333285507)
--(axis cs:5200000,1169.64056438629)
--(axis cs:5100000,1128.01068017288)
--(axis cs:5000000,1094.79827539131)
--(axis cs:4900000,1055.21569077946)
--(axis cs:4800000,1017.30192764043)
--(axis cs:4700000,993.890621231988)
--(axis cs:4600000,987.981811749357)
--(axis cs:4500000,967.077369123903)
--(axis cs:4400000,941.802760060103)
--(axis cs:4300000,922.143344727979)
--(axis cs:4200000,887.691873707687)
--(axis cs:4100000,849.029602274139)
--(axis cs:4000000,804.910680057517)
--(axis cs:3900000,745.34838361994)
--(axis cs:3800000,688.795524212361)
--(axis cs:3700000,628.407748507367)
--(axis cs:3600000,576.277381652796)
--(axis cs:3500000,526.25813927915)
--(axis cs:3400000,499.835851392641)
--(axis cs:3300000,477.068113733941)
--(axis cs:3200000,459.474437188442)
--(axis cs:3100000,435.24237469588)
--(axis cs:3000000,416.528033262917)
--(axis cs:2900000,395.328737579911)
--(axis cs:2800000,376.041631743966)
--(axis cs:2700000,364.130895801261)
--(axis cs:2600000,353.117286612454)
--(axis cs:2500000,346.153217831155)
--(axis cs:2400000,323.04472301101)
--(axis cs:2300000,303.143791558583)
--(axis cs:2200000,282.721436527323)
--(axis cs:2100000,274.917213453671)
--(axis cs:2000000,258.033568552531)
--(axis cs:1900000,244.182748054667)
--(axis cs:1800000,235.906029377673)
--(axis cs:1700000,228.168995499369)
--(axis cs:1600000,222.786256460182)
--(axis cs:1500000,207.272630873791)
--(axis cs:1400000,199.664629249148)
--(axis cs:1300000,195.629982549396)
--(axis cs:1200000,186.277959197485)
--(axis cs:1100000,176.937838099172)
--(axis cs:1000000,175.015751596722)
--(axis cs:900000,165.462680562625)
--(axis cs:800000,149.74888693278)
--(axis cs:700000,135.462495708807)
--(axis cs:600000,119.821429969987)
--(axis cs:500000,114.88353864622)
--(axis cs:400000,109.087938767681)
--(axis cs:300000,97.9449356129469)
--(axis cs:200000,91.461105657373)
--(axis cs:100000,78.909357907448)
--cycle;

\addplot [semithick, darkorange]
table {%
100000 580.12972557579
200000 675.401639194863
300000 744.822943088774
400000 811.838922479014
500000 867.459223842608
600000 917.642627648231
700000 1045.27396843898
800000 1122.74599765657
900000 1167.85377845109
1000000 1210.50116007093
1100000 1220.50265386553
1200000 1232.90540768459
1300000 1280.83967818657
1400000 1318.37866102378
1500000 1343.95753376171
1600000 1376.78458267903
1700000 1412.49456747518
1800000 1470.64781039691
1900000 1532.53741409441
2000000 1585.49648760652
2100000 1648.97643974327
2200000 1684.12014921061
2300000 1712.88796291401
2400000 1751.14103858778
2500000 1788.83470386422
2600000 1833.19246520619
2700000 1875.93430301873
2800000 1933.49995706082
2900000 1983.32953155979
3000000 2025.04218332886
3100000 2080.15141207436
3200000 2134.74020764133
3300000 2168.15880316281
3400000 2182.36893966246
3500000 2211.77108595432
3600000 2223.36739186166
3700000 2210.04344958582
3800000 2201.26578668643
3900000 2190.839317409
4000000 2197.10356485968
4100000 2224.17387248914
4200000 2257.66747130042
4300000 2288.41459244399
4400000 2332.59746618917
4500000 2329.53343788299
4600000 2343.53747803048
4700000 2353.32819549926
4800000 2359.93688856305
4900000 2377.99718420987
5000000 2387.22782133413
5100000 2390.79521836179
5200000 2400.5771139523
5300000 2400.14117051381
5400000 2374.83857065191
5500000 2408.5750878693
5600000 2442.48814998686
5700000 2479.08484240635
5800000 2525.41835255444
5900000 2577.31439584395
6000000 2617.21077020058
6100000 2647.15077941651
6200000 2674.8786362411
6300000 2701.97088620192
6400000 2761.41303354747
6500000 2805.1165759223
6600000 2809.07856638682
6700000 2811.29050400683
6800000 2800.7912653847
6900000 2796.02362810774
7000000 2803.06470785782
7100000 2819.82363428021
7200000 2827.99741655779
7300000 2835.13044975806
7400000 2811.63727081909
7500000 2767.01009788591
7600000 2768.99897112466
7700000 2773.84061264115
7800000 2778.74225039714
7900000 2784.88486223932
8000000 2775.61107089619
8100000 2757.21974841607
8200000 2719.3355341142
8300000 2705.5515937013
8400000 2714.65059247143
8500000 2734.71550440744
8600000 2729.60889801684
8700000 2761.74530399348
8800000 2774.59688406655
8900000 2790.29547736703
9000000 2834.04196555128
9100000 2860.71967911906
9200000 2909.17758712533
9300000 2930.55358546843
9400000 2958.56735940034
9500000 2983.51671113962
9600000 2992.44938781273
9700000 2992.71811697887
9800000 3000.50601048106
9900000 3001.35936503886
10000000 2961.89582331753
10100000 2949.80909445776
10200000 2944.11574399014
10300000 2954.02282791074
10400000 2922.37440422121
10500000 2907.67333947677
10600000 2902.16605063043
10700000 2900.98699440054
10800000 2908.10590037121
10900000 2887.83080246065
11000000 2915.9291551112
11100000 2919.86225016968
11200000 2888.26768544404
11300000 2858.27961348564
11400000 2893.95793116114
11500000 2915.76714342217
11600000 2946.50430012715
11700000 2937.88946130185
11800000 2918.11656965728
11900000 2912.92153898953
12000000 2885.46167384595
12100000 2884.95236419586
12200000 2903.50450038041
12300000 2903.60430120605
12400000 2883.94286503494
12500000 2847.30320814787
12600000 2825.52858790795
12700000 2821.55069890266
12800000 2846.53500217445
12900000 2864.00996945879
13000000 2880.86469022048
13100000 2876.95875061565
13200000 2850.66434545165
13300000 2870.9774592934
13400000 2870.39616260633
13500000 2889.16968501229
13600000 2887.11296660282
13700000 2884.25680058219
13800000 2859.77895146763
13900000 2841.44722638348
14000000 2807.53228681387
14100000 2797.18457088093
14200000 2845.277789568
14300000 2841.34844414001
14400000 2842.81231379431
14500000 2854.36317009611
14600000 2887.20568863245
14700000 2907.44452802808
14800000 2908.71155748452
14900000 2920.916025832
15000000 2959.01660408981
15100000 2972.72253148227
15200000 2969.65685052685
15300000 2986.9939213264
15400000 3001.50471211023
15500000 3019.90311994893
15600000 3032.18721155964
15700000 3053.02164096523
15800000 3064.25692444771
15900000 3054.71629279968
16000000 3051.52099397901
16100000 3064.46624636999
16200000 3056.67174111915
16300000 3028.41100679937
16400000 3012.30685068551
16500000 2997.92647561983
16600000 2978.47151523038
16700000 2964.30854207202
16800000 2989.9152208033
16900000 2991.00471802543
17000000 2970.7331287182
17100000 2943.85819528103
17200000 2934.36414202843
17300000 2937.73396257031
17400000 2927.6280374853
17500000 2906.55767466403
17600000 2884.26123607277
17700000 2860.04582842792
17800000 2848.3841758395
17900000 2869.25950155506
18000000 2904.1561994025
18100000 2924.97327044674
18200000 2919.05555429428
18300000 2940.16343976288
18400000 2951.59063291571
18500000 2969.49488730421
18600000 3002.9706490115
18700000 3031.94986592843
18800000 3047.14491304267
18900000 3070.11253451102
19000000 3077.68867793304
19100000 3089.81061584248
19200000 3121.22115240364
19300000 3127.60666288839
19400000 3153.88465940218
19500000 3138.91398366114
19600000 3103.16307034969
19700000 3103.4995226172
19800000 3093.73926055861
19900000 3074.40154834408
20000000 3063.55116365181
};
\addplot [semithick, steelblue31119180]
table {%
100000 48.7066818599236
200000 55.1596929464354
300000 59.2689525929372
400000 65.0045090505421
500000 68.0823069828379
600000 71.1378332464021
700000 79.2742987685777
800000 87.1570000795945
900000 95.2358364851178
1000000 100.386997732107
1100000 102.639108597932
1200000 107.456350155576
1300000 112.199966631303
1400000 114.952367267061
1500000 118.96312486461
1600000 124.963488996183
1700000 127.266924852233
1800000 131.992989778458
1900000 138.119508047109
2000000 146.939808396098
2100000 156.805256773831
2200000 164.092275918932
2300000 176.273591072457
2400000 189.527212190922
2500000 204.182560736752
2600000 212.163366790995
2700000 222.593523655145
2800000 232.154586507186
2900000 245.67896133385
3000000 261.131954042454
3100000 274.602603658104
3200000 291.179290407367
3300000 306.441542392115
3400000 323.265599409083
3500000 345.668768446207
3600000 377.208568365171
3700000 410.232556625128
3800000 447.63342809344
3900000 481.634684042669
4000000 515.032737542769
4100000 544.850104930625
4200000 569.444756597112
4300000 593.117303234394
4400000 606.350305311362
4500000 619.27694250167
4600000 632.317953391148
4700000 640.408350082621
4800000 656.2703466109
4900000 676.762395308528
5000000 695.379708697789
5100000 709.156885189327
5200000 727.609786723519
5300000 740.345008697893
5400000 768.903177897391
5500000 806.973316288724
5600000 829.612146891994
5700000 875.811035251729
5800000 900.267227531259
5900000 921.051027178488
6000000 931.280057933092
6100000 958.414788080826
6200000 979.978592073477
6300000 998.756206817586
6400000 1024.09019529089
6500000 1022.42274565204
6600000 1037.23189164262
6700000 1036.29989420654
6800000 1054.14882744399
6900000 1064.71893821531
7000000 1086.86309944735
7100000 1103.33079356365
7200000 1125.6321098333
7300000 1157.71539200904
7400000 1183.21673296292
7500000 1220.51776941652
7600000 1249.44424042926
7700000 1282.02972160891
7800000 1299.21235237009
7900000 1314.99294778531
8000000 1340.36131282684
8100000 1361.89096331497
8200000 1380.92471622769
8300000 1412.57853826603
8400000 1433.60547049723
8500000 1452.41407709219
8600000 1474.49211124967
8700000 1480.1205324037
8800000 1502.44756832186
8900000 1535.93500486034
9000000 1559.6200068721
9100000 1595.69146799799
9200000 1635.17898992824
9300000 1679.10123750989
9400000 1721.57881761719
9500000 1783.74941352598
9600000 1838.29901042239
9700000 1894.56363512776
9800000 1960.96137131159
9900000 2016.64668124811
10000000 2077.05676711419
10100000 2122.24359000578
10200000 2158.69785945605
10300000 2181.7877567432
10400000 2208.5417959159
10500000 2220.22839949502
10600000 2228.26020680834
10700000 2254.71245676681
10800000 2269.72196221268
10900000 2289.35968914612
11000000 2312.01941578189
11100000 2320.45865018927
11200000 2357.86461912193
11300000 2386.98391903401
11400000 2422.15107326157
11500000 2470.23170064928
11600000 2527.61289564287
11700000 2572.7498755434
11800000 2620.93378819593
11900000 2659.27314086921
12000000 2700.85437378742
12100000 2773.09336728838
12200000 2819.62047186597
12300000 2863.49754116883
12400000 2887.30540030263
12500000 2905.16658810046
12600000 2954.21698349657
12700000 2974.28344729571
12800000 2967.8386595428
12900000 2984.25422777292
13000000 3006.8489126567
13100000 3005.73262992707
13200000 3012.33225493702
13300000 3045.80000254657
13400000 3058.69114117837
13500000 3094.31971278913
13600000 3111.52228530807
13700000 3161.18805614524
13800000 3210.03696158401
13900000 3221.55813604795
14000000 3206.17564566913
14100000 3224.301692047
14200000 3249.41517301339
14300000 3222.3299307906
14400000 3262.54235664762
14500000 3270.88585959513
14600000 3226.40131011418
14700000 3188.61248385997
14800000 3173.20264694167
14900000 3173.96377221247
15000000 3223.28125997302
15100000 3249.25631163989
15200000 3246.37884209908
15300000 3284.82794340177
15400000 3292.60056989207
15500000 3344.4493498288
15600000 3433.85348055316
15700000 3502.45509039513
15800000 3568.38847455231
15900000 3654.76488288246
16000000 3675.08760167844
16100000 3717.41655180436
16200000 3784.87677032182
16300000 3822.816141464
16400000 3868.06606445714
16500000 3861.50609883039
16600000 3858.40150183221
};
\end{axis}

==> figures/dataefficiency_cost_ballhitting.tex <==
\begin{axis}[%
name =ax2,
scaled y ticks=base 10:\Factor,
at={(ax1.south east)},
xlabel near ticks, ylabel near ticks,
every y tick scale label/.style={at={(yticklabel* cs:1.03,0cm)},anchor=near yticklabel},
title style={at={(0.5,0.93)}},
xshift=1cm,
width=0.607\figW,
height=\figH,
scale only axis,
xmin=0,
xmax=100,
xtick={  0,  20,  40,  60,  80, 100},
xlabel style={font=\color{white!15!black}},
xlabel={generations},
ymin=-10000,
ymax=-1000,
ylabel style={font=\color{white!15!black}},
ylabel={cost},
axis background/.style={fill=white},
title={(b) ball-hitting (OC)},
legend style={at={(1.03,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]

\addplot[area legend, draw=none, fill=mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	-5291.80866933026\\
2	-5682.42633331395\\
3	-5837.20113326777\\
4	-5803.22843335161\\
5	-5789.249535679\\
6	-6147.63419089572\\
7	-6152.52926727062\\
8	-6133.96438865605\\
9	-6150.75821956043\\
10	-6150.75821956043\\
11	-6173.64997251582\\
12	-6537.20378219882\\
13	-6537.20378219882\\
14	-6589.34195964146\\
15	-6591.55129737832\\
16	-6591.55129737832\\
17	-6585.67569970645\\
18	-6641.89388141719\\
19	-6641.89388141719\\
20	-6697.34177127907\\
21	-6726.00612730319\\
22	-6726.00612730319\\
23	-6743.54171007751\\
24	-6743.54171007751\\
25	-6745.73075582727\\
26	-6745.73075582727\\
27	-6796.18244824027\\
28	-6820.01124081681\\
29	-6989.03458841424\\
30	-7034.01119668308\\
31	-7224.46831778737\\
32	-7224.46831778737\\
33	-7224.46831778737\\
34	-7224.46831778737\\
35	-7224.70007629762\\
36	-7224.70007629762\\
37	-7230.03028201104\\
38	-7233.3222184378\\
39	-7257.87609644284\\
40	-7257.87609644284\\
41	-7288.248435168\\
42	-7288.248435168\\
43	-7288.248435168\\
44	-7288.248435168\\
45	-7288.248435168\\
46	-7292.89704841534\\
47	-7292.89704841534\\
48	-7292.89704841534\\
49	-7292.89704841534\\
50	-7292.89704841534\\
51	-7292.89704841534\\
52	-7292.89704841534\\
53	-7292.89704841534\\
54	-7292.89704841534\\
55	-7292.89704841534\\
56	-7294.9905358738\\
57	-7294.9905358738\\
58	-7294.9905358738\\
59	-7294.9905358738\\
60	-7294.9905358738\\
61	-7294.9905358738\\
62	-7294.9905358738\\
63	-7432.09987431843\\
64	-7432.09987431843\\
65	-7432.09987431843\\
66	-7432.09987431843\\
67	-7432.09987431843\\
68	-7432.09987431843\\
69	-7432.09987431843\\
70	-7432.09987431843\\
71	-7432.09987431843\\
72	-7467.77938128918\\
73	-7468.5627805501\\
74	-7468.5627805501\\
75	-7533.30925428655\\
76	-7533.30925428655\\
77	-7533.30925428655\\
78	-7533.30925428655\\
79	-7533.30925428655\\
80	-7533.30925428655\\
81	-7555.22848346429\\
82	-7555.22848346429\\
83	-7555.22848346429\\
84	-7555.22848346429\\
85	-7555.22848346429\\
86	-7555.22848346429\\
87	-7566.52229168068\\
88	-7566.52229168068\\
89	-7572.68825441383\\
90	-7572.68825441383\\
91	-7572.68825441383\\
92	-7586.27791922631\\
93	-7584.41193195032\\
94	-7583.29662509572\\
95	-7581.10524257536\\
96	-7579.54559988984\\
97	-7579.54559988984\\
98	-7574.84356675803\\
99	-7574.84356675803\\
100	-7574.84356675803\\
100	-6250.81592047582\\
99	-6250.81592047582\\
98	-6250.81592047582\\
97	-6190.60276738598\\
96	-6190.60276738598\\
95	-6174.2057487676\\
94	-6152.83296029553\\
93	-6142.54383005048\\
92	-6126.04314743321\\
91	-6127.60099723615\\
90	-6127.60099723615\\
89	-6127.60099723615\\
88	-6128.28693297425\\
87	-6128.28693297425\\
86	-6129.50824431597\\
85	-6129.50824431597\\
84	-6129.50824431597\\
83	-6129.50824431597\\
82	-6129.50824431597\\
81	-6129.50824431597\\
80	-6124.77065149052\\
79	-6124.77065149052\\
78	-6124.77065149052\\
77	-6124.77065149052\\
76	-6124.77065149052\\
75	-6124.77065149052\\
74	-6105.38604624322\\
73	-6105.38604624322\\
72	-6102.40177142112\\
71	-6087.28642276343\\
70	-6087.28642276343\\
69	-6087.28642276343\\
68	-6087.28642276343\\
67	-6087.28642276343\\
66	-6087.28642276343\\
65	-6087.28642276343\\
64	-6087.28642276343\\
63	-6087.28642276343\\
62	-6109.61544415595\\
61	-6109.61544415595\\
60	-6109.61544415595\\
59	-6109.61544415595\\
58	-6109.61544415595\\
57	-6109.61544415595\\
56	-6109.61544415595\\
55	-6102.44689064979\\
54	-6102.44689064979\\
53	-6102.44689064979\\
52	-6102.44689064979\\
51	-6102.44689064979\\
50	-6102.44689064979\\
49	-6102.44689064979\\
48	-6102.44689064979\\
47	-6102.44689064979\\
46	-6102.44689064979\\
45	-6103.11774391304\\
44	-6103.11774391304\\
43	-6103.11774391304\\
42	-6103.11774391304\\
41	-6103.11774391304\\
40	-6089.56440406807\\
39	-6089.56440406807\\
38	-6092.80657355251\\
37	-6078.85319336211\\
36	-6066.37211560995\\
35	-6066.37211560995\\
34	-6065.18384053871\\
33	-6065.18384053871\\
32	-6065.18384053871\\
31	-6065.18384053871\\
30	-6080.23027302313\\
29	-6079.61051449441\\
28	-6056.45042321527\\
27	-6045.99301072775\\
26	-6054.20099771085\\
25	-6054.20099771085\\
24	-6048.57896351531\\
23	-6048.57896351531\\
22	-6041.36224480827\\
21	-6041.36224480827\\
20	-6045.35803598094\\
19	-6047.65769441455\\
18	-6047.65769441455\\
17	-5959.97412119738\\
16	-5885.2343833084\\
15	-5885.2343833084\\
14	-5874.57044848043\\
13	-5880.59140816471\\
12	-5880.59140816471\\
11	-5866.21951777297\\
10	-5868.9949080003\\
9	-5868.9949080003\\
8	-5740.79970906635\\
7	-5461.31924873367\\
6	-5268.4031629468\\
5	-5167.80007163422\\
4	-5111.21133401378\\
3	-4976.95384085547\\
2	-4606.82749670308\\
1	-3901.85126895938\\
}--cycle;
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	-4597\\
2	-5145\\
3	-5407\\
4	-5457\\
5	-5479\\
6	-5708\\
7	-5807\\
8	-5937\\
9	-6010\\
10	-6010\\
11	-6020\\
12	-6209\\
13	-6209\\
14	-6232\\
15	-6238\\
16	-6238\\
17	-6273\\
18	-6345\\
19	-6345\\
20	-6371\\
21	-6384\\
22	-6384\\
23	-6396\\
24	-6396\\
25	-6400\\
26	-6400\\
27	-6421\\
28	-6438\\
29	-6534\\
30	-6557\\
31	-6645\\
32	-6645\\
33	-6645\\
34	-6645\\
35	-6646\\
36	-6646\\
37	-6654\\
38	-6663\\
39	-6674\\
40	-6674\\
41	-6696\\
42	-6696\\
43	-6696\\
44	-6696\\
45	-6696\\
46	-6698\\
47	-6698\\
48	-6698\\
49	-6698\\
50	-6698\\
51	-6698\\
52	-6698\\
53	-6698\\
54	-6698\\
55	-6698\\
56	-6702\\
57	-6702\\
58	-6702\\
59	-6702\\
60	-6702\\
61	-6702\\
62	-6702\\
63	-6760\\
64	-6760\\
65	-6760\\
66	-6760\\
67	-6760\\
68	-6760\\
69	-6760\\
70	-6760\\
71	-6760\\
72	-6785\\
73	-6787\\
74	-6787\\
75	-6829\\
76	-6829\\
77	-6829\\
78	-6829\\
79	-6829\\
80	-6829\\
81	-6842\\
82	-6842\\
83	-6842\\
84	-6842\\
85	-6842\\
86	-6842\\
87	-6847\\
88	-6847\\
89	-6850\\
90	-6850\\
91	-6850\\
92	-6856\\
93	-6863\\
94	-6868\\
95	-6878\\
96	-6885\\
97	-6885\\
98	-6913\\
99	-6913\\
100	-6913\\
};
\addlegendentry{torques, c = 0.05 s}


\addplot[area legend, draw=none, fill=blue!50!mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	-5110.65371499423\\
2	-6074.74734219291\\
3	-6074.74734219291\\
4	-6173.1634604619\\
5	-6026.26737655751\\
6	-6417.25280911772\\
7	-6417.25280911772\\
8	-6417.25280911772\\
9	-6606.42622969041\\
10	-6822.13487770116\\
11	-7023.97909079323\\
12	-7147.60735081257\\
13	-7142.99578616611\\
14	-7131.55415988453\\
15	-7131.55415988453\\
16	-7131.55415988453\\
17	-7131.55415988453\\
18	-7131.55415988453\\
19	-7131.28776910424\\
20	-7131.28776910424\\
21	-7131.87615852651\\
22	-7131.20447311537\\
23	-7131.20447311537\\
24	-7131.15065599522\\
25	-7131.15065599522\\
26	-7289.3219825376\\
27	-7289.3219825376\\
28	-7298.73778409705\\
29	-7298.66796224901\\
30	-7411.77190145223\\
31	-7411.77190145223\\
32	-7411.61473614177\\
33	-7411.61473614177\\
34	-7411.61473614177\\
35	-7411.61473614177\\
36	-7411.61473614177\\
37	-7411.396193212\\
38	-7411.32904714833\\
39	-7411.32904714833\\
40	-7411.29050844223\\
41	-7411.29050844223\\
42	-7411.18325343266\\
43	-7411.18325343266\\
44	-7427.24132673789\\
45	-7608.68545210971\\
46	-7608.68545210971\\
47	-7608.68545210971\\
48	-7608.68545210971\\
49	-7608.68545210971\\
50	-7630.81435223842\\
51	-7630.81435223842\\
52	-7630.81435223842\\
53	-7630.81435223842\\
54	-7719.61759442506\\
55	-7719.56523659587\\
56	-7719.56523659587\\
57	-7719.56523659587\\
58	-7878.21370799831\\
59	-7878.18132516523\\
60	-7878.18132516523\\
61	-7903.41126082517\\
62	-7918.51818430577\\
63	-7929.95018014088\\
64	-8048.65512396284\\
65	-8048.65512396284\\
66	-8082.62105126177\\
67	-8204.6063435231\\
68	-8306.03438115618\\
69	-8328.25317456692\\
70	-8402.07555539747\\
71	-8402.07555539747\\
72	-8402.07555539747\\
73	-8402.07555539747\\
74	-8570.86545882292\\
75	-8659.35464255626\\
76	-8659.35464255626\\
77	-8774.80966298532\\
78	-8843.8066117998\\
79	-8861.75073651849\\
80	-8861.75073651849\\
81	-9233.56191237865\\
82	-9236.33795520149\\
83	-9236.33795520149\\
84	-9250.27540244738\\
85	-9250.27540244738\\
86	-9250.27540244738\\
87	-9263.98241270393\\
88	-9285.0157078952\\
89	-9315.33375987776\\
90	-9327.05315487201\\
91	-9490.57778731199\\
92	-9519.51169607784\\
93	-9610.17865242254\\
94	-9610.17865242254\\
95	-9610.17865242254\\
96	-9681.18833837768\\
97	-9681.18833837768\\
98	-9814.22797132082\\
99	-9814.22797132082\\
100	-9814.22797132082\\
100	-7068.33187679025\\
99	-7068.33187679025\\
98	-7068.33187679025\\
97	-7030.06119041174\\
96	-7030.06119041174\\
95	-6964.75434245284\\
94	-6964.75434245284\\
93	-6964.75434245284\\
92	-6840.49774269315\\
91	-6784.11014953833\\
90	-6730.77048735127\\
89	-6725.55764048134\\
88	-6667.28234320697\\
87	-6648.88891925396\\
86	-6615.0633255978\\
85	-6615.0633255978\\
84	-6615.0633255978\\
83	-6575.73079576071\\
82	-6575.73079576071\\
81	-6567.16867171832\\
80	-6616.47612511761\\
79	-6616.47612511761\\
78	-6560.526405326\\
77	-6543.74628683667\\
76	-6500.9679569263\\
75	-6500.9679569263\\
74	-6515.42628730601\\
73	-6497.65810079195\\
72	-6497.65810079195\\
71	-6497.65810079195\\
70	-6497.65810079195\\
69	-6491.76044842767\\
68	-6478.67084759729\\
67	-6454.08005115572\\
66	-6463.24043203116\\
65	-6434.21364077625\\
64	-6434.21364077625\\
63	-6457.09045590383\\
62	-6459.18262008572\\
61	-6461.91293063369\\
60	-6466.38066654253\\
59	-6466.38066654253\\
58	-6466.18285764922\\
57	-6490.95070978997\\
56	-6490.95070978997\\
55	-6490.95070978997\\
54	-6490.68482650707\\
53	-6501.03553606515\\
52	-6501.03553606515\\
51	-6501.03553606515\\
50	-6501.03553606515\\
49	-6503.02978361111\\
48	-6503.02978361111\\
47	-6503.02978361111\\
46	-6503.02978361111\\
45	-6503.02978361111\\
44	-6505.75554821497\\
43	-6504.17015312023\\
42	-6504.17015312023\\
41	-6503.7539947998\\
40	-6503.7539947998\\
39	-6503.60446619422\\
38	-6503.60446619422\\
37	-6503.34394822137\\
36	-6502.49608293705\\
35	-6502.49608293705\\
34	-6502.49608293705\\
33	-6502.49608293705\\
32	-6502.49608293705\\
31	-6501.88638978254\\
30	-6501.88638978254\\
29	-6313.11034643839\\
28	-6312.50054718087\\
27	-6212.5447921964\\
26	-6212.5447921964\\
25	-6188.07738497029\\
24	-6188.07738497029\\
23	-6180.67985861462\\
22	-6180.67985861462\\
21	-6152.82472084501\\
20	-6146.65271488914\\
19	-6146.65271488914\\
18	-6138.77332975262\\
17	-6138.77332975262\\
16	-6138.77332975262\\
15	-6138.77332975262\\
14	-6138.77332975262\\
13	-6000.21301665309\\
12	-5963.59839253815\\
11	-5967.91362854108\\
10	-5555.29314130306\\
9	-5566.76585675245\\
8	-5579.82030073729\\
7	-5579.82030073729\\
6	-5579.82030073729\\
5	-5225.46723876403\\
4	-3728.62678003309\\
3	-3508.93673315372\\
2	-3508.93673315372\\
1	-2236.71209206163\\
}--cycle;
\addplot [color=blue!50!mycolor1]
  table[row sep=crcr]{%
1	-3674\\
2	-4792\\
3	-4792\\
4	-4951\\
5	-5626\\
6	-5999\\
7	-5999\\
8	-5999\\
9	-6087\\
10	-6189\\
11	-6496\\
12	-6556\\
13	-6572\\
14	-6635\\
15	-6635\\
16	-6635\\
17	-6635\\
18	-6635\\
19	-6639\\
20	-6639\\
21	-6642\\
22	-6656\\
23	-6656\\
24	-6660\\
25	-6660\\
26	-6751\\
27	-6751\\
28	-6806\\
29	-6806\\
30	-6957\\
31	-6957\\
32	-6957\\
33	-6957\\
34	-6957\\
35	-6957\\
36	-6957\\
37	-6957\\
38	-6957\\
39	-6957\\
40	-6958\\
41	-6958\\
42	-6958\\
43	-6958\\
44	-6966\\
45	-7056\\
46	-7056\\
47	-7056\\
48	-7056\\
49	-7056\\
50	-7066\\
51	-7066\\
52	-7066\\
53	-7066\\
54	-7105\\
55	-7105\\
56	-7105\\
57	-7105\\
58	-7172\\
59	-7172\\
60	-7172\\
61	-7183\\
62	-7189\\
63	-7194\\
64	-7241\\
65	-7241\\
66	-7273\\
67	-7329\\
68	-7392\\
69	-7410\\
70	-7450\\
71	-7450\\
72	-7450\\
73	-7450\\
74	-7543\\
75	-7580\\
76	-7580\\
77	-7659\\
78	-7702\\
79	-7739\\
80	-7739\\
81	-7900\\
82	-7906\\
83	-7906\\
84	-7933\\
85	-7933\\
86	-7933\\
87	-7956\\
88	-7976\\
89	-8020\\
90	-8029\\
91	-8137\\
92	-8180\\
93	-8287\\
94	-8287\\
95	-8287\\
96	-8356\\
97	-8356\\
98	-8441\\
99	-8441\\
100	-8441\\
};
\addlegendentry{torques, c = 0.15 s}


\addplot[area legend, draw=none, fill=blue, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	-4582.41423247614\\
2	-4431.85794163209\\
3	-4319.38033889836\\
4	-4319.38033889836\\
5	-4387.16421325558\\
6	-4387.16421325558\\
7	-4387.16421325558\\
8	-4395.9934800607\\
9	-4395.9934800607\\
10	-4412.40413210778\\
11	-4412.40413210778\\
12	-4452.81360089379\\
13	-4452.81360089379\\
14	-4486.09923286474\\
15	-4486.09923286474\\
16	-4486.09923286474\\
17	-4501.5262952278\\
18	-4516.43290851342\\
19	-4577.66573780541\\
20	-4578.97786648918\\
21	-4580.55472467406\\
22	-4581.423231931\\
23	-4581.65337814504\\
24	-4582.07059140358\\
25	-4582.32476042336\\
26	-4583.02044655903\\
27	-4583.4192206446\\
28	-4583.52379911224\\
29	-4583.45706400877\\
30	-4583.73115206138\\
31	-4583.70485378078\\
32	-4583.70485378078\\
33	-4583.70937978208\\
34	-4583.79809336942\\
35	-4583.75727880228\\
36	-4583.76171727911\\
37	-4583.77427178349\\
38	-4583.85835376448\\
39	-4583.85835376448\\
40	-4583.89684570363\\
41	-4583.89684570363\\
42	-4583.89684570363\\
43	-4583.89684570363\\
44	-4583.89684570363\\
45	-4583.89684570363\\
46	-4583.89684570363\\
47	-4583.89684570363\\
48	-4583.89684570363\\
49	-4583.89838790799\\
50	-4583.94133503181\\
51	-4583.94535503461\\
52	-4583.94535503461\\
53	-4583.94535503461\\
54	-4583.94535503461\\
55	-4583.94535503461\\
56	-4583.94535503461\\
57	-4583.94535503461\\
58	-4583.94569840913\\
59	-4583.96724774459\\
60	-4583.96724774459\\
61	-4583.96724774459\\
62	-4583.96724774459\\
63	-4583.96724774459\\
64	-4583.96893137935\\
65	-4583.96893137935\\
66	-4583.96893137935\\
67	-4583.96893137935\\
68	-4583.98929929962\\
69	-4583.98929929962\\
70	-4583.99164538735\\
71	-4583.99164538735\\
72	-4583.99164538735\\
73	-4583.99377992879\\
74	-4583.99377992879\\
75	-4583.99377992879\\
76	-4583.99377992879\\
77	-4583.99377992879\\
78	-4583.99377992879\\
79	-4583.99377992879\\
80	-4583.99377992879\\
81	-4583.99377992879\\
82	-4583.99377992879\\
83	-4583.99387218202\\
84	-4583.99387629429\\
85	-4583.99387629429\\
86	-4583.99387629429\\
87	-4583.99387629429\\
88	-4583.99387629429\\
89	-4583.99387629429\\
90	-4583.99387629429\\
91	-4583.99387629429\\
92	-4583.99573620738\\
93	-4583.99573620738\\
94	-4583.99658221912\\
95	-4583.99658221912\\
96	-4583.99699477244\\
97	-4583.99700223355\\
98	-4583.99700223355\\
99	-4583.99700223355\\
100	-4583.99709691545\\
100	-4266.76918220078\\
99	-4266.76917263519\\
98	-4266.76917263519\\
97	-4266.76917263519\\
96	-4266.76917188145\\
95	-4266.76913020098\\
94	-4266.76913020098\\
93	-4266.76904472427\\
92	-4266.76904472427\\
91	-4266.76885679134\\
90	-4266.76885679134\\
89	-4266.76885679134\\
88	-4266.76885679134\\
87	-4266.76885679134\\
86	-4266.76885679134\\
85	-4266.76885679134\\
84	-4266.76885679134\\
83	-4266.76885637596\\
82	-4266.76884705725\\
81	-4266.76884705725\\
80	-4266.76884705725\\
79	-4266.76884705725\\
78	-4266.76884705725\\
77	-4266.76884705725\\
76	-4266.76884705725\\
75	-4266.76884705725\\
74	-4266.76884705725\\
73	-4266.76884705725\\
72	-4266.76863141717\\
71	-4266.76863141717\\
70	-4266.76863141717\\
69	-4266.76839433178\\
68	-4266.76839433178\\
67	-4266.76633441591\\
66	-4266.76633441591\\
65	-4266.76633441591\\
64	-4266.76633441591\\
63	-4266.76616401075\\
62	-4266.76616401075\\
61	-4266.76616401075\\
60	-4266.76616401075\\
59	-4266.76616401075\\
58	-4266.76398118795\\
57	-4266.76394655414\\
56	-4266.76394655414\\
55	-4266.76394655414\\
54	-4266.76394655414\\
53	-4266.76394655414\\
52	-4266.76394655414\\
51	-4266.76394655414\\
50	-4266.76354102284\\
49	-4266.75844585866\\
48	-4266.75828978812\\
47	-4266.75828978812\\
46	-4266.75828978812\\
45	-4266.75828978812\\
44	-4266.75828978812\\
43	-4266.75828978812\\
42	-4266.75828978812\\
41	-4266.75828978812\\
40	-4266.75828978812\\
39	-4266.75438927115\\
38	-4266.75438927115\\
37	-4266.74586628135\\
36	-4266.35268215713\\
35	-4266.3522292518\\
34	-4265.94687936972\\
33	-4265.93485606277\\
32	-4265.93439470542\\
31	-4265.93439470542\\
30	-4265.6740930233\\
29	-4265.43123380542\\
28	-4264.78292586323\\
27	-4264.77226138495\\
26	-4264.4989021618\\
25	-4264.42712748445\\
24	-4264.40017907672\\
23	-4264.36055107089\\
22	-4264.33706340017\\
21	-4264.24861622991\\
20	-4263.49589471638\\
19	-4263.3730186832\\
18	-4231.58522130978\\
17	-4232.75347674113\\
16	-4232.89558917191\\
15	-4232.89558917191\\
14	-4232.89558917191\\
13	-4236.35683518717\\
12	-4236.35683518717\\
11	-4228.09299931623\\
10	-4228.09299931623\\
9	-4232.16871684692\\
8	-4232.16871684692\\
7	-4193.62080166221\\
6	-4193.62080166221\\
5	-4193.62080166221\\
4	-4200.00872427376\\
3	-4200.00872427376\\
2	-3727.75444484907\\
1	-1586.12566185704\\
}--cycle;
\addplot [color=blue]
  table[row sep=crcr]{%
1	-3084\\
2	-4080\\
3	-4260\\
4	-4260\\
5	-4290\\
6	-4290\\
7	-4290\\
8	-4314\\
9	-4314\\
10	-4320\\
11	-4320\\
12	-4345\\
13	-4345\\
14	-4359\\
15	-4359\\
16	-4359\\
17	-4367\\
18	-4374\\
19	-4421\\
20	-4421\\
21	-4422\\
22	-4423\\
23	-4423\\
24	-4423\\
25	-4423\\
26	-4424\\
27	-4424\\
28	-4424\\
29	-4424\\
30	-4425\\
31	-4425\\
32	-4425\\
33	-4425\\
34	-4425\\
35	-4425\\
36	-4425\\
37	-4425\\
38	-4425\\
39	-4425\\
40	-4425\\
41	-4425\\
42	-4425\\
43	-4425\\
44	-4425\\
45	-4425\\
46	-4425\\
47	-4425\\
48	-4425\\
49	-4425\\
50	-4425\\
51	-4425\\
52	-4425\\
53	-4425\\
54	-4425\\
55	-4425\\
56	-4425\\
57	-4425\\
58	-4425\\
59	-4425\\
60	-4425\\
61	-4425\\
62	-4425\\
63	-4425\\
64	-4425\\
65	-4425\\
66	-4425\\
67	-4425\\
68	-4425\\
69	-4425\\
70	-4425\\
71	-4425\\
72	-4425\\
73	-4425\\
74	-4425\\
75	-4425\\
76	-4425\\
77	-4425\\
78	-4425\\
79	-4425\\
80	-4425\\
81	-4425\\
82	-4425\\
83	-4425\\
84	-4425\\
85	-4425\\
86	-4425\\
87	-4425\\
88	-4425\\
89	-4425\\
90	-4425\\
91	-4425\\
92	-4425\\
93	-4425\\
94	-4425\\
95	-4425\\
96	-4425\\
97	-4425\\
98	-4425\\
99	-4425\\
100	-4425\\
};
\addlegendentry{torques, c = 0.3 s}


\addplot[area legend, draw=none, fill=orange, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	-3139.52602254716\\
2	-3437.12027218734\\
3	-3559.69571387806\\
4	-4162.9757032568\\
5	-4173.85933837253\\
6	-4386.09330080767\\
7	-4396.2359365395\\
8	-4444.87934107649\\
9	-4630.97375501588\\
10	-4630.63814326178\\
11	-4633.68248924309\\
12	-4836.82147361801\\
13	-4836.82147361801\\
14	-4838.1704724497\\
15	-4831.944400709\\
16	-4831.944400709\\
17	-4886.30418617878\\
18	-5197.46013603824\\
19	-5230.77617898608\\
20	-5457.9221146822\\
21	-5442.96567799683\\
22	-5534.90904288198\\
23	-5543.22002943968\\
24	-5528.76654748578\\
25	-5702.38674773179\\
26	-5745.55605765711\\
27	-5745.55605765711\\
28	-5745.55605765711\\
29	-5745.55605765711\\
30	-5729.30693533391\\
31	-5711.05826453185\\
32	-5793.76425394591\\
33	-5900.60820313088\\
34	-5876.56323080572\\
35	-5876.56323080572\\
36	-5876.56323080572\\
37	-5852.76430433529\\
38	-5946.71230753108\\
39	-5946.71230753108\\
40	-5991.03007986144\\
41	-5991.8931744239\\
42	-5991.8931744239\\
43	-5991.8931744239\\
44	-6078.5579454484\\
45	-6078.5579454484\\
46	-6054.20628259357\\
47	-6057.77017301976\\
48	-6012.83928205139\\
49	-6133.95633557593\\
50	-6133.95633557593\\
51	-6133.95633557593\\
52	-6161.56842028672\\
53	-6221.72173265648\\
54	-6210.98624420377\\
55	-6207.63491274155\\
56	-6207.63491274155\\
57	-6207.63491274155\\
58	-6207.63491274155\\
59	-6207.63491274155\\
60	-6237.18210626414\\
61	-6391.12709556377\\
62	-6455.97395325694\\
63	-6455.97395325694\\
64	-6455.97395325694\\
65	-6455.97395325694\\
66	-6455.97395325694\\
67	-6758.6666248501\\
68	-6758.6666248501\\
69	-6846.85172121906\\
70	-6846.85172121906\\
71	-6846.85172121906\\
72	-6846.85172121906\\
73	-6897.58491938491\\
74	-6897.58491938491\\
75	-6896.42937195216\\
76	-6912.70198524777\\
77	-6923.56469656583\\
78	-7097.7117368635\\
79	-7097.7117368635\\
80	-7097.7117368635\\
81	-7100.09347760029\\
82	-7255.14090699775\\
83	-7255.14090699775\\
84	-7255.14090699775\\
85	-7352.8732141017\\
86	-7352.8732141017\\
87	-7352.8732141017\\
88	-7352.8732141017\\
89	-7352.8732141017\\
90	-7352.8732141017\\
91	-7352.8732141017\\
92	-7437.11024745626\\
93	-7437.11024745626\\
94	-7437.11024745626\\
95	-7437.11024745626\\
96	-7437.11024745626\\
97	-7409.01697187461\\
98	-7409.01697187461\\
99	-7409.01697187461\\
100	-7406.97436925563\\
100	-6572.8379455515\\
99	-6564.66734745335\\
98	-6564.66734745335\\
97	-6564.66734745335\\
96	-6453.5469535586\\
95	-6453.5469535586\\
94	-6453.5469535586\\
93	-6453.5469535586\\
92	-6453.5469535586\\
91	-6419.87964293092\\
90	-6419.87964293092\\
89	-6419.87964293092\\
88	-6419.87964293092\\
87	-6419.87964293092\\
86	-6419.87964293092\\
85	-6419.87964293092\\
84	-6361.61477139391\\
83	-6361.61477139391\\
82	-6361.61477139391\\
81	-6292.25274086998\\
80	-6289.75553680523\\
79	-6289.75553680523\\
78	-6289.75553680523\\
77	-6229.79756557853\\
76	-6218.51549105896\\
75	-6220.30015553941\\
74	-6214.84766860093\\
73	-6214.84766860093\\
72	-6100.61549643702\\
71	-6100.61549643702\\
70	-6100.61549643702\\
69	-6100.61549643702\\
68	-6050.44112354865\\
67	-6050.44112354865\\
66	-6106.70911846153\\
65	-6106.70911846153\\
64	-6106.70911846153\\
63	-6106.70911846153\\
62	-6106.70911846153\\
61	-6067.37290377703\\
60	-6085.42157133798\\
59	-6062.26310056454\\
58	-6062.26310056454\\
57	-6062.26310056454\\
56	-6062.26310056454\\
55	-6062.26310056454\\
54	-6044.82880968721\\
53	-5870.25079716836\\
52	-5851.65824752221\\
51	-5854.99414807717\\
50	-5854.99414807717\\
49	-5854.99414807717\\
48	-5828.01188622583\\
47	-5574.21527728959\\
46	-5572.95541078165\\
45	-5478.6525890019\\
44	-5478.6525890019\\
43	-5458.40686971453\\
42	-5458.40686971453\\
41	-5458.40686971453\\
40	-5325.62302633509\\
39	-5260.06787994392\\
38	-5260.06787994392\\
37	-5195.32939391303\\
36	-5091.43244956778\\
35	-5091.43244956778\\
34	-5091.43244956778\\
33	-4973.62952677715\\
32	-4945.95365518287\\
31	-4880.6080252192\\
30	-4792.62262672397\\
29	-4718.90505221705\\
28	-4718.90505221705\\
27	-4718.90505221705\\
26	-4718.90505221705\\
25	-4721.19145910363\\
24	-4425.43877738069\\
23	-4221.22191700828\\
22	-3984.19324968572\\
21	-3985.38429005265\\
20	-3850.21618574375\\
19	-3619.25271171019\\
18	-3612.07601380872\\
17	-3637.38411118899\\
16	-3636.28332621949\\
15	-3636.28332621949\\
14	-3251.0797769409\\
13	-3237.83805730965\\
12	-3237.83805730965\\
11	-3214.41575134078\\
10	-3168.27069584966\\
9	-3135.00666149739\\
8	-3085.30099121452\\
7	-2899.37830386928\\
6	-2900.56666739697\\
5	-2773.13150520142\\
4	-2717.1435433971\\
3	-2534.41242516551\\
2	-2158.70316341115\\
1	-1093.963261449\\
}--cycle;
\addplot [color=orange]
  table[row sep=crcr]{%
1	-2117\\
2	-2798\\
3	-3047\\
4	-3440\\
5	-3473\\
6	-3643\\
7	-3648\\
8	-3765\\
9	-3883\\
10	-3899\\
11	-3924\\
12	-4037\\
13	-4037\\
14	-4045\\
15	-4234\\
16	-4234\\
17	-4262\\
18	-4405\\
19	-4425\\
20	-4654\\
21	-4714\\
22	-4760\\
23	-4882\\
24	-4977\\
25	-5212\\
26	-5232\\
27	-5232\\
28	-5232\\
29	-5232\\
30	-5261\\
31	-5296\\
32	-5370\\
33	-5437\\
34	-5484\\
35	-5484\\
36	-5484\\
37	-5524\\
38	-5603\\
39	-5603\\
40	-5658\\
41	-5725\\
42	-5725\\
43	-5725\\
44	-5779\\
45	-5779\\
46	-5814\\
47	-5816\\
48	-5920\\
49	-5994\\
50	-5994\\
51	-5994\\
52	-6007\\
53	-6046\\
54	-6128\\
55	-6135\\
56	-6135\\
57	-6135\\
58	-6135\\
59	-6135\\
60	-6161\\
61	-6229\\
62	-6281\\
63	-6281\\
64	-6281\\
65	-6281\\
66	-6281\\
67	-6405\\
68	-6405\\
69	-6474\\
70	-6474\\
71	-6474\\
72	-6474\\
73	-6556\\
74	-6556\\
75	-6558\\
76	-6566\\
77	-6577\\
78	-6694\\
79	-6694\\
80	-6694\\
81	-6696\\
82	-6808\\
83	-6808\\
84	-6808\\
85	-6886\\
86	-6886\\
87	-6886\\
88	-6886\\
89	-6886\\
90	-6886\\
91	-6886\\
92	-6945\\
93	-6945\\
94	-6945\\
95	-6945\\
96	-6945\\
97	-6987\\
98	-6987\\
99	-6987\\
100	-6990\\
};
\addlegendentry{muscles, c = 0.05 s}


\addplot[area legend, draw=none, fill=red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	-4282.57904728777\\
2	-5443.36471358105\\
3	-5458.90750870273\\
4	-5458.90750870273\\
5	-5725.26411033104\\
6	-5828.62943684691\\
7	-5835.72648073652\\
8	-5922.95853951417\\
9	-6363.91241853273\\
10	-6373.05133809314\\
11	-6456.684852007\\
12	-6456.684852007\\
13	-6678.22566951122\\
14	-6678.22566951122\\
15	-6674.96178929033\\
16	-6674.96178929033\\
17	-6674.96178929033\\
18	-6674.96178929033\\
19	-6674.96178929033\\
20	-6674.96178929033\\
21	-6674.96178929033\\
22	-6807.69389913169\\
23	-6895.86295059955\\
24	-6895.86295059955\\
25	-6895.86295059955\\
26	-6882.01720876026\\
27	-6882.01720876026\\
28	-6906.26050141658\\
29	-7003.14003095929\\
30	-7149.92224931354\\
31	-7149.92224931354\\
32	-7591.7033082859\\
33	-7625.22428532694\\
34	-7627.70778703185\\
35	-7645.58552215956\\
36	-7669.55257805323\\
37	-7704.78036900014\\
38	-7704.78036900014\\
39	-7798.53255091449\\
40	-7832.32051679256\\
41	-7834.20749675584\\
42	-7853.10840486858\\
43	-7879.20641438858\\
44	-7867.64220507391\\
45	-7919.35683247907\\
46	-7885.61590343593\\
47	-7879.06637257348\\
48	-7883.88000725778\\
49	-7830.73163268277\\
50	-7830.73163268277\\
51	-7833.15151445794\\
52	-7852.40979832097\\
53	-7871.51556190107\\
54	-7925.88784193477\\
55	-7925.88784193477\\
56	-7857.49641422645\\
57	-7829.85571744554\\
58	-7834.50184346103\\
59	-7894.74530556976\\
60	-7952.97741771012\\
61	-7908.11849554606\\
62	-7908.11849554606\\
63	-7949.24475796418\\
64	-7940.09392149461\\
65	-7933.97215342437\\
66	-7957.95534319953\\
67	-7958.16948889282\\
68	-7959.79202868747\\
69	-8001.59403856592\\
70	-8052.14568798587\\
71	-8052.14568798587\\
72	-8102.98646814014\\
73	-8119.6713382809\\
74	-8137.17240873148\\
75	-8126.43541129084\\
76	-8126.75124982894\\
77	-8126.75124982894\\
78	-8127.2722272983\\
79	-8127.2722272983\\
80	-8127.2722272983\\
81	-8128.59953675659\\
82	-8135.74295315796\\
83	-8137.04938382904\\
84	-8148.08148390218\\
85	-8148.79637939122\\
86	-8165.21391270311\\
87	-8165.21391270311\\
88	-8165.21391270311\\
89	-8172.92108432258\\
90	-8173.21548729218\\
91	-8173.21548729218\\
92	-8169.89263423003\\
93	-8184.15793933373\\
94	-8184.15793933373\\
95	-8184.15793933373\\
96	-8183.09827444768\\
97	-8185.276524813\\
98	-8190.4549378295\\
99	-8188.20899344392\\
100	-8188.20899344392\\
100	-6663.41151225292\\
99	-6663.41151225292\\
98	-6652.072658305\\
97	-6643.79876154944\\
96	-6642.52423043303\\
95	-6637.1272683319\\
94	-6637.1272683319\\
93	-6637.1272683319\\
92	-6632.37399312619\\
91	-6615.6436735601\\
90	-6615.6436735601\\
89	-6614.16893062201\\
88	-6609.71915663742\\
87	-6609.71915663742\\
86	-6609.71915663742\\
85	-6611.52082913723\\
84	-6607.91056754792\\
83	-6604.72411923023\\
82	-6603.55538258321\\
81	-6598.24822007576\\
80	-6597.49763506675\\
79	-6597.49763506675\\
78	-6597.49763506675\\
77	-6594.7311531324\\
76	-6594.7311531324\\
75	-6593.01469442579\\
74	-6535.75239179495\\
73	-6530.0987205755\\
72	-6520.70447112847\\
71	-6499.42117712915\\
70	-6499.42117712915\\
69	-6467.3287387578\\
68	-6426.26897524972\\
67	-6421.4754291546\\
66	-6420.82761524508\\
65	-6387.1117498687\\
64	-6331.25746736339\\
63	-6280.62179454886\\
62	-6256.69409176993\\
61	-6256.69409176993\\
60	-6041.57428968786\\
59	-6052.56079876014\\
58	-5956.986129557\\
57	-5794.66185948427\\
56	-5699.04772032047\\
55	-5464.17064079621\\
54	-5464.17064079621\\
53	-5423.91791069259\\
52	-5417.70018374968\\
51	-5410.74119844736\\
50	-5409.81419299135\\
49	-5409.81419299135\\
48	-5231.76739122842\\
47	-5228.14122955015\\
46	-5078.6615358341\\
45	-4969.95368759033\\
44	-4881.52509373625\\
43	-4843.73071004039\\
42	-4835.09453114881\\
41	-4828.19195029583\\
40	-4827.47098376106\\
39	-4813.50326129747\\
38	-4803.8118230559\\
37	-4803.8118230559\\
36	-4774.55850515427\\
35	-4754.96660942096\\
34	-4746.70329299062\\
33	-4745.57592335623\\
32	-4728.20017362702\\
31	-4701.39439295035\\
30	-4701.39439295035\\
29	-4550.20777247671\\
28	-4525.69857409559\\
27	-4517.17276110436\\
26	-4517.17276110436\\
25	-4461.11504623414\\
24	-4461.11504623414\\
23	-4461.11504623414\\
22	-4446.1725583677\\
21	-4331.08548593714\\
20	-4331.08548593714\\
19	-4331.08548593714\\
18	-4331.08548593714\\
17	-4331.08548593714\\
16	-4331.08548593714\\
15	-4331.08548593714\\
14	-4319.97574978293\\
13	-4319.97574978293\\
12	-4255.92255709346\\
11	-4255.92255709346\\
10	-4020.10020696575\\
9	-3939.2572143647\\
8	-3699.89161591684\\
7	-3643.0645645454\\
6	-3321.02241463156\\
5	-3224.56181712101\\
4	-3208.6513290335\\
3	-3208.6513290335\\
2	-3052.68403409097\\
1	-2175.33987577862\\
}--cycle;
\addplot [color=red]
  table[row sep=crcr]{%
1	-3229\\
2	-4248\\
3	-4334\\
4	-4334\\
5	-4475\\
6	-4575\\
7	-4739\\
8	-4811\\
9	-5152\\
10	-5197\\
11	-5356\\
12	-5356\\
13	-5499\\
14	-5499\\
15	-5503\\
16	-5503\\
17	-5503\\
18	-5503\\
19	-5503\\
20	-5503\\
21	-5503\\
22	-5627\\
23	-5678\\
24	-5678\\
25	-5678\\
26	-5700\\
27	-5700\\
28	-5716\\
29	-5777\\
30	-5926\\
31	-5926\\
32	-6160\\
33	-6185\\
34	-6187\\
35	-6200\\
36	-6222\\
37	-6254\\
38	-6254\\
39	-6306\\
40	-6330\\
41	-6331\\
42	-6344\\
43	-6361\\
44	-6375\\
45	-6445\\
46	-6482\\
47	-6554\\
48	-6558\\
49	-6620\\
50	-6620\\
51	-6622\\
52	-6635\\
53	-6648\\
54	-6695\\
55	-6695\\
56	-6778\\
57	-6812\\
58	-6896\\
59	-6974\\
60	-6997\\
61	-7082\\
62	-7082\\
63	-7115\\
64	-7136\\
65	-7161\\
66	-7189\\
67	-7190\\
68	-7193\\
69	-7234\\
70	-7276\\
71	-7276\\
72	-7312\\
73	-7325\\
74	-7336\\
75	-7360\\
76	-7361\\
77	-7361\\
78	-7362\\
79	-7362\\
80	-7362\\
81	-7363\\
82	-7370\\
83	-7371\\
84	-7378\\
85	-7380\\
86	-7387\\
87	-7387\\
88	-7387\\
89	-7394\\
90	-7394\\
91	-7394\\
92	-7401\\
93	-7411\\
94	-7411\\
95	-7411\\
96	-7413\\
97	-7415\\
98	-7421\\
99	-7426\\
100	-7426\\
};
\addlegendentry{muscles, c = 0.15 s}


\addplot[area legend, draw=none, fill=black!50!red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	-5309.59710680297\\
2	-5379.28128514495\\
3	-5519.44814420699\\
4	-6041.98976644551\\
5	-6733.6294484453\\
6	-6733.6294484453\\
7	-6733.6294484453\\
8	-6741.82657628771\\
9	-6906.10567793555\\
10	-6906.10567793555\\
11	-7295.80768970971\\
12	-7352.6430224026\\
13	-7352.6430224026\\
14	-7357.92227143345\\
15	-7357.92227143345\\
16	-7432.20069883609\\
17	-7613.39251804853\\
18	-7622.38940511394\\
19	-7731.79290177511\\
20	-7794.36578999014\\
21	-7814.13244094272\\
22	-7847.3015802137\\
23	-7847.3015802137\\
24	-7847.3015802137\\
25	-7847.3015802137\\
26	-7804.76702631933\\
27	-7809.84600501291\\
28	-7809.84600501291\\
29	-7809.84600501291\\
30	-7811.13017402449\\
31	-7811.13017402449\\
32	-7813.29107655562\\
33	-7813.29107655562\\
34	-7813.29107655562\\
35	-7813.29107655562\\
36	-7846.49424563946\\
37	-7840.79734515155\\
38	-7840.79734515155\\
39	-7843.5626975946\\
40	-7843.5626975946\\
41	-7843.5258835903\\
42	-7845.42545724994\\
43	-7846.23102574522\\
44	-7846.40747315233\\
45	-7827.22505909749\\
46	-7828.30649412116\\
47	-7830.63397973825\\
48	-7831.8219969198\\
49	-7832.13986383814\\
50	-7819.95919616775\\
51	-7821.50829305867\\
52	-7822.07512609144\\
53	-7864.1259110343\\
54	-7860.54241355738\\
55	-7860.54241355738\\
56	-7860.54241355738\\
57	-7864.31363785612\\
58	-7846.97189481667\\
59	-7846.97189481667\\
60	-7846.97189481667\\
61	-7868.42025232306\\
62	-7862.35126188295\\
63	-7862.35126188295\\
64	-7838.30326958868\\
65	-7838.30326958868\\
66	-7837.74767625577\\
67	-7817.73834986893\\
68	-7817.73834986893\\
69	-7817.73834986893\\
70	-7817.73834986893\\
71	-7817.73834986893\\
72	-7817.73834986893\\
73	-7814.78251185104\\
74	-7814.78251185104\\
75	-7814.78251185104\\
76	-7812.87585011352\\
77	-7812.87585011352\\
78	-7812.87585011352\\
79	-7812.87585011352\\
80	-7809.19513516924\\
81	-7809.19513516924\\
82	-7808.70251430469\\
83	-7808.5706056456\\
84	-7807.99424511231\\
85	-7807.80931235394\\
86	-7807.80931235394\\
87	-7805.04217466169\\
88	-7805.04217466169\\
89	-7804.68728357225\\
90	-7843.7600194191\\
91	-7843.74134932852\\
92	-7843.4644270063\\
93	-7842.89997590362\\
94	-7842.89997590362\\
95	-7842.89997590362\\
96	-7842.89997590362\\
97	-7843.70749122684\\
98	-7843.26115206107\\
99	-7843.26115206107\\
100	-7843.20881193135\\
100	-5847.24432133752\\
99	-5847.05112394328\\
98	-5847.05112394328\\
97	-5845.40412236979\\
96	-5845.29162451994\\
95	-5845.29162451994\\
94	-5845.29162451994\\
93	-5845.29162451994\\
92	-5843.21041544856\\
91	-5842.18990477454\\
90	-5842.12111473928\\
89	-5832.62501630621\\
88	-5831.32630143474\\
87	-5831.32630143474\\
86	-5821.21896594376\\
85	-5821.21896594376\\
84	-5817.49560690121\\
83	-5815.39709937174\\
82	-5814.91702143148\\
81	-5813.12478583578\\
80	-5813.12478583578\\
79	-5799.76538710685\\
78	-5799.76538710685\\
77	-5799.76538710685\\
76	-5799.76538710685\\
75	-5792.86647225437\\
74	-5792.86647225437\\
73	-5792.86647225437\\
72	-5782.19930092719\\
71	-5782.19930092719\\
70	-5782.19930092719\\
69	-5782.19930092719\\
68	-5782.19930092719\\
67	-5782.19930092719\\
66	-5710.80727295383\\
65	-5708.84367859661\\
64	-5708.84367859661\\
63	-5624.68890287976\\
62	-5624.68890287976\\
61	-5603.68558015585\\
60	-5588.99576381535\\
59	-5588.99576381535\\
58	-5588.99576381535\\
57	-5529.76231450584\\
56	-5529.00798889822\\
55	-5529.00798889822\\
54	-5529.00798889822\\
53	-5515.10038499534\\
52	-5508.53860972818\\
51	-5508.43544598041\\
50	-5508.15195778118\\
49	-5466.48506595528\\
48	-5466.42576527296\\
47	-5466.20619568646\\
46	-5465.76717748444\\
45	-5465.56652618585\\
44	-5401.64985240588\\
43	-5401.61701865984\\
42	-5400.08356199187\\
41	-5399.72480341775\\
40	-5382.67132807623\\
39	-5382.67132807623\\
38	-5382.13683135287\\
37	-5382.13683135287\\
36	-5329.80707284186\\
35	-5324.40013507403\\
34	-5324.40013507403\\
33	-5324.40013507403\\
32	-5324.40013507403\\
31	-5324.00682676828\\
30	-5324.00682676828\\
29	-5323.77050069582\\
28	-5323.77050069582\\
27	-5323.77050069582\\
26	-5322.81665693656\\
25	-5175.07361460724\\
24	-5175.07361460724\\
23	-5175.07361460724\\
22	-5175.07361460724\\
21	-5168.37923849664\\
20	-5164.79129437871\\
19	-5151.32232652045\\
18	-5115.7528982233\\
17	-5114.44695878186\\
16	-4981.22660931562\\
15	-4904.93058250629\\
14	-4904.93058250629\\
13	-4904.82972392869\\
12	-4904.82972392869\\
11	-3877.89798880436\\
10	-3378.59406577079\\
9	-3378.59406577079\\
8	-3383.62885493996\\
7	-3358.98236105882\\
6	-3358.98236105882\\
5	-3358.98236105882\\
4	-3113.58416434772\\
3	-3083.48450582187\\
2	-2620.65160097923\\
1	-1683.12966794915\\
}--cycle;
\addplot [color=black!50!red]
  table[row sep=crcr]{%
1	-3496\\
2	-4000\\
3	-4301\\
4	-4578\\
5	-5046\\
6	-5046\\
7	-5046\\
8	-5063\\
9	-5142\\
10	-5142\\
11	-5587\\
12	-6129\\
13	-6129\\
14	-6131\\
15	-6131\\
16	-6207\\
17	-6364\\
18	-6369\\
19	-6442\\
20	-6480\\
21	-6491\\
22	-6511\\
23	-6511\\
24	-6511\\
25	-6511\\
26	-6564\\
27	-6567\\
28	-6567\\
29	-6567\\
30	-6568\\
31	-6568\\
32	-6569\\
33	-6569\\
34	-6569\\
35	-6569\\
36	-6588\\
37	-6611\\
38	-6611\\
39	-6613\\
40	-6613\\
41	-6622\\
42	-6623\\
43	-6624\\
44	-6624\\
45	-6646\\
46	-6647\\
47	-6648\\
48	-6649\\
49	-6649\\
50	-6664\\
51	-6665\\
52	-6665\\
53	-6690\\
54	-6695\\
55	-6695\\
56	-6695\\
57	-6697\\
58	-6718\\
59	-6718\\
60	-6718\\
61	-6736\\
62	-6744\\
63	-6744\\
64	-6774\\
65	-6774\\
66	-6774\\
67	-6800\\
68	-6800\\
69	-6800\\
70	-6800\\
71	-6800\\
72	-6800\\
73	-6804\\
74	-6804\\
75	-6804\\
76	-6806\\
77	-6806\\
78	-6806\\
79	-6806\\
80	-6811\\
81	-6811\\
82	-6812\\
83	-6812\\
84	-6813\\
85	-6815\\
86	-6815\\
87	-6818\\
88	-6818\\
89	-6819\\
90	-6843\\
91	-6843\\
92	-6843\\
93	-6844\\
94	-6844\\
95	-6844\\
96	-6844\\
97	-6845\\
98	-6845\\
99	-6845\\
100	-6845\\
};
\addlegendentry{muscles, c = 0.3 s}

\legend{}
\end{axis}


==> figures/dataefficiency_cost_jumping.tex <==
\begin{axis}[%
name =ax4,
scaled y ticks=base 10:\Factor,
at={(ax3.south east)},
xlabel near ticks, ylabel near ticks,
every y tick scale label/.style={at={(yticklabel* cs:1.03,0cm)},anchor=near yticklabel},
title style={at={(0.5,0.93)}},
xshift=1cm,
width=0.639\figW,
height=\figH,
scale only axis,
xmin=0,
xmax=100,
xtick={  0,  20,  40,  60,  80, 100},
xlabel style={font=\color{white!15!black}},
xlabel={generations},
ymin=-900,
ymax=-550,
ylabel style={font=\color{white!15!black}},
ylabel={cost},
axis background/.style={fill=white},
title={(d) high-jumping (OC)},
legend style={at={(1.03,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]

\addplot[area legend, draw=none, fill=mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	-753.543601147122\\
2	-772.474500357352\\
3	-780.158213461913\\
4	-775.628937685188\\
5	-804.833106928538\\
6	-804.599119462824\\
7	-809.014372845352\\
8	-818.726511896109\\
9	-818.726511896109\\
10	-818.780427254835\\
11	-819.746956224431\\
12	-820.18836165223\\
13	-820.928726406177\\
14	-825.641573502176\\
15	-835.728843692383\\
16	-837.346921977322\\
17	-837.346921977322\\
18	-837.373261373717\\
19	-838.583771669756\\
20	-839.537183803368\\
21	-842.522122689122\\
22	-842.522122689122\\
23	-846.420654842828\\
24	-853.468341962171\\
25	-853.468341962171\\
26	-859.563244398069\\
27	-859.563244398069\\
28	-859.582614106301\\
29	-860.194883586149\\
30	-860.194883586149\\
31	-860.143743014562\\
32	-860.125782230632\\
33	-860.123817096334\\
34	-860.121960895829\\
35	-860.048799563657\\
36	-860.509635465477\\
37	-860.459857164925\\
38	-860.459857164925\\
39	-860.459857164925\\
40	-860.455162202813\\
41	-863.002258112952\\
42	-863.002258112952\\
43	-862.984314719321\\
44	-863.148556825207\\
45	-863.540459593506\\
46	-864.891676853018\\
47	-865.90211215866\\
48	-865.967538489961\\
49	-865.967538489961\\
50	-866.924474070165\\
51	-868.631518223413\\
52	-869.896110410499\\
53	-871.200294374917\\
54	-871.189092099342\\
55	-871.189092099342\\
56	-873.846622911436\\
57	-873.846622911436\\
58	-873.73319654968\\
59	-873.73319654968\\
60	-873.73319654968\\
61	-873.73319654968\\
62	-873.73319654968\\
63	-873.73319654968\\
64	-873.884465009038\\
65	-873.884465009038\\
66	-874.6408885573\\
67	-874.736435952819\\
68	-875.070042412107\\
69	-875.070042412107\\
70	-875.066618098467\\
71	-875.066618098467\\
72	-875.065764702497\\
73	-875.577208047799\\
74	-876.496670092324\\
75	-876.496670092324\\
76	-876.496670092324\\
77	-876.496670092324\\
78	-876.495553025306\\
79	-876.458918192838\\
80	-876.458918192838\\
81	-876.458918192838\\
82	-876.822419009708\\
83	-876.821962918725\\
84	-876.821962918725\\
85	-876.821962918725\\
86	-876.837989918273\\
87	-876.835416372807\\
88	-877.440082183856\\
89	-877.627375502769\\
90	-877.669425804138\\
91	-878.457332314997\\
92	-878.457332314997\\
93	-878.454491221318\\
94	-878.59014460358\\
95	-878.575190771217\\
96	-878.63951789865\\
97	-878.652565306025\\
98	-878.650372162999\\
99	-878.74137253596\\
100	-878.74137253596\\
100	-801.826196812417\\
99	-801.826196812417\\
98	-801.8170687097\\
97	-801.795170539114\\
96	-801.777958337296\\
95	-801.77137471565\\
94	-801.625555508872\\
93	-801.608735875429\\
92	-801.581211902873\\
91	-801.581211902873\\
90	-801.492117336102\\
89	-801.486824192784\\
88	-801.474102614821\\
87	-801.362837980793\\
86	-801.336686693084\\
85	-801.334845832553\\
84	-801.334845832553\\
83	-801.334845832553\\
82	-801.330219910793\\
81	-801.293438373286\\
80	-801.293438373286\\
79	-801.293438373286\\
78	-800.941577028065\\
77	-800.929805827103\\
76	-800.929805827103\\
75	-800.929805827103\\
74	-800.929805827103\\
73	-800.862687358854\\
72	-800.786298500163\\
71	-800.777349399422\\
70	-800.777349399422\\
69	-800.741546433137\\
68	-800.741546433137\\
67	-800.698444779952\\
66	-800.685415232149\\
65	-800.609055265312\\
64	-800.609055265312\\
63	-800.587308093748\\
62	-800.587308093748\\
61	-800.587308093748\\
60	-800.587308093748\\
59	-800.587308093748\\
58	-800.587308093748\\
57	-799.571086913884\\
56	-799.571086913884\\
55	-799.239507202346\\
54	-799.239507202346\\
53	-799.103550339863\\
52	-798.957161737618\\
51	-798.839449091143\\
50	-798.685358976183\\
49	-798.556194698895\\
48	-798.556194698895\\
47	-798.546100063444\\
46	-798.4444366252\\
45	-798.340165137155\\
44	-797.56610591468\\
43	-797.55135276564\\
42	-797.313020646095\\
41	-797.313020646095\\
40	-797.022679798348\\
39	-796.961164381371\\
38	-796.961164381371\\
37	-796.961164381371\\
36	-796.5627909446\\
35	-796.491920374017\\
34	-795.124742263947\\
33	-795.091536368014\\
32	-795.056757329458\\
31	-794.927183935211\\
30	-794.103098726965\\
29	-794.103098726965\\
28	-794.064857667246\\
27	-793.551986375364\\
26	-793.551986375364\\
25	-792.238659465141\\
24	-792.238659465141\\
23	-789.456975593055\\
22	-784.044433195823\\
21	-784.044433195823\\
20	-783.825428766694\\
19	-776.55934387754\\
18	-776.808365469414\\
17	-776.576872951022\\
16	-776.576872951022\\
15	-776.666829043099\\
14	-777.479191215923\\
13	-772.130112263376\\
12	-772.323841511928\\
11	-772.438138516576\\
10	-770.284375834242\\
9	-769.860343836257\\
8	-769.860343836257\\
7	-772.11977384204\\
6	-769.171437131607\\
5	-765.313821638897\\
4	-763.291251127515\\
3	-712.753580252051\\
2	-669.868154246509\\
1	-653.921249783981\\
}--cycle;
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	-704\\
2	-721\\
3	-746\\
4	-769\\
5	-785\\
6	-787\\
7	-791\\
8	-794\\
9	-794\\
10	-795\\
11	-796\\
12	-796\\
13	-797\\
14	-802\\
15	-806\\
16	-807\\
17	-807\\
18	-807\\
19	-808\\
20	-812\\
21	-813\\
22	-813\\
23	-818\\
24	-823\\
25	-823\\
26	-827\\
27	-827\\
28	-827\\
29	-827\\
30	-827\\
31	-828\\
32	-828\\
33	-828\\
34	-828\\
35	-828\\
36	-829\\
37	-829\\
38	-829\\
39	-829\\
40	-829\\
41	-830\\
42	-830\\
43	-830\\
44	-830\\
45	-831\\
46	-832\\
47	-832\\
48	-832\\
49	-832\\
50	-833\\
51	-834\\
52	-834\\
53	-835\\
54	-835\\
55	-835\\
56	-837\\
57	-837\\
58	-837\\
59	-837\\
60	-837\\
61	-837\\
62	-837\\
63	-837\\
64	-837\\
65	-837\\
66	-838\\
67	-838\\
68	-838\\
69	-838\\
70	-838\\
71	-838\\
72	-838\\
73	-838\\
74	-839\\
75	-839\\
76	-839\\
77	-839\\
78	-839\\
79	-839\\
80	-839\\
81	-839\\
82	-839\\
83	-839\\
84	-839\\
85	-839\\
86	-839\\
87	-839\\
88	-839\\
89	-840\\
90	-840\\
91	-840\\
92	-840\\
93	-840\\
94	-840\\
95	-840\\
96	-840\\
97	-840\\
98	-840\\
99	-840\\
100	-840\\
};
\addlegendentry{torques, c = 0.05 s}


\addplot[area legend, draw=none, fill=blue!50!mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	-759.757826733523\\
2	-788.547134222445\\
3	-782.683643269468\\
4	-791.159490649548\\
5	-791.159490649548\\
6	-792.906362585732\\
7	-792.906362585732\\
8	-792.920978167089\\
9	-792.920978167089\\
10	-793.596470346167\\
11	-793.596470346167\\
12	-793.700205047308\\
13	-794.301993243866\\
14	-794.301993243866\\
15	-794.273315877461\\
16	-796.256687171359\\
17	-796.256687171359\\
18	-796.256687171359\\
19	-796.26416346224\\
20	-796.26416346224\\
21	-796.26416346224\\
22	-796.381491548702\\
23	-796.421252450346\\
24	-797.103449332433\\
25	-797.103449332433\\
26	-797.34160309593\\
27	-797.34160309593\\
28	-797.435239758362\\
29	-797.575133333627\\
30	-797.575133333627\\
31	-797.575133333627\\
32	-797.575133333627\\
33	-797.658275592705\\
34	-797.72959118091\\
35	-797.775496361665\\
36	-797.879708350343\\
37	-797.898928686393\\
38	-797.915025301594\\
39	-797.972356667978\\
40	-798.113121211093\\
41	-798.230525408044\\
42	-798.230525408044\\
43	-798.28148166424\\
44	-798.32676919206\\
45	-798.333185548245\\
46	-798.333185548245\\
47	-798.626233834549\\
48	-798.626233834549\\
49	-798.626233834549\\
50	-798.672268632452\\
51	-798.675662114552\\
52	-798.783652321941\\
53	-798.840414144956\\
54	-798.840414144956\\
55	-798.994495183783\\
56	-798.994495183783\\
57	-798.994495183783\\
58	-798.994495183783\\
59	-799.011606321531\\
60	-799.011606321531\\
61	-799.026969474645\\
62	-799.03214626679\\
63	-799.067642483695\\
64	-799.067642483695\\
65	-799.073845775723\\
66	-799.085147082843\\
67	-799.086005709509\\
68	-799.086005709509\\
69	-799.086005709509\\
70	-799.134137644947\\
71	-799.137255646893\\
72	-799.137602369588\\
73	-799.137602369588\\
74	-799.138330739949\\
75	-799.149984617068\\
76	-799.149984617068\\
77	-799.152614945243\\
78	-799.193987456739\\
79	-799.193987456739\\
80	-799.196394364663\\
81	-799.3258319672\\
82	-799.4411500551\\
83	-799.520821402233\\
84	-799.661257441792\\
85	-799.662029580639\\
86	-799.686053767062\\
87	-799.686832356413\\
88	-799.700299614079\\
89	-799.700299614079\\
90	-799.700299614079\\
91	-799.759718805277\\
92	-799.759849625\\
93	-799.86239717776\\
94	-799.865645203415\\
95	-799.885297398399\\
96	-799.885297398399\\
97	-799.885421382668\\
98	-799.885687084081\\
99	-799.88586516357\\
100	-799.959022500143\\
100	-792.616717503065\\
99	-792.588459918567\\
98	-792.58840347305\\
97	-792.58832431926\\
96	-792.588285012034\\
95	-792.588285012034\\
94	-792.580043936755\\
93	-792.579093484759\\
92	-792.531111206924\\
91	-792.531073063387\\
90	-792.499121544086\\
89	-792.499121544086\\
88	-792.499121544086\\
87	-792.491340286305\\
86	-792.49112437671\\
85	-792.47716602991\\
84	-792.476955156425\\
83	-792.378647326256\\
82	-792.309679816633\\
81	-792.19241903909\\
80	-792.008551591523\\
79	-792.008124811341\\
78	-792.008124811341\\
77	-791.933631717192\\
76	-791.933184102155\\
75	-791.933184102155\\
74	-791.931274362385\\
73	-791.931152798634\\
72	-791.931152798634\\
71	-791.931094859484\\
70	-791.930571742443\\
69	-791.826294233721\\
68	-791.826294233721\\
67	-791.826294233721\\
66	-791.826158521452\\
65	-791.824350747332\\
64	-791.823366927521\\
63	-791.823366927521\\
62	-791.754749214371\\
61	-791.75392487813\\
60	-791.751419350065\\
59	-791.751419350065\\
58	-791.748522852127\\
57	-791.748522852127\\
56	-791.748522852127\\
55	-791.748522852127\\
54	-791.719193025262\\
53	-791.719193025262\\
52	-791.712259966585\\
51	-791.68804994271\\
50	-791.687731483425\\
49	-791.681793146993\\
48	-791.681793146993\\
47	-791.681793146993\\
46	-791.625788972883\\
45	-791.625788972883\\
44	-791.624333031741\\
43	-791.613480500305\\
42	-791.601053981816\\
41	-791.601053981816\\
40	-791.573552352565\\
39	-791.526118539917\\
38	-791.503768750684\\
37	-791.496687165008\\
36	-791.487920926544\\
35	-791.440537785582\\
34	-791.413485092007\\
33	-791.271964207612\\
32	-791.275502436033\\
31	-791.275502436033\\
30	-791.275502436033\\
29	-791.275502436033\\
28	-791.184192184198\\
27	-791.188499413004\\
26	-791.188499413004\\
25	-790.629321976107\\
24	-790.629321976107\\
23	-790.445067877011\\
22	-790.444506774588\\
21	-790.440231304733\\
20	-790.440231304733\\
19	-790.440231304733\\
18	-790.439816125244\\
17	-790.439816125244\\
16	-790.439816125244\\
15	-787.443274759876\\
14	-787.321032721225\\
13	-787.321032721225\\
12	-787.17041026706\\
11	-787.119778505454\\
10	-787.119778505454\\
9	-787.213924595436\\
8	-787.213924595436\\
7	-781.790547313988\\
6	-781.790547313988\\
5	-780.674136913919\\
4	-780.674136913919\\
3	-749.072164957931\\
2	-686.894713119302\\
1	-629.093251302187\\
}--cycle;
\addplot [color=blue!50!mycolor1]
  table[row sep=crcr]{%
1	-694\\
2	-738\\
3	-766\\
4	-786\\
5	-786\\
6	-787\\
7	-787\\
8	-790\\
9	-790\\
10	-790\\
11	-790\\
12	-790\\
13	-791\\
14	-791\\
15	-791\\
16	-793\\
17	-793\\
18	-793\\
19	-793\\
20	-793\\
21	-793\\
22	-793\\
23	-793\\
24	-794\\
25	-794\\
26	-794\\
27	-794\\
28	-794\\
29	-794\\
30	-794\\
31	-794\\
32	-794\\
33	-794\\
34	-795\\
35	-795\\
36	-795\\
37	-795\\
38	-795\\
39	-795\\
40	-795\\
41	-795\\
42	-795\\
43	-795\\
44	-795\\
45	-795\\
46	-795\\
47	-795\\
48	-795\\
49	-795\\
50	-795\\
51	-795\\
52	-795\\
53	-795\\
54	-795\\
55	-795\\
56	-795\\
57	-795\\
58	-795\\
59	-795\\
60	-795\\
61	-795\\
62	-795\\
63	-795\\
64	-795\\
65	-795\\
66	-795\\
67	-795\\
68	-795\\
69	-795\\
70	-796\\
71	-796\\
72	-796\\
73	-796\\
74	-796\\
75	-796\\
76	-796\\
77	-796\\
78	-796\\
79	-796\\
80	-796\\
81	-796\\
82	-796\\
83	-796\\
84	-796\\
85	-796\\
86	-796\\
87	-796\\
88	-796\\
89	-796\\
90	-796\\
91	-796\\
92	-796\\
93	-796\\
94	-796\\
95	-796\\
96	-796\\
97	-796\\
98	-796\\
99	-796\\
100	-796\\
};
\addlegendentry{torques, c = 0.15 s}


\addplot[area legend, draw=none, fill=blue, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	-731.499455985821\\
2	-791.164664865091\\
3	-787.022601994071\\
4	-782.542977251791\\
5	-786.398548315949\\
6	-786.765702889886\\
7	-790.690892583936\\
8	-791.610155911823\\
9	-792.825546699632\\
10	-792.943927616574\\
11	-793.686534384616\\
12	-793.895028145098\\
13	-793.895028145098\\
14	-794.276988918297\\
15	-794.661580232331\\
16	-794.970099736483\\
17	-794.423199508611\\
18	-794.423199508611\\
19	-794.437461737118\\
20	-795.719972516121\\
21	-795.746570144545\\
22	-796.662327437982\\
23	-796.555845790859\\
24	-796.555845790859\\
25	-796.638716679954\\
26	-796.811008757536\\
27	-797.087965249344\\
28	-797.411641836127\\
29	-797.563939966771\\
30	-797.596209526762\\
31	-797.646749110497\\
32	-797.813051437196\\
33	-797.92948712263\\
34	-797.932163328437\\
35	-797.932163328437\\
36	-797.978014688038\\
37	-798.097491188887\\
38	-798.09564304104\\
39	-798.114689250099\\
40	-798.126256829257\\
41	-798.105724952097\\
42	-798.107028100298\\
43	-798.107062302278\\
44	-798.130120962898\\
45	-798.141528050625\\
46	-798.144877617108\\
47	-798.150267803124\\
48	-798.158863751363\\
49	-798.158672476224\\
50	-798.158335045036\\
51	-798.157459083634\\
52	-798.157894887814\\
53	-798.163284102127\\
54	-798.163368773883\\
55	-798.163368773883\\
56	-798.163479762286\\
57	-798.165020796099\\
58	-798.165373367581\\
59	-798.168712130143\\
60	-798.170372536084\\
61	-798.181774278697\\
62	-798.182036674032\\
63	-798.18229687113\\
64	-798.182371308597\\
65	-798.184054714035\\
66	-798.184240684434\\
67	-798.184324033687\\
68	-798.18902812262\\
69	-798.189079241881\\
70	-798.18913941269\\
71	-798.189243420446\\
72	-798.189305028302\\
73	-798.189305028302\\
74	-798.190246023699\\
75	-798.190296503505\\
76	-798.190320918452\\
77	-798.190347760038\\
78	-798.190381226819\\
79	-798.190891274899\\
80	-798.191358504089\\
81	-798.191358504089\\
82	-798.191364739859\\
83	-798.191816415629\\
84	-798.191824654291\\
85	-798.191829777683\\
86	-798.191830670271\\
87	-798.192032505623\\
88	-798.192032661284\\
89	-798.192144451201\\
90	-798.192169902637\\
91	-798.192172149034\\
92	-798.192172149034\\
93	-798.192172411166\\
94	-798.19217379957\\
95	-798.192174086698\\
96	-798.192239321801\\
97	-798.192287930208\\
98	-798.192288173286\\
99	-798.192293071609\\
100	-798.192299781819\\
100	-798.114246093556\\
99	-798.114247540802\\
98	-798.11424915599\\
97	-798.114248247899\\
96	-798.114264276007\\
95	-798.114285204011\\
94	-798.114284130711\\
93	-798.114278940786\\
92	-798.114277960832\\
91	-798.114277960832\\
90	-798.1142695656\\
89	-798.114270908336\\
88	-798.11430613362\\
87	-798.114305551265\\
86	-798.114361576364\\
85	-798.114358228082\\
84	-798.114339032333\\
83	-798.114308178465\\
82	-798.114440116072\\
81	-798.114416642538\\
80	-798.114416642538\\
79	-798.114547318358\\
78	-798.114651615208\\
77	-798.114662638565\\
76	-798.114560634936\\
75	-798.11446834908\\
74	-798.114351408914\\
73	-798.114501375828\\
72	-798.114501375828\\
71	-798.114263163226\\
70	-798.113866087755\\
69	-798.113634017724\\
68	-798.113429672399\\
67	-798.114437144826\\
66	-798.114082006568\\
65	-798.113349988754\\
64	-798.113541753089\\
63	-798.113233885989\\
62	-798.113318451168\\
61	-798.111866335871\\
60	-798.115514500904\\
59	-798.113089483565\\
58	-798.113962484591\\
57	-798.114070514566\\
56	-798.111912771057\\
55	-798.111432617106\\
54	-798.111432617106\\
53	-798.110814259485\\
52	-798.111612356504\\
51	-798.103814071902\\
50	-798.096647013886\\
49	-798.094719770903\\
48	-798.090404440108\\
47	-798.070644576877\\
46	-798.060784353686\\
45	-798.043598347371\\
44	-798.042530006804\\
43	-798.047156767502\\
42	-798.046497503782\\
41	-798.046620098245\\
40	-797.964351657439\\
39	-797.92014320456\\
38	-797.89600199945\\
37	-797.861152561013\\
36	-797.820819393861\\
35	-797.751717417915\\
34	-797.751717417915\\
33	-797.592816264308\\
32	-797.528745723378\\
31	-797.34363908491\\
30	-797.053939520383\\
29	-796.969604369127\\
28	-796.699958009387\\
27	-796.154605488717\\
26	-795.42938344571\\
25	-795.325431518954\\
24	-795.297651118876\\
23	-795.297651118876\\
22	-794.927816320983\\
21	-793.672805369\\
20	-793.618509884824\\
19	-793.841855849606\\
18	-793.453719595254\\
17	-793.453719595254\\
16	-791.66332260937\\
15	-791.464887769349\\
14	-791.404930788575\\
13	-789.808144992792\\
12	-789.808144992792\\
11	-788.970738754892\\
10	-786.332517744587\\
9	-786.307322334763\\
8	-781.839727060877\\
7	-781.746320263575\\
6	-780.227606141889\\
5	-771.97465567629\\
4	-761.59585308032\\
3	-739.86412611626\\
2	-678.30249045831\\
1	-621.251017233866\\
}--cycle;
\addplot [color=blue]
  table[row sep=crcr]{%
1	-676\\
2	-735\\
3	-763\\
4	-772\\
5	-779\\
6	-783\\
7	-786\\
8	-787\\
9	-790\\
10	-790\\
11	-791\\
12	-792\\
13	-792\\
14	-793\\
15	-793\\
16	-793\\
17	-794\\
18	-794\\
19	-794\\
20	-795\\
21	-795\\
22	-796\\
23	-796\\
24	-796\\
25	-796\\
26	-796\\
27	-797\\
28	-797\\
29	-797\\
30	-797\\
31	-797\\
32	-798\\
33	-798\\
34	-798\\
35	-798\\
36	-798\\
37	-798\\
38	-798\\
39	-798\\
40	-798\\
41	-798\\
42	-798\\
43	-798\\
44	-798\\
45	-798\\
46	-798\\
47	-798\\
48	-798\\
49	-798\\
50	-798\\
51	-798\\
52	-798\\
53	-798\\
54	-798\\
55	-798\\
56	-798\\
57	-798\\
58	-798\\
59	-798\\
60	-798\\
61	-798\\
62	-798\\
63	-798\\
64	-798\\
65	-798\\
66	-798\\
67	-798\\
68	-798\\
69	-798\\
70	-798\\
71	-798\\
72	-798\\
73	-798\\
74	-798\\
75	-798\\
76	-798\\
77	-798\\
78	-798\\
79	-798\\
80	-798\\
81	-798\\
82	-798\\
83	-798\\
84	-798\\
85	-798\\
86	-798\\
87	-798\\
88	-798\\
89	-798\\
90	-798\\
91	-798\\
92	-798\\
93	-798\\
94	-798\\
95	-798\\
96	-798\\
97	-798\\
98	-798\\
99	-798\\
100	-798\\
};
\addlegendentry{torques, c = 0.3 s}


\addplot[area legend, draw=none, fill=orange, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	-648.867475672273\\
2	-661.970698612087\\
3	-664.560188119164\\
4	-668.685258170005\\
5	-673.701665765283\\
6	-676.301206434345\\
7	-678.48093834866\\
8	-679.474406289435\\
9	-679.866775760397\\
10	-680.29321717645\\
11	-681.763548232217\\
12	-681.734636498514\\
13	-682.112078069803\\
14	-682.741596794527\\
15	-682.208321282798\\
16	-682.966319202954\\
17	-681.696080074082\\
18	-678.070192902368\\
19	-676.732102543846\\
20	-676.45986860805\\
21	-677.219848302105\\
22	-676.394884277334\\
23	-675.801978607594\\
24	-676.192675596236\\
25	-675.590781856875\\
26	-675.06166942062\\
27	-674.407197155528\\
28	-674.407197155528\\
29	-674.407197155528\\
30	-674.407197155528\\
31	-674.450956330678\\
32	-674.450956330678\\
33	-674.450956330678\\
34	-674.897673422648\\
35	-675.040979583985\\
36	-674.840877157744\\
37	-674.840877157744\\
38	-675.105383572075\\
39	-674.910515952919\\
40	-674.971002758648\\
41	-675.776697720445\\
42	-675.776697720445\\
43	-675.82782098165\\
44	-675.82782098165\\
45	-675.854328179028\\
46	-675.9304018353\\
47	-675.9304018353\\
48	-676.561325780289\\
49	-676.67683572799\\
50	-676.41959758522\\
51	-676.452999382409\\
52	-676.452999382409\\
53	-676.452999382409\\
54	-676.452999382409\\
55	-676.549050751927\\
56	-676.645237057777\\
57	-676.645237057777\\
58	-676.645237057777\\
59	-677.276215930991\\
60	-676.914529735169\\
61	-676.914529735169\\
62	-676.914529735169\\
63	-676.918571059275\\
64	-676.992258183347\\
65	-677.004902164424\\
66	-677.137573732738\\
67	-677.137573732738\\
68	-677.137573732738\\
69	-677.26018337939\\
70	-677.328894080856\\
71	-677.328894080856\\
72	-677.377395194075\\
73	-677.377395194075\\
74	-677.377395194075\\
75	-678.079896521143\\
76	-678.079896521143\\
77	-678.233737277926\\
78	-678.168613843338\\
79	-678.168613843338\\
80	-678.282790149224\\
81	-678.282790149224\\
82	-678.282790149224\\
83	-678.282790149224\\
84	-678.314867345039\\
85	-678.314867345039\\
86	-678.314867345039\\
87	-678.314867345039\\
88	-678.314867345039\\
89	-678.314867345039\\
90	-678.594745154036\\
91	-678.690478313357\\
92	-679.092629259202\\
93	-679.183898404313\\
94	-679.069465241729\\
95	-679.069465241729\\
96	-679.084009908659\\
97	-679.087170999327\\
98	-679.088249752532\\
99	-679.14116275206\\
100	-679.041188159286\\
100	-678.614040331596\\
99	-678.274220494872\\
98	-678.242324751754\\
97	-678.241339913423\\
96	-678.23833943449\\
95	-678.238499408732\\
94	-678.238499408732\\
93	-677.128990247083\\
92	-677.113333530769\\
91	-676.792074844589\\
90	-676.377076511185\\
89	-676.334325152386\\
88	-676.334325152386\\
87	-676.334325152386\\
86	-676.334325152386\\
85	-676.334325152386\\
84	-676.334325152386\\
83	-676.320874705413\\
82	-676.320874705413\\
81	-676.320874705413\\
80	-676.320874705413\\
79	-675.598351329325\\
78	-675.598351329325\\
77	-675.218898667589\\
76	-675.166293324845\\
75	-675.166293324845\\
74	-675.211763863889\\
73	-675.211763863889\\
72	-675.211763863889\\
71	-675.204499684748\\
70	-675.204499684748\\
69	-675.188492705406\\
68	-675.148168510237\\
67	-675.148168510237\\
66	-675.148168510237\\
65	-675.029003630497\\
64	-675.029426284543\\
63	-674.403640772754\\
62	-674.269421839961\\
61	-674.269421839961\\
60	-674.269421839961\\
59	-672.711038645597\\
58	-672.548384593908\\
57	-672.548384593908\\
56	-672.548384593908\\
55	-672.478104137036\\
54	-672.314466445876\\
53	-672.314466445876\\
52	-672.314466445876\\
51	-672.314466445876\\
50	-672.28750991581\\
49	-671.342394184934\\
48	-671.250042115341\\
47	-670.93599523306\\
46	-670.93599523306\\
45	-670.933251206296\\
44	-670.909715585742\\
43	-670.909715585742\\
42	-670.911226810107\\
41	-670.911226810107\\
40	-670.772699353175\\
39	-670.737802803033\\
38	-670.050231054685\\
37	-670.067290255776\\
36	-670.067290255776\\
35	-669.424107588139\\
34	-669.285305440033\\
33	-668.95684035351\\
32	-668.95684035351\\
31	-668.95684035351\\
30	-668.570166018677\\
29	-668.570166018677\\
28	-668.570166018677\\
27	-668.570166018677\\
26	-664.606864073415\\
25	-662.987466091401\\
24	-661.156718633981\\
23	-660.162701608244\\
22	-658.344231815877\\
21	-655.198579994316\\
20	-654.720201201866\\
19	-651.338444890942\\
18	-646.74188271142\\
17	-632.828141305196\\
16	-627.652316942352\\
15	-627.28967901483\\
14	-624.959877166422\\
13	-624.665399224195\\
12	-624.449428329499\\
11	-621.155824870449\\
10	-619.735896024308\\
9	-619.424472843622\\
8	-618.731347141921\\
7	-616.599979214539\\
6	-614.58799887034\\
5	-612.88901479472\\
4	-609.755183821167\\
3	-606.837771059347\\
2	-583.677679797349\\
1	-611.719388271458\\
}--cycle;
\addplot [color=orange]
  table[row sep=crcr]{%
1	-630\\
2	-623\\
3	-636\\
4	-639\\
5	-643\\
6	-645\\
7	-648\\
8	-649\\
9	-650\\
10	-650\\
11	-651\\
12	-653\\
13	-653\\
14	-654\\
15	-655\\
16	-655\\
17	-657\\
18	-662\\
19	-664\\
20	-666\\
21	-666\\
22	-667\\
23	-668\\
24	-669\\
25	-669\\
26	-670\\
27	-671\\
28	-671\\
29	-671\\
30	-671\\
31	-672\\
32	-672\\
33	-672\\
34	-672\\
35	-672\\
36	-672\\
37	-672\\
38	-673\\
39	-673\\
40	-673\\
41	-673\\
42	-673\\
43	-673\\
44	-673\\
45	-673\\
46	-673\\
47	-673\\
48	-674\\
49	-674\\
50	-674\\
51	-674\\
52	-674\\
53	-674\\
54	-674\\
55	-675\\
56	-675\\
57	-675\\
58	-675\\
59	-675\\
60	-676\\
61	-676\\
62	-676\\
63	-676\\
64	-676\\
65	-676\\
66	-676\\
67	-676\\
68	-676\\
69	-676\\
70	-676\\
71	-676\\
72	-676\\
73	-676\\
74	-676\\
75	-677\\
76	-677\\
77	-677\\
78	-677\\
79	-677\\
80	-677\\
81	-677\\
82	-677\\
83	-677\\
84	-677\\
85	-677\\
86	-677\\
87	-677\\
88	-677\\
89	-677\\
90	-677\\
91	-678\\
92	-678\\
93	-678\\
94	-679\\
95	-679\\
96	-679\\
97	-679\\
98	-679\\
99	-679\\
100	-679\\
};
\addlegendentry{muscles, c = 0.05 s}


\addplot[area legend, draw=none, fill=red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	-657.148784887039\\
2	-664.878663431419\\
3	-670.181906016692\\
4	-674.717172244748\\
5	-675.418916846534\\
6	-677.459615309737\\
7	-677.939229668205\\
8	-677.939229668205\\
9	-681.329621517177\\
10	-686.622753609086\\
11	-686.489501143565\\
12	-686.202759682578\\
13	-691.884794044075\\
14	-691.669925054672\\
15	-691.546228776848\\
16	-691.546228776848\\
17	-691.346788087051\\
18	-691.346788087051\\
19	-691.346788087051\\
20	-691.43595756089\\
21	-691.423289448747\\
22	-691.423289448747\\
23	-691.411641736596\\
24	-691.408628753138\\
25	-691.435629877849\\
26	-691.435629877849\\
27	-701.72337695156\\
28	-701.721665326097\\
29	-701.721665326097\\
30	-701.845103838447\\
31	-701.853871742669\\
32	-701.853871742669\\
33	-701.853871742669\\
34	-701.853871742669\\
35	-701.853871742669\\
36	-701.853871742669\\
37	-703.061906749133\\
38	-703.061906749133\\
39	-707.866632356526\\
40	-707.86756792822\\
41	-707.877492597301\\
42	-707.877492597301\\
43	-707.877983312084\\
44	-707.878032403884\\
45	-707.878032403884\\
46	-707.879725045691\\
47	-707.879725045691\\
48	-707.882696174608\\
49	-707.884970684727\\
50	-707.884970684727\\
51	-707.884970684727\\
52	-707.885529342222\\
53	-707.885529342222\\
54	-707.885529342222\\
55	-707.885529342222\\
56	-707.885569752172\\
57	-707.885569752172\\
58	-707.888282806664\\
59	-707.888282806664\\
60	-707.888282806664\\
61	-707.888282806664\\
62	-708.559454854307\\
63	-708.559454854307\\
64	-708.807725384465\\
65	-708.807725384465\\
66	-708.808514663787\\
67	-708.808514663787\\
68	-708.808567479712\\
69	-708.808567479712\\
70	-708.80976714084\\
71	-708.810853362693\\
72	-708.810853362693\\
73	-708.8109172864\\
74	-708.8109172864\\
75	-708.8109172864\\
76	-708.8109172864\\
77	-708.811048566125\\
78	-708.811048566125\\
79	-708.811048566125\\
80	-708.811048566125\\
81	-708.811048566125\\
82	-708.920462879624\\
83	-708.920908838201\\
84	-708.959034684774\\
85	-708.959124132733\\
86	-709.30941193917\\
87	-709.30941193917\\
88	-709.309610628876\\
89	-709.309610628876\\
90	-709.309610628876\\
91	-709.309610628876\\
92	-709.309610628876\\
93	-709.309610628876\\
94	-709.309610628876\\
95	-709.309610628876\\
96	-709.309888189116\\
97	-709.309888189116\\
98	-709.30994835458\\
99	-709.30994835458\\
100	-709.30994835458\\
100	-678.285543535521\\
99	-678.285543535521\\
98	-678.285543535521\\
97	-678.284501283567\\
96	-678.284501283567\\
95	-678.280455912072\\
94	-678.280455912072\\
93	-678.280455912072\\
92	-678.280455912072\\
91	-678.280455912072\\
90	-678.280455912072\\
89	-678.280455912072\\
88	-678.280455912072\\
87	-678.277008434969\\
86	-678.277008434969\\
85	-678.340561274424\\
84	-678.338961429943\\
83	-678.34583443746\\
82	-678.337791904159\\
81	-678.357372188975\\
80	-678.357372188975\\
79	-678.357372188975\\
78	-678.357372188975\\
77	-678.357372188975\\
76	-678.355511447347\\
75	-678.355511447347\\
74	-678.355511447347\\
73	-678.355511447347\\
72	-678.354604237587\\
71	-678.354604237587\\
70	-678.334568434304\\
69	-678.311893027954\\
68	-678.311893027954\\
67	-678.310880901306\\
66	-678.310880901306\\
65	-678.299859521929\\
64	-678.299859521929\\
63	-678.310392912071\\
62	-678.310392912071\\
61	-678.410846111319\\
60	-678.410846111319\\
59	-678.410846111319\\
58	-678.410846111319\\
57	-678.370400571331\\
56	-678.370400571331\\
55	-678.369785631684\\
54	-678.369785631684\\
53	-678.369785631684\\
52	-678.369785631684\\
51	-678.361244854781\\
50	-678.361244854781\\
49	-678.361244854781\\
48	-678.325681632675\\
47	-678.277140363081\\
46	-678.277140363081\\
45	-678.248307938693\\
44	-678.248307938693\\
43	-678.247457912185\\
42	-678.238916734327\\
41	-678.238916734327\\
40	-678.044634838281\\
39	-678.023591225827\\
38	-678.433920308756\\
37	-678.433920308756\\
36	-678.296083762381\\
35	-678.296083762381\\
34	-678.296083762381\\
33	-678.296083762381\\
32	-678.296083762381\\
31	-678.296083762381\\
30	-677.575305301962\\
29	-677.560037099174\\
28	-677.560037099174\\
27	-677.436227935788\\
26	-674.646472569722\\
25	-674.646472569722\\
24	-673.773635998329\\
23	-673.594192361255\\
22	-673.267147898237\\
21	-673.267147898237\\
20	-673.03468158479\\
19	-672.662024239825\\
18	-672.662024239825\\
17	-672.662024239825\\
16	-670.608030504478\\
15	-670.608030504478\\
14	-669.800676066724\\
13	-668.383622448594\\
12	-664.007290144331\\
11	-661.383493260556\\
10	-658.97408280278\\
9	-660.010706396671\\
8	-659.424853559413\\
7	-659.424853559413\\
6	-657.989704682615\\
5	-652.38716203146\\
4	-646.893588089114\\
3	-628.747232346274\\
2	-622.892736314217\\
1	-606.659047560016\\
}--cycle;
\addplot [color=red]
  table[row sep=crcr]{%
1	-632\\
2	-644\\
3	-649\\
4	-661\\
5	-664\\
6	-668\\
7	-669\\
8	-669\\
9	-671\\
10	-673\\
11	-674\\
12	-675\\
13	-680\\
14	-681\\
15	-681\\
16	-681\\
17	-682\\
18	-682\\
19	-682\\
20	-682\\
21	-682\\
22	-682\\
23	-683\\
24	-683\\
25	-683\\
26	-683\\
27	-690\\
28	-690\\
29	-690\\
30	-690\\
31	-690\\
32	-690\\
33	-690\\
34	-690\\
35	-690\\
36	-690\\
37	-691\\
38	-691\\
39	-693\\
40	-693\\
41	-693\\
42	-693\\
43	-693\\
44	-693\\
45	-693\\
46	-693\\
47	-693\\
48	-693\\
49	-693\\
50	-693\\
51	-693\\
52	-693\\
53	-693\\
54	-693\\
55	-693\\
56	-693\\
57	-693\\
58	-693\\
59	-693\\
60	-693\\
61	-693\\
62	-693\\
63	-693\\
64	-694\\
65	-694\\
66	-694\\
67	-694\\
68	-694\\
69	-694\\
70	-694\\
71	-694\\
72	-694\\
73	-694\\
74	-694\\
75	-694\\
76	-694\\
77	-694\\
78	-694\\
79	-694\\
80	-694\\
81	-694\\
82	-694\\
83	-694\\
84	-694\\
85	-694\\
86	-694\\
87	-694\\
88	-694\\
89	-694\\
90	-694\\
91	-694\\
92	-694\\
93	-694\\
94	-694\\
95	-694\\
96	-694\\
97	-694\\
98	-694\\
99	-694\\
100	-694\\
};
\addlegendentry{muscles, c = 0.15 s}


\addplot[area legend, draw=none, fill=black!50!red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	-670.618786448199\\
2	-673.348999497823\\
3	-678.143880916682\\
4	-678.187043665748\\
5	-689.364992824725\\
6	-689.634839170512\\
7	-689.781271239989\\
8	-694.759403438864\\
9	-694.783636093308\\
10	-694.991636499651\\
11	-695.715070511022\\
12	-699.086294053486\\
13	-700.148704684562\\
14	-693.544212760033\\
15	-693.57482722592\\
16	-692.73195560023\\
17	-692.73195560023\\
18	-694.198919041487\\
19	-694.372407008789\\
20	-699.021159166991\\
21	-699.021755228225\\
22	-699.021755228225\\
23	-699.024080906782\\
24	-699.048871182569\\
25	-699.048871182569\\
26	-699.049905502265\\
27	-699.049905502265\\
28	-699.049905502265\\
29	-699.049905502265\\
30	-699.05030603697\\
31	-699.05030603697\\
32	-699.050317318349\\
33	-699.050861827023\\
34	-699.050861827023\\
35	-702.894352074502\\
36	-702.894352074502\\
37	-702.89436994356\\
38	-702.89436994356\\
39	-702.894874084202\\
40	-702.894874084202\\
41	-702.895039780615\\
42	-702.895039780615\\
43	-702.895039780615\\
44	-702.895039780615\\
45	-702.895039780615\\
46	-705.327338712104\\
47	-705.327338712104\\
48	-706.366188381995\\
49	-708.377744579185\\
50	-709.258136320611\\
51	-709.783697134209\\
52	-709.783783213705\\
53	-709.783783213705\\
54	-709.783783213705\\
55	-709.78388454749\\
56	-710.039969687649\\
57	-710.128447510374\\
58	-710.128488745489\\
59	-710.128499604729\\
60	-710.128537621725\\
61	-710.697094744343\\
62	-710.772106552249\\
63	-710.772109144829\\
64	-711.021644680441\\
65	-711.250192602834\\
66	-711.250192602834\\
67	-711.250192602834\\
68	-711.341611182019\\
69	-711.341611727299\\
70	-711.341611727299\\
71	-711.341611727299\\
72	-711.341611727299\\
73	-711.420612133138\\
74	-711.526143644282\\
75	-711.53553691617\\
76	-711.535538681411\\
77	-711.64582955585\\
78	-711.64582955585\\
79	-711.645832361668\\
80	-711.645837170385\\
81	-711.645847868143\\
82	-711.645847993477\\
83	-711.778389894102\\
84	-711.875951026123\\
85	-711.875951026123\\
86	-711.892121893532\\
87	-711.908163135476\\
88	-711.91667915141\\
89	-711.977587463561\\
90	-711.998667918553\\
91	-712.02051504189\\
92	-712.044271621306\\
93	-712.044271621306\\
94	-712.044271621306\\
95	-712.047565567102\\
96	-712.047565567102\\
97	-712.047568009688\\
98	-712.071840503767\\
99	-712.071840503767\\
100	-712.075300759627\\
100	-678.463973215626\\
99	-678.464500623778\\
98	-678.464500623778\\
97	-678.46826601539\\
96	-678.468225521043\\
95	-678.468225521043\\
94	-678.468737063385\\
93	-678.468737063385\\
92	-678.468737063385\\
91	-678.471125546719\\
90	-678.471834972916\\
89	-678.472414493162\\
88	-678.479620591077\\
87	-678.480948646059\\
86	-678.481456853369\\
85	-678.481834714757\\
84	-678.481834714757\\
83	-678.497029879694\\
82	-678.510550879748\\
81	-678.510548780788\\
80	-678.510369610014\\
79	-678.510289061382\\
78	-678.510242059515\\
77	-678.510242059515\\
76	-678.527196698787\\
75	-678.527166961317\\
74	-678.527381438407\\
73	-678.531012282827\\
72	-678.53344194599\\
71	-678.53344194599\\
70	-678.53344194599\\
69	-678.53344194599\\
68	-678.533432784216\\
67	-678.53485418656\\
66	-678.53485418656\\
65	-678.53485418656\\
64	-678.570423005016\\
63	-678.608621115493\\
62	-678.608576425174\\
61	-678.619619635761\\
60	-678.637038267774\\
59	-678.636385856095\\
58	-678.636199419088\\
57	-678.635491145156\\
56	-678.649897573738\\
55	-678.690847921859\\
54	-678.689068252172\\
53	-678.689068252172\\
52	-678.689068252172\\
51	-678.687553820966\\
50	-678.696211039362\\
49	-678.839687034058\\
48	-678.803891596459\\
47	-678.671808619447\\
46	-678.671808619447\\
45	-679.217212008354\\
44	-679.217212008354\\
43	-679.217212008354\\
42	-679.217212008354\\
41	-679.217212008354\\
40	-679.213891257366\\
39	-679.213891257366\\
38	-679.203680201908\\
37	-679.203680201908\\
36	-679.203315245608\\
35	-679.203315245608\\
34	-679.797509692673\\
33	-679.797509692673\\
32	-679.775575708955\\
31	-679.775102850504\\
30	-679.775102850504\\
29	-679.757758409673\\
28	-679.757758409673\\
27	-679.757758409673\\
26	-679.757758409673\\
25	-679.706490219082\\
24	-679.706490219082\\
23	-679.574475540203\\
22	-679.458868640983\\
21	-679.458868640983\\
20	-679.414780516121\\
19	-678.50667966327\\
18	-677.815934100951\\
17	-673.865904341409\\
16	-673.865904341409\\
15	-667.73877401332\\
14	-667.700184557483\\
13	-644.498184540451\\
12	-640.702697735693\\
11	-640.662041680177\\
10	-639.825711616906\\
9	-639.696353523064\\
8	-638.703869073679\\
7	-635.300937020742\\
6	-634.829872369035\\
5	-634.685157767441\\
4	-629.066954001499\\
3	-613.758788542872\\
2	-596.125649685636\\
1	-585.036788306048\\
}--cycle;
\addplot [color=black!50!red]
  table[row sep=crcr]{%
1	-628\\
2	-635\\
3	-646\\
4	-654\\
5	-662\\
6	-662\\
7	-663\\
8	-667\\
9	-667\\
10	-667\\
11	-668\\
12	-670\\
13	-672\\
14	-681\\
15	-681\\
16	-683\\
17	-683\\
18	-686\\
19	-686\\
20	-689\\
21	-689\\
22	-689\\
23	-689\\
24	-689\\
25	-689\\
26	-689\\
27	-689\\
28	-689\\
29	-689\\
30	-689\\
31	-689\\
32	-689\\
33	-689\\
34	-689\\
35	-691\\
36	-691\\
37	-691\\
38	-691\\
39	-691\\
40	-691\\
41	-691\\
42	-691\\
43	-691\\
44	-691\\
45	-691\\
46	-692\\
47	-692\\
48	-693\\
49	-694\\
50	-694\\
51	-694\\
52	-694\\
53	-694\\
54	-694\\
55	-694\\
56	-694\\
57	-694\\
58	-694\\
59	-694\\
60	-694\\
61	-695\\
62	-695\\
63	-695\\
64	-695\\
65	-695\\
66	-695\\
67	-695\\
68	-695\\
69	-695\\
70	-695\\
71	-695\\
72	-695\\
73	-695\\
74	-695\\
75	-695\\
76	-695\\
77	-695\\
78	-695\\
79	-695\\
80	-695\\
81	-695\\
82	-695\\
83	-695\\
84	-695\\
85	-695\\
86	-695\\
87	-695\\
88	-695\\
89	-695\\
90	-695\\
91	-695\\
92	-695\\
93	-695\\
94	-695\\
95	-695\\
96	-695\\
97	-695\\
98	-695\\
99	-695\\
100	-695\\
};
\addlegendentry{muscles, c = 0.3 s}
\legend{}
\end{axis}



==> figures/dataefficiency_cost_pointreaching.tex <==
\begin{axis}[%
name =ax1,
scaled y ticks=base 10:\Factor,
xlabel near ticks, ylabel near ticks,
every y tick scale label/.style={at={(yticklabel* cs:1.03,0cm)},anchor=near yticklabel},
title style={at={(0.5,0.93)}},
width=0.631\figW,
height=\figH,
scale only axis,
xmin=0,
xmax=100,
xtick={  0,  20,  40,  60,  80, 100},
xlabel style={font=\color{white!15!black}},
xlabel={generations},
ymin=0,
ymax=5000,
ylabel style={font=\color{white!15!black}},
ylabel={cost},
axis background/.style={fill=white},
title={(a) smooth point-reaching (OC)},
legend style={at={(1.03,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]

\addplot[area legend, draw=none, fill=mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	5170.03227375288\\
2	3643.14937266689\\
3	3013.88527938524\\
4	2783.06302901892\\
5	2549.27558055067\\
6	2205.76574250587\\
7	1736.53564003158\\
8	2025.07266339973\\
9	1933.88406465493\\
10	1862.31313228524\\
11	1813.45295146484\\
12	1535.58352075129\\
13	1419.20393942324\\
14	1302.38076622633\\
15	1260.28962879832\\
16	1216.52422340768\\
17	1216.52422340768\\
18	1140.17085108422\\
19	1026.54299533562\\
20	1026.54299533562\\
21	989.444818262883\\
22	964.4433972427\\
23	1011.36789330552\\
24	1028.30328882717\\
25	995.364425543746\\
26	995.364425543746\\
27	861.221345909889\\
28	823.945474588184\\
29	782.86172469087\\
30	782.86172469087\\
31	672.346402142427\\
32	680.882151120109\\
33	668.05050271671\\
34	647.775849970312\\
35	661.863514329305\\
36	673.36497392303\\
37	650.899122928831\\
38	566.681462789805\\
39	565.824814884483\\
40	565.824814884483\\
41	581.248166400597\\
42	589.111342550479\\
43	568.737250729501\\
44	581.285834479515\\
45	624.045399513396\\
46	605.210537505279\\
47	605.210537505279\\
48	605.210537505279\\
49	575.082734050564\\
50	575.082734050564\\
51	522.021632429589\\
52	494.714663446711\\
53	492.470394688581\\
54	487.464935565014\\
55	450.039038431918\\
56	438.747085867178\\
57	433.1179991205\\
58	422.485130389727\\
59	417.929148202331\\
60	431.177789871439\\
61	458.839303277193\\
62	458.839303277193\\
63	460.71701090311\\
64	460.71701090311\\
65	463.58723210839\\
66	516.538182005144\\
67	475.511449975345\\
68	475.511449975345\\
69	475.511449975345\\
70	416.417408383608\\
71	403.575941395932\\
72	399.111668085704\\
73	384.812067099911\\
74	417.763251132279\\
75	408.163147211992\\
76	408.163147211992\\
77	393.830605810589\\
78	413.536109632479\\
79	413.536109632479\\
80	413.536109632479\\
81	408.284445260311\\
82	389.082529534418\\
83	388.288298937817\\
84	417.8818916726\\
85	417.8818916726\\
86	417.636749850663\\
87	397.310580403872\\
88	397.192368692042\\
89	393.936863880994\\
90	413.376581858168\\
91	413.376581858168\\
92	405.190150470063\\
93	433.503949282877\\
94	433.503949282877\\
95	430.256629385682\\
96	430.256629385682\\
97	430.247981309142\\
98	424.62876209212\\
99	416.460492542109\\
100	431.15899699201\\
100	1197.84165586544\\
99	1257.97137573982\\
98	1260.58849430647\\
97	1262.54808321891\\
96	1262.55085180562\\
95	1262.55085180562\\
94	1263.61816175387\\
93	1263.61816175387\\
92	1390.56130791087\\
91	1393.21489136149\\
90	1393.21489136149\\
89	1451.54191816615\\
88	1452.71548167627\\
87	1452.75223077959\\
86	1459.81164653627\\
85	1459.90206577437\\
84	1459.90206577437\\
83	1549.50567257604\\
82	1549.7937327662\\
81	1556.50279462597\\
80	1558.54644637074\\
79	1558.54644637074\\
78	1558.54644637074\\
77	1644.4319506761\\
76	1650.38071209823\\
75	1650.38071209823\\
74	1653.82364503072\\
73	1752.97187263258\\
72	1757.42776226991\\
71	1759.15794742782\\
70	1764.57193898686\\
69	1785.45032960566\\
68	1785.45032960566\\
67	1785.45032960566\\
66	1796.39057309957\\
65	1971.64672289783\\
64	1980.26674830263\\
63	1980.26674830263\\
62	1985.90591930752\\
61	1985.90591930752\\
60	2090.36077908667\\
59	2130.15679684688\\
58	2131.78529674959\\
57	2136.09402329121\\
56	2137.85312466122\\
55	2142.7685853537\\
54	2153.76840739466\\
53	2155.19037026667\\
52	2155.95160872277\\
51	2165.13087277362\\
50	2181.52532096602\\
49	2181.52532096602\\
48	2192.40522106257\\
47	2192.40522106257\\
46	2192.40522106257\\
45	2200.65619943934\\
44	2486.53412169753\\
43	2527.30643768789\\
42	2577.68449966283\\
41	2601.3313908603\\
40	2647.7088956018\\
39	2647.7088956018\\
38	2648.05186856348\\
37	2675.28029988324\\
36	2683.6543589496\\
35	2718.2407792816\\
34	2774.1504087651\\
33	2782.95884486911\\
32	2786.4183029955\\
31	2812.11423213712\\
30	2853.46061567132\\
29	2853.46061567132\\
28	2867.26835056141\\
27	2881.38937961344\\
26	2918.27442389441\\
25	2918.27442389441\\
24	2932.83070250423\\
23	2983.93259459486\\
22	3125.42726114772\\
21	3134.70195505357\\
20	3150.21711913398\\
19	3150.21711913398\\
18	3210.1664588243\\
17	3225.86509212053\\
16	3225.86509212053\\
15	3233.50488148559\\
14	3244.18632076094\\
13	3315.37838555635\\
12	3395.02896668288\\
11	3502.76422321806\\
10	3911.99422186422\\
9	3948.92765822696\\
8	3999.63463916276\\
7	4993.00451050724\\
6	5242.57856212147\\
5	5319.98328006031\\
4	5374.79535934662\\
3	5486.10505602762\\
2	5970.80733529359\\
1	7826.03005114544\\
}--cycle;
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	6498\\
2	4807\\
3	4250\\
4	4079\\
5	3935\\
6	3724\\
7	3365\\
8	3012\\
9	2941\\
10	2887\\
11	2658\\
12	2465\\
13	2367\\
14	2273\\
15	2247\\
16	2221\\
17	2221\\
18	2175\\
19	2088\\
20	2088\\
21	2062\\
22	2045\\
23	1998\\
24	1981\\
25	1957\\
26	1957\\
27	1871\\
28	1846\\
29	1818\\
30	1818\\
31	1742\\
32	1734\\
33	1726\\
34	1711\\
35	1690\\
36	1679\\
37	1663\\
38	1607\\
39	1607\\
40	1607\\
41	1591\\
42	1583\\
43	1548\\
44	1534\\
45	1412\\
46	1399\\
47	1399\\
48	1399\\
49	1378\\
50	1378\\
51	1344\\
52	1325\\
53	1324\\
54	1321\\
55	1296\\
56	1288\\
57	1285\\
58	1277\\
59	1274\\
60	1261\\
61	1222\\
62	1222\\
63	1220\\
64	1220\\
65	1218\\
66	1156\\
67	1130\\
68	1130\\
69	1130\\
70	1090\\
71	1081\\
72	1078\\
73	1069\\
74	1036\\
75	1029\\
76	1029\\
77	1019\\
78	986\\
79	986\\
80	986\\
81	982\\
82	969\\
83	969\\
84	939\\
85	939\\
86	939\\
87	925\\
88	925\\
89	923\\
90	903\\
91	903\\
92	898\\
93	849\\
94	849\\
95	846\\
96	846\\
97	846\\
98	843\\
99	837\\
100	815\\
};
\addlegendentry{torques, c = 0.05 s}


\addplot[area legend, draw=none, fill=blue!50!mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	661.289616605163\\
2	977.246670931292\\
3	944.509069720273\\
4	797.088050841908\\
5	756.338211651292\\
6	756.338211651292\\
7	756.338211651292\\
8	713.338547394196\\
9	713.338547394196\\
10	732.614609950776\\
11	715.301703223654\\
12	715.301703223654\\
13	702.04431388911\\
14	684.770629381988\\
15	684.770629381988\\
16	685.317806528589\\
17	685.296116283732\\
18	662.233568320906\\
19	638.193654648692\\
20	633.014868592728\\
21	606.912306113397\\
22	584.742583739849\\
23	569.358785490491\\
24	566.87175227992\\
25	567.543842129013\\
26	567.543842129013\\
27	559.377762114584\\
28	554.973517325879\\
29	549.430901562195\\
30	545.424750257415\\
31	535.130794937847\\
32	528.045998842465\\
33	499.541660773917\\
34	489.238779114913\\
35	489.238779114913\\
36	493.922469729725\\
37	487.667479342535\\
38	486.397742459972\\
39	482.25104375025\\
40	479.047266542927\\
41	473.912832585759\\
42	489.806071925413\\
43	485.994712020022\\
44	469.405351037119\\
45	466.924573839571\\
46	461.895387821864\\
47	458.641032793744\\
48	452.323403061573\\
49	466.297711812363\\
50	450.639343158452\\
51	444.714664229167\\
52	439.839705700187\\
53	434.163446939647\\
54	389.77671703227\\
55	389.43363113756\\
56	389.744117920342\\
57	379.565692149799\\
58	342.279714205261\\
59	341.263581062384\\
60	329.105281336259\\
61	329.105281336259\\
62	324.465824693138\\
63	319.731088165226\\
64	321.711910102816\\
65	306.460308832485\\
66	304.988682722165\\
67	297.841720067647\\
68	298.091739237359\\
69	295.810940046274\\
70	295.964379056398\\
71	292.467723135313\\
72	291.961612840659\\
73	289.398128391543\\
74	288.918906132034\\
75	289.957864677694\\
76	287.262161123179\\
77	287.949082455263\\
78	288.004801819658\\
79	288.785248081413\\
80	287.699492653192\\
81	282.961945109615\\
82	281.889179708085\\
83	278.498393780664\\
84	278.57793028674\\
85	277.977567743912\\
86	275.1564070434\\
87	275.584023680347\\
88	273.586872250078\\
89	274.910214462076\\
90	274.910214462076\\
91	281.775586771367\\
92	279.425920195026\\
93	279.015757859746\\
94	278.635098154042\\
95	277.971443148872\\
96	277.969019823314\\
97	281.596297494516\\
98	284.819534000973\\
99	286.920146941799\\
100	286.580071340258\\
100	317.462913720376\\
99	317.556895364824\\
98	325.16357294226\\
97	348.676930738359\\
96	359.794350418751\\
95	359.795300566413\\
94	359.928093064211\\
93	360.067454042013\\
92	360.23173629622\\
91	369.587352887379\\
90	390.57323362271\\
89	390.57323362271\\
88	396.609671945447\\
87	397.406504780326\\
86	401.918404220232\\
85	403.077125648195\\
84	404.587142917951\\
83	404.830091701385\\
82	405.612187192105\\
81	406.030556139149\\
80	408.999185946104\\
79	417.602487608854\\
78	420.051272581233\\
77	420.225884117689\\
76	422.376279145479\\
75	423.226866337677\\
74	426.956258223376\\
73	427.02582965994\\
72	431.633091881714\\
71	431.988604231846\\
70	434.515388717464\\
69	436.130594478499\\
68	436.397404468093\\
67	437.183445970326\\
66	445.230281212171\\
65	445.91758916621\\
64	453.360502221058\\
63	469.048411168029\\
62	474.655871765328\\
61	481.322114569626\\
60	481.322114569626\\
59	503.941235621222\\
58	506.985183138122\\
57	534.127543197494\\
56	542.435333706015\\
55	546.133272723632\\
54	546.864736280153\\
53	553.79549207305\\
52	563.129994386468\\
51	568.262945993505\\
50	588.867367345949\\
49	588.071885361522\\
48	672.472730837903\\
47	682.582472158894\\
46	757.754189750951\\
45	759.435735920918\\
44	763.559698148652\\
43	765.370703547091\\
42	767.28504273211\\
41	820.234724090187\\
40	850.267694936585\\
39	850.415459155712\\
38	851.784669890548\\
37	856.111071147276\\
36	856.446090931515\\
35	871.217185250978\\
34	871.217185250978\\
33	873.995361148473\\
32	921.695713159492\\
31	921.763689415109\\
30	956.176790981338\\
29	966.964219813359\\
28	990.055513813827\\
27	990.368403938458\\
26	1003.38219992896\\
25	1003.38219992896\\
24	1005.76929383791\\
23	1006.05697110472\\
22	1010.57962817735\\
21	1010.65809201974\\
20	1022.35374868098\\
19	1022.91042944751\\
18	1026.62994856721\\
17	1034.13282897698\\
16	1034.15667088096\\
15	1075.64058534475\\
14	1075.64058534475\\
13	1075.75650922861\\
12	1094.62157339565\\
11	1094.62157339565\\
10	1322.2349201139\\
9	1505.05801564296\\
8	1505.05801564296\\
7	1596.18568083774\\
6	1596.18568083774\\
5	1596.18568083774\\
4	1615.70612566641\\
3	2324.15102345855\\
2	3680.9530728926\\
1	6491.36035484248\\
}--cycle;
\addplot [color=blue!50!mycolor1]
  table[row sep=crcr]{%
1	3576\\
2	2329\\
3	1634\\
4	1206\\
5	1176\\
6	1176\\
7	1176\\
8	1109\\
9	1109\\
10	1027\\
11	905\\
12	905\\
13	889\\
14	880\\
15	880\\
16	860\\
17	860\\
18	844\\
19	831\\
20	828\\
21	809\\
22	798\\
23	788\\
24	786\\
25	785\\
26	785\\
27	775\\
28	773\\
29	758\\
30	751\\
31	728\\
32	725\\
33	687\\
34	680\\
35	680\\
36	675\\
37	672\\
38	669\\
39	666\\
40	665\\
41	647\\
42	629\\
43	626\\
44	616\\
45	613\\
46	610\\
47	571\\
48	562\\
49	527\\
50	520\\
51	506\\
52	501\\
53	494\\
54	468\\
55	468\\
56	466\\
57	457\\
58	425\\
59	423\\
60	405\\
61	405\\
62	400\\
63	394\\
64	388\\
65	376\\
66	375\\
67	368\\
68	367\\
69	366\\
70	365\\
71	362\\
72	362\\
73	358\\
74	358\\
75	357\\
76	355\\
77	354\\
78	354\\
79	353\\
80	348\\
81	344\\
82	344\\
83	342\\
84	342\\
85	341\\
86	339\\
87	336\\
88	335\\
89	333\\
90	333\\
91	326\\
92	320\\
93	320\\
94	319\\
95	319\\
96	319\\
97	315\\
98	305\\
99	302\\
100	302\\
};
\addlegendentry{torques, c = 0.15 s}


\addplot[area legend, draw=none, fill=blue, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1083.94164841792\\
2	794.545435134731\\
3	704.192255409083\\
4	701.134326487207\\
5	694.808452919495\\
6	652.209499657079\\
7	648.888903551531\\
8	656.45155232808\\
9	656.920038632598\\
10	649.40664047447\\
11	649.40664047447\\
12	645.434130799015\\
13	645.434130799015\\
14	645.699902211598\\
15	645.542333450434\\
16	645.542333450434\\
17	636.415999106652\\
18	637.603189663503\\
19	637.778933691178\\
20	636.635836780502\\
21	614.495885603808\\
22	614.107635046692\\
23	572.580531743537\\
24	555.324258364133\\
25	536.071943719922\\
26	536.071943719922\\
27	535.336137312279\\
28	526.774258154144\\
29	514.285240413715\\
30	502.249790877919\\
31	502.249790877919\\
32	500.236038119568\\
33	479.344870023028\\
34	454.021923366868\\
35	455.237778680672\\
36	451.012544814158\\
37	450.710770075302\\
38	449.941725825424\\
39	450.413910826878\\
40	447.926388059455\\
41	434.272252263923\\
42	427.015894526178\\
43	426.387885160478\\
44	432.339144158234\\
45	432.029235590877\\
46	429.779197357935\\
47	424.231140827622\\
48	423.969410390353\\
49	423.969410390353\\
50	423.914239015292\\
51	421.37221510034\\
52	418.876497373984\\
53	416.192693428237\\
54	410.405103097919\\
55	409.966573650248\\
56	407.441313763792\\
57	402.385715395574\\
58	395.372603645508\\
59	394.961683309964\\
60	394.547491419885\\
61	394.336376450156\\
62	388.698095262638\\
63	388.50793500901\\
64	388.482677424752\\
65	388.478373721849\\
66	388.393843902907\\
67	388.318082207792\\
68	388.318082207792\\
69	388.231559875928\\
70	386.9228618396\\
71	385.966217080338\\
72	385.935400238512\\
73	385.895337634896\\
74	384.393837711543\\
75	381.68983822879\\
76	381.68743000909\\
77	381.575900482241\\
78	381.561644666656\\
79	381.519729874943\\
80	380.613914828196\\
81	380.02435361736\\
82	379.308840419949\\
83	379.011322748535\\
84	378.999782004617\\
85	378.999085191276\\
86	378.649916635589\\
87	378.581360010999\\
88	378.581360010999\\
89	378.484445050155\\
90	378.479237041359\\
91	378.478819593061\\
92	378.408931554198\\
93	378.391918974319\\
94	378.284118355776\\
95	378.186739329333\\
96	378.186739329333\\
97	378.178320436045\\
98	378.178320436045\\
99	378.172674021632\\
100	378.155784640731\\
100	466.869762461439\\
99	466.868974866717\\
98	466.902174999279\\
97	466.902174999279\\
96	466.931627562019\\
95	466.931627562019\\
94	466.921870728478\\
93	466.930828323438\\
92	466.936404268747\\
91	466.929550821431\\
90	466.929507280735\\
89	466.982290626576\\
88	467.023049044693\\
87	467.023049044693\\
86	467.016439061075\\
85	466.983549807674\\
84	466.990458006029\\
83	467.109115724308\\
82	467.252465621823\\
81	467.191270294799\\
80	467.145337579885\\
79	467.083068623541\\
78	467.077432366927\\
77	467.223219271684\\
76	467.320123743087\\
75	467.345179076365\\
74	467.428115916062\\
73	467.821871928179\\
72	467.87042884477\\
71	467.865112595187\\
70	468.378195083874\\
69	468.40740774632\\
68	468.488377925865\\
67	468.488377925865\\
66	469.182100103753\\
65	470.163152307302\\
64	470.189892572444\\
63	470.47930675546\\
62	473.47906893478\\
61	473.732402600548\\
60	476.420549491272\\
59	476.327097226378\\
58	476.489479051228\\
57	479.35959615439\\
56	483.19165356278\\
55	486.747300965976\\
54	490.473817954474\\
53	502.652926565333\\
52	502.582830860023\\
51	508.298520830002\\
50	507.748011685474\\
49	507.942358863781\\
48	507.942358863781\\
47	508.798787017036\\
46	516.896462757442\\
45	516.285607989744\\
44	516.202348079164\\
43	556.935876311467\\
42	557.649180713919\\
41	558.043721890984\\
40	565.202346335247\\
39	567.859633281839\\
38	570.436632407033\\
37	570.326255688148\\
36	570.771422077133\\
35	616.422455480104\\
34	627.572379348708\\
33	638.816652783296\\
32	646.677998694583\\
31	650.74489237834\\
30	650.74489237834\\
29	653.579133632443\\
28	650.968912436178\\
27	670.113057525592\\
26	669.954442762706\\
25	669.954442762706\\
24	678.720269805939\\
23	673.437200496022\\
22	663.06998283479\\
21	667.775571933131\\
20	678.25224407229\\
19	690.962253191531\\
18	692.343556652675\\
17	699.187313669683\\
16	702.860691206039\\
15	702.860691206039\\
14	709.895225790493\\
13	712.652724679152\\
12	712.652724679152\\
11	714.091371662041\\
10	714.091371662041\\
9	724.854655488439\\
8	741.628495624467\\
7	811.155073642865\\
6	820.179777899462\\
5	826.308457721423\\
4	1021.05984776962\\
3	1062.36690407385\\
2	1628.79830806761\\
1	2046.4385193762\\
}--cycle;
\addplot [color=blue]
  table[row sep=crcr]{%
1	1565\\
2	1212\\
3	883\\
4	861\\
5	761\\
6	736\\
7	730\\
8	699\\
9	691\\
10	682\\
11	682\\
12	679\\
13	679\\
14	678\\
15	674\\
16	674\\
17	668\\
18	665\\
19	664\\
20	657\\
21	641\\
22	639\\
23	623\\
24	617\\
25	603\\
26	603\\
27	603\\
28	589\\
29	584\\
30	576\\
31	576\\
32	573\\
33	559\\
34	541\\
35	536\\
36	511\\
37	511\\
38	510\\
39	509\\
40	507\\
41	496\\
42	492\\
43	492\\
44	474\\
45	474\\
46	473\\
47	467\\
48	466\\
49	466\\
50	466\\
51	465\\
52	461\\
53	459\\
54	450\\
55	448\\
56	445\\
57	441\\
58	436\\
59	436\\
60	435\\
61	434\\
62	431\\
63	429\\
64	429\\
65	429\\
66	429\\
67	428\\
68	428\\
69	428\\
70	428\\
71	427\\
72	427\\
73	427\\
74	426\\
75	425\\
76	425\\
77	424\\
78	424\\
79	424\\
80	424\\
81	424\\
82	423\\
83	423\\
84	423\\
85	423\\
86	423\\
87	423\\
88	423\\
89	423\\
90	423\\
91	423\\
92	423\\
93	423\\
94	423\\
95	423\\
96	423\\
97	423\\
98	423\\
99	423\\
100	423\\
};
\addlegendentry{torques, c = 0.3 s}


\addplot[area legend, draw=none, fill=orange, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	891.813524513513\\
2	819.409843551937\\
3	766.927512436109\\
4	681.790680263488\\
5	649.033795495181\\
6	592.132559512566\\
7	484.435877900163\\
8	472.088364883036\\
9	443.342397611295\\
10	426.391575269901\\
11	402.090747821125\\
12	385.924804431583\\
13	372.144984684559\\
14	359.458853051741\\
15	354.447215788007\\
16	347.479898170432\\
17	346.02794573735\\
18	336.158708629221\\
19	334.376507703783\\
20	329.870870084657\\
21	330.012487688409\\
22	329.471144850914\\
23	329.471144850914\\
24	328.405149708682\\
25	326.029065632327\\
26	323.784277314758\\
27	322.755013130461\\
28	321.875611921904\\
29	322.473074096898\\
30	321.665435072793\\
31	321.896634485784\\
32	321.621919715792\\
33	320.982561993955\\
34	320.982561993955\\
35	319.493867874908\\
36	318.652385910739\\
37	318.808018437192\\
38	318.808018437192\\
39	320.76094240268\\
40	319.860838462048\\
41	319.912091285084\\
42	320.07549917476\\
43	320.07549917476\\
44	320.07549917476\\
45	318.08163196237\\
46	318.08163196237\\
47	317.770448196243\\
48	317.291240761116\\
49	317.291240761116\\
50	316.171163054462\\
51	316.171163054462\\
52	316.171163054462\\
53	316.890828061565\\
54	315.960066347777\\
55	315.710672576696\\
56	315.710672576696\\
57	313.161472150081\\
58	312.509780109113\\
59	312.080489574408\\
60	311.585451287641\\
61	311.682414500046\\
62	311.682414500046\\
63	311.682414500046\\
64	310.544425483001\\
65	310.544425483001\\
66	310.246696193509\\
67	309.74268026204\\
68	309.74268026204\\
69	309.74268026204\\
70	309.739933175232\\
71	308.618275932413\\
72	308.618275932413\\
73	306.975277029445\\
74	306.975277029445\\
75	306.173589656686\\
76	306.562741648895\\
77	305.664372923498\\
78	305.664372923498\\
79	305.664372923498\\
80	305.640874469217\\
81	305.77782594072\\
82	305.77782594072\\
83	305.77782594072\\
84	305.880275684867\\
85	305.880275684867\\
86	305.579299824209\\
87	305.051837259119\\
88	304.551919087331\\
89	304.583425846264\\
90	304.583425846264\\
91	304.583425846264\\
92	304.583425846264\\
93	304.573778178\\
94	304.411291306328\\
95	304.411291306328\\
96	304.411291306328\\
97	304.411291306328\\
98	304.411291306328\\
99	304.411291306328\\
100	304.257610128137\\
100	309.523233804604\\
99	310.392556236287\\
98	310.392556236287\\
97	310.392556236287\\
96	310.392556236287\\
95	310.392556236287\\
94	310.392556236287\\
93	311.409361324253\\
92	311.578967880502\\
91	311.578967880502\\
90	311.578967880502\\
89	311.578967880502\\
88	312.35798113371\\
87	312.478676873282\\
86	312.807456768638\\
85	314.563128518639\\
84	314.563128518639\\
83	315.513123869668\\
82	315.513123869668\\
81	315.513123869668\\
80	316.308225496201\\
79	316.367888818264\\
78	316.367888818264\\
77	316.367888818264\\
76	316.177295979946\\
75	317.782385189032\\
74	318.633615309913\\
73	318.633615309913\\
72	321.168133906284\\
71	321.168133906284\\
70	321.714134862103\\
69	321.714234646203\\
68	321.714234646203\\
67	321.714234646203\\
66	322.348366315542\\
65	322.308677800564\\
64	322.308677800564\\
63	322.366906446803\\
62	322.366906446803\\
61	322.366906446803\\
60	323.3095213827\\
59	324.402983224711\\
58	329.43727699767\\
57	329.566591977709\\
56	329.539424948941\\
55	329.539424948941\\
54	329.555785881415\\
53	329.717094672125\\
52	332.929442762828\\
51	332.929442762828\\
50	332.929442762828\\
49	334.766872048467\\
48	334.766872048467\\
47	334.864782639788\\
46	334.953214384808\\
45	334.953214384808\\
44	339.141598778996\\
43	339.141598778996\\
42	339.141598778996\\
41	340.317282215621\\
40	340.486070378614\\
39	340.691905353095\\
38	346.90083866664\\
37	346.90083866664\\
36	347.386392996367\\
35	348.179239330056\\
34	351.944118040282\\
33	351.944118040282\\
32	353.560847305629\\
31	356.711858038168\\
30	360.366751381295\\
29	360.566123651921\\
28	366.714319688962\\
27	366.70049718591\\
26	366.845950420562\\
25	367.044018866555\\
24	369.097458938452\\
23	369.538389581555\\
22	369.538389581555\\
21	369.828437691072\\
20	372.882659133978\\
19	372.752109694634\\
18	381.884984204696\\
17	404.386836655814\\
16	414.595925807957\\
15	426.023966372821\\
14	441.544066109695\\
13	451.289982961733\\
12	462.47911059179\\
11	497.017208028262\\
10	535.203306088386\\
9	564.393761209783\\
8	570.317601196132\\
7	652.606919628772\\
6	673.567520911265\\
5	709.307959696982\\
4	798.762127891694\\
3	871.949668402133\\
2	957.603899121031\\
1	1021.93461883201\\
}--cycle;
\addplot [color=orange]
  table[row sep=crcr]{%
1	957\\
2	889\\
3	819\\
4	740\\
5	679\\
6	633\\
7	569\\
8	521\\
9	504\\
10	481\\
11	450\\
12	424\\
13	412\\
14	401\\
15	390\\
16	381\\
17	375\\
18	359\\
19	354\\
20	351\\
21	350\\
22	350\\
23	350\\
24	349\\
25	347\\
26	345\\
27	345\\
28	344\\
29	342\\
30	341\\
31	339\\
32	338\\
33	336\\
34	336\\
35	334\\
36	333\\
37	333\\
38	333\\
39	331\\
40	330\\
41	330\\
42	330\\
43	330\\
44	330\\
45	327\\
46	327\\
47	326\\
48	326\\
49	326\\
50	325\\
51	325\\
52	325\\
53	323\\
54	323\\
55	323\\
56	323\\
57	321\\
58	321\\
59	318\\
60	317\\
61	317\\
62	317\\
63	317\\
64	316\\
65	316\\
66	316\\
67	316\\
68	316\\
69	316\\
70	316\\
71	315\\
72	315\\
73	313\\
74	313\\
75	312\\
76	311\\
77	311\\
78	311\\
79	311\\
80	311\\
81	311\\
82	311\\
83	311\\
84	310\\
85	310\\
86	309\\
87	309\\
88	308\\
89	308\\
90	308\\
91	308\\
92	308\\
93	308\\
94	307\\
95	307\\
96	307\\
97	307\\
98	307\\
99	307\\
100	307\\
};
\addlegendentry{muscles, c = 0.05 s}


\addplot[area legend, draw=none, fill=red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	552.682241146824\\
2	532.195486728073\\
3	494.982852784691\\
4	458.861138435318\\
5	431.997275946587\\
6	408.396995591456\\
7	387.742175484299\\
8	370.309003353631\\
9	370.545132782615\\
10	362.592665080047\\
11	359.049052768056\\
12	340.88791327695\\
13	334.886017540123\\
14	332.314620106687\\
15	330.910297188282\\
16	330.910297188282\\
17	326.180634119869\\
18	321.805250128372\\
19	322.760608780375\\
20	317.313798359896\\
21	314.943710728092\\
22	314.435600535633\\
23	313.271744527597\\
24	312.58056132806\\
25	307.93361519106\\
26	307.892618440559\\
27	307.628295892923\\
28	307.628295892923\\
29	307.628295892923\\
30	305.829809290952\\
31	305.829809290952\\
32	306.427226186994\\
33	305.290178087892\\
34	302.86729123274\\
35	301.836009686807\\
36	301.358685655954\\
37	298.639750364164\\
38	297.088710303267\\
39	296.666613933378\\
40	296.666613933378\\
41	296.666613933378\\
42	296.666613933378\\
43	295.922884928342\\
44	295.922884928342\\
45	295.922884928342\\
46	298.904607297776\\
47	298.635085760101\\
48	298.635085760101\\
49	297.458750244978\\
50	297.409053523348\\
51	297.409053523348\\
52	297.274088662947\\
53	296.432088012206\\
54	295.895319641192\\
55	295.966679079473\\
56	295.82187808108\\
57	295.82187808108\\
58	295.82187808108\\
59	295.730491087913\\
60	295.930767620448\\
61	295.930767620448\\
62	295.021567464205\\
63	293.849212335177\\
64	293.849212335177\\
65	293.431147503788\\
66	293.431147503788\\
67	293.431147503788\\
68	292.870840882251\\
69	292.870840882251\\
70	292.870840882251\\
71	293.882471050094\\
72	293.762743690591\\
73	293.762743690591\\
74	293.614047478722\\
75	293.614047478722\\
76	293.614047478722\\
77	293.614047478722\\
78	293.583204800804\\
79	293.145118731767\\
80	293.0431027717\\
81	292.832716719971\\
82	293.03983837787\\
83	293.255007749399\\
84	293.255007749399\\
85	293.255007749399\\
86	292.908873796951\\
87	293.746636735984\\
88	293.399802072843\\
89	293.65941124007\\
90	293.65941124007\\
91	293.503528032247\\
92	293.521369224434\\
93	293.479526562105\\
94	293.479526562105\\
95	293.479526562105\\
96	293.378389847049\\
97	293.201098692096\\
98	293.201098692096\\
99	293.201098692096\\
100	293.208612584878\\
100	299.285750487676\\
99	299.343445420326\\
98	299.343445420326\\
97	299.343445420326\\
96	299.361803134541\\
95	299.431758787246\\
94	299.431758787246\\
93	299.431758787246\\
92	299.451103280379\\
91	299.506681995384\\
90	299.546107857017\\
89	299.546107857017\\
88	300.404192729822\\
87	300.601863677189\\
86	303.309530787653\\
85	303.449296759838\\
84	303.449296759838\\
83	303.449296759838\\
82	304.110987259452\\
81	304.975048644508\\
80	305.004153976787\\
79	305.026975227037\\
78	305.202122411977\\
77	305.206083655068\\
76	305.206083655068\\
75	305.206083655068\\
74	305.206083655068\\
73	305.255049799549\\
72	305.255049799549\\
71	305.301043688151\\
70	308.377474589691\\
69	308.377474589691\\
68	308.377474589691\\
67	308.656411476383\\
66	308.656411476383\\
65	308.656411476383\\
64	308.839302789658\\
63	308.839302789658\\
62	309.322895227011\\
61	309.792279942395\\
60	309.792279942395\\
59	311.9418471586\\
58	314.941545698064\\
57	314.941545698064\\
56	314.941545698064\\
55	315.000080653988\\
54	316.474834998047\\
53	316.809738331155\\
52	316.917644447434\\
51	317.016328129872\\
50	317.016328129872\\
49	317.022703541049\\
48	317.356134907148\\
47	317.356134907148\\
46	317.411298747907\\
45	328.602764805711\\
44	328.602764805711\\
43	328.602764805711\\
42	328.924306078856\\
41	328.924306078856\\
40	328.924306078856\\
39	328.924306078856\\
38	329.205093740657\\
37	329.71848713306\\
36	330.532495137564\\
35	330.741080513088\\
34	331.161791898278\\
33	331.855676971329\\
32	332.147620707169\\
31	337.038802431629\\
30	337.038802431629\\
29	337.885464925427\\
28	337.885464925427\\
27	337.885464925427\\
26	338.151817382729\\
25	338.196639034067\\
24	340.154745016621\\
23	340.538991652407\\
22	341.603028507782\\
21	341.537554335023\\
20	345.757949292655\\
19	345.255106311983\\
18	349.063446075038\\
17	351.276562073804\\
16	353.493318791377\\
15	353.493318791377\\
14	359.717515949388\\
13	362.380356689992\\
12	368.414944249113\\
11	374.885869760552\\
10	392.274111948794\\
9	399.382479588957\\
8	448.306287795917\\
7	494.469893338674\\
6	560.959781508393\\
5	628.047365255794\\
4	681.189497337559\\
3	760.867271863049\\
2	842.521082164984\\
1	927.149794195054\\
}--cycle;
\addplot [color=red]
  table[row sep=crcr]{%
1	740\\
2	687\\
3	628\\
4	570\\
5	530\\
6	485\\
7	441\\
8	409\\
9	385\\
10	377\\
11	367\\
12	355\\
13	349\\
14	346\\
15	342\\
16	342\\
17	339\\
18	335\\
19	334\\
20	332\\
21	328\\
22	328\\
23	327\\
24	326\\
25	323\\
26	323\\
27	323\\
28	323\\
29	323\\
30	321\\
31	321\\
32	319\\
33	319\\
34	317\\
35	316\\
36	316\\
37	314\\
38	313\\
39	313\\
40	313\\
41	313\\
42	313\\
43	312\\
44	312\\
45	312\\
46	308\\
47	308\\
48	308\\
49	307\\
50	307\\
51	307\\
52	307\\
53	307\\
54	306\\
55	305\\
56	305\\
57	305\\
58	305\\
59	304\\
60	303\\
61	303\\
62	302\\
63	301\\
64	301\\
65	301\\
66	301\\
67	301\\
68	301\\
69	301\\
70	301\\
71	300\\
72	300\\
73	300\\
74	299\\
75	299\\
76	299\\
77	299\\
78	299\\
79	299\\
80	299\\
81	299\\
82	299\\
83	298\\
84	298\\
85	298\\
86	298\\
87	297\\
88	297\\
89	297\\
90	297\\
91	297\\
92	296\\
93	296\\
94	296\\
95	296\\
96	296\\
97	296\\
98	296\\
99	296\\
100	296\\
};
\addlegendentry{muscles, c = 0.15 s}


\addplot[area legend, draw=none, fill=black!50!red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	478.784964605733\\
2	405.471064872286\\
3	371.293077597947\\
4	334.211355718086\\
5	307.72086890057\\
6	314.992386608893\\
7	309.494558607774\\
8	314.80792297688\\
9	316.945715123061\\
10	320.254359515838\\
11	320.254359515838\\
12	321.522045810314\\
13	321.522045810314\\
14	321.593397134307\\
15	315.080002510151\\
16	315.440630126395\\
17	315.052452168554\\
18	315.768254645231\\
19	314.982019815006\\
20	312.292325636975\\
21	311.250962132487\\
22	311.20627700475\\
23	309.546729077254\\
24	307.864576436952\\
25	307.733989558666\\
26	307.738727936513\\
27	306.968471738838\\
28	306.903692317399\\
29	306.903692317399\\
30	302.720290737671\\
31	302.049444733298\\
32	301.098596324628\\
33	300.86232388654\\
34	300.896349498827\\
35	301.2500477729\\
36	299.493512580349\\
37	299.493512580349\\
38	299.058271870041\\
39	299.971851466504\\
40	299.27014701626\\
41	298.7326150187\\
42	298.688094535372\\
43	298.688094535372\\
44	298.872348590486\\
45	298.818975230423\\
46	298.663696096775\\
47	298.632724864559\\
48	298.30039004882\\
49	298.263747831709\\
50	298.054445519377\\
51	297.769434461424\\
52	297.645645914504\\
53	297.645645914504\\
54	297.798436488542\\
55	297.441368811099\\
56	297.474038740806\\
57	297.463196541043\\
58	297.075002375787\\
59	297.075002375787\\
60	297.091501870633\\
61	297.14738620463\\
62	297.063581419628\\
63	297.063581419628\\
64	297.066901738977\\
65	296.96040675893\\
66	296.905477221653\\
67	296.73239123112\\
68	296.679288939549\\
69	296.38193836614\\
70	296.38193836614\\
71	296.258263077049\\
72	296.258263077049\\
73	296.096515432179\\
74	296.064794076049\\
75	295.878982979178\\
76	295.878982979178\\
77	295.874079302839\\
78	295.807449262563\\
79	295.807449262563\\
80	295.829974509044\\
81	295.80705517866\\
82	295.748636480224\\
83	295.690104573764\\
84	295.620965874913\\
85	295.531053499314\\
86	295.507753271011\\
87	295.503806281136\\
88	295.490050992914\\
89	295.471324035258\\
90	295.469055603906\\
91	295.466708822964\\
92	295.322785658597\\
93	295.322785658597\\
94	295.319357104251\\
95	295.213290065541\\
96	295.225047984934\\
97	295.218750949224\\
98	295.241732960207\\
99	295.185141706945\\
100	295.207515905097\\
100	296.586373624062\\
99	296.744789154563\\
98	296.758481322761\\
97	296.830223682989\\
96	296.84529919263\\
95	296.881890366744\\
94	296.926320742229\\
93	296.927465114184\\
92	296.927465114184\\
91	297.046559951219\\
90	297.046520721542\\
89	297.144622496289\\
88	297.271015503229\\
87	297.271253964249\\
86	297.272554508571\\
85	297.274976148588\\
84	297.31587165495\\
83	297.37105387912\\
82	297.534131463404\\
81	297.528366169792\\
80	297.52850887704\\
79	297.702675576991\\
78	297.702675576991\\
77	297.744711387975\\
76	297.808055619363\\
75	297.808055619363\\
74	297.824411043288\\
73	297.82029600616\\
72	298.112071739658\\
71	298.112071739658\\
70	298.127744495144\\
69	298.127744495144\\
68	298.444783258253\\
67	298.51816438613\\
66	298.791119361473\\
65	298.864810448537\\
64	299.448562220308\\
63	299.486941558375\\
62	299.486941558375\\
61	299.466518094596\\
60	299.822723559806\\
59	299.932578654324\\
58	299.932578654324\\
57	300.324016439382\\
56	300.473936213258\\
55	300.758478320026\\
54	300.957036842652\\
53	301.79806761209\\
52	301.79806761209\\
51	301.883617082383\\
50	301.938875423132\\
49	302.019544363849\\
48	302.090969132876\\
47	302.124407350267\\
46	302.155450503061\\
45	302.430556773513\\
44	303.155189568671\\
43	304.468835760873\\
42	304.468835760873\\
41	304.925579773449\\
40	306.661043106797\\
39	306.864639193877\\
38	309.949401243958\\
37	310.070071099272\\
36	310.070071099272\\
35	310.768267538967\\
34	311.925858288884\\
33	312.392857328035\\
32	312.415955980691\\
31	313.335379799198\\
30	313.493741306611\\
29	315.426303195577\\
28	315.426303195577\\
27	317.791511387295\\
26	318.864199388826\\
25	319.057883109539\\
24	319.347361658081\\
23	321.478311072659\\
22	321.941704326059\\
21	322.468406608785\\
20	327.116203869101\\
19	328.277876371554\\
18	329.64644410863\\
17	332.763691791231\\
16	333.545560136616\\
15	341.132416208063\\
14	349.101152806001\\
13	349.792668213235\\
12	349.792668213235\\
11	363.250716867875\\
10	363.250716867875\\
9	395.456901363967\\
8	402.427850686458\\
7	434.902433668952\\
6	463.030045055925\\
5	504.219555150483\\
4	581.319239144814\\
3	636.122637822107\\
2	724.181215955365\\
1	875.388880002082\\
}--cycle;
\addplot [color=black!50!red]
  table[row sep=crcr]{%
1	677\\
2	565\\
3	504\\
4	458\\
5	406\\
6	389\\
7	372\\
8	359\\
9	356\\
10	342\\
11	342\\
12	336\\
13	336\\
14	335\\
15	328\\
16	324\\
17	324\\
18	323\\
19	322\\
20	320\\
21	317\\
22	317\\
23	316\\
24	314\\
25	313\\
26	313\\
27	312\\
28	311\\
29	311\\
30	308\\
31	308\\
32	307\\
33	307\\
34	306\\
35	306\\
36	305\\
37	305\\
38	305\\
39	303\\
40	303\\
41	302\\
42	302\\
43	302\\
44	301\\
45	301\\
46	300\\
47	300\\
48	300\\
49	300\\
50	300\\
51	300\\
52	300\\
53	300\\
54	299\\
55	299\\
56	299\\
57	299\\
58	299\\
59	299\\
60	298\\
61	298\\
62	298\\
63	298\\
64	298\\
65	298\\
66	298\\
67	298\\
68	298\\
69	297\\
70	297\\
71	297\\
72	297\\
73	297\\
74	297\\
75	297\\
76	297\\
77	297\\
78	297\\
79	297\\
80	297\\
81	297\\
82	297\\
83	297\\
84	296\\
85	296\\
86	296\\
87	296\\
88	296\\
89	296\\
90	296\\
91	296\\
92	296\\
93	296\\
94	296\\
95	296\\
96	296\\
97	296\\
98	296\\
99	296\\
100	296\\
};
\addlegendentry{muscles, c = 0.3 s}

\legend{}
\end{axis}


==> figures/dataefficiency_cost_squatting.tex <==
\begin{axis}[%
name =ax3,
at={(ax2.south east)},
xlabel near ticks, ylabel near ticks,
every y tick scale label/.style={at={(yticklabel* cs:1.03,0cm)},anchor=near yticklabel},
title style={at={(0.5,0.93)}},
xshift=1cm,
width=0.652\figW,
height=\figH,
scale only axis,
xmin=0,
xmax=100,
xtick={  0,  20,  40,  60,  80, 100},
xlabel style={font=\color{white!15!black}},
xlabel={generations},
ymin=0,
ymax=500000,
ylabel style={font=\color{white!15!black}},
ylabel={cost},
axis background/.style={fill=white},
title={(c) squatting(OC)},
legend style={at={(1.03,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]

\addplot[area legend, draw=none, fill=mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1447724.42201543\\
2	922940.598363457\\
3	841731.302688755\\
4	771025.685605582\\
5	756283.570654325\\
6	725764.010068513\\
7	664998.909426936\\
8	657906.513362481\\
9	657906.513362481\\
10	578379.196913774\\
11	571372.88025311\\
12	544618.643672315\\
13	524804.337703379\\
14	529731.392568539\\
15	540272.085124177\\
16	536948.183209817\\
17	522971.815808422\\
18	530423.69295344\\
19	524795.150453576\\
20	512236.097851383\\
21	500447.23600771\\
22	484124.950812001\\
23	425623.679673401\\
24	424399.639110464\\
25	433846.738005775\\
26	433846.738005775\\
27	420557.938028925\\
28	420557.938028925\\
29	421494.178506131\\
30	396960.065021628\\
31	399272.650394326\\
32	382351.958331378\\
33	371486.558607142\\
34	347116.882839836\\
35	332263.664826977\\
36	327380.653798195\\
37	289525.238904202\\
38	292640.688539948\\
39	292640.688539948\\
40	292640.688539948\\
41	261026.286227108\\
42	257152.446857674\\
43	257532.157170409\\
44	244697.77479383\\
45	244187.790371526\\
46	243289.485435928\\
47	220119.939891415\\
48	216249.824372932\\
49	216249.824372932\\
50	209094.469053494\\
51	189724.010510146\\
52	195747.746844009\\
53	193886.582902801\\
54	180546.519738594\\
55	180546.519738594\\
56	179371.786979935\\
57	172695.46573651\\
58	172113.194798593\\
59	165865.07575237\\
60	165835.853139741\\
61	163420.286382651\\
62	158102.326694028\\
63	157338.561693157\\
64	146587.068768074\\
65	137638.55494966\\
66	137638.55494966\\
67	131074.985437452\\
68	125424.32851333\\
69	126147.409061972\\
70	126147.409061972\\
71	126147.409061972\\
72	126372.637848402\\
73	126372.637848402\\
74	124488.517775573\\
75	124488.517775573\\
76	125493.319984365\\
77	121723.615325621\\
78	121723.615325621\\
79	115809.048399424\\
80	115809.048399424\\
81	114602.336611126\\
82	114602.336611126\\
83	113843.970290151\\
84	112174.327876418\\
85	112716.674883327\\
86	112716.674883327\\
87	112716.674883327\\
88	112122.74111828\\
89	112122.74111828\\
90	111639.143626957\\
91	111639.143626957\\
92	110811.75801552\\
93	111269.954423585\\
94	109344.393857794\\
95	104260.469333025\\
96	104476.160232706\\
97	104419.855119653\\
98	103996.161818146\\
99	103996.161818146\\
100	103996.161818146\\
100	121886.817595737\\
99	121886.817595737\\
98	121886.817595737\\
97	122214.494324834\\
96	131204.899002314\\
95	132121.046023024\\
94	133232.761197244\\
93	135476.217146172\\
92	137715.576722686\\
91	138449.839865704\\
90	138449.839865704\\
89	140059.688215361\\
88	140059.688215361\\
87	140772.525992274\\
86	140772.525992274\\
85	140772.525992274\\
84	143348.262411276\\
83	143458.847568\\
82	144595.090505426\\
81	144595.090505426\\
80	148438.431737211\\
79	148438.431737211\\
78	147306.054751903\\
77	147306.054751903\\
76	153697.721320983\\
75	160803.83157586\\
74	160803.83157586\\
73	175497.829081679\\
72	175497.829081679\\
71	176319.415326972\\
70	176319.415326972\\
69	176319.415326972\\
68	189373.229929698\\
67	194017.183078695\\
66	215580.284043802\\
65	215580.284043802\\
64	228654.310966417\\
63	229555.415484593\\
62	229773.875484916\\
61	232584.626003755\\
60	240940.074799936\\
59	250883.515506656\\
58	273476.42073607\\
57	275858.729639495\\
56	302714.692850603\\
55	305074.720830818\\
54	305074.720830818\\
53	301489.972311058\\
52	301016.433511466\\
51	328532.930984531\\
50	330745.208590895\\
49	338736.987215902\\
48	338736.987215902\\
47	353093.937305952\\
46	369196.267094636\\
45	373930.79220567\\
44	379704.491725423\\
43	376867.431923174\\
42	386023.601513807\\
41	399926.825216405\\
40	432020.763594259\\
39	432020.763594259\\
38	432020.763594259\\
37	446774.829664166\\
36	449508.572274065\\
35	452155.615578795\\
34	483634.826200882\\
33	506101.755786113\\
32	504690.935161143\\
31	504499.312802029\\
30	526013.991367374\\
29	523735.098844856\\
28	527784.37333365\\
27	527784.37333365\\
26	530674.438849467\\
25	530674.438849467\\
24	577929.073010163\\
23	578617.311669705\\
22	594061.73224156\\
21	599232.391548404\\
20	601405.723187903\\
19	638218.426043636\\
18	641140.089081756\\
17	679042.949823988\\
16	695221.967633697\\
15	694858.161682567\\
14	739528.870954543\\
13	757450.706777133\\
12	771255.209112581\\
11	781324.407987672\\
10	818905.046381847\\
9	852636.3185359\\
8	852636.3185359\\
7	869938.41441583\\
6	956738.868435267\\
5	1187680.62066785\\
4	1236920.62754701\\
3	1448355.95467162\\
2	1550713.31513768\\
1	1858724.94016062\\
}--cycle;
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	1653225\\
2	1236827\\
3	1145044\\
4	1003973\\
5	971982\\
6	841251\\
7	767469\\
8	755271\\
9	755271\\
10	698642\\
11	676349\\
12	657937\\
13	641128\\
14	634630\\
15	617565\\
16	616085\\
17	601007\\
18	585782\\
19	581507\\
20	556821\\
21	549840\\
22	539093\\
23	502120\\
24	501164\\
25	482261\\
26	482261\\
27	474171\\
28	474171\\
29	472615\\
30	461487\\
31	451886\\
32	443521\\
33	438794\\
34	415376\\
35	392210\\
36	388445\\
37	368150\\
38	362331\\
39	362331\\
40	362331\\
41	330477\\
42	321588\\
43	317200\\
44	312201\\
45	309059\\
46	306243\\
47	286607\\
48	277493\\
49	277493\\
50	269920\\
51	259128\\
52	248382\\
53	247688\\
54	242811\\
55	242811\\
56	241043\\
57	224277\\
58	222795\\
59	208374\\
60	203388\\
61	198002\\
62	193938\\
63	193447\\
64	187621\\
65	176609\\
66	176609\\
67	162546\\
68	157399\\
69	151233\\
70	151233\\
71	151233\\
72	150935\\
73	150935\\
74	142646\\
75	142646\\
76	139596\\
77	134515\\
78	134515\\
79	132124\\
80	132124\\
81	129599\\
82	129599\\
83	128651\\
84	127761\\
85	126745\\
86	126745\\
87	126745\\
88	126091\\
89	126091\\
90	125044\\
91	125044\\
92	124264\\
93	123373\\
94	121289\\
95	118191\\
96	117841\\
97	113317\\
98	112941\\
99	112941\\
100	112941\\
};
\addlegendentry{torques, c = 0.05 s}


\addplot[area legend, draw=none, fill=blue!50!mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	700638.620934816\\
2	538365.924947887\\
3	411232.551167037\\
4	379701.002596309\\
5	334938.915552502\\
6	273281.131487146\\
7	200864.628746381\\
8	172715.840433511\\
9	163025.848072981\\
10	116174.832793357\\
11	111435.746142339\\
12	111435.746142339\\
13	100598.390065403\\
14	87265.7747681576\\
15	82493.5753394731\\
16	66461.4565711776\\
17	73839.8516857203\\
18	73839.8516857203\\
19	77028.7098727748\\
20	67520.9054038944\\
21	81720.2422585866\\
22	83011.1087755603\\
23	84258.030187254\\
24	75855.9060102928\\
25	75159.1396430369\\
26	75159.1396430369\\
27	82828.0631665499\\
28	82828.0631665499\\
29	82800.5579104628\\
30	84668.538169571\\
31	86094.1470349014\\
32	86094.1470349014\\
33	86094.1470349014\\
34	81905.1339930141\\
35	81905.1339930141\\
36	81905.1339930141\\
37	86386.0073723063\\
38	85764.63462302\\
39	85764.63462302\\
40	84502.3652300763\\
41	84502.3652300763\\
42	84300.7932566449\\
43	84921.7325518523\\
44	82010.4239376088\\
45	79130.9682746518\\
46	78902.2738395165\\
47	78902.2738395165\\
48	78227.8960967484\\
49	77849.4711718511\\
50	77709.9915810581\\
51	77658.5321332734\\
52	75824.4289182154\\
53	75824.4289182154\\
54	75100.7967817753\\
55	74432.7453875476\\
56	74804.2501743843\\
57	74376.7738942269\\
58	73851.9495657201\\
59	73851.9495657201\\
60	71815.6207800841\\
61	70885.8490946836\\
62	70704.5016751719\\
63	66468.0419783574\\
64	66468.0419783574\\
65	65239.6654140161\\
66	63964.2210193328\\
67	63686.3143025129\\
68	63686.3143025129\\
69	62375.8139706868\\
70	62375.8139706868\\
71	62375.8139706868\\
72	61961.1853842543\\
73	61961.1853842543\\
74	61961.1853842543\\
75	61810.2008813132\\
76	61541.6862715813\\
77	58167.024992679\\
78	54740.344476792\\
79	53576.7590048403\\
80	50356.2645601747\\
81	50431.3833592086\\
82	50431.3833592086\\
83	49220.6405703588\\
84	49089.9873328185\\
85	49089.9873328185\\
86	49089.9873328185\\
87	49089.9873328185\\
88	50151.0862946448\\
89	50151.0862946448\\
90	50151.0862946448\\
91	48769.7466250372\\
92	47672.3374532023\\
93	47672.3374532023\\
94	48775.8859051047\\
95	48775.8859051047\\
96	48775.8859051047\\
97	48036.0292530373\\
98	46276.4578671076\\
99	45521.7175297582\\
100	45521.7175297582\\
100	61427.6865412564\\
99	61427.6865412564\\
98	62393.0804275615\\
97	62219.5089038468\\
96	62447.7165729769\\
95	62447.7165729769\\
94	62447.7165729769\\
93	66509.7728696202\\
92	66509.7728696202\\
91	66501.9009005825\\
90	67778.6696707877\\
89	67778.6696707877\\
88	67778.6696707877\\
87	71516.7036657543\\
86	71516.7036657543\\
85	71516.7036657543\\
84	71516.7036657543\\
83	71680.5981125278\\
82	72492.8711493916\\
81	72492.8711493916\\
80	72947.8452871559\\
79	73774.7517352097\\
78	73641.5253692109\\
77	78412.6463004112\\
76	77994.5714097101\\
75	78027.934210286\\
74	80554.72635096\\
73	80554.72635096\\
72	80554.72635096\\
71	80613.364906458\\
70	80613.364906458\\
69	80613.364906458\\
68	81109.0401468382\\
67	81109.0401468382\\
66	81219.8576097849\\
65	84668.6065561765\\
64	85011.2885497496\\
63	85011.2885497496\\
62	84894.8773193855\\
61	85147.954379883\\
60	85669.4783837523\\
59	87254.806007384\\
58	87254.806007384\\
57	87263.3595577101\\
56	88551.0113055358\\
55	90242.0998792235\\
54	90574.9490660891\\
53	90474.3257976333\\
52	90474.3257976333\\
51	92658.7644965708\\
50	92704.7541994429\\
49	95355.5207315415\\
48	96027.3619526969\\
47	96356.5488246141\\
46	96356.5488246141\\
45	98087.7297525732\\
44	97566.4850614248\\
43	98506.9613246256\\
42	101161.495131522\\
41	104070.078664601\\
40	104070.078664601\\
39	112861.082273484\\
38	112861.082273484\\
37	112917.976581685\\
36	127682.524368458\\
35	127682.524368458\\
34	127682.524368458\\
33	129116.569228941\\
32	129116.569228941\\
31	129116.569228941\\
30	141787.790982688\\
29	147476.893807238\\
28	147491.630981852\\
27	147491.630981852\\
26	190445.67704926\\
25	190445.67704926\\
24	190669.744287364\\
23	195472.158421307\\
22	199439.203208957\\
21	203523.585767902\\
20	247577.916078195\\
19	251563.235940181\\
18	261426.834504699\\
17	261426.834504699\\
16	285755.270722265\\
15	307398.509279813\\
14	308686.669640989\\
13	355430.014972186\\
12	416768.975482665\\
11	416768.975482665\\
10	426711.487932101\\
9	465244.883328096\\
8	502183.343060328\\
7	541679.423913219\\
6	756633.725148182\\
5	763832.93041314\\
4	791544.360852764\\
3	806347.381118965\\
2	892458.220158536\\
1	1002985.34340266\\
}--cycle;
\addplot [color=blue!50!mycolor1]
  table[row sep=crcr]{%
1	851812\\
2	715412\\
3	608790\\
4	585623\\
5	549386\\
6	514957\\
7	371272\\
8	337450\\
9	314135\\
10	271443\\
11	264102\\
12	264102\\
13	228014\\
14	197976\\
15	194946\\
16	176108\\
17	167633\\
18	167633\\
19	164296\\
20	157549\\
21	142622\\
22	141225\\
23	139865\\
24	133263\\
25	132802\\
26	132802\\
27	115160\\
28	115160\\
29	115139\\
30	113228\\
31	107605\\
32	107605\\
33	107605\\
34	104794\\
35	104794\\
36	104794\\
37	99652\\
38	99313\\
39	99313\\
40	94286\\
41	94286\\
42	92731\\
43	91714\\
44	89788\\
45	88609\\
46	87629\\
47	87629\\
48	87128\\
49	86602\\
50	85207\\
51	85159\\
52	83149\\
53	83149\\
54	82838\\
55	82337\\
56	81678\\
57	80820\\
58	80553\\
59	80553\\
60	78743\\
61	78017\\
62	77800\\
63	75740\\
64	75740\\
65	74954\\
66	72592\\
67	72398\\
68	72398\\
69	71495\\
70	71495\\
71	71495\\
72	71258\\
73	71258\\
74	71258\\
75	69919\\
76	69768\\
77	68290\\
78	64191\\
79	63676\\
80	61652\\
81	61462\\
82	61462\\
83	60451\\
84	60303\\
85	60303\\
86	60303\\
87	60303\\
88	58965\\
89	58965\\
90	58965\\
91	57636\\
92	57091\\
93	57091\\
94	55612\\
95	55612\\
96	55612\\
97	55128\\
98	54335\\
99	53475\\
100	53475\\
};
\addlegendentry{torques, c = 0.15 s}


\addplot[area legend, draw=none, fill=blue, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	358959.278683098\\
2	229377.059570268\\
3	135603.953582104\\
4	71534.0839196269\\
5	71826.3554801458\\
6	108656.991265732\\
7	84768.7900341027\\
8	81542.4982912049\\
9	81515.5318732062\\
10	81515.5318732062\\
11	81301.5802493061\\
12	77819.4197466439\\
13	77025.7213801929\\
14	74276.1034957577\\
15	74276.1034957577\\
16	74659.8190259415\\
17	74779.0943572894\\
18	74409.2254990317\\
19	73530.5350157804\\
20	73530.5350157804\\
21	73530.5350157804\\
22	73850.205880149\\
23	73850.205880149\\
24	72888.7435368092\\
25	68360.9876001021\\
26	68128.020843706\\
27	68128.020843706\\
28	68128.020843706\\
29	68318.2277492005\\
30	68318.2277492005\\
31	68318.2277492005\\
32	68318.2277492005\\
33	68318.2277492005\\
34	68318.2277492005\\
35	68234.1005367559\\
36	67998.8513514217\\
37	67504.2463249365\\
38	67504.2463249365\\
39	67540.8023698209\\
40	67216.4278883962\\
41	65396.6983433137\\
42	65396.6983433137\\
43	63632.9319706304\\
44	63632.92924772\\
45	63609.9683487668\\
46	63390.6467124228\\
47	63267.031263326\\
48	60698.1761958733\\
49	59883.842966989\\
50	59392.5090728625\\
51	59310.2278891124\\
52	59310.2278891124\\
53	56228.8681687733\\
54	56228.8681687733\\
55	56228.8681687733\\
56	55530.5433603415\\
57	53906.207159414\\
58	53906.207159414\\
59	52372.7100624048\\
60	52357.4639398241\\
61	51744.3821586947\\
62	50196.9757304565\\
63	49996.9390298422\\
64	50106.14981681\\
65	49963.0742322064\\
66	46175.9522285541\\
67	46011.8738621853\\
68	45816.921620599\\
69	45754.9442936424\\
70	45734.9298253094\\
71	44901.6876642417\\
72	44728.5890302365\\
73	42562.2284636813\\
74	42542.5354293257\\
75	42013.2543583568\\
76	41715.1388267473\\
77	40983.3310449979\\
78	38400.276935326\\
79	37319.426552537\\
80	36244.2339455235\\
81	36549.7788764203\\
82	36549.7788764203\\
83	36649.0956108596\\
84	36864.2241619072\\
85	36864.2241619072\\
86	36864.2241619072\\
87	36864.2241619072\\
88	36864.2241619072\\
89	36864.2241619072\\
90	36844.1434486538\\
91	36325.4021519622\\
92	36081.7456446812\\
93	36022.1329478772\\
94	36147.9394365459\\
95	36147.9394365459\\
96	35456.4249890004\\
97	35393.6420635544\\
98	35422.1734490809\\
99	34267.7470176612\\
100	33715.8265253913\\
100	43663.4607871681\\
99	43864.8186181474\\
98	44422.9130434101\\
97	45495.144573616\\
96	45566.9370325243\\
95	45406.7456400078\\
94	45406.7456400078\\
93	46498.1128604934\\
92	46560.5642786538\\
91	47959.6671491696\\
90	47921.585067765\\
89	47916.8662271476\\
88	47916.8662271476\\
87	47916.8662271476\\
86	47916.8662271476\\
85	47916.8662271476\\
84	47916.8662271476\\
83	49646.0054691458\\
82	50178.8692825496\\
81	50178.8692825496\\
80	51590.5105705785\\
79	52270.3554020328\\
78	53003.6014331735\\
77	52579.7578628139\\
76	53297.4817290328\\
75	53594.701524149\\
74	54350.5513764465\\
73	54985.2125561292\\
72	54469.0134381423\\
71	54801.2153547015\\
70	55524.1877875331\\
69	55585.1211631666\\
68	55635.5777568151\\
67	56515.2327996851\\
66	56994.09713863\\
65	56734.8023844481\\
64	60646.1434491369\\
63	66352.469136188\\
62	66426.446306799\\
61	66747.8888749859\\
60	67757.1385628044\\
59	67755.5508942215\\
58	67762.6788584144\\
57	67762.6788584144\\
56	68308.5167257836\\
55	69083.8082046471\\
54	69083.8082046471\\
53	69083.8082046471\\
52	68997.0570505603\\
51	68997.0570505603\\
50	69102.7670858308\\
49	69264.551948302\\
48	70015.2489923288\\
47	69677.578303521\\
46	69853.1095418865\\
45	70583.2340966729\\
44	70934.4815188588\\
43	70934.6152510579\\
42	71968.9171751594\\
41	71968.9171751594\\
40	73289.2810322066\\
39	74778.0594611857\\
38	75245.0614441876\\
37	75245.0614441876\\
36	75909.5308540112\\
35	76511.8061586088\\
34	77475.0325333101\\
33	77475.0325333101\\
32	77475.0325333101\\
31	77475.0325333101\\
30	77475.0325333101\\
29	77475.0325333101\\
28	79247.3343856044\\
27	79247.3343856044\\
26	79247.3343856044\\
25	81318.2700958627\\
24	80929.2850142337\\
23	81749.6173893994\\
22	81749.6173893994\\
21	84025.3944564139\\
20	84025.3944564139\\
19	84025.3944564139\\
18	86375.7106667354\\
17	87217.7367107415\\
16	87781.4763543289\\
15	89388.2888604017\\
14	89388.2888604017\\
13	92342.3290056658\\
12	104292.716306678\\
11	112467.304587777\\
10	115306.286724579\\
9	115306.286724579\\
8	117932.4504432\\
7	118644.934969502\\
6	125935.651802915\\
5	272431.479186538\\
4	343367.242704701\\
3	487899.450457063\\
2	653075.07193112\\
1	812972.479396005\\
}--cycle;
\addplot [color=blue]
  table[row sep=crcr]{%
1	585966\\
2	441226\\
3	311752\\
4	207451\\
5	172129\\
6	117296\\
7	101707\\
8	99737\\
9	98411\\
10	98411\\
11	96884\\
12	91056\\
13	84684\\
14	81832\\
15	81832\\
16	81221\\
17	80998\\
18	80392\\
19	78778\\
20	78778\\
21	78778\\
22	77800\\
23	77800\\
24	76909\\
25	74840\\
26	73688\\
27	73688\\
28	73688\\
29	72897\\
30	72897\\
31	72897\\
32	72897\\
33	72897\\
34	72897\\
35	72373\\
36	71954\\
37	71375\\
38	71375\\
39	71159\\
40	70253\\
41	68683\\
42	68683\\
43	67284\\
44	67284\\
45	67097\\
46	66622\\
47	66472\\
48	65357\\
49	64574\\
50	64248\\
51	64154\\
52	64154\\
53	62656\\
54	62656\\
55	62656\\
56	61920\\
57	60834\\
58	60834\\
59	60064\\
60	60057\\
61	59246\\
62	58312\\
63	58175\\
64	55376\\
65	53349\\
66	51585\\
67	51264\\
68	50726\\
69	50670\\
70	50630\\
71	49851\\
72	49599\\
73	48774\\
74	48447\\
75	47804\\
76	47506\\
77	46782\\
78	45702\\
79	44795\\
80	43917\\
81	43364\\
82	43364\\
83	43148\\
84	42391\\
85	42391\\
86	42391\\
87	42391\\
88	42391\\
89	42391\\
90	42383\\
91	42143\\
92	41321\\
93	41260\\
94	40777\\
95	40777\\
96	40512\\
97	40444\\
98	39923\\
99	39066\\
100	38690\\
};
\addlegendentry{torques, c = 0.3 s}


\addplot[area legend, draw=none, fill=orange, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	58099.8909158242\\
2	48583.3029635151\\
3	46639.2223165527\\
4	26487.6168326215\\
5	23508.7197956599\\
6	18388.2869318008\\
7	17376.3228648759\\
8	15437.8865195928\\
9	13903.3644829503\\
10	13269.2113915556\\
11	12529.9726166424\\
12	10952.7982604868\\
13	10025.4175234838\\
14	9350.69884464666\\
15	9844.09316053676\\
16	10204.0181256217\\
17	9095.58495585027\\
18	8063.66104070144\\
19	8148.36209831073\\
20	7992.31557867388\\
21	7608.79629650789\\
22	7574.21997055817\\
23	7882.88430958063\\
24	7980.23531797548\\
25	7980.23531797548\\
26	8188.35634029343\\
27	8188.35634029343\\
28	7796.85559163755\\
29	7796.85559163755\\
30	7796.85559163755\\
31	7796.85559163755\\
32	7796.85559163755\\
33	7796.85559163755\\
34	7796.85559163755\\
35	7796.85559163755\\
36	7604.46194739503\\
37	7604.46194739503\\
38	7584.17838200133\\
39	7403.3297577612\\
40	7403.3297577612\\
41	7403.3297577612\\
42	7403.3297577612\\
43	7403.3297577612\\
44	7403.3297577612\\
45	7403.3297577612\\
46	7147.59926476259\\
47	7147.59926476259\\
48	6813.33080545443\\
49	6798.52330991897\\
50	6798.52330991897\\
51	6798.52330991897\\
52	6800.51406299042\\
53	6800.51406299042\\
54	6800.51406299042\\
55	6800.51406299042\\
56	6789.21057669039\\
57	6789.21057669039\\
58	6789.21057669039\\
59	6789.21057669039\\
60	6789.21057669039\\
61	6789.21057669039\\
62	6411.36553976832\\
63	6306.97885481107\\
64	5901.69828182759\\
65	5901.69828182759\\
66	5901.69828182759\\
67	5901.69828182759\\
68	5901.69828182759\\
69	5901.69828182759\\
70	5910.68121097019\\
71	5905.33680380175\\
72	5905.33680380175\\
73	5906.86482504756\\
74	5906.86482504756\\
75	5906.86482504756\\
76	5906.86482504756\\
77	5906.86482504756\\
78	5906.86482504756\\
79	5906.86482504756\\
80	5906.86482504756\\
81	5840.33393230709\\
82	5838.74621388157\\
83	5838.74621388157\\
84	5838.74621388157\\
85	5838.74621388157\\
86	5838.74621388157\\
87	5838.74621388157\\
88	5799.81073529991\\
89	5647.19888718142\\
90	5351.33795344227\\
91	5296.65064616646\\
92	5296.65064616646\\
93	5296.65064616646\\
94	5296.65064616646\\
95	5286.77636200838\\
96	5286.77636200838\\
97	5286.77636200838\\
98	5286.77636200838\\
99	5286.77636200838\\
100	5286.77636200838\\
100	6932.97258474458\\
99	6932.97258474458\\
98	6932.97258474458\\
97	6932.97258474458\\
96	6932.97258474458\\
95	6932.97258474458\\
94	7051.539126515\\
93	7051.539126515\\
92	7051.539126515\\
91	7051.539126515\\
90	7043.34217424467\\
89	7031.07197965053\\
88	7078.02544928191\\
87	7107.88721431363\\
86	7107.88721431363\\
85	7107.88721431363\\
84	7107.88721431363\\
83	7107.88721431363\\
82	7107.88721431363\\
81	7140.78017799611\\
80	7241.5689228981\\
79	7241.5689228981\\
78	7241.5689228981\\
77	7241.5689228981\\
76	7241.5689228981\\
75	7241.5689228981\\
74	7241.5689228981\\
73	7241.5689228981\\
72	7263.96212834492\\
71	7263.96212834492\\
70	7378.91036246918\\
69	7528.04011822842\\
68	7528.04011822842\\
67	7528.04011822842\\
66	7528.04011822842\\
65	7528.04011822842\\
64	7528.04011822842\\
63	7562.52806129704\\
62	7680.13267577188\\
61	7583.74679930671\\
60	7583.74679930671\\
59	7583.74679930671\\
58	7583.74679930671\\
57	7583.74679930671\\
56	7583.74679930671\\
55	7673.18108976284\\
54	7673.18108976284\\
53	7673.18108976284\\
52	7673.18108976284\\
51	7733.83982584658\\
50	7733.83982584658\\
49	7733.83982584658\\
48	7731.30085061221\\
47	7949.69570247372\\
46	7949.69570247372\\
45	7988.79263098049\\
44	7988.79263098049\\
43	7988.79263098049\\
42	7988.79263098049\\
41	7988.79263098049\\
40	7988.79263098049\\
39	7988.79263098049\\
38	8021.71648676945\\
37	8332.10476926389\\
36	8332.10476926389\\
35	8587.95857622037\\
34	8587.95857622037\\
33	8587.95857622037\\
32	8587.95857622037\\
31	8587.95857622037\\
30	8587.95857622037\\
29	8587.95857622037\\
28	8587.95857622037\\
27	8815.54532458111\\
26	8815.54532458111\\
25	9895.75278384838\\
24	9895.75278384838\\
23	10632.1542612145\\
22	11577.2610164922\\
21	11864.1356850076\\
20	12123.4451163043\\
19	12147.4794111525\\
18	14754.1660920881\\
17	15253.1781775531\\
16	15863.6857006346\\
15	17410.5825763013\\
14	19203.4222815572\\
13	20365.1057851505\\
12	21231.22339625\\
11	24163.3491907038\\
10	26772.1775192312\\
9	30137.8485013781\\
8	31171.28789456\\
7	35323.8171556874\\
6	46030.8645462191\\
5	58680.9716759425\\
4	61180.6703127824\\
3	73969.0522042086\\
2	97722.4634559649\\
1	112408.744396179\\
}--cycle;
\addplot [color=orange]
  table[row sep=crcr]{%
1	85254\\
2	73153\\
3	60304\\
4	43834\\
5	41095\\
6	32210\\
7	26350\\
8	23305\\
9	22021\\
10	20021\\
11	18347\\
12	16092\\
13	15195\\
14	14277\\
15	13627\\
16	13034\\
17	12174\\
18	11409\\
19	10148\\
20	10058\\
21	9736\\
22	9576\\
23	9258\\
24	8938\\
25	8938\\
26	8502\\
27	8502\\
28	8192\\
29	8192\\
30	8192\\
31	8192\\
32	8192\\
33	8192\\
34	8192\\
35	8192\\
36	7968\\
37	7968\\
38	7803\\
39	7696\\
40	7696\\
41	7696\\
42	7696\\
43	7696\\
44	7696\\
45	7696\\
46	7549\\
47	7549\\
48	7272\\
49	7266\\
50	7266\\
51	7266\\
52	7237\\
53	7237\\
54	7237\\
55	7237\\
56	7186\\
57	7186\\
58	7186\\
59	7186\\
60	7186\\
61	7186\\
62	7046\\
63	6935\\
64	6715\\
65	6715\\
66	6715\\
67	6715\\
68	6715\\
69	6715\\
70	6645\\
71	6585\\
72	6585\\
73	6574\\
74	6574\\
75	6574\\
76	6574\\
77	6574\\
78	6574\\
79	6574\\
80	6574\\
81	6491\\
82	6473\\
83	6473\\
84	6473\\
85	6473\\
86	6473\\
87	6473\\
88	6439\\
89	6339\\
90	6197\\
91	6174\\
92	6174\\
93	6174\\
94	6174\\
95	6110\\
96	6110\\
97	6110\\
98	6110\\
99	6110\\
100	6110\\
};
\addlegendentry{muscles, c = 0.05 s}


\addplot[area legend, draw=none, fill=red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	39038.6978666228\\
2	26206.4088911111\\
3	27121.2135767713\\
4	23069.1389383349\\
5	18275.2703992514\\
6	16409.214516669\\
7	16316.4638915634\\
8	14132.001190993\\
9	13185.3754098875\\
10	12529.6493332672\\
11	12529.6493332672\\
12	12044.94573996\\
13	12609.338974452\\
14	13499.9590015651\\
15	12994.9813162196\\
16	12249.5534475536\\
17	12275.2865459426\\
18	12275.2865459426\\
19	12275.2865459426\\
20	12275.2865459426\\
21	12275.2865459426\\
22	11398.7537320113\\
23	11457.4517841254\\
24	11457.6555679709\\
25	11457.6555679709\\
26	11457.6555679709\\
27	10677.5928156614\\
28	10677.5928156614\\
29	10611.4344893367\\
30	10369.3179881632\\
31	10369.3179881632\\
32	10369.3179881632\\
33	10349.8035852173\\
34	9996.0590380323\\
35	9996.0590380323\\
36	9996.0590380323\\
37	8694.09185164534\\
38	8694.09185164534\\
39	8694.09185164534\\
40	8694.09185164534\\
41	8694.09185164534\\
42	8694.09185164534\\
43	8694.09185164534\\
44	8694.09185164534\\
45	8687.14787651183\\
46	8687.14787651183\\
47	8687.14787651183\\
48	8687.14787651183\\
49	8687.14787651183\\
50	8558.07629664552\\
51	8410.68651001978\\
52	8410.68651001978\\
53	8225.20054139584\\
54	8225.20054139584\\
55	8225.20054139584\\
56	8225.20054139584\\
57	7948.4947665629\\
58	7948.4947665629\\
59	7948.4947665629\\
60	7948.4947665629\\
61	7948.4947665629\\
62	7913.35721160844\\
63	7818.15968281751\\
64	7805.42536089019\\
65	7805.42536089019\\
66	7805.42536089019\\
67	7805.42536089019\\
68	7805.42536089019\\
69	7805.42536089019\\
70	7805.42536089019\\
71	7744.57017994756\\
72	7744.57017994756\\
73	7744.57017994756\\
74	7744.57017994756\\
75	7922.89353960444\\
76	7279.75777309317\\
77	7279.75777309317\\
78	7279.75777309317\\
79	6830.05627213985\\
80	6830.05627213985\\
81	6830.05627213985\\
82	6683.52420332243\\
83	6683.52420332243\\
84	6639.43056766319\\
85	6735.76010673011\\
86	6735.76010673011\\
87	6735.76010673011\\
88	6735.76010673011\\
89	6675.02036092904\\
90	6772.18762767314\\
91	6606.77114541509\\
92	6606.77114541509\\
93	6606.77114541509\\
94	6665.07135430276\\
95	6665.07135430276\\
96	6665.07135430276\\
97	6665.07135430276\\
98	6665.07135430276\\
99	6591.44589087011\\
100	6317.07472918638\\
100	11167.0457201205\\
99	11483.0663878044\\
98	11966.7179452384\\
97	11966.7179452384\\
96	11966.7179452384\\
95	11966.7179452384\\
94	11966.7179452384\\
93	12201.1185569482\\
92	12201.1185569482\\
91	12201.1185569482\\
90	12192.1249015259\\
89	12554.9883469498\\
88	12571.9454088852\\
87	12571.9454088852\\
86	12571.9454088852\\
85	12571.9454088852\\
84	12917.747342748\\
83	12917.4788664706\\
82	12917.4788664706\\
81	13404.0739474686\\
80	13404.0739474686\\
79	13404.0739474686\\
78	13579.6863461676\\
77	13579.6863461676\\
76	13579.6863461676\\
75	13565.2018254391\\
74	14253.6599067209\\
73	14253.6599067209\\
72	14253.6599067209\\
71	14253.6599067209\\
70	14261.8678533477\\
69	14261.8678533477\\
68	14261.8678533477\\
67	14261.8678533477\\
66	14261.8678533477\\
65	14261.8678533477\\
64	14261.8678533477\\
63	14267.0051482865\\
62	14278.4077578434\\
61	14283.4993948667\\
60	14283.4993948667\\
59	14283.4993948667\\
58	14283.4993948667\\
57	14283.4993948667\\
56	14344.1684406526\\
55	14344.1684406526\\
54	14344.1684406526\\
53	14344.1684406526\\
52	14416.025499229\\
51	14416.025499229\\
50	14460.6619388413\\
49	14833.3188967913\\
48	14833.3188967913\\
47	14833.3188967913\\
46	14833.3188967913\\
45	14833.3188967913\\
44	14866.134962104\\
43	14866.134962104\\
42	14866.134962104\\
41	14866.134962104\\
40	14866.134962104\\
39	14866.134962104\\
38	14866.134962104\\
37	14866.134962104\\
36	14954.4524481689\\
35	14954.4524481689\\
34	14954.4524481689\\
33	14988.3923986151\\
32	15052.1329641615\\
31	15052.1329641615\\
30	15052.1329641615\\
29	15117.0189364186\\
28	15994.4754371712\\
27	15994.4754371712\\
26	16458.3517699599\\
25	16458.3517699599\\
24	16458.3517699599\\
23	16463.1830471067\\
22	17050.9918832742\\
21	16972.8148659797\\
20	16972.8148659797\\
19	16972.8148659797\\
18	16972.8148659797\\
17	16972.8148659797\\
16	17109.6075237108\\
15	19997.6143227977\\
14	20072.6177735664\\
13	23290.0781647853\\
12	26718.5655799727\\
11	27185.6767804641\\
10	27185.6767804641\\
9	31708.8950824103\\
8	32474.641764848\\
7	35425.6813554003\\
6	41540.792198278\\
5	55743.9041224712\\
4	67656.2884647296\\
3	80734.3771502692\\
2	99957.0007078124\\
1	151841.655115874\\
}--cycle;
\addplot [color=red]
  table[row sep=crcr]{%
1	95440\\
2	63082\\
3	53928\\
4	45363\\
5	37010\\
6	28975\\
7	25871\\
8	23303\\
9	22447\\
10	19858\\
11	19858\\
12	19382\\
13	17950\\
14	16786\\
15	16496\\
16	14680\\
17	14624\\
18	14624\\
19	14624\\
20	14624\\
21	14624\\
22	14225\\
23	13960\\
24	13958\\
25	13958\\
26	13958\\
27	13336\\
28	13336\\
29	12864\\
30	12711\\
31	12711\\
32	12711\\
33	12669\\
34	12475\\
35	12475\\
36	12475\\
37	11780\\
38	11780\\
39	11780\\
40	11780\\
41	11780\\
42	11780\\
43	11780\\
44	11780\\
45	11760\\
46	11760\\
47	11760\\
48	11760\\
49	11760\\
50	11509\\
51	11413\\
52	11413\\
53	11285\\
54	11285\\
55	11285\\
56	11285\\
57	11116\\
58	11116\\
59	11116\\
60	11116\\
61	11116\\
62	11096\\
63	11043\\
64	11034\\
65	11034\\
66	11034\\
67	11034\\
68	11034\\
69	11034\\
70	11034\\
71	10999\\
72	10999\\
73	10999\\
74	10999\\
75	10744\\
76	10430\\
77	10430\\
78	10430\\
79	10117\\
80	10117\\
81	10117\\
82	9801\\
83	9801\\
84	9779\\
85	9654\\
86	9654\\
87	9654\\
88	9654\\
89	9615\\
90	9482\\
91	9404\\
92	9404\\
93	9404\\
94	9316\\
95	9316\\
96	9316\\
97	9316\\
98	9316\\
99	9037\\
100	8742\\
};
\addlegendentry{muscles, c = 0.15 s}


\addplot[area legend, draw=none, fill=black!50!red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	32409.9773523096\\
2	19093.726710256\\
3	19490.7276556974\\
4	19638.8246850694\\
5	19510.9739545577\\
6	18272.7309347136\\
7	16857.673610433\\
8	17838.2073208368\\
9	17002.3758813245\\
10	16133.8355074427\\
11	14612.118037285\\
12	14585.0179561027\\
13	13267.5912769976\\
14	13287.8137005144\\
15	13163.8509002434\\
16	12719.839733898\\
17	11284.7946556503\\
18	11171.4680828372\\
19	11171.4680828372\\
20	10945.7008094498\\
21	10945.7008094498\\
22	11126.6601902055\\
23	10536.4693943565\\
24	10536.4693943565\\
25	10536.4693943565\\
26	10058.511901203\\
27	10036.0932842277\\
28	9313.03714637765\\
29	9313.03714637765\\
30	9184.26588542084\\
31	9184.26588542084\\
32	9184.26588542084\\
33	9872.52793281687\\
34	9872.52793281687\\
35	9872.52793281687\\
36	9872.52793281687\\
37	9872.52793281687\\
38	9872.52793281687\\
39	9406.53655512588\\
40	9406.53655512588\\
41	8749.56011319259\\
42	8749.56011319259\\
43	8749.56011319259\\
44	8501.69280572227\\
45	8501.69280572227\\
46	8119.8777065336\\
47	8119.8777065336\\
48	8119.8777065336\\
49	8098.68836669767\\
50	8098.68836669767\\
51	8098.68836669767\\
52	7577.75485877996\\
53	7358.96429174964\\
54	7358.96429174964\\
55	7358.96429174964\\
56	7289.29641842024\\
57	7045.7769341272\\
58	7045.7769341272\\
59	6618.1542221581\\
60	6432.76618513758\\
61	6432.76618513758\\
62	6494.74482124043\\
63	6343.95734865338\\
64	6232.3725763929\\
65	5681.42487796507\\
66	5330.12875535045\\
67	5330.12875535045\\
68	5330.12875535045\\
69	5229.52183453016\\
70	5364.70270182742\\
71	5364.70270182742\\
72	5341.13636230651\\
73	5326.78533202575\\
74	5124.38361638911\\
75	5314.07868439254\\
76	5306.57551306739\\
77	5297.58132590791\\
78	5167.88308768613\\
79	5157.00974458699\\
80	5130.24695451394\\
81	5130.24695451394\\
82	5132.69108438804\\
83	5020.96198055196\\
84	5003.43437766377\\
85	4970.83455232328\\
86	5012.85236819907\\
87	4928.38329319778\\
88	4768.2850455299\\
89	4751.7894636527\\
90	4736.69251764955\\
91	4695.55157455806\\
92	4682.30458059491\\
93	4698.159680853\\
94	4649.19172711406\\
95	4614.58843295227\\
96	4528.81049890763\\
97	4485.12657521981\\
98	4500.82641944397\\
99	4441.44852888779\\
100	4436.15215882098\\
100	5754.75462825104\\
99	5755.27807145481\\
98	5754.50453738665\\
97	5813.00760814349\\
96	5815.80086436887\\
95	5822.93375355553\\
94	5829.60016627109\\
93	5918.7357285139\\
92	6221.36222946063\\
91	6267.50448101428\\
90	6269.35111167784\\
89	6270.55492865522\\
88	6272.23864811564\\
87	6319.92391961456\\
86	6324.04469099616\\
85	6567.11448948958\\
84	6713.82510607201\\
83	6720.26490858573\\
82	6754.06889083278\\
81	6948.65205659272\\
80	6948.65205659272\\
79	6960.0855694229\\
78	6965.40197699144\\
77	7341.80508613118\\
76	7344.27509780744\\
75	7442.5209334096\\
74	8247.36416104403\\
73	8256.99355880185\\
72	8258.72146825739\\
71	8263.1027860579\\
70	8263.1027860579\\
69	8721.72458919496\\
68	8740.27998969953\\
67	8740.27998969953\\
66	8740.27998969953\\
65	8865.0656814271\\
64	9045.26000907318\\
63	9051.52871561925\\
62	9133.08474918637\\
61	9428.19807021419\\
60	9428.19807021419\\
59	10303.2029041642\\
58	10735.7308260243\\
57	10735.7308260243\\
56	10838.2223744768\\
55	10831.6780332972\\
54	10831.6780332972\\
53	10831.6780332972\\
52	11055.3959493616\\
51	11155.9229671021\\
50	11155.9229671021\\
49	11155.9229671021\\
48	11681.0911611214\\
47	11681.0911611214\\
46	11681.0911611214\\
45	12068.0138622615\\
44	12068.0138622615\\
43	11997.0975826076\\
42	11997.0975826076\\
41	11997.0975826076\\
40	12027.6724886677\\
39	12027.6724886677\\
38	11887.4304316495\\
37	11887.4304316495\\
36	11887.4304316495\\
35	11887.4304316495\\
34	11887.4304316495\\
33	11887.4304316495\\
32	14959.5585320706\\
31	14959.5585320706\\
30	14959.5585320706\\
29	19862.2188052406\\
28	19862.2188052406\\
27	19884.581790272\\
26	19897.6885432724\\
25	20309.4315060871\\
24	20309.4315060871\\
23	20309.4315060871\\
22	20383.7799196153\\
21	20982.7870061961\\
20	20982.7870061961\\
19	21151.9923946855\\
18	21151.9923946855\\
17	21260.8890101233\\
16	22157.7658802488\\
15	22526.8182118585\\
14	22692.003273735\\
13	24466.7834446847\\
12	24293.4396249346\\
11	24344.6205578556\\
10	25175.8694996602\\
9	30026.1720360182\\
8	30334.2455935335\\
7	40607.0752839117\\
6	40770.4802818937\\
5	44572.9238979105\\
4	57225.5377678844\\
3	71772.9658040574\\
2	93833.131679137\\
1	96788.6155752725\\
}--cycle;
\addplot [color=black!50!red]
  table[row sep=crcr]{%
1	64599\\
2	56463\\
3	45632\\
4	38432\\
5	32042\\
6	29522\\
7	28732\\
8	24086\\
9	23514\\
10	20655\\
11	19478\\
12	19439\\
13	18867\\
14	17990\\
15	17845\\
16	17439\\
17	16273\\
18	16162\\
19	16162\\
20	15964\\
21	15964\\
22	15755\\
23	15423\\
24	15423\\
25	15423\\
26	14978\\
27	14960\\
28	14588\\
29	14588\\
30	12072\\
31	12072\\
32	12072\\
33	10880\\
34	10880\\
35	10880\\
36	10880\\
37	10880\\
38	10880\\
39	10717\\
40	10717\\
41	10373\\
42	10373\\
43	10373\\
44	10285\\
45	10285\\
46	9900\\
47	9900\\
48	9900\\
49	9627\\
50	9627\\
51	9627\\
52	9317\\
53	9095\\
54	9095\\
55	9095\\
56	9064\\
57	8891\\
58	8891\\
59	8461\\
60	7930\\
61	7930\\
62	7814\\
63	7698\\
64	7639\\
65	7273\\
66	7035\\
67	7035\\
68	7035\\
69	6976\\
70	6814\\
71	6814\\
72	6800\\
73	6792\\
74	6686\\
75	6378\\
76	6325\\
77	6320\\
78	6067\\
79	6059\\
80	6039\\
81	6039\\
82	5943\\
83	5871\\
84	5859\\
85	5769\\
86	5668\\
87	5624\\
88	5520\\
89	5511\\
90	5503\\
91	5482\\
92	5452\\
93	5308\\
94	5239\\
95	5219\\
96	5172\\
97	5149\\
98	5128\\
99	5098\\
100	5095\\
};
\addlegendentry{muscles, c = 0.3 s}

\legend{}
\end{axis}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}


==> new_figures/dataefficiency_cost_pointreaching_modifs0_05.tex <==
\begin{axis}[%
name =ax3,
scaled y ticks=base 10:\Factor,
at={(ax2.south east)},
xlabel near ticks, ylabel near ticks,
every y tick scale label/.style={at={(yticklabel* cs:1.03,0cm)},anchor=near yticklabel},
title style={at={(0.5,0.93)}},
xshift=1cm,
width=0.951\figW,
height=\figH,
scale only axis,
xmin=0,
xmax=100,
xtick={  0,  20,  40,  60,  80, 100},
xlabel style={font=\color{white!15!black}},
xlabel={generations},
ymin=0,
ymax=3000,
ylabel style={font=\color{white!15!black}},
ylabel={cost},
axis background/.style={fill=white},
title={pointreaching, c = 0.05 s},
legend style={legend cell align=left, align=left, draw=white!15!black}
]

\addplot[area legend, draw=none, fill=red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	642.866578749281\\
2	590.707193481988\\
3	497.921988153405\\
4	445.005763842037\\
5	420.417487833177\\
6	389.725041192492\\
7	371.539056706871\\
8	329.842506045259\\
9	311.403918943119\\
10	295.89834525183\\
11	276.848715334484\\
12	281.252041995415\\
13	281.296649806739\\
14	263.488368866393\\
15	254.245991440816\\
16	256.343363484288\\
17	237.97692486871\\
18	241.70256985005\\
19	240.647614805128\\
20	241.859693010864\\
21	248.001485120905\\
22	248.001485120905\\
23	248.001485120905\\
24	233.241782902748\\
25	234.862553381831\\
26	236.668953913741\\
27	237.391457000369\\
28	237.60706265212\\
29	237.60706265212\\
30	237.60706265212\\
31	237.60706265212\\
32	237.60706265212\\
33	239.635802139177\\
34	239.635802139177\\
35	239.635802139177\\
36	239.635802139177\\
37	240.300423974689\\
38	237.75733081042\\
39	237.395292979239\\
40	236.153147368055\\
41	236.244085834875\\
42	231.622237623476\\
43	232.173825445932\\
44	230.8410727162\\
45	230.8410727162\\
46	228.369999624787\\
47	228.369999624787\\
48	228.369999624787\\
49	228.369999624787\\
50	228.369999624787\\
51	228.369999624787\\
52	228.369999624787\\
53	228.493594128341\\
54	227.162686523694\\
55	227.057427886947\\
56	225.293415311547\\
57	225.293415311547\\
58	225.293415311547\\
59	225.293415311547\\
60	225.293415311547\\
61	221.152894167682\\
62	221.152894167682\\
63	221.152894167682\\
64	221.152894167682\\
65	221.152894167682\\
66	221.152894167682\\
67	221.152894167682\\
68	221.152894167682\\
69	221.152894167682\\
70	221.152894167682\\
71	222.219974038653\\
72	222.219974038653\\
73	222.378843808914\\
74	222.258097001116\\
75	222.258097001116\\
76	222.258097001116\\
77	222.258097001116\\
78	222.258097001116\\
79	222.258097001116\\
80	222.258097001116\\
81	222.258097001116\\
82	222.258097001116\\
83	222.258097001116\\
84	222.258097001116\\
85	222.258097001116\\
86	222.258097001116\\
87	222.038864351467\\
88	222.038864351467\\
89	222.038864351467\\
90	222.038864351467\\
91	222.038864351467\\
92	221.561931523725\\
93	221.561931523725\\
94	219.107645306085\\
95	219.107645306085\\
96	219.107645306085\\
97	218.551554071215\\
98	218.551554071215\\
99	218.551554071215\\
100	218.541687062182\\
100	233.484018340512\\
99	234.342381367368\\
98	234.342381367368\\
97	234.342381367368\\
96	234.195193499767\\
95	234.195193499767\\
94	234.195193499767\\
93	234.219807040601\\
92	234.219807040601\\
91	234.097804534797\\
90	234.097804534797\\
89	234.097804534797\\
88	234.097804534797\\
87	234.097804534797\\
86	238.355888889135\\
85	238.355888889135\\
84	238.355888889135\\
83	238.355888889135\\
82	238.355888889135\\
81	238.355888889135\\
80	238.355888889135\\
79	238.355888889135\\
78	238.355888889135\\
77	238.355888889135\\
76	238.355888889135\\
75	238.355888889135\\
74	238.355888889135\\
73	238.733955364523\\
72	240.393883739207\\
71	240.393883739207\\
70	246.59566182251\\
69	246.59566182251\\
68	246.59566182251\\
67	246.59566182251\\
66	246.59566182251\\
65	246.59566182251\\
64	246.59566182251\\
63	246.59566182251\\
62	246.59566182251\\
61	246.59566182251\\
60	276.995275940653\\
59	276.995275940653\\
58	276.995275940653\\
57	276.995275940653\\
56	276.995275940653\\
55	276.522611455776\\
54	280.269800842792\\
53	280.049081384413\\
52	283.121611738339\\
51	283.121611738339\\
50	283.121611738339\\
49	283.121611738339\\
48	283.121611738339\\
47	283.121611738339\\
46	283.121611738339\\
45	282.481517614534\\
44	282.481517614534\\
43	294.201324879307\\
42	305.095980042663\\
41	307.590651712899\\
40	309.029887748045\\
39	308.709325727702\\
38	310.030731488143\\
37	322.447871217492\\
36	326.618010760745\\
35	326.618010760745\\
34	326.618010760745\\
33	326.618010760745\\
32	337.698222204513\\
31	337.698222204513\\
30	337.698222204513\\
29	337.698222204513\\
28	337.698222204513\\
27	338.789463344671\\
26	342.367186796002\\
25	350.909420842945\\
24	358.23502910277\\
23	358.752321310398\\
22	358.752321310398\\
21	358.752321310398\\
20	411.473275587299\\
19	416.185652305174\\
18	442.705442423782\\
17	465.702880690611\\
16	484.714013384724\\
15	501.729685754669\\
14	544.222344963036\\
13	545.385846119312\\
12	594.92757723156\\
11	617.558009627804\\
10	645.954988072133\\
9	715.105245298374\\
8	814.891404727537\\
7	870.837355269283\\
6	890.045209231861\\
5	918.387016969088\\
4	971.682344630206\\
3	1014.61991872096\\
2	1053.81588791214\\
1	1152.09680323745\\
}--cycle;
\addplot [color=red]
  table[row sep=crcr]{%
1	897\\
2	822\\
3	756\\
4	708\\
5	669\\
6	640\\
7	621\\
8	572\\
9	513\\
10	471\\
11	447\\
12	438\\
13	413\\
14	404\\
15	378\\
16	371\\
17	352\\
18	342\\
19	328\\
20	327\\
21	303\\
22	303\\
23	303\\
24	296\\
25	293\\
26	290\\
27	288\\
28	288\\
29	288\\
30	288\\
31	288\\
32	288\\
33	283\\
34	283\\
35	283\\
36	283\\
37	281\\
38	274\\
39	273\\
40	273\\
41	272\\
42	268\\
43	263\\
44	257\\
45	257\\
46	256\\
47	256\\
48	256\\
49	256\\
50	256\\
51	256\\
52	256\\
53	254\\
54	254\\
55	252\\
56	251\\
57	251\\
58	251\\
59	251\\
60	251\\
61	234\\
62	234\\
63	234\\
64	234\\
65	234\\
66	234\\
67	234\\
68	234\\
69	234\\
70	234\\
71	231\\
72	231\\
73	231\\
74	230\\
75	230\\
76	230\\
77	230\\
78	230\\
79	230\\
80	230\\
81	230\\
82	230\\
83	230\\
84	230\\
85	230\\
86	230\\
87	228\\
88	228\\
89	228\\
90	228\\
91	228\\
92	228\\
93	228\\
94	227\\
95	227\\
96	227\\
97	226\\
98	226\\
99	226\\
100	226\\
};
\addlegendentry{muscles}


\addplot[area legend, draw=none, fill=mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	3619.05743823495\\
2	2636.20738241187\\
3	2162.82232385495\\
4	1955.92727377236\\
5	1328.73423534295\\
6	1200.58211556448\\
7	1200.58211556448\\
8	1200.58211556448\\
9	1200.58211556448\\
10	1100.75243615817\\
11	1100.75243615817\\
12	1054.10928661941\\
13	1054.10928661941\\
14	1054.10928661941\\
15	1054.10928661941\\
16	1058.39211932963\\
17	1058.39211932963\\
18	1058.39211932963\\
19	1058.39211932963\\
20	1057.43736797524\\
21	1057.43736797524\\
22	995.27249034752\\
23	980.915293047479\\
24	986.51270573265\\
25	908.529557865736\\
26	908.529557865736\\
27	870.22873396208\\
28	900.198694670013\\
29	874.875074384925\\
30	835.614050799492\\
31	835.614050799492\\
32	836.275342105298\\
33	836.275342105298\\
34	836.221484161008\\
35	798.633228748723\\
36	798.633228748723\\
37	784.082381824754\\
38	784.082381824754\\
39	784.082381824754\\
40	784.082381824754\\
41	784.082381824754\\
42	787.254518168369\\
43	790.269444561684\\
44	790.269444561684\\
45	790.269444561684\\
46	790.269444561684\\
47	767.10365168895\\
48	767.10365168895\\
49	761.536389831056\\
50	782.107181332705\\
51	782.763008556772\\
52	782.763008556772\\
53	782.763008556772\\
54	782.249338990118\\
55	758.437771438699\\
56	758.437771438699\\
57	722.303915716928\\
58	721.563686955837\\
59	715.986061938968\\
60	695.243995746983\\
61	666.601866276671\\
62	666.601866276671\\
63	656.498808185896\\
64	656.813087215282\\
65	645.621972325175\\
66	643.238031272534\\
67	641.374762241729\\
68	622.665319341988\\
69	622.665319341988\\
70	617.544243684146\\
71	614.088991717277\\
72	601.801681946432\\
73	572.990479275375\\
74	564.645864089157\\
75	564.645864089157\\
76	555.584088330034\\
77	555.584088330034\\
78	557.322696314148\\
79	558.785055846485\\
80	549.630350085581\\
81	549.942603544811\\
82	551.527523173501\\
83	551.527523173501\\
84	551.74913624288\\
85	534.186573038847\\
86	534.186573038847\\
87	532.842876697007\\
88	531.447158386545\\
89	523.852200518069\\
90	523.852200518069\\
91	523.746411626629\\
92	521.9941004721\\
93	523.673832989532\\
94	523.673832989532\\
95	523.673832989532\\
96	523.073448508201\\
97	523.402838137374\\
98	523.382804323258\\
99	522.298798277848\\
100	526.310889098176\\
100	567.641917239045\\
99	583.277164945479\\
98	596.312471559173\\
97	596.32019173821\\
96	597.628458346799\\
95	597.863471695689\\
94	597.863471695689\\
93	597.863471695689\\
92	616.294003361161\\
91	616.216426654796\\
90	616.2125896125\\
89	616.2125896125\\
88	616.520651789874\\
87	616.798495780774\\
86	617.11720423739\\
85	617.11720423739\\
84	660.655946623924\\
83	662.812864715529\\
82	662.812864715529\\
81	668.777330106638\\
80	669.951679889054\\
79	670.351055633457\\
78	675.812113318389\\
77	689.876579240037\\
76	689.876579240037\\
75	691.516760278436\\
74	691.516760278436\\
73	694.588631371458\\
72	693.120020665199\\
71	695.245682461409\\
70	701.537133503401\\
69	705.458563898319\\
68	705.458563898319\\
67	702.183804838449\\
66	703.257312810037\\
65	717.707422506957\\
64	727.101358597325\\
63	729.43151826189\\
62	735.218152931183\\
61	735.218152931183\\
60	727.821095880521\\
59	733.672310187571\\
58	757.167757782914\\
57	757.441530686758\\
56	788.045390126426\\
55	788.045390126426\\
54	796.759329856547\\
53	796.671783968295\\
52	796.671783968295\\
51	796.671783968295\\
50	799.456816916122\\
49	878.149245218218\\
48	879.057736231217\\
47	879.057736231217\\
46	892.421925127425\\
45	892.421925127425\\
44	892.421925127425\\
43	892.421925127425\\
42	904.388717995852\\
41	916.792469478679\\
40	916.792469478679\\
39	916.792469478679\\
38	916.792469478679\\
37	916.792469478679\\
36	921.913199718419\\
35	921.913199718419\\
34	954.682991370727\\
33	955.252164413491\\
32	955.252164413491\\
31	982.939325777429\\
30	982.939325777429\\
29	1011.58783431544\\
28	1009.05934068571\\
27	1219.4639834224\\
26	1240.85577842995\\
25	1240.85577842995\\
24	1230.22361915064\\
23	1251.75655010071\\
22	1256.62930808706\\
21	1313.38473032201\\
20	1313.38473032201\\
19	1320.6997117982\\
18	1320.6997117982\\
17	1320.6997117982\\
16	1320.6997117982\\
15	1410.77406473653\\
14	1410.77406473653\\
13	1410.77406473653\\
12	1410.77406473653\\
11	1606.52185524545\\
10	1606.52185524545\\
9	1616.98159180459\\
8	1616.98159180459\\
7	1616.98159180459\\
6	1616.98159180459\\
5	2125.31584059348\\
4	3409.71541789831\\
3	3453.60757274624\\
2	3522.07063352559\\
1	4960.87919070535\\
}--cycle;
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	4290\\
2	3079\\
3	2808\\
4	2683\\
5	1727\\
6	1409\\
7	1409\\
8	1409\\
9	1409\\
10	1354\\
11	1354\\
12	1232\\
13	1232\\
14	1232\\
15	1232\\
16	1190\\
17	1190\\
18	1190\\
19	1190\\
20	1185\\
21	1185\\
22	1126\\
23	1116\\
24	1108\\
25	1075\\
26	1075\\
27	1045\\
28	955\\
29	943\\
30	909\\
31	909\\
32	896\\
33	896\\
34	895\\
35	860\\
36	860\\
37	850\\
38	850\\
39	850\\
40	850\\
41	850\\
42	846\\
43	841\\
44	841\\
45	841\\
46	841\\
47	823\\
48	823\\
49	820\\
50	791\\
51	790\\
52	790\\
53	790\\
54	790\\
55	773\\
56	773\\
57	740\\
58	739\\
59	725\\
60	712\\
61	701\\
62	701\\
63	693\\
64	692\\
65	682\\
66	673\\
67	672\\
68	664\\
69	664\\
70	660\\
71	655\\
72	647\\
73	634\\
74	628\\
75	628\\
76	623\\
77	623\\
78	617\\
79	615\\
80	610\\
81	609\\
82	607\\
83	607\\
84	606\\
85	576\\
86	576\\
87	575\\
88	574\\
89	570\\
90	570\\
91	570\\
92	569\\
93	561\\
94	561\\
95	561\\
96	560\\
97	560\\
98	560\\
99	553\\
100	547\\
};
\addlegendentry{torques}


\addplot[area legend, draw=none, fill=mycolor2, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	987.578506111497\\
2	759.371962060912\\
3	537.574994954481\\
4	445.979227164362\\
5	422.180038722295\\
6	400.711146346784\\
7	370.190423014177\\
8	367.084827237556\\
9	354.124805592198\\
10	348.959718767334\\
11	342.385756961685\\
12	342.026751249255\\
13	342.026751249255\\
14	337.598639576595\\
15	337.598639576595\\
16	325.105432974428\\
17	308.080550269266\\
18	308.122847229132\\
19	169.539009239549\\
20	178.627719249902\\
21	178.627719249902\\
22	178.627719249902\\
23	217.832644313319\\
24	217.832644313319\\
25	254.459795797069\\
26	254.459795797069\\
27	254.459795797069\\
28	259.631094133496\\
29	259.631094133496\\
30	261.927195614295\\
31	249.613935464651\\
32	249.613935464651\\
33	252.588863868752\\
34	252.588863868752\\
35	252.588863868752\\
36	252.588863868752\\
37	252.588863868752\\
38	252.588863868752\\
39	252.588863868752\\
40	249.983097067354\\
41	249.983097067354\\
42	249.983097067354\\
43	249.983097067354\\
44	249.983097067354\\
45	249.983097067354\\
46	251.568609163778\\
47	251.568609163778\\
48	248.646942218519\\
49	248.646942218519\\
50	248.646942218519\\
51	251.093385516442\\
52	251.093385516442\\
53	251.093385516442\\
54	251.093385516442\\
55	251.093385516442\\
56	251.093385516442\\
57	251.093385516442\\
58	250.713021133043\\
59	250.713021133043\\
60	250.713021133043\\
61	250.713021133043\\
62	250.713021133043\\
63	250.713021133043\\
64	250.713021133043\\
65	250.713021133043\\
66	251.64775757918\\
67	251.64775757918\\
68	251.64775757918\\
69	251.64775757918\\
70	251.64775757918\\
71	251.64775757918\\
72	251.64775757918\\
73	251.64775757918\\
74	251.64775757918\\
75	251.376842077825\\
76	251.376842077825\\
77	251.376842077825\\
78	251.376842077825\\
79	251.376842077825\\
80	250.90499123434\\
81	251.74333820585\\
82	251.74333820585\\
83	251.74333820585\\
84	251.74333820585\\
85	251.74333820585\\
86	251.74333820585\\
87	249.377006981784\\
88	249.377006981784\\
89	249.377006981784\\
90	249.377006981784\\
91	249.377006981784\\
92	249.377006981784\\
93	249.377006981784\\
94	249.377006981784\\
95	249.377006981784\\
96	249.377006981784\\
97	249.377006981784\\
98	250.496379252499\\
99	250.496379252499\\
100	250.496379252499\\
100	257.245125275379\\
99	257.245125275379\\
98	257.245125275379\\
97	261.857332120015\\
96	261.857332120015\\
95	261.857332120015\\
94	261.857332120015\\
93	261.857332120015\\
92	261.857332120015\\
91	261.857332120015\\
90	261.857332120015\\
89	261.857332120015\\
88	261.857332120015\\
87	261.857332120015\\
86	265.918032092303\\
85	265.918032092303\\
84	265.918032092303\\
83	265.918032092303\\
82	265.918032092303\\
81	265.918032092303\\
80	274.487868037433\\
79	275.106985260763\\
78	275.106985260763\\
77	275.106985260763\\
76	275.106985260763\\
75	275.106985260763\\
74	275.556731010682\\
73	275.556731010682\\
72	275.556731010682\\
71	275.556731010682\\
70	275.556731010682\\
69	275.556731010682\\
68	275.556731010682\\
67	275.556731010682\\
66	275.556731010682\\
65	280.915482086774\\
64	280.915482086774\\
63	280.915482086774\\
62	280.915482086774\\
61	280.915482086774\\
60	280.915482086774\\
59	280.915482086774\\
58	280.915482086774\\
57	281.337218096041\\
56	281.337218096041\\
55	281.337218096041\\
54	281.337218096041\\
53	281.337218096041\\
52	281.337218096041\\
51	281.337218096041\\
50	292.779391190216\\
49	292.779391190216\\
48	292.779391190216\\
47	292.367273391767\\
46	292.367273391767\\
45	298.756513159358\\
44	298.756513159358\\
43	298.756513159358\\
42	298.756513159358\\
41	298.756513159358\\
40	298.756513159358\\
39	300.073154700619\\
38	300.073154700619\\
37	300.073154700619\\
36	300.073154700619\\
35	300.073154700619\\
34	300.073154700619\\
33	300.073154700619\\
32	312.516897191953\\
31	312.516897191953\\
30	311.899353847978\\
29	320.471252939363\\
28	320.471252939363\\
27	339.774403981774\\
26	339.774403981774\\
25	339.774403981774\\
24	476.47479562254\\
23	476.47479562254\\
22	622.79080164106\\
21	622.79080164106\\
20	622.79080164106\\
19	656.710481023929\\
18	912.289583390342\\
17	912.740958221579\\
16	1019.99244364555\\
15	1191.10496433034\\
14	1191.10496433034\\
13	1293.54756560219\\
12	1293.54756560219\\
11	1366.91615577835\\
10	1413.65590873973\\
9	1438.89925469472\\
8	1578.31727112955\\
7	1613.9692930052\\
6	1636.57241888183\\
5	1703.36249764259\\
4	1885.15211308462\\
3	2131.6054066985\\
2	2177.68919631217\\
1	2279.38931529364\\
}--cycle;
\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	1633\\
2	1469\\
3	1335\\
4	1166\\
5	1063\\
6	1019\\
7	992\\
8	973\\
9	897\\
10	881\\
11	855\\
12	818\\
13	818\\
14	764\\
15	764\\
16	673\\
17	610\\
18	610\\
19	413\\
20	401\\
21	401\\
22	401\\
23	347\\
24	347\\
25	297\\
26	297\\
27	297\\
28	290\\
29	290\\
30	287\\
31	281\\
32	281\\
33	276\\
34	276\\
35	276\\
36	276\\
37	276\\
38	276\\
39	276\\
40	274\\
41	274\\
42	274\\
43	274\\
44	274\\
45	274\\
46	272\\
47	272\\
48	271\\
49	271\\
50	271\\
51	266\\
52	266\\
53	266\\
54	266\\
55	266\\
56	266\\
57	266\\
58	266\\
59	266\\
60	266\\
61	266\\
62	266\\
63	266\\
64	266\\
65	266\\
66	264\\
67	264\\
68	264\\
69	264\\
70	264\\
71	264\\
72	264\\
73	264\\
74	264\\
75	263\\
76	263\\
77	263\\
78	263\\
79	263\\
80	263\\
81	259\\
82	259\\
83	259\\
84	259\\
85	259\\
86	259\\
87	256\\
88	256\\
89	256\\
90	256\\
91	256\\
92	256\\
93	256\\
94	256\\
95	256\\
96	256\\
97	256\\
98	254\\
99	254\\
100	254\\
};
\addlegendentry{no Fl}


\addplot[area legend, draw=none, fill=red!50!mycolor2, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	432.735611278581\\
2	391.250082784748\\
3	365.04040866047\\
4	330.174649779079\\
5	316.80934971498\\
6	302.712813634785\\
7	287.885927936067\\
8	276.227325269678\\
9	264.215503556908\\
10	250.90282398733\\
11	250.905203170123\\
12	250.675264870128\\
13	248.697725835537\\
14	235.709258822862\\
15	235.401700710818\\
16	234.112856187943\\
17	233.162992278333\\
18	222.220536509819\\
19	221.928853393006\\
20	221.880151243745\\
21	221.880151243745\\
22	221.880151243745\\
23	219.77166983165\\
24	219.77166983165\\
25	219.77166983165\\
26	219.610973247936\\
27	219.53020708352\\
28	219.53020708352\\
29	219.53020708352\\
30	219.389360153508\\
31	218.931883601745\\
32	218.931883601745\\
33	218.931883601745\\
34	218.931883601745\\
35	218.668445042818\\
36	218.469537352997\\
37	218.185555231863\\
38	218.185555231863\\
39	217.453870734013\\
40	217.005585352093\\
41	217.005585352093\\
42	217.005585352093\\
43	217.005585352093\\
44	217.005585352093\\
45	217.005585352093\\
46	217.005585352093\\
47	207.519734077219\\
48	207.559445749057\\
49	206.959057104314\\
50	207.06489417974\\
51	204.908272308278\\
52	204.908272308278\\
53	204.908272308278\\
54	204.958097152277\\
55	204.838164351015\\
56	204.838164351015\\
57	204.289677705823\\
58	203.547834181291\\
59	203.547834181291\\
60	203.547834181291\\
61	203.547834181291\\
62	203.547834181291\\
63	203.547834181291\\
64	201.831764513357\\
65	198.941803559864\\
66	194.934275922818\\
67	194.934275922818\\
68	195.091108853213\\
69	195.091108853213\\
70	195.091108853213\\
71	195.091108853213\\
72	195.151739596866\\
73	192.5779466916\\
74	192.5779466916\\
75	192.5779466916\\
76	192.5779466916\\
77	192.5779466916\\
78	192.5779466916\\
79	192.5779466916\\
80	192.5779466916\\
81	192.5779466916\\
82	192.5779466916\\
83	192.5779466916\\
84	192.5779466916\\
85	192.5779466916\\
86	192.5779466916\\
87	192.5779466916\\
88	192.5779466916\\
89	192.5779466916\\
90	192.5779466916\\
91	191.866104601598\\
92	191.866104601598\\
93	191.866104601598\\
94	192.22178630903\\
95	192.22178630903\\
96	186.731672542492\\
97	186.731672542492\\
98	186.731672542492\\
99	187.255482987044\\
100	187.255482987044\\
100	222.312267794734\\
99	222.312267794734\\
98	227.885113015177\\
97	227.885113015177\\
96	227.885113015177\\
95	226.583846022614\\
94	226.583846022614\\
93	228.704440295388\\
92	228.704440295388\\
91	228.704440295388\\
90	228.548994349091\\
89	228.548994349091\\
88	228.548994349091\\
87	228.548994349091\\
86	228.548994349091\\
85	228.548994349091\\
84	228.548994349091\\
83	228.548994349091\\
82	228.548994349091\\
81	228.548994349091\\
80	228.548994349091\\
79	228.548994349091\\
78	228.548994349091\\
77	228.548994349091\\
76	228.548994349091\\
75	228.548994349091\\
74	228.548994349091\\
73	228.548994349091\\
72	241.753008124107\\
71	242.798482129184\\
70	242.798482129184\\
69	242.798482129184\\
68	242.798482129184\\
67	244.777586377273\\
66	244.777586377273\\
65	243.76608516283\\
64	243.046506097821\\
63	253.779379392023\\
62	253.779379392023\\
61	253.779379392023\\
60	253.779379392023\\
59	253.779379392023\\
58	253.779379392023\\
57	267.05697918576\\
56	271.585367631728\\
55	271.585367631728\\
54	274.800536649413\\
53	278.380039146482\\
52	278.380039146482\\
51	278.380039146482\\
50	277.813297509108\\
49	279.891905025569\\
48	282.518006899076\\
47	284.014945264105\\
46	281.527821964297\\
45	281.527821964297\\
44	281.527821964297\\
43	281.527821964297\\
42	281.527821964297\\
41	281.527821964297\\
40	281.527821964297\\
39	283.633913812575\\
38	296.151480640336\\
37	296.151480640336\\
36	297.683176692093\\
35	299.013331875202\\
34	301.414089160604\\
33	301.414089160604\\
32	301.414089160604\\
31	301.414089160604\\
30	301.291539845011\\
29	303.313046653366\\
28	303.313046653366\\
27	303.313046653366\\
26	305.442619291322\\
25	322.743538183705\\
24	322.743538183705\\
23	322.743538183705\\
22	336.031246622395\\
21	336.031246622395\\
20	336.031246622395\\
19	336.611806369826\\
18	343.588819664164\\
17	344.686222020658\\
16	356.841724919198\\
15	367.783791220356\\
14	373.792780177563\\
13	377.071698251963\\
12	395.72321094933\\
11	402.685771926388\\
10	403.391242615175\\
9	427.119032229811\\
8	447.088053677783\\
7	447.511907634087\\
6	454.447748575119\\
5	464.881237301576\\
4	497.425520623688\\
3	505.810229601008\\
2	499.057829975704\\
1	516.697767970644\\
}--cycle;
\addplot [color=red!50!mycolor2]
  table[row sep=crcr]{%
1	475\\
2	445\\
3	435\\
4	414\\
5	391\\
6	379\\
7	368\\
8	362\\
9	346\\
10	327\\
11	327\\
12	323\\
13	313\\
14	305\\
15	302\\
16	295\\
17	289\\
18	283\\
19	279\\
20	279\\
21	279\\
22	279\\
23	271\\
24	271\\
25	271\\
26	263\\
27	261\\
28	261\\
29	261\\
30	260\\
31	260\\
32	260\\
33	260\\
34	260\\
35	259\\
36	258\\
37	257\\
38	257\\
39	251\\
40	249\\
41	249\\
42	249\\
43	249\\
44	249\\
45	249\\
46	249\\
47	246\\
48	245\\
49	243\\
50	242\\
51	242\\
52	242\\
53	242\\
54	240\\
55	238\\
56	238\\
57	236\\
58	229\\
59	229\\
60	229\\
61	229\\
62	229\\
63	229\\
64	222\\
65	221\\
66	220\\
67	220\\
68	219\\
69	219\\
70	219\\
71	219\\
72	218\\
73	211\\
74	211\\
75	211\\
76	211\\
77	211\\
78	211\\
79	211\\
80	211\\
81	211\\
82	211\\
83	211\\
84	211\\
85	211\\
86	211\\
87	211\\
88	211\\
89	211\\
90	211\\
91	210\\
92	210\\
93	210\\
94	209\\
95	209\\
96	207\\
97	207\\
98	207\\
99	205\\
100	205\\
};
\addlegendentry{const r}


\addplot[area legend, draw=none, fill=mycolor3, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1280.54394418587\\
2	1253.4835580422\\
3	1283.21753283186\\
4	1320.17895303592\\
5	1297.34824187978\\
6	1297.34824187978\\
7	1297.34824187978\\
8	1191.35638416065\\
9	1191.35638416065\\
10	1199.928570523\\
11	1057.14438164483\\
12	1057.36197858773\\
13	1057.36197858773\\
14	1057.09717059123\\
15	1051.17888706313\\
16	1051.17888706313\\
17	1035.95660878441\\
18	1040.37742377648\\
19	1040.37742377648\\
20	1040.37742377648\\
21	1040.37742377648\\
22	1040.37742377648\\
23	1040.37742377648\\
24	1040.37742377648\\
25	1040.37742377648\\
26	1040.37742377648\\
27	1040.37742377648\\
28	1040.37742377648\\
29	1028.13635904719\\
30	1026.74217514214\\
31	1027.16109080005\\
32	1025.13767413407\\
33	1035.21844315363\\
34	1018.36645707941\\
35	1018.36645707941\\
36	1018.36645707941\\
37	1006.28651371567\\
38	1006.28651371567\\
39	1006.28651371567\\
40	1006.28651371567\\
41	1006.28651371567\\
42	1006.28651371567\\
43	1006.28651371567\\
44	1006.28651371567\\
45	1006.28651371567\\
46	1006.28651371567\\
47	973.582332197642\\
48	973.582332197642\\
49	973.582332197642\\
50	953.667845830782\\
51	953.667845830782\\
52	950.525623574953\\
53	940.374090533193\\
54	943.551805888213\\
55	943.551805888213\\
56	943.551805888213\\
57	929.19683849196\\
58	940.007823628413\\
59	940.007823628413\\
60	940.007823628413\\
61	940.007823628413\\
62	940.007823628413\\
63	945.965346427167\\
64	945.965346427167\\
65	953.505723393405\\
66	953.505723393405\\
67	956.03744544922\\
68	956.03744544922\\
69	956.03744544922\\
70	956.03744544922\\
71	956.03744544922\\
72	956.03744544922\\
73	956.03744544922\\
74	963.115309361373\\
75	963.115309361373\\
76	954.268598784587\\
77	963.443332522282\\
78	966.382993692336\\
79	966.382993692336\\
80	966.382993692336\\
81	966.382993692336\\
82	966.382993692336\\
83	966.382993692336\\
84	966.382993692336\\
85	966.382993692336\\
86	966.382993692336\\
87	966.382993692336\\
88	966.382993692336\\
89	967.146537322002\\
90	967.146537322002\\
91	967.805751056848\\
92	967.805751056848\\
93	967.805751056848\\
94	967.805751056848\\
95	967.805751056848\\
96	967.805751056848\\
97	968.206936407305\\
98	968.206936407305\\
99	968.236347090665\\
100	968.236347090665\\
100	1052.45584749845\\
99	1052.45584749845\\
98	1052.62024555921\\
97	1052.62024555921\\
96	1054.81973145188\\
95	1054.81973145188\\
94	1054.81973145188\\
93	1054.81973145188\\
92	1054.81973145188\\
91	1054.81973145188\\
90	1058.28912800615\\
89	1058.28912800615\\
88	1062.1372262045\\
87	1062.1372262045\\
86	1062.1372262045\\
85	1062.1372262045\\
84	1062.1372262045\\
83	1062.1372262045\\
82	1062.1372262045\\
81	1062.1372262045\\
80	1062.1372262045\\
79	1062.1372262045\\
78	1062.1372262045\\
77	1075.91405723091\\
76	1114.62664626752\\
75	1113.70614733216\\
74	1113.70614733216\\
73	1141.21219983029\\
72	1141.21219983029\\
71	1141.21219983029\\
70	1141.21219983029\\
69	1141.21219983029\\
68	1141.21219983029\\
67	1141.21219983029\\
66	1150.95346861231\\
65	1150.95346861231\\
64	1179.77789376782\\
63	1179.77789376782\\
62	1202.41386233065\\
61	1202.41386233065\\
60	1202.41386233065\\
59	1202.41386233065\\
58	1202.41386233065\\
57	1243.30019099245\\
56	1243.43013769346\\
55	1243.43013769346\\
54	1243.43013769346\\
53	1255.30954177736\\
52	1255.8879151422\\
51	1256.15994344522\\
50	1256.15994344522\\
49	1258.13503731568\\
48	1258.13503731568\\
47	1258.13503731568\\
46	1268.33369931456\\
45	1268.33369931456\\
44	1268.33369931456\\
43	1268.33369931456\\
42	1268.33369931456\\
41	1268.33369931456\\
40	1268.33369931456\\
39	1268.33369931456\\
38	1268.33369931456\\
37	1268.33369931456\\
36	1276.6198033478\\
35	1276.6198033478\\
34	1276.6198033478\\
33	1300.00029292168\\
32	1363.35991704961\\
31	1365.77003224959\\
30	1368.06640941724\\
29	1369.81031735837\\
28	1418.42750846342\\
27	1418.42750846342\\
26	1418.42750846342\\
25	1418.42750846342\\
24	1418.42750846342\\
23	1418.42750846342\\
22	1418.42750846342\\
21	1418.42750846342\\
20	1418.42750846342\\
19	1418.42750846342\\
18	1418.42750846342\\
17	1450.01006838887\\
16	1604.83560056371\\
15	1604.83560056371\\
14	1620.86690740506\\
13	1621.70012942502\\
12	1621.70012942502\\
11	1624.41678833603\\
10	1592.81180022574\\
9	1650.4292392558\\
8	1650.4292392558\\
7	1628.9834639472\\
6	1628.9834639472\\
5	1628.9834639472\\
4	1654.79918869887\\
3	1869.34788164072\\
2	1994.10419165522\\
1	2903.69045209899\\
}--cycle;
\addplot [color=mycolor3]
  table[row sep=crcr]{%
1	2092\\
2	1624\\
3	1576\\
4	1487\\
5	1463\\
6	1463\\
7	1463\\
8	1421\\
9	1421\\
10	1396\\
11	1341\\
12	1340\\
13	1340\\
14	1339\\
15	1328\\
16	1328\\
17	1243\\
18	1229\\
19	1229\\
20	1229\\
21	1229\\
22	1229\\
23	1229\\
24	1229\\
25	1229\\
26	1229\\
27	1229\\
28	1229\\
29	1199\\
30	1197\\
31	1196\\
32	1194\\
33	1168\\
34	1147\\
35	1147\\
36	1147\\
37	1137\\
38	1137\\
39	1137\\
40	1137\\
41	1137\\
42	1137\\
43	1137\\
44	1137\\
45	1137\\
46	1137\\
47	1116\\
48	1116\\
49	1116\\
50	1105\\
51	1105\\
52	1103\\
53	1098\\
54	1093\\
55	1093\\
56	1093\\
57	1086\\
58	1071\\
59	1071\\
60	1071\\
61	1071\\
62	1071\\
63	1063\\
64	1063\\
65	1052\\
66	1052\\
67	1049\\
68	1049\\
69	1049\\
70	1049\\
71	1049\\
72	1049\\
73	1049\\
74	1038\\
75	1038\\
76	1034\\
77	1020\\
78	1014\\
79	1014\\
80	1014\\
81	1014\\
82	1014\\
83	1014\\
84	1014\\
85	1014\\
86	1014\\
87	1014\\
88	1014\\
89	1013\\
90	1013\\
91	1011\\
92	1011\\
93	1011\\
94	1011\\
95	1011\\
96	1011\\
97	1010\\
98	1010\\
99	1010\\
100	1010\\
};
\addlegendentry{no Fv}


\addplot[area legend, draw=none, fill=red!50!mycolor3, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1204.61798514594\\
2	1206.3244916745\\
3	1162.64976106702\\
4	1148.318144638\\
5	902.747930536171\\
6	863.681899951815\\
7	826.120056432591\\
8	751.183250654134\\
9	748.768614159915\\
10	629.996408107125\\
11	599.129297100181\\
12	571.019842894471\\
13	478.765771107677\\
14	458.443081277232\\
15	446.69883436257\\
16	396.561570407025\\
17	384.283572534289\\
18	386.004080853254\\
19	381.100974962063\\
20	380.328259835127\\
21	356.144589175066\\
22	356.144589175066\\
23	356.144589175066\\
24	361.170901554035\\
25	361.170901554035\\
26	365.773017135612\\
27	332.496126746454\\
28	332.496126746454\\
29	332.496126746454\\
30	332.496126746454\\
31	311.324457955305\\
32	311.324457955305\\
33	317.91109965289\\
34	304.082048596106\\
35	289.390006468954\\
36	289.390006468954\\
37	289.390006468954\\
38	282.440078256365\\
39	282.440078256365\\
40	282.440078256365\\
41	282.440078256365\\
42	283.623606056265\\
43	293.292598137113\\
44	296.077277158262\\
45	295.91654522956\\
46	286.023778114667\\
47	271.529186177167\\
48	281.536864270126\\
49	286.269335766117\\
50	286.269335766117\\
51	296.170783941484\\
52	296.170783941484\\
53	296.170783941484\\
54	291.071699484053\\
55	290.543507134154\\
56	290.543507134154\\
57	290.543507134154\\
58	279.665459636714\\
59	279.665459636714\\
60	279.665459636714\\
61	279.665459636714\\
62	273.370310029798\\
63	273.370310029798\\
64	273.680398319534\\
65	273.680398319534\\
66	273.680398319534\\
67	267.753399483524\\
68	275.356473817355\\
69	275.356473817355\\
70	275.356473817355\\
71	278.298073594759\\
72	277.307127853404\\
73	277.307127853404\\
74	277.307127853404\\
75	277.307127853404\\
76	276.497179153281\\
77	276.497179153281\\
78	276.497179153281\\
79	276.497179153281\\
80	269.453648370852\\
81	271.343277201073\\
82	270.19885265897\\
83	268.777269857701\\
84	268.777269857701\\
85	268.777269857701\\
86	261.500693752716\\
87	263.714600014918\\
88	263.714600014918\\
89	263.714600014918\\
90	261.380388548185\\
91	253.995007611234\\
92	253.995007611234\\
93	253.995007611234\\
94	253.995007611234\\
95	252.547276170616\\
96	248.090014093216\\
97	248.090014093216\\
98	248.090014093216\\
99	248.090014093216\\
100	251.606762534519\\
100	281.290459993199\\
99	303.841733071315\\
98	303.841733071315\\
97	303.841733071315\\
96	303.841733071315\\
95	303.110502607457\\
94	303.418659857648\\
93	303.418659857648\\
92	303.418659857648\\
91	303.418659857648\\
90	302.474400334409\\
89	302.317246806239\\
88	302.317246806239\\
87	302.317246806239\\
86	310.730187130448\\
85	314.185039653556\\
84	314.185039653556\\
83	314.185039653556\\
82	315.873745445741\\
81	317.956577092042\\
80	331.96998073606\\
79	330.581003772181\\
78	330.581003772181\\
77	330.581003772181\\
76	330.581003772181\\
75	331.311671244508\\
74	331.311671244508\\
73	331.311671244508\\
72	331.311671244508\\
71	332.405037775202\\
70	351.09595412655\\
69	351.09595412655\\
68	351.09595412655\\
67	382.168655304919\\
66	384.999050412053\\
65	384.999050412053\\
64	384.999050412053\\
63	386.329788405506\\
62	386.329788405506\\
61	391.491490577982\\
60	391.491490577982\\
59	391.491490577982\\
58	391.491490577982\\
57	389.327062782872\\
56	389.327062782872\\
55	389.327062782872\\
54	389.799492616969\\
53	388.844040149998\\
52	388.844040149998\\
51	388.844040149998\\
50	430.784603311807\\
49	430.784603311807\\
48	449.63088646188\\
47	488.588382783425\\
46	494.290805928507\\
45	501.17211833532\\
44	501.31579121484\\
43	524.04343897482\\
42	565.46022573374\\
41	570.374789325554\\
40	570.374789325554\\
39	570.374789325554\\
38	570.374789325554\\
37	574.356430475173\\
36	574.356430475173\\
35	574.356430475173\\
34	587.09360750563\\
33	611.138442608049\\
32	660.213341852688\\
31	660.213341852688\\
30	655.458781622386\\
29	655.458781622386\\
28	655.458781622386\\
27	655.458781622386\\
26	685.727023572436\\
25	730.138176196795\\
24	730.138176196795\\
23	763.420950033891\\
22	763.420950033891\\
21	763.420950033891\\
20	844.902095444493\\
19	854.529844716668\\
18	961.233395807213\\
17	994.861702595332\\
16	1070.01200953368\\
15	1152.6720681816\\
14	1290.635446442\\
13	1353.30330233464\\
12	1359.45222656484\\
11	1423.13111971479\\
10	1486.9937201428\\
9	1636.90749419117\\
8	1659.22046011277\\
7	1725.5383107486\\
6	1780.0964030132\\
5	1866.94803838439\\
4	1879.97489703494\\
3	2028.33907086129\\
2	2103.83045164427\\
1	2151.84055953502\\
}--cycle;
\addplot [color=red!50!mycolor3]
  table[row sep=crcr]{%
1	1678\\
2	1655\\
3	1595\\
4	1514\\
5	1385\\
6	1322\\
7	1276\\
8	1205\\
9	1193\\
10	1058\\
11	1011\\
12	965\\
13	916\\
14	875\\
15	800\\
16	733\\
17	690\\
18	674\\
19	618\\
20	613\\
21	560\\
22	560\\
23	560\\
24	546\\
25	546\\
26	526\\
27	494\\
28	494\\
29	494\\
30	494\\
31	486\\
32	486\\
33	465\\
34	446\\
35	432\\
36	432\\
37	432\\
38	426\\
39	426\\
40	426\\
41	426\\
42	425\\
43	409\\
44	399\\
45	399\\
46	390\\
47	380\\
48	366\\
49	359\\
50	359\\
51	343\\
52	343\\
53	343\\
54	340\\
55	340\\
56	340\\
57	340\\
58	336\\
59	336\\
60	336\\
61	336\\
62	330\\
63	330\\
64	329\\
65	329\\
66	329\\
67	325\\
68	313\\
69	313\\
70	313\\
71	305\\
72	304\\
73	304\\
74	304\\
75	304\\
76	304\\
77	304\\
78	304\\
79	304\\
80	301\\
81	295\\
82	293\\
83	291\\
84	291\\
85	291\\
86	286\\
87	283\\
88	283\\
89	283\\
90	282\\
91	279\\
92	279\\
93	279\\
94	279\\
95	278\\
96	276\\
97	276\\
98	276\\
99	276\\
100	266\\
};
\addlegendentry{no actdyn}

\legend{}
\end{axis}


==> new_figures/dataefficiency_cost_pointreaching_modifs0_15.tex <==
\begin{axis}[%
name =ax2,
scaled y ticks=base 10:\Factor,
at={(ax1.south east)},
xlabel near ticks, ylabel near ticks,
every y tick scale label/.style={at={(yticklabel* cs:1.03,0cm)},anchor=near yticklabel},
title style={at={(0.5,0.93)}},
xshift=1cm,
width=0.951\figW,
height=\figH,
scale only axis,
xmin=0,
xmax=100,
xlabel style={font=\color{white!15!black}},
xlabel={\# generations},
ymin=0,
ymax=3000,
ylabel style={font=\color{white!15!black}},
ylabel={cost},
axis background/.style={fill=white},
title={pointreaching, c = 0.15 s},
legend style={legend cell align=left, align=left, draw=white!15!black}
]

\addplot[area legend, draw=none, fill=red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	384.747435246807\\
2	339.424854684054\\
3	300.422374193527\\
4	284.450527203695\\
5	263.099614353156\\
6	265.644393884321\\
7	249.943877589622\\
8	254.787569506639\\
9	259.307030365723\\
10	245.386067115261\\
11	245.432802595148\\
12	256.500550643941\\
13	248.015677273998\\
14	245.331560258835\\
15	245.331560258835\\
16	245.331560258835\\
17	247.807519913313\\
18	247.807519913313\\
19	247.807519913313\\
20	247.807519913313\\
21	247.937373223286\\
22	247.937373223286\\
23	247.937373223286\\
24	247.937373223286\\
25	247.937373223286\\
26	244.642611603449\\
27	243.801449409563\\
28	243.801449409563\\
29	243.801449409563\\
30	243.801449409563\\
31	243.801449409563\\
32	231.208812571634\\
33	231.208812571634\\
34	231.208812571634\\
35	231.208812571634\\
36	231.775664286117\\
37	231.775664286117\\
38	231.775664286117\\
39	231.775664286117\\
40	231.673316352279\\
41	231.673316352279\\
42	231.673316352279\\
43	231.673316352279\\
44	231.673316352279\\
45	231.704373704106\\
46	231.704373704106\\
47	231.704373704106\\
48	227.927131848709\\
49	227.927131848709\\
50	228.529557455665\\
51	228.529557455665\\
52	228.529557455665\\
53	228.529557455665\\
54	228.529557455665\\
55	228.529557455665\\
56	228.529557455665\\
57	228.529557455665\\
58	230.729532769935\\
59	230.729532769935\\
60	224.517919348254\\
61	224.517919348254\\
62	222.400244445131\\
63	221.812715238426\\
64	221.812715238426\\
65	221.812715238426\\
66	221.812715238426\\
67	221.812715238426\\
68	221.812715238426\\
69	221.781917354377\\
70	221.781917354377\\
71	221.781917354377\\
72	221.246520651224\\
73	221.246520651224\\
74	221.246520651224\\
75	221.246520651224\\
76	221.246520651224\\
77	221.430541407762\\
78	221.430541407762\\
79	221.430541407762\\
80	221.430541407762\\
81	221.430541407762\\
82	219.935387120559\\
83	219.935387120559\\
84	219.935387120559\\
85	219.935387120559\\
86	219.935387120559\\
87	219.935387120559\\
88	219.935387120559\\
89	219.935387120559\\
90	219.935387120559\\
91	219.935387120559\\
92	219.887685088105\\
93	219.887685088105\\
94	219.887685088105\\
95	219.887685088105\\
96	219.772700389049\\
97	219.772700389049\\
98	219.772700389049\\
99	219.497517912194\\
100	219.020590877557\\
100	228.320541387127\\
99	228.203123355293\\
98	229.736959745198\\
97	229.736959745198\\
96	229.736959745198\\
95	230.543571207291\\
94	230.543571207291\\
93	230.543571207291\\
92	230.543571207291\\
91	231.53890202697\\
90	231.53890202697\\
89	231.53890202697\\
88	231.53890202697\\
87	231.53890202697\\
86	231.53890202697\\
85	231.53890202697\\
84	231.53890202697\\
83	231.53890202697\\
82	231.53890202697\\
81	231.14213521207\\
80	231.14213521207\\
79	231.14213521207\\
78	231.14213521207\\
77	231.14213521207\\
76	233.260216600647\\
75	233.260216600647\\
74	233.260216600647\\
73	233.260216600647\\
72	233.260216600647\\
71	235.573844435881\\
70	235.573844435881\\
69	235.573844435881\\
68	237.206523310084\\
67	237.206523310084\\
66	237.206523310084\\
65	237.206523310084\\
64	237.206523310084\\
63	237.206523310084\\
62	237.052163545348\\
61	236.498999580589\\
60	236.498999580589\\
59	234.990003611823\\
58	234.990003611823\\
57	243.711714863732\\
56	243.711714863732\\
55	243.711714863732\\
54	243.711714863732\\
53	243.711714863732\\
52	243.711714863732\\
51	243.711714863732\\
50	243.711714863732\\
49	245.989601902591\\
48	245.989601902591\\
47	248.764602696789\\
46	248.764602696789\\
45	248.764602696789\\
44	249.038010254848\\
43	249.038010254848\\
42	249.038010254848\\
41	249.038010254848\\
40	249.038010254848\\
39	249.287992231122\\
38	249.287992231122\\
37	249.287992231122\\
36	249.287992231122\\
35	253.189075995287\\
34	253.189075995287\\
33	253.189075995287\\
32	253.189075995287\\
31	257.366632462755\\
30	257.366632462755\\
29	257.366632462755\\
28	257.366632462755\\
27	257.366632462755\\
26	257.142410441939\\
25	256.267042897981\\
24	256.267042897981\\
23	256.267042897981\\
22	256.267042897981\\
21	256.267042897981\\
20	257.84006744138\\
19	257.84006744138\\
18	257.84006744138\\
17	257.84006744138\\
16	269.241922489019\\
15	269.241922489019\\
14	269.241922489019\\
13	290.175377162416\\
12	288.521055148962\\
11	372.68884252355\\
10	374.556651174359\\
9	384.758486067506\\
8	464.15064843449\\
7	498.777782488596\\
6	496.320832049358\\
5	552.956923827991\\
4	648.530357321565\\
3	651.663700436703\\
2	744.871273688348\\
1	880.574075740346\\
}--cycle;
\addplot [color=red]
  table[row sep=crcr]{%
1	633\\
2	542\\
3	476\\
4	466\\
5	408\\
6	381\\
7	374\\
8	359\\
9	322\\
10	310\\
11	309\\
12	273\\
13	269\\
14	257\\
15	257\\
16	257\\
17	253\\
18	253\\
19	253\\
20	253\\
21	252\\
22	252\\
23	252\\
24	252\\
25	252\\
26	251\\
27	251\\
28	251\\
29	251\\
30	251\\
31	251\\
32	242\\
33	242\\
34	242\\
35	242\\
36	241\\
37	241\\
38	241\\
39	241\\
40	240\\
41	240\\
42	240\\
43	240\\
44	240\\
45	240\\
46	240\\
47	240\\
48	237\\
49	237\\
50	236\\
51	236\\
52	236\\
53	236\\
54	236\\
55	236\\
56	236\\
57	236\\
58	233\\
59	233\\
60	231\\
61	231\\
62	230\\
63	230\\
64	230\\
65	230\\
66	230\\
67	230\\
68	230\\
69	229\\
70	229\\
71	229\\
72	227\\
73	227\\
74	227\\
75	227\\
76	227\\
77	226\\
78	226\\
79	226\\
80	226\\
81	226\\
82	226\\
83	226\\
84	226\\
85	226\\
86	226\\
87	226\\
88	226\\
89	226\\
90	226\\
91	226\\
92	225\\
93	225\\
94	225\\
95	225\\
96	225\\
97	225\\
98	225\\
99	224\\
100	224\\
};
\addlegendentry{muscles}


\addplot[area legend, draw=none, fill=mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1627.9035999872\\
2	1306.03979490931\\
3	985.047178798434\\
4	885.00425279036\\
5	822.912325839988\\
6	822.912325839988\\
7	822.912325839988\\
8	822.912325839988\\
9	740.942304698452\\
10	629.495784381323\\
11	623.701354273899\\
12	621.731692487156\\
13	625.33797792972\\
14	625.633342253642\\
15	625.633342253642\\
16	555.797419790942\\
17	555.797419790942\\
18	555.797419790942\\
19	555.797419790942\\
20	555.402039122708\\
21	553.28193463323\\
22	553.28193463323\\
23	527.459980888294\\
24	539.377215430268\\
25	544.547647548207\\
26	544.547647548207\\
27	544.547647548207\\
28	540.01569980221\\
29	540.01569980221\\
30	504.463461762259\\
31	504.463461762259\\
32	504.463461762259\\
33	504.463461762259\\
34	497.330112100446\\
35	482.88197334922\\
36	480.45605514176\\
37	480.45605514176\\
38	467.77508734465\\
39	457.199503118067\\
40	454.1663831086\\
41	448.140664283474\\
42	441.806101604861\\
43	440.486770671938\\
44	414.983551948044\\
45	414.983551948044\\
46	409.252533558267\\
47	404.032351850354\\
48	401.042248222403\\
49	401.042248222403\\
50	404.993876769914\\
51	408.924269107181\\
52	404.149693354237\\
53	399.664266957255\\
54	354.889361499188\\
55	350.531184615838\\
56	339.057763828909\\
57	339.057763828909\\
58	336.435177063763\\
59	336.435177063763\\
60	336.832456334285\\
61	337.25849846261\\
62	289.421806022332\\
63	289.421806022332\\
64	289.421806022332\\
65	289.421806022332\\
66	289.421806022332\\
67	289.421806022332\\
68	289.421806022332\\
69	289.421806022332\\
70	289.421806022332\\
71	253.25786913572\\
72	253.323659310481\\
73	240.123637797606\\
74	240.123637797606\\
75	241.77020867946\\
76	241.77020867946\\
77	245.230462939749\\
78	247.748858324345\\
79	249.113371616652\\
80	249.113371616652\\
81	250.257554412069\\
82	250.321421567257\\
83	250.829266467742\\
84	242.683568882563\\
85	237.499088505556\\
86	236.855630659301\\
87	237.004112316009\\
88	232.833152785509\\
89	225.86461570931\\
90	227.553208443771\\
91	227.553208443771\\
92	227.553208443771\\
93	227.553208443771\\
94	227.474490157456\\
95	227.474490157456\\
96	227.474490157456\\
97	227.474490157456\\
98	227.102894039326\\
99	227.102894039326\\
100	227.102894039326\\
100	255.674740089919\\
99	255.674740089919\\
98	255.674740089919\\
97	256.880154328381\\
96	256.880154328381\\
95	256.880154328381\\
94	256.880154328381\\
93	257.215864807367\\
92	257.215864807367\\
91	257.215864807367\\
90	257.215864807367\\
89	278.430596146927\\
88	283.816373190382\\
87	283.131961753066\\
86	284.616680211385\\
85	286.52835485118\\
84	285.189562415738\\
83	283.128741419984\\
82	286.807450881911\\
81	287.207481345602\\
80	293.464760791295\\
79	293.464760791295\\
78	300.285925435638\\
77	311.127585631651\\
76	325.180742902234\\
75	325.180742902234\\
74	331.700003042962\\
73	331.700003042962\\
72	342.974366378365\\
71	348.626810943452\\
70	341.086749356241\\
69	341.086749356241\\
68	341.086749356241\\
67	341.086749356241\\
66	341.086749356241\\
65	341.086749356241\\
64	341.086749356241\\
63	341.086749356241\\
62	341.086749356241\\
61	342.818823894487\\
60	344.476987672312\\
59	358.200190166244\\
58	358.200190166244\\
57	373.452698727883\\
56	373.452698727883\\
55	373.909398110691\\
54	419.935655009371\\
53	430.533484177651\\
52	431.662256117659\\
51	431.965161446216\\
50	447.557272976395\\
49	462.629013470953\\
48	462.629013470953\\
47	488.165439071937\\
46	489.342122076614\\
45	497.648331791112\\
44	497.648331791112\\
43	496.025876317506\\
42	496.070844530183\\
41	497.002855157589\\
40	563.599404325607\\
39	562.997479177848\\
38	567.768593176536\\
37	568.186882804324\\
36	568.186882804324\\
35	574.07877988034\\
34	570.382981461825\\
33	568.596411010906\\
32	568.596411010906\\
31	568.596411010906\\
30	568.596411010906\\
29	561.79099834118\\
28	561.79099834118\\
27	580.861934180802\\
26	580.861934180802\\
25	580.861934180802\\
24	603.688665805533\\
23	650.123513948921\\
22	685.984222943395\\
21	685.984222943395\\
20	700.599999511509\\
19	709.046267805671\\
18	709.046267805671\\
17	709.046267805671\\
16	709.046267805671\\
15	703.44167746633\\
14	703.44167746633\\
13	709.357203014808\\
12	735.011483122504\\
11	826.394482560801\\
10	835.598039867015\\
9	952.962674726712\\
8	968.511333420183\\
7	968.511333420183\\
6	968.511333420183\\
5	968.511333420183\\
4	1107.8772439859\\
3	1419.56877596391\\
2	1764.43022145879\\
1	1986.14351338173\\
}--cycle;
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	1807\\
2	1535\\
3	1202\\
4	996\\
5	896\\
6	896\\
7	896\\
8	896\\
9	847\\
10	733\\
11	725\\
12	678\\
13	667\\
14	665\\
15	665\\
16	632\\
17	632\\
18	632\\
19	632\\
20	628\\
21	620\\
22	620\\
23	589\\
24	572\\
25	563\\
26	563\\
27	563\\
28	551\\
29	551\\
30	537\\
31	537\\
32	537\\
33	537\\
34	534\\
35	528\\
36	524\\
37	524\\
38	518\\
39	510\\
40	509\\
41	473\\
42	469\\
43	468\\
44	456\\
45	456\\
46	449\\
47	446\\
48	432\\
49	432\\
50	426\\
51	420\\
52	418\\
53	415\\
54	387\\
55	362\\
56	356\\
57	356\\
58	347\\
59	347\\
60	341\\
61	340\\
62	315\\
63	315\\
64	315\\
65	315\\
66	315\\
67	315\\
68	315\\
69	315\\
70	315\\
71	301\\
72	298\\
73	286\\
74	286\\
75	283\\
76	283\\
77	278\\
78	274\\
79	271\\
80	271\\
81	269\\
82	269\\
83	267\\
84	264\\
85	262\\
86	261\\
87	260\\
88	258\\
89	252\\
90	242\\
91	242\\
92	242\\
93	242\\
94	242\\
95	242\\
96	242\\
97	242\\
98	241\\
99	241\\
100	241\\
};
\addlegendentry{torques}


\addplot[area legend, draw=none, fill=mycolor2, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	373.217478830767\\
2	276.520388823272\\
3	278.860100671472\\
4	274.613620603099\\
5	239.23826875398\\
6	268.663903315261\\
7	207.389595114721\\
8	256.227849661939\\
9	268.651718391085\\
10	268.847911495738\\
11	253.869388594095\\
12	253.869388594095\\
13	253.869388594095\\
14	253.869388594095\\
15	253.869388594095\\
16	253.869388594095\\
17	253.869388594095\\
18	258.700250920593\\
19	258.700250920593\\
20	259.375115701406\\
21	259.884630245875\\
22	259.884630245875\\
23	259.884630245875\\
24	259.884630245875\\
25	259.884630245875\\
26	259.913208316247\\
27	260.406279277716\\
28	255.976816758818\\
29	251.197450153958\\
30	251.197450153958\\
31	251.197450153958\\
32	251.197450153958\\
33	251.197450153958\\
34	251.197450153958\\
35	244.230272926517\\
36	244.230272926517\\
37	244.230272926517\\
38	244.230272926517\\
39	242.228694282336\\
40	242.228694282336\\
41	242.228694282336\\
42	242.228694282336\\
43	242.228694282336\\
44	242.228694282336\\
45	242.228694282336\\
46	242.228694282336\\
47	242.228694282336\\
48	242.228694282336\\
49	242.228694282336\\
50	242.228694282336\\
51	244.55038565349\\
52	244.55038565349\\
53	244.169663279219\\
54	244.169663279219\\
55	244.169663279219\\
56	244.169663279219\\
57	240.208757356587\\
58	240.208757356587\\
59	240.208757356587\\
60	240.208757356587\\
61	240.208757356587\\
62	240.208757356587\\
63	240.208757356587\\
64	240.208757356587\\
65	240.208757356587\\
66	240.208757356587\\
67	240.208757356587\\
68	240.208757356587\\
69	240.208757356587\\
70	240.208757356587\\
71	240.208757356587\\
72	238.50208248849\\
73	238.50208248849\\
74	238.50208248849\\
75	238.50208248849\\
76	238.50208248849\\
77	238.50208248849\\
78	236.921695055715\\
79	236.921695055715\\
80	236.921695055715\\
81	236.921695055715\\
82	237.340948831358\\
83	237.340948831358\\
84	237.340948831358\\
85	237.340948831358\\
86	237.340948831358\\
87	237.340948831358\\
88	238.108424287874\\
89	238.108424287874\\
90	238.108424287874\\
91	238.108424287874\\
92	238.108424287874\\
93	238.108424287874\\
94	238.108424287874\\
95	238.108424287874\\
96	238.076277352432\\
97	238.076277352432\\
98	238.076277352432\\
99	238.076277352432\\
100	238.076277352432\\
100	245.330729876256\\
99	245.330729876256\\
98	245.330729876256\\
97	245.330729876256\\
96	245.330729876256\\
95	246.754168408382\\
94	246.754168408382\\
93	246.754168408382\\
92	246.754168408382\\
91	246.754168408382\\
90	246.754168408382\\
89	246.754168408382\\
88	246.754168408382\\
87	251.527209894262\\
86	251.527209894262\\
85	251.527209894262\\
84	251.527209894262\\
83	251.527209894262\\
82	251.527209894262\\
81	253.429601021331\\
80	253.429601021331\\
79	253.429601021331\\
78	253.429601021331\\
77	253.199598405832\\
76	253.199598405832\\
75	253.199598405832\\
74	253.199598405832\\
73	253.199598405832\\
72	253.199598405832\\
71	253.041870287744\\
70	253.041870287744\\
69	253.041870287744\\
68	253.041870287744\\
67	253.041870287744\\
66	253.041870287744\\
65	253.041870287744\\
64	253.041870287744\\
63	253.041870287744\\
62	253.041870287744\\
61	253.041870287744\\
60	253.041870287744\\
59	253.041870287744\\
58	253.041870287744\\
57	253.041870287744\\
56	254.026773512153\\
55	254.026773512153\\
54	254.026773512153\\
53	254.026773512153\\
52	261.193564552833\\
51	261.193564552833\\
50	271.97571848325\\
49	271.97571848325\\
48	271.97571848325\\
47	271.97571848325\\
46	271.97571848325\\
45	271.97571848325\\
44	271.97571848325\\
43	271.97571848325\\
42	271.97571848325\\
41	271.97571848325\\
40	271.97571848325\\
39	271.97571848325\\
38	273.469064945211\\
37	273.469064945211\\
36	273.469064945211\\
35	273.469064945211\\
34	272.262720683706\\
33	272.262720683706\\
32	272.262720683706\\
31	272.262720683706\\
30	272.262720683706\\
29	272.262720683706\\
28	272.066227458402\\
27	279.328372125561\\
26	283.360642514423\\
25	283.537646357138\\
24	283.537646357138\\
23	283.537646357138\\
22	283.537646357138\\
21	283.537646357138\\
20	305.099539011621\\
19	308.435578815448\\
18	308.435578815448\\
17	329.403649375832\\
16	329.403649375832\\
15	329.403649375832\\
14	329.403649375832\\
13	329.403649375832\\
12	329.403649375832\\
11	329.403649375832\\
10	328.497283261349\\
9	329.230484328138\\
8	375.628546700524\\
7	793.081740499191\\
6	821.061083726775\\
5	994.889402189574\\
4	1128.01336203156\\
3	1162.14757718931\\
2	1534.19891249322\\
1	1788.92936796945\\
}--cycle;
\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	1081\\
2	905\\
3	721\\
4	701\\
5	617\\
6	545\\
7	500\\
8	316\\
9	299\\
10	299\\
11	292\\
12	292\\
13	292\\
14	292\\
15	292\\
16	292\\
17	292\\
18	284\\
19	284\\
20	282\\
21	272\\
22	272\\
23	272\\
24	272\\
25	272\\
26	272\\
27	270\\
28	264\\
29	262\\
30	262\\
31	262\\
32	262\\
33	262\\
34	262\\
35	259\\
36	259\\
37	259\\
38	259\\
39	257\\
40	257\\
41	257\\
42	257\\
43	257\\
44	257\\
45	257\\
46	257\\
47	257\\
48	257\\
49	257\\
50	257\\
51	253\\
52	253\\
53	249\\
54	249\\
55	249\\
56	249\\
57	247\\
58	247\\
59	247\\
60	247\\
61	247\\
62	247\\
63	247\\
64	247\\
65	247\\
66	247\\
67	247\\
68	247\\
69	247\\
70	247\\
71	247\\
72	246\\
73	246\\
74	246\\
75	246\\
76	246\\
77	246\\
78	245\\
79	245\\
80	245\\
81	245\\
82	244\\
83	244\\
84	244\\
85	244\\
86	244\\
87	244\\
88	242\\
89	242\\
90	242\\
91	242\\
92	242\\
93	242\\
94	242\\
95	242\\
96	242\\
97	242\\
98	242\\
99	242\\
100	242\\
};
\addlegendentry{no Fl}


\addplot[area legend, draw=none, fill=red!50!mycolor2, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	382.099469136191\\
2	309.508122332534\\
3	284.790427784845\\
4	284.600505107235\\
5	272.622625715761\\
6	266.180794521983\\
7	259.793090653779\\
8	259.793090653779\\
9	258.905547509207\\
10	232.263364953561\\
11	238.111140482498\\
12	238.64548077136\\
13	230.804017350777\\
14	230.804017350777\\
15	231.188665463399\\
16	231.550366273618\\
17	231.797436881678\\
18	231.797436881678\\
19	231.797436881678\\
20	231.797436881678\\
21	223.772621658219\\
22	223.772621658219\\
23	221.094009576847\\
24	221.094009576847\\
25	221.094009576847\\
26	218.107564038673\\
27	207.31399277002\\
28	207.31399277002\\
29	207.31399277002\\
30	207.31399277002\\
31	209.069740873613\\
32	208.519861500376\\
33	208.993910619099\\
34	208.354433232933\\
35	206.14175174992\\
36	204.434168627648\\
37	197.789422348852\\
38	197.789422348852\\
39	197.789422348852\\
40	198.258954513702\\
41	195.103841347893\\
42	194.620386941689\\
43	193.730281184771\\
44	193.730281184771\\
45	192.286080908941\\
46	192.286080908941\\
47	188.072016003434\\
48	187.245878774939\\
49	187.245878774939\\
50	187.245878774939\\
51	187.245878774939\\
52	188.807077778001\\
53	188.807077778001\\
54	188.807077778001\\
55	186.55251685335\\
56	184.749190765144\\
57	184.749190765144\\
58	185.651376336592\\
59	185.651376336592\\
60	185.651376336592\\
61	185.651376336592\\
62	185.035566778531\\
63	185.035566778531\\
64	185.035566778531\\
65	185.035566778531\\
66	184.666747570528\\
67	184.647154384587\\
68	184.647154384587\\
69	184.160026314058\\
70	180.255026468521\\
71	180.255026468521\\
72	180.160229681443\\
73	180.025636054347\\
74	180.22424173355\\
75	180.22424173355\\
76	180.362161141056\\
77	180.362161141056\\
78	178.982039629345\\
79	178.620421775282\\
80	177.605375151373\\
81	177.605375151373\\
82	178.338248338722\\
83	178.338248338722\\
84	178.338248338722\\
85	178.338248338722\\
86	177.227693461614\\
87	177.227693461614\\
88	176.290059702072\\
89	176.290059702072\\
90	176.290059702072\\
91	176.290059702072\\
92	176.290059702072\\
93	176.290059702072\\
94	176.290059702072\\
95	175.730106546535\\
96	176.540270384722\\
97	176.540270384722\\
98	176.540270384722\\
99	175.10356489774\\
100	175.42633363003\\
100	199.056237155205\\
99	200.303230947058\\
98	200.72074097667\\
97	200.72074097667\\
96	200.72074097667\\
95	203.95607151044\\
94	203.905579525041\\
93	203.905579525041\\
92	203.905579525041\\
91	203.905579525041\\
90	203.905579525041\\
89	203.905579525041\\
88	203.905579525041\\
87	204.27320982948\\
86	204.27320982948\\
85	204.147541817416\\
84	204.147541817416\\
83	204.147541817416\\
82	204.147541817416\\
81	207.038005154731\\
80	207.038005154731\\
79	206.962641744577\\
78	206.94176577705\\
77	207.396908775834\\
76	207.396908775834\\
75	207.950020096791\\
74	207.950020096791\\
73	208.742892997145\\
72	208.729116786179\\
71	213.376645358181\\
70	213.376645358181\\
69	214.232776790184\\
68	215.741598799711\\
67	215.741598799711\\
66	215.738959083045\\
65	215.938394054082\\
64	215.938394054082\\
63	215.938394054082\\
62	215.938394054082\\
61	216.169112684985\\
60	216.169112684985\\
59	216.169112684985\\
58	216.169112684985\\
57	220.006162862745\\
56	220.006162862745\\
55	221.252196184904\\
54	220.838662318141\\
53	220.838662318141\\
52	220.838662318141\\
51	227.589985801769\\
50	227.589985801769\\
49	227.589985801769\\
48	227.589985801769\\
47	227.478577617509\\
46	231.451586979268\\
45	231.451586979268\\
44	235.366450803195\\
43	235.366450803195\\
42	236.568003149677\\
41	238.926974764321\\
40	238.182774411095\\
39	241.021772666958\\
38	241.021772666958\\
37	241.021772666958\\
36	240.1617403837\\
35	247.135834285404\\
34	246.603464668937\\
33	248.005838654227\\
32	251.832451805362\\
31	252.957979491139\\
30	264.019128932328\\
29	264.019128932328\\
28	264.019128932328\\
27	264.019128932328\\
26	261.98646976924\\
25	264.864675921584\\
24	264.864675921584\\
23	264.864675921584\\
22	280.758099197536\\
21	280.758099197536\\
20	278.680399281218\\
19	278.680399281218\\
18	278.680399281218\\
17	278.680399281218\\
16	281.307231650274\\
15	284.253603543584\\
14	286.908393193184\\
13	286.908393193184\\
12	285.14673127318\\
11	287.958154581048\\
10	313.77278417814\\
9	326.290628284862\\
8	332.786872487974\\
7	332.786872487974\\
6	347.34651143028\\
5	371.533281728663\\
4	402.138274677483\\
3	441.195703979094\\
2	472.111375135387\\
1	477.794047504056\\
}--cycle;
\addplot [color=red!50!mycolor2]
  table[row sep=crcr]{%
1	430\\
2	391\\
3	363\\
4	343\\
5	322\\
6	307\\
7	296\\
8	296\\
9	293\\
10	273\\
11	263\\
12	262\\
13	259\\
14	259\\
15	258\\
16	256\\
17	255\\
18	255\\
19	255\\
20	255\\
21	252\\
22	252\\
23	243\\
24	243\\
25	243\\
26	240\\
27	236\\
28	236\\
29	236\\
30	236\\
31	231\\
32	230\\
33	228\\
34	227\\
35	227\\
36	222\\
37	219\\
38	219\\
39	219\\
40	218\\
41	217\\
42	216\\
43	215\\
44	215\\
45	212\\
46	212\\
47	208\\
48	207\\
49	207\\
50	207\\
51	207\\
52	205\\
53	205\\
54	205\\
55	204\\
56	202\\
57	202\\
58	201\\
59	201\\
60	201\\
61	201\\
62	200\\
63	200\\
64	200\\
65	200\\
66	200\\
67	200\\
68	200\\
69	199\\
70	197\\
71	197\\
72	194\\
73	194\\
74	194\\
75	194\\
76	194\\
77	194\\
78	193\\
79	193\\
80	192\\
81	192\\
82	191\\
83	191\\
84	191\\
85	191\\
86	191\\
87	191\\
88	190\\
89	190\\
90	190\\
91	190\\
92	190\\
93	190\\
94	190\\
95	190\\
96	189\\
97	189\\
98	189\\
99	188\\
100	187\\
};
\addlegendentry{const r}


\addplot[area legend, draw=none, fill=mycolor3, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1475.49126948748\\
2	1375.2428540141\\
3	1171.26251548779\\
4	1171.26251548779\\
5	1135.78197386618\\
6	1135.78197386618\\
7	1210.55675241997\\
8	1264.28021921567\\
9	1254.68475344274\\
10	1206.3025457244\\
11	1206.3025457244\\
12	1206.3025457244\\
13	1159.01201026011\\
14	1159.01201026011\\
15	1160.01665656418\\
16	1160.01665656418\\
17	1165.42508327941\\
18	1165.42508327941\\
19	1023.07338137601\\
20	1023.07338137601\\
21	1023.07338137601\\
22	1023.07338137601\\
23	1023.07338137601\\
24	1023.98416796808\\
25	1017.03478513057\\
26	1015.63749046636\\
27	1009.0818809942\\
28	1009.0818809942\\
29	1009.0818809942\\
30	1009.0818809942\\
31	1009.77801647575\\
32	1009.77801647575\\
33	1009.77801647575\\
34	1012.08659121626\\
35	999.541598059154\\
36	999.541598059154\\
37	999.541598059154\\
38	983.873942973365\\
39	983.873942973365\\
40	925.155325467839\\
41	925.155325467839\\
42	928.527068572823\\
43	929.96476280658\\
44	929.96476280658\\
45	924.336673119626\\
46	886.776162684675\\
47	876.807710896321\\
48	878.445375196033\\
49	882.022472624744\\
50	882.022472624744\\
51	785.415287171523\\
52	782.589465430545\\
53	782.589465430545\\
54	781.874452854545\\
55	781.611590866219\\
56	781.611590866219\\
57	781.611590866219\\
58	781.472225050497\\
59	781.472225050497\\
60	781.472225050497\\
61	772.136292962431\\
62	772.136292962431\\
63	772.136292962431\\
64	739.648135694805\\
65	739.648135694805\\
66	734.957196857105\\
67	705.186176430937\\
68	705.186176430937\\
69	705.186176430937\\
70	705.186176430937\\
71	705.186176430937\\
72	672.635551640185\\
73	672.635551640185\\
74	672.635551640185\\
75	672.635551640185\\
76	672.635551640185\\
77	672.635551640185\\
78	672.635551640185\\
79	667.846408680327\\
80	651.708717555413\\
81	651.708717555413\\
82	653.288496058516\\
83	653.288496058516\\
84	654.248966974312\\
85	654.248966974312\\
86	654.248966974312\\
87	654.248966974312\\
88	654.248966974312\\
89	654.248966974312\\
90	656.017572258742\\
91	656.017572258742\\
92	656.017572258742\\
93	650.705411156285\\
94	650.705411156285\\
95	650.705411156285\\
96	619.156616603273\\
97	599.819520152459\\
98	599.819520152459\\
99	599.819520152459\\
100	599.819520152459\\
100	962.704553296672\\
99	962.704553296672\\
98	962.704553296672\\
97	962.704553296672\\
96	962.856103260979\\
95	969.265759326598\\
94	969.265759326598\\
93	969.265759326598\\
92	971.139857355098\\
91	971.139857355098\\
90	971.139857355098\\
89	978.15438566603\\
88	978.15438566603\\
87	978.15438566603\\
86	978.15438566603\\
85	978.15438566603\\
84	978.15438566603\\
83	981.953553604224\\
82	981.953553604224\\
81	988.187957459803\\
80	988.187957459803\\
79	1003.40442781942\\
78	1006.38108259179\\
77	1006.38108259179\\
76	1006.38108259179\\
75	1006.38108259179\\
74	1006.38108259179\\
73	1006.38108259179\\
72	1006.38108259179\\
71	1010.48703439302\\
70	1010.48703439302\\
69	1010.48703439302\\
68	1010.48703439302\\
67	1010.48703439302\\
66	1061.91181605721\\
65	1103.84224655303\\
64	1103.84224655303\\
63	1095.16462907115\\
62	1095.16462907115\\
61	1095.16462907115\\
60	1106.90070456369\\
59	1106.90070456369\\
58	1106.90070456369\\
57	1109.16369338918\\
56	1109.16369338918\\
55	1109.16369338918\\
54	1112.45316533358\\
53	1132.86587992121\\
52	1132.86587992121\\
51	1180.74328009224\\
50	1155.27793096023\\
49	1155.27793096023\\
48	1196.18941924304\\
47	1208.33244701358\\
46	1227.08448051876\\
45	1225.24495301402\\
44	1241.39894138671\\
43	1241.39894138671\\
42	1249.25935023479\\
41	1266.82821018483\\
40	1266.82821018483\\
39	1256.17540710478\\
38	1256.17540710478\\
37	1269.34292584094\\
36	1269.34292584094\\
35	1269.34292584094\\
34	1290.55569903225\\
33	1309.59735733368\\
32	1309.59735733368\\
31	1309.59735733368\\
30	1314.60139806791\\
29	1314.60139806791\\
28	1314.60139806791\\
27	1314.60139806791\\
26	1329.66286607521\\
25	1334.04625346244\\
24	1389.55349346064\\
23	1420.82022392988\\
22	1420.82022392988\\
21	1420.82022392988\\
20	1420.82022392988\\
19	1420.82022392988\\
18	1389.78169106338\\
17	1389.78169106338\\
16	1426.53332644711\\
15	1426.53332644711\\
14	1432.27935897521\\
13	1432.27935897521\\
12	1422.67019048667\\
11	1422.67019048667\\
10	1422.67019048667\\
9	1459.7552521251\\
8	1619.11445701911\\
7	1823.40468503371\\
6	2316.98785255777\\
5	2316.98785255777\\
4	2319.52536357764\\
3	2319.52536357764\\
2	3211.79188435871\\
1	3326.65676371465\\
}--cycle;
\addplot [color=mycolor3]
  table[row sep=crcr]{%
1	2401\\
2	2294\\
3	1745\\
4	1745\\
5	1726\\
6	1726\\
7	1517\\
8	1442\\
9	1357\\
10	1314\\
11	1314\\
12	1314\\
13	1296\\
14	1296\\
15	1293\\
16	1293\\
17	1278\\
18	1278\\
19	1222\\
20	1222\\
21	1222\\
22	1222\\
23	1222\\
24	1207\\
25	1176\\
26	1173\\
27	1162\\
28	1162\\
29	1162\\
30	1162\\
31	1160\\
32	1160\\
33	1160\\
34	1151\\
35	1134\\
36	1134\\
37	1134\\
38	1120\\
39	1120\\
40	1096\\
41	1096\\
42	1089\\
43	1086\\
44	1086\\
45	1075\\
46	1057\\
47	1043\\
48	1037\\
49	1019\\
50	1019\\
51	983\\
52	958\\
53	958\\
54	947\\
55	945\\
56	945\\
57	945\\
58	944\\
59	944\\
60	944\\
61	934\\
62	934\\
63	934\\
64	922\\
65	922\\
66	898\\
67	858\\
68	858\\
69	858\\
70	858\\
71	858\\
72	840\\
73	840\\
74	840\\
75	840\\
76	840\\
77	840\\
78	840\\
79	836\\
80	820\\
81	820\\
82	818\\
83	818\\
84	816\\
85	816\\
86	816\\
87	816\\
88	816\\
89	816\\
90	814\\
91	814\\
92	814\\
93	810\\
94	810\\
95	810\\
96	791\\
97	781\\
98	781\\
99	781\\
100	781\\
};
\addlegendentry{no Fv}


\addplot[area legend, draw=none, fill=red!50!mycolor3, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	787.491413316323\\
2	667.748681151948\\
3	484.834816192383\\
4	399.807913652924\\
5	306.350313945322\\
6	231.347111635291\\
7	176.153075442396\\
8	105.236529875014\\
9	182.171401442951\\
10	196.695210918013\\
11	203.414730658481\\
12	197.936747119484\\
13	208.88021133064\\
14	225.81484391894\\
15	230.247051267522\\
16	233.861385741007\\
17	233.861385741007\\
18	220.077665670592\\
19	234.324259930807\\
20	234.324259930807\\
21	234.324259930807\\
22	234.324259930807\\
23	234.324259930807\\
24	234.324259930807\\
25	230.151257882368\\
26	230.151257882368\\
27	230.151257882368\\
28	222.035376090476\\
29	222.035376090476\\
30	222.035376090476\\
31	222.035376090476\\
32	222.035376090476\\
33	222.035376090476\\
34	222.035376090476\\
35	222.737755934466\\
36	222.737183582173\\
37	218.678804559759\\
38	218.678804559759\\
39	218.678804559759\\
40	218.896745102547\\
41	218.896745102547\\
42	218.164649518883\\
43	218.164649518883\\
44	217.401549197262\\
45	217.977484430739\\
46	213.801602342179\\
47	213.801602342179\\
48	213.801602342179\\
49	214.831592297413\\
50	212.413741486989\\
51	207.957593709194\\
52	207.957593709194\\
53	206.180873359654\\
54	203.051057314837\\
55	199.217307343537\\
56	199.386861219985\\
57	199.70661895784\\
58	199.70661895784\\
59	199.70661895784\\
60	199.70661895784\\
61	199.70661895784\\
62	199.62730668354\\
63	199.62730668354\\
64	199.62730668354\\
65	198.691924202531\\
66	198.691924202531\\
67	198.691924202531\\
68	198.691924202531\\
69	198.254580372786\\
70	197.958756678804\\
71	197.958756678804\\
72	193.285502050019\\
73	193.285502050019\\
74	193.947943252734\\
75	193.947943252734\\
76	194.047461648077\\
77	194.047461648077\\
78	194.047461648077\\
79	194.047156301142\\
80	190.743444961196\\
81	190.743444961196\\
82	190.743444961196\\
83	190.796388180691\\
84	190.796388180691\\
85	188.808594504569\\
86	188.808594504569\\
87	188.808594504569\\
88	188.808594504569\\
89	188.808594504569\\
90	188.808594504569\\
91	188.808594504569\\
92	188.808594504569\\
93	188.808594504569\\
94	188.399360848\\
95	188.399360848\\
96	186.892845874846\\
97	186.892845874846\\
98	186.508287533649\\
99	185.999792501063\\
100	186.632698582258\\
100	187.964970197823\\
99	190.349374117946\\
98	190.645934332641\\
97	190.959120067569\\
96	190.959120067569\\
95	190.697086427871\\
94	190.697086427871\\
93	192.19734096122\\
92	192.19734096122\\
91	192.19734096122\\
90	192.19734096122\\
89	192.19734096122\\
88	192.19734096122\\
87	192.19734096122\\
86	192.19734096122\\
85	192.19734096122\\
84	193.392218200357\\
83	193.392218200357\\
82	199.933386940162\\
81	199.933386940162\\
80	199.933386940162\\
79	202.036529261865\\
78	202.400477601085\\
77	202.400477601085\\
76	202.400477601085\\
75	205.64794714656\\
74	205.64794714656\\
73	209.32309577592\\
72	209.32309577592\\
71	210.460874823277\\
70	210.460874823277\\
69	210.506164755256\\
68	210.600845482883\\
67	210.600845482883\\
66	210.600845482883\\
65	210.600845482883\\
64	221.023078471994\\
63	221.023078471994\\
62	221.023078471994\\
61	221.443621617405\\
60	221.443621617405\\
59	221.443621617405\\
58	221.443621617405\\
57	221.443621617405\\
56	222.839020072967\\
55	223.564603039761\\
54	223.139087272497\\
53	225.29353891266\\
52	227.918321108214\\
51	227.918321108214\\
50	227.307918246725\\
49	227.320974837998\\
48	231.170551416319\\
47	231.170551416319\\
46	231.170551416319\\
45	232.726518436383\\
44	235.558805854251\\
43	237.614338453293\\
42	237.614338453293\\
41	238.917750928229\\
40	238.917750928229\\
39	240.643716907933\\
38	240.643716907933\\
37	240.643716907933\\
36	241.51756682214\\
35	242.759051428173\\
34	247.673547298917\\
33	247.673547298917\\
32	247.673547298917\\
31	247.673547298917\\
30	247.673547298917\\
29	247.673547298917\\
28	247.673547298917\\
27	246.218614010096\\
26	246.218614010096\\
25	246.218614010096\\
24	246.27689697559\\
23	246.27689697559\\
22	246.27689697559\\
21	246.27689697559\\
20	246.27689697559\\
19	246.27689697559\\
18	299.633242668232\\
17	302.822562412939\\
16	302.822562412939\\
15	317.548361326533\\
14	358.713841640067\\
13	424.372678519524\\
12	465.9751044013\\
11	467.210754677895\\
10	553.888002646118\\
9	608.717787580362\\
8	897.323626340391\\
7	1002.71785645187\\
6	1165.42116300133\\
5	1193.04217328007\\
4	1305.75268585737\\
3	1436.26150233293\\
2	1440.06975843205\\
1	1456.84054882895\\
}--cycle;
\addplot [color=red!50!mycolor3]
  table[row sep=crcr]{%
1	1122\\
2	1054\\
3	961\\
4	853\\
5	750\\
6	698\\
7	589\\
8	501\\
9	395\\
10	375\\
11	335\\
12	332\\
13	317\\
14	292\\
15	274\\
16	268\\
17	268\\
18	260\\
19	240\\
20	240\\
21	240\\
22	240\\
23	240\\
24	240\\
25	238\\
26	238\\
27	238\\
28	235\\
29	235\\
30	235\\
31	235\\
32	235\\
33	235\\
34	235\\
35	233\\
36	232\\
37	230\\
38	230\\
39	230\\
40	229\\
41	229\\
42	228\\
43	228\\
44	226\\
45	225\\
46	222\\
47	222\\
48	222\\
49	221\\
50	220\\
51	218\\
52	218\\
53	216\\
54	213\\
55	211\\
56	211\\
57	211\\
58	211\\
59	211\\
60	211\\
61	211\\
62	210\\
63	210\\
64	210\\
65	205\\
66	205\\
67	205\\
68	205\\
69	204\\
70	204\\
71	204\\
72	201\\
73	201\\
74	200\\
75	200\\
76	198\\
77	198\\
78	198\\
79	198\\
80	195\\
81	195\\
82	195\\
83	192\\
84	192\\
85	191\\
86	191\\
87	191\\
88	191\\
89	191\\
90	191\\
91	191\\
92	191\\
93	191\\
94	190\\
95	190\\
96	189\\
97	189\\
98	189\\
99	188\\
100	187\\
};
\addlegendentry{no actdyn}

\legend{}
\end{axis}


==> new_figures/dataefficiency_cost_pointreaching_modifs0_3.tex <==
\begin{axis}[%
name =ax1,
scaled y ticks=base 10:\Factor,
xlabel near ticks, ylabel near ticks,
every y tick scale label/.style={at={(yticklabel* cs:1.03,0cm)},anchor=near yticklabel},
title style={at={(0.5,0.93)}},
width=0.951\figW,
height=\figH,
scale only axis,
xmin=0,
xmax=100,
xlabel style={font=\color{white!15!black}},
xlabel={\# generations},
ymin=0,
ymax=3000,
ylabel style={font=\color{white!15!black}},
ylabel={cost},
axis background/.style={fill=white},
title={pointreaching, c = 0.3 s},
legend style={legend cell align=left, align=left, draw=white!15!black}
]

\addplot[area legend, draw=none, fill=red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	539.901681728496\\
2	447.608976489532\\
3	305.154305379838\\
4	282.107922937995\\
5	250.399134947236\\
6	252.829601820532\\
7	250.975436813109\\
8	246.756327078151\\
9	248.019084489374\\
10	248.019084489374\\
11	240.1204398279\\
12	240.1204398279\\
13	240.1204398279\\
14	239.786053373221\\
15	239.790530560781\\
16	239.684401621894\\
17	239.31521377393\\
18	238.588541355541\\
19	238.388867282901\\
20	238.388867282901\\
21	237.618249079702\\
22	237.712119372395\\
23	236.127048526241\\
24	236.473412282625\\
25	236.473412282625\\
26	236.473412282625\\
27	236.473412282625\\
28	228.0946238668\\
29	228.0946238668\\
30	228.0946238668\\
31	227.125901398227\\
32	227.125901398227\\
33	227.125901398227\\
34	227.125901398227\\
35	227.125901398227\\
36	227.474393824839\\
37	227.592508571131\\
38	227.998902209542\\
39	227.998902209542\\
40	227.998902209542\\
41	227.998902209542\\
42	227.998902209542\\
43	227.998902209542\\
44	228.027790946634\\
45	228.027790946634\\
46	228.027790946634\\
47	228.027790946634\\
48	228.027790946634\\
49	228.027790946634\\
50	228.027790946634\\
51	228.169267760588\\
52	223.728039452001\\
53	223.728039452001\\
54	223.728039452001\\
55	223.963739998543\\
56	223.682377667554\\
57	223.682377667554\\
58	223.682377667554\\
59	223.682377667554\\
60	220.877512160915\\
61	220.88193086036\\
62	218.269704346714\\
63	218.269704346714\\
64	214.879026745485\\
65	214.90443897752\\
66	215.274230983754\\
67	213.843083722953\\
68	213.843083722953\\
69	214.000096505607\\
70	214.000096505607\\
71	213.468231633436\\
72	214.602561190893\\
73	214.602561190893\\
74	213.978635846854\\
75	214.752266546445\\
76	214.219353738112\\
77	214.219353738112\\
78	214.564117535231\\
79	214.564117535231\\
80	214.564117535231\\
81	213.681956873721\\
82	213.644638035192\\
83	212.375444869295\\
84	212.885768128358\\
85	211.725887772255\\
86	211.725887772255\\
87	211.725887772255\\
88	211.405702897994\\
89	211.119018013197\\
90	211.364830287416\\
91	211.364830287416\\
92	211.347089262577\\
93	210.368640074645\\
94	209.711030133804\\
95	209.959404238186\\
96	209.959404238186\\
97	209.959404238186\\
98	209.959404238186\\
99	209.959404238186\\
100	209.959404238186\\
100	211.248011700908\\
99	211.248011700908\\
98	211.248011700908\\
97	211.248011700908\\
96	211.248011700908\\
95	211.248011700908\\
94	212.209914126554\\
93	212.337803869808\\
92	212.684884985415\\
91	213.059142450371\\
90	213.059142450371\\
89	214.484558106035\\
88	214.816598376023\\
87	214.776653666411\\
86	214.776653666411\\
85	214.776653666411\\
84	214.529508686809\\
83	216.536749171202\\
82	216.906865813033\\
81	216.959550611198\\
80	216.819421886721\\
79	216.819421886721\\
78	216.819421886721\\
77	222.122491025048\\
76	222.122491025048\\
75	224.137228150283\\
74	227.073049402737\\
73	227.077429287257\\
72	227.077429287257\\
71	231.316383541012\\
70	231.35060016772\\
69	231.35060016772\\
68	231.93669573455\\
67	231.93669573455\\
66	232.159019182399\\
65	233.568760336467\\
64	233.665425220519\\
63	233.929490255728\\
62	233.929490255728\\
61	234.024073462293\\
60	234.040711576794\\
59	236.035577950929\\
58	236.035577950929\\
57	236.035577950929\\
56	236.035577950929\\
55	236.98677841309\\
54	239.653265939484\\
53	239.653265939484\\
52	239.653265939484\\
51	238.655303089548\\
50	239.339917353697\\
49	239.339917353697\\
48	239.339917353697\\
47	239.339917353697\\
46	239.339917353697\\
45	239.339917353697\\
44	239.339917353697\\
43	239.475720248588\\
42	239.475720248588\\
41	239.475720248588\\
40	239.475720248588\\
39	239.475720248588\\
38	239.475720248588\\
37	241.295036577379\\
36	241.80176956813\\
35	243.261595985273\\
34	243.261595985273\\
33	243.261595985273\\
32	243.261595985273\\
31	243.261595985273\\
30	243.927682095174\\
29	243.927682095174\\
28	243.927682095174\\
27	245.280706418835\\
26	245.280706418835\\
25	245.280706418835\\
24	245.280706418835\\
23	248.195086694085\\
22	247.859105406852\\
21	248.318335884375\\
20	249.520823520607\\
19	249.520823520607\\
18	253.710099687597\\
17	266.194723705969\\
16	267.472799830811\\
15	267.991862137461\\
14	268.223002892517\\
13	272.025015217783\\
12	272.025015217783\\
11	272.025015217783\\
10	278.559005431787\\
9	278.559005431787\\
8	293.960549442888\\
7	308.651607315587\\
6	362.282087350534\\
5	379.856531662819\\
4	436.595838958061\\
3	430.807981063977\\
2	541.114308259387\\
1	669.229589580062\\
}--cycle;
\addplot [color=red]
  table[row sep=crcr]{%
1	604.565635654279\\
2	494.36164237446\\
3	367.981143221908\\
4	359.351880948028\\
5	315.127833305028\\
6	307.555844585533\\
7	279.813522064348\\
8	270.358438260519\\
9	263.28904496058\\
10	263.28904496058\\
11	256.072727522841\\
12	256.072727522841\\
13	256.072727522841\\
14	254.004528132869\\
15	253.891196349121\\
16	253.578600726352\\
17	252.754968739949\\
18	246.149320521569\\
19	243.954845401754\\
20	243.954845401754\\
21	242.968292482039\\
22	242.785612389624\\
23	242.161067610163\\
24	240.87705935073\\
25	240.87705935073\\
26	240.87705935073\\
27	240.87705935073\\
28	236.011152980987\\
29	236.011152980987\\
30	236.011152980987\\
31	235.19374869175\\
32	235.19374869175\\
33	235.19374869175\\
34	235.19374869175\\
35	235.19374869175\\
36	234.638081696484\\
37	234.443772574255\\
38	233.737311229065\\
39	233.737311229065\\
40	233.737311229065\\
41	233.737311229065\\
42	233.737311229065\\
43	233.737311229065\\
44	233.683854150166\\
45	233.683854150166\\
46	233.683854150166\\
47	233.683854150166\\
48	233.683854150166\\
49	233.683854150166\\
50	233.683854150166\\
51	233.412285425068\\
52	231.690652695743\\
53	231.690652695743\\
54	231.690652695743\\
55	230.475259205817\\
56	229.858977809242\\
57	229.858977809242\\
58	229.858977809242\\
59	229.858977809242\\
60	227.459111868855\\
61	227.453002161327\\
62	226.099597301221\\
63	226.099597301221\\
64	224.272225983002\\
65	224.236599656994\\
66	223.716625083077\\
67	222.889889728751\\
68	222.889889728751\\
69	222.675348336663\\
70	222.675348336663\\
71	222.392307587224\\
72	220.839995239075\\
73	220.839995239075\\
74	220.525842624796\\
75	219.444747348364\\
76	218.17092238158\\
77	218.17092238158\\
78	215.691769710976\\
79	215.691769710976\\
80	215.691769710976\\
81	215.320753742459\\
82	215.275751924112\\
83	214.456097020248\\
84	213.707638407584\\
85	213.251270719333\\
86	213.251270719333\\
87	213.251270719333\\
88	213.111150637009\\
89	212.801788059616\\
90	212.211986368893\\
91	212.211986368893\\
92	212.015987123996\\
93	211.353221972226\\
94	210.960472130179\\
95	210.603707969547\\
96	210.603707969547\\
97	210.603707969547\\
98	210.603707969547\\
99	210.603707969547\\
100	210.603707969547\\
};
\addlegendentry{muscles}


\addplot[area legend, draw=none, fill=mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1175.29848510726\\
2	725.056869604282\\
3	652.353631216891\\
4	640.271160102066\\
5	671.50263846622\\
6	616.915055920658\\
7	623.823109750204\\
8	623.823109750204\\
9	632.120783476859\\
10	636.666632339653\\
11	636.666632339653\\
12	635.437578860113\\
13	635.437578860113\\
14	635.437578860113\\
15	635.437578860113\\
16	635.437578860113\\
17	625.776761360403\\
18	625.776761360403\\
19	625.776761360403\\
20	625.776761360403\\
21	605.720974567993\\
22	607.902287635937\\
23	538.815571647037\\
24	511.737482024253\\
25	511.737482024253\\
26	511.737482024253\\
27	510.430278434456\\
28	503.793149645335\\
29	482.034543999652\\
30	481.670810914795\\
31	481.670810914795\\
32	482.601884319995\\
33	483.309197992213\\
34	466.639262172347\\
35	468.183530147143\\
36	477.284340738423\\
37	477.302213465006\\
38	477.302213465006\\
39	476.860887545517\\
40	474.709075277144\\
41	467.020517457859\\
42	467.738032036546\\
43	468.050769277198\\
44	463.631094499659\\
45	463.631094499659\\
46	463.631094499659\\
47	463.500412921739\\
48	463.458118600624\\
49	463.458118600624\\
50	463.481823778448\\
51	462.662161105005\\
52	462.697103937448\\
53	462.57195515427\\
54	462.256883355426\\
55	461.099438684306\\
56	460.713366807164\\
57	459.881864443482\\
58	460.027783903452\\
59	460.03537956538\\
60	460.03537956538\\
61	459.180703539837\\
62	459.157141884717\\
63	459.364730881319\\
64	459.294893039224\\
65	459.224753990567\\
66	459.138634405552\\
67	459.030285838539\\
68	459.030285838539\\
69	458.98735553787\\
70	458.98735553787\\
71	458.942561730234\\
72	458.942561730234\\
73	458.88253440728\\
74	458.844462871819\\
75	458.815508545642\\
76	458.81520027932\\
77	458.788945899519\\
78	458.778720152408\\
79	458.778720152408\\
80	458.778720152408\\
81	458.778720152408\\
82	458.778720152408\\
83	458.671809215254\\
84	458.73348599039\\
85	458.727912213843\\
86	458.727912213843\\
87	458.727912213843\\
88	458.727912213843\\
89	458.668516965352\\
90	458.702418441779\\
91	458.702418441779\\
92	458.702418441779\\
93	458.687570500961\\
94	458.659717800603\\
95	458.659717800603\\
96	458.659717800603\\
97	458.679551661505\\
98	458.679551661505\\
99	458.700583744366\\
100	458.698607001284\\
100	458.761587716918\\
99	458.761273436436\\
98	458.843605292641\\
97	458.843605292641\\
96	458.918414401337\\
95	458.918414401337\\
94	458.918414401337\\
93	458.926272912223\\
92	458.924615437255\\
91	458.924615437255\\
90	458.924615437255\\
89	459.055169171409\\
88	459.087027271229\\
87	459.087027271229\\
86	459.087027271229\\
85	459.087027271229\\
84	459.094128514178\\
83	459.372802726308\\
82	459.575770979888\\
81	459.575770979888\\
80	459.575770979888\\
79	459.575770979888\\
78	459.575770979888\\
77	459.832283100014\\
76	460.007999957144\\
75	460.053464279118\\
74	460.402169312723\\
73	461.159504281333\\
72	461.200006298796\\
71	461.200006298796\\
70	462.096433462139\\
69	462.096433462139\\
68	462.229314524938\\
67	462.229314524938\\
66	463.388734506209\\
65	465.078584958679\\
64	465.060185856764\\
63	465.514800960126\\
62	471.038927344975\\
61	471.033722115767\\
60	475.01114919098\\
59	475.01114919098\\
58	475.457362756902\\
57	477.428275547369\\
56	477.221815439593\\
55	484.645678035103\\
54	490.429977424266\\
53	490.345598033627\\
52	491.746895018489\\
51	493.101146112814\\
50	492.886592376443\\
49	493.326161809882\\
48	493.326161809882\\
47	495.14746513964\\
46	498.237179932063\\
45	498.237179932063\\
44	498.237179932063\\
43	497.113573334245\\
42	499.661833521816\\
41	504.065895578934\\
40	523.624833013544\\
39	530.047703601865\\
38	529.930385583962\\
37	529.930385583962\\
36	531.193160190281\\
35	596.77322490867\\
34	603.418199520444\\
33	627.409545205397\\
32	637.001926205382\\
31	645.596825935256\\
30	645.596825935256\\
29	646.41633439078\\
28	641.122389652039\\
27	680.661967942165\\
26	680.316750426964\\
25	680.316750426964\\
24	680.316750426964\\
23	673.194000919991\\
22	655.939014146897\\
21	666.610059973935\\
20	664.880858512835\\
19	664.880858512835\\
18	664.880858512835\\
17	664.880858512835\\
16	671.084493861893\\
15	671.084493861893\\
14	671.084493861893\\
13	671.084493861893\\
12	671.084493861893\\
11	678.874034812925\\
10	678.874034812925\\
9	713.881020316598\\
8	749.354283762434\\
7	749.354283762434\\
6	776.837838195555\\
5	787.707948013456\\
4	1034.37752678134\\
3	1040.6290793196\\
2	1571.78860844591\\
1	2048.59460812448\\
}--cycle;
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	1612\\
2	1148\\
3	846\\
4	837\\
5	730\\
6	697\\
7	687\\
8	687\\
9	673\\
10	658\\
11	658\\
12	653\\
13	653\\
14	653\\
15	653\\
16	653\\
17	645\\
18	645\\
19	645\\
20	645\\
21	636\\
22	632\\
23	606\\
24	596\\
25	596\\
26	596\\
27	596\\
28	572\\
29	564\\
30	564\\
31	564\\
32	560\\
33	555\\
34	535\\
35	532\\
36	504\\
37	504\\
38	504\\
39	503\\
40	499\\
41	486\\
42	484\\
43	483\\
44	481\\
45	481\\
46	481\\
47	479\\
48	478\\
49	478\\
50	478\\
51	478\\
52	477\\
53	476\\
54	476\\
55	473\\
56	469\\
57	469\\
58	468\\
59	468\\
60	468\\
61	465\\
62	465\\
63	462\\
64	462\\
65	462\\
66	461\\
67	461\\
68	461\\
69	461\\
70	461\\
71	460\\
72	460\\
73	460\\
74	460\\
75	459\\
76	459\\
77	459\\
78	459\\
79	459\\
80	459\\
81	459\\
82	459\\
83	459\\
84	459\\
85	459\\
86	459\\
87	459\\
88	459\\
89	459\\
90	459\\
91	459\\
92	459\\
93	459\\
94	459\\
95	459\\
96	459\\
97	459\\
98	459\\
99	459\\
100	459\\
};
\addlegendentry{torques}


\addplot[area legend, draw=none, fill=mycolor2, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	550.094588901682\\
2	560.640431278917\\
3	499.144937766364\\
4	326.436463085823\\
5	326.436463085823\\
6	283.238888048267\\
7	283.238888048267\\
8	256.043712549961\\
9	256.043712549961\\
10	264.856265562427\\
11	264.856265562427\\
12	264.856265562427\\
13	251.525888264431\\
14	253.681275877079\\
15	253.681275877079\\
16	253.681275877079\\
17	293.182074906979\\
18	268.096004570635\\
19	266.940719372421\\
20	266.940719372421\\
21	266.940719372421\\
22	265.342583613011\\
23	265.342583613011\\
24	265.342583613011\\
25	259.566872848763\\
26	259.566872848763\\
27	254.920971521862\\
28	254.920971521862\\
29	258.163645610751\\
30	258.163645610751\\
31	258.163645610751\\
32	259.216615485353\\
33	259.216615485353\\
34	260.199127342111\\
35	260.199127342111\\
36	260.199127342111\\
37	260.199127342111\\
38	260.199127342111\\
39	251.012065704464\\
40	251.012065704464\\
41	251.012065704464\\
42	251.012065704464\\
43	250.955841706307\\
44	250.955841706307\\
45	250.955841706307\\
46	250.955841706307\\
47	250.955841706307\\
48	251.701040620149\\
49	251.72157296716\\
50	251.72157296716\\
51	245.061263419384\\
52	247.062050320173\\
53	247.062050320173\\
54	247.062050320173\\
55	247.062050320173\\
56	247.062050320173\\
57	247.062050320173\\
58	247.062050320173\\
59	247.062050320173\\
60	247.062050320173\\
61	247.062050320173\\
62	247.062050320173\\
63	247.062050320173\\
64	247.062050320173\\
65	244.460831565831\\
66	244.460831565831\\
67	242.35646167704\\
68	242.35646167704\\
69	242.35646167704\\
70	242.35646167704\\
71	242.35646167704\\
72	242.40645757895\\
73	242.40645757895\\
74	242.40645757895\\
75	242.40645757895\\
76	242.40645757895\\
77	242.40645757895\\
78	242.40645757895\\
79	242.40645757895\\
80	242.482534346528\\
81	242.482534346528\\
82	242.464053780359\\
83	242.464053780359\\
84	241.17477652512\\
85	241.17477652512\\
86	241.111485712537\\
87	241.111485712537\\
88	241.111485712537\\
89	241.111485712537\\
90	241.111485712537\\
91	241.111485712537\\
92	241.111485712537\\
93	241.039150900052\\
94	240.729935231088\\
95	240.452470343841\\
96	239.722207403507\\
97	239.722207403507\\
98	239.7668122002\\
99	239.7668122002\\
100	239.936373599942\\
100	244.991994670261\\
99	246.745325050395\\
98	246.745325050395\\
97	247.010971734231\\
96	247.010971734231\\
95	248.07475612461\\
94	248.001016997103\\
93	248.401654219736\\
92	251.020164500712\\
91	251.020164500712\\
90	251.020164500712\\
89	251.020164500712\\
88	251.020164500712\\
87	251.020164500712\\
86	251.020164500712\\
85	260.476298643585\\
84	260.476298643585\\
83	262.278909705662\\
82	262.278909705662\\
81	262.274322421597\\
80	262.274322421597\\
79	262.900635620555\\
78	262.900635620555\\
77	262.900635620555\\
76	262.900635620555\\
75	262.900635620555\\
74	262.900635620555\\
73	262.900635620555\\
72	262.900635620555\\
71	263.27817279027\\
70	263.27817279027\\
69	263.27817279027\\
68	263.27817279027\\
67	263.27817279027\\
66	262.780811457703\\
65	262.780811457703\\
64	262.201175722386\\
63	262.201175722386\\
62	262.201175722386\\
61	262.201175722386\\
60	262.201175722386\\
59	262.201175722386\\
58	262.201175722386\\
57	262.201175722386\\
56	262.201175722386\\
55	262.201175722386\\
54	262.201175722386\\
53	262.201175722386\\
52	262.201175722386\\
51	271.144193732993\\
50	270.952241456919\\
49	270.952241456919\\
48	271.029293622504\\
47	276.167565426967\\
46	276.167565426967\\
45	276.167565426967\\
44	276.167565426967\\
43	276.167565426967\\
42	276.177284490349\\
41	276.177284490349\\
40	276.177284490349\\
39	276.177284490349\\
38	290.541630904172\\
37	290.541630904172\\
36	290.541630904172\\
35	290.541630904172\\
34	290.541630904172\\
33	296.153587056986\\
32	296.153587056986\\
31	320.273940865542\\
30	320.273940865542\\
29	320.273940865542\\
28	334.636473673994\\
27	334.636473673994\\
26	338.310262815569\\
25	338.310262815569\\
24	351.097205250625\\
23	351.097205250625\\
22	351.097205250625\\
21	380.748716683004\\
20	380.748716683004\\
19	380.748716683004\\
18	414.673063345985\\
17	408.361842442751\\
16	585.046952210931\\
15	585.046952210931\\
14	585.046952210931\\
13	593.501290556901\\
12	618.054921631719\\
11	618.054921631719\\
10	618.054921631719\\
9	651.472156836504\\
8	651.472156836504\\
7	651.766696005706\\
6	651.766696005706\\
5	658.760888673508\\
4	658.760888673508\\
3	825.961036176583\\
2	926.869516950019\\
1	1261.34779905523\\
}--cycle;
\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	906\\
2	744\\
3	663\\
4	493\\
5	493\\
6	468\\
7	468\\
8	454\\
9	454\\
10	441\\
11	441\\
12	441\\
13	423\\
14	419\\
15	419\\
16	419\\
17	351\\
18	341\\
19	324\\
20	324\\
21	324\\
22	308\\
23	308\\
24	308\\
25	299\\
26	299\\
27	295\\
28	295\\
29	289\\
30	289\\
31	289\\
32	278\\
33	278\\
34	275\\
35	275\\
36	275\\
37	275\\
38	275\\
39	264\\
40	264\\
41	264\\
42	264\\
43	264\\
44	264\\
45	264\\
46	264\\
47	264\\
48	261\\
49	261\\
50	261\\
51	258\\
52	255\\
53	255\\
54	255\\
55	255\\
56	255\\
57	255\\
58	255\\
59	255\\
60	255\\
61	255\\
62	255\\
63	255\\
64	255\\
65	254\\
66	254\\
67	253\\
68	253\\
69	253\\
70	253\\
71	253\\
72	253\\
73	253\\
74	253\\
75	253\\
76	253\\
77	253\\
78	253\\
79	253\\
80	252\\
81	252\\
82	252\\
83	252\\
84	251\\
85	251\\
86	246\\
87	246\\
88	246\\
89	246\\
90	246\\
91	246\\
92	246\\
93	245\\
94	244\\
95	244\\
96	243\\
97	243\\
98	243\\
99	243\\
100	242\\
};
\addlegendentry{no Fl}


\addplot[area legend, draw=none, fill=red!50!mycolor2, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	253.30848870893\\
2	264.326103901602\\
3	267.296576166107\\
4	249.410259597735\\
5	251.784574439014\\
6	251.935073373572\\
7	251.935073373572\\
8	247.825168614065\\
9	247.825168614065\\
10	227.143588119667\\
11	228.416695477301\\
12	228.416695477301\\
13	228.416695477301\\
14	228.416695477301\\
15	225.360825358342\\
16	223.853203331633\\
17	226.094161766908\\
18	226.094161766908\\
19	226.094161766908\\
20	226.094161766908\\
21	226.094161766908\\
22	226.094161766908\\
23	224.611043021453\\
24	226.160785850919\\
25	226.160785850919\\
26	211.343424260166\\
27	211.343424260166\\
28	210.523135459591\\
29	210.523135459591\\
30	209.118900828254\\
31	209.118900828254\\
32	209.118900828254\\
33	208.703559183989\\
34	208.703559183989\\
35	212.532162844215\\
36	208.84452715925\\
37	207.102009077296\\
38	207.102009077296\\
39	207.102009077296\\
40	207.102009077296\\
41	206.467667853215\\
42	206.163505204046\\
43	205.579873696823\\
44	201.43245537806\\
45	201.43245537806\\
46	202.425739646936\\
47	202.425739646936\\
48	199.473827472565\\
49	193.953124494433\\
50	193.723975849522\\
51	193.425714177059\\
52	189.7015899047\\
53	189.7015899047\\
54	189.7015899047\\
55	189.975158699124\\
56	190.105905062585\\
57	190.395068669225\\
58	188.239684318926\\
59	188.239684318926\\
60	188.239684318926\\
61	187.486788141769\\
62	187.486788141769\\
63	187.486788141769\\
64	187.983975443508\\
65	187.983975443508\\
66	187.983975443508\\
67	187.927260267195\\
68	188.021964627245\\
69	188.021964627245\\
70	188.196663166588\\
71	188.485117307175\\
72	188.350056520794\\
73	188.309383023746\\
74	187.777459241202\\
75	186.242214597152\\
76	186.242214597152\\
77	186.242214597152\\
78	186.242214597152\\
79	186.242214597152\\
80	186.242214597152\\
81	186.242214597152\\
82	186.242214597152\\
83	186.242214597152\\
84	186.002492371459\\
85	185.645060329803\\
86	185.692036090521\\
87	185.692036090521\\
88	185.692036090521\\
89	185.692036090521\\
90	185.617640186648\\
91	185.437629634842\\
92	185.437629634842\\
93	185.437629634842\\
94	185.481391190903\\
95	185.481391190903\\
96	185.481391190903\\
97	185.481391190903\\
98	185.3116891257\\
99	185.3356907007\\
100	185.171105420345\\
100	207.498638195365\\
99	207.699230586213\\
98	208.554187342359\\
97	208.512193479431\\
96	208.512193479431\\
95	208.512193479431\\
94	208.512193479431\\
93	208.874365723766\\
92	208.874365723766\\
91	208.874365723766\\
90	208.830324660109\\
89	208.812148216662\\
88	208.812148216662\\
87	208.812148216662\\
86	208.812148216662\\
85	209.174096477672\\
84	209.087870019099\\
83	209.03026232688\\
82	209.03026232688\\
81	209.03026232688\\
80	209.03026232688\\
79	209.03026232688\\
78	209.03026232688\\
77	209.03026232688\\
76	209.03026232688\\
75	209.03026232688\\
74	208.666147997066\\
73	209.827737129516\\
72	209.948060293455\\
71	214.883889152922\\
70	217.328192693977\\
69	218.487514701046\\
68	218.487514701046\\
67	219.077384081445\\
66	219.06448418765\\
65	219.06448418765\\
64	219.06448418765\\
63	221.884605420927\\
62	221.884605420927\\
61	221.884605420927\\
60	222.909537762461\\
59	222.909537762461\\
58	222.909537762461\\
57	224.159617235107\\
56	225.852815951546\\
55	226.578680507018\\
54	228.039163941293\\
53	228.039163941293\\
52	228.039163941293\\
51	227.947593561819\\
50	227.886301515778\\
49	228.140287321612\\
48	227.066610681669\\
47	227.572181953224\\
46	227.572181953224\\
45	232.129685458008\\
44	232.129685458008\\
43	231.565994061845\\
42	231.510221652382\\
41	231.48426258272\\
40	231.437741376963\\
39	231.437741376963\\
38	231.437741376963\\
37	231.437741376963\\
36	231.375111392699\\
35	231.762670496114\\
34	246.274640387937\\
33	246.274640387937\\
32	248.192461503711\\
31	248.192461503711\\
30	248.192461503711\\
29	248.261285848818\\
28	248.261285848818\\
27	248.3341534498\\
26	248.3341534498\\
25	249.596081273983\\
24	249.596081273983\\
23	255.511892805664\\
22	260.837548901276\\
21	260.837548901276\\
20	260.837548901276\\
19	260.837548901276\\
18	260.837548901276\\
17	260.837548901276\\
16	269.200996312583\\
15	269.35084056393\\
14	269.956699037699\\
13	269.956699037699\\
12	269.956699037699\\
11	269.956699037699\\
10	274.851340088404\\
9	291.36494176434\\
8	291.36494176434\\
7	294.052990612232\\
6	294.052990612232\\
5	333.045216368817\\
4	342.342473733679\\
3	390.515337857749\\
2	401.918221791719\\
1	536.189809862186\\
}--cycle;
\addplot [color=red!50!mycolor2]
  table[row sep=crcr]{%
1	395\\
2	333\\
3	329\\
4	296\\
5	292\\
6	273\\
7	273\\
8	270\\
9	270\\
10	251\\
11	249\\
12	249\\
13	249\\
14	249\\
15	247\\
16	247\\
17	243\\
18	243\\
19	243\\
20	243\\
21	243\\
22	243\\
23	240\\
24	238\\
25	238\\
26	230\\
27	230\\
28	229\\
29	229\\
30	229\\
31	229\\
32	229\\
33	227\\
34	227\\
35	222\\
36	220\\
37	219\\
38	219\\
39	219\\
40	219\\
41	219\\
42	219\\
43	219\\
44	217\\
45	217\\
46	215\\
47	215\\
48	213\\
49	211\\
50	211\\
51	211\\
52	209\\
53	209\\
54	209\\
55	208\\
56	208\\
57	207\\
58	206\\
59	206\\
60	206\\
61	205\\
62	205\\
63	205\\
64	204\\
65	204\\
66	204\\
67	204\\
68	203\\
69	203\\
70	203\\
71	202\\
72	199\\
73	199\\
74	198\\
75	198\\
76	198\\
77	198\\
78	198\\
79	198\\
80	198\\
81	198\\
82	198\\
83	198\\
84	198\\
85	197\\
86	197\\
87	197\\
88	197\\
89	197\\
90	197\\
91	197\\
92	197\\
93	197\\
94	197\\
95	197\\
96	197\\
97	197\\
98	197\\
99	197\\
100	196\\
};
\addlegendentry{const r}


\addplot[area legend, draw=none, fill=mycolor3, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1616.51718568243\\
2	1383.4412649575\\
3	1383.4412649575\\
4	1382.19964855009\\
5	1340.17178786178\\
6	1340.17178786178\\
7	1340.17178786178\\
8	1340.17178786178\\
9	1340.17178786178\\
10	1340.17178786178\\
11	1340.17178786178\\
12	1340.17178786178\\
13	1340.17178786178\\
14	1340.17178786178\\
15	1340.17178786178\\
16	1327.47304700877\\
17	1321.7772647794\\
18	1321.7772647794\\
19	1321.7772647794\\
20	1321.7772647794\\
21	1321.7772647794\\
22	1281.77546251626\\
23	1281.77546251626\\
24	1132.48310042478\\
25	1132.48310042478\\
26	1132.48310042478\\
27	1133.88339953797\\
28	1133.88339953797\\
29	1133.88339953797\\
30	1133.88339953797\\
31	1087.5808077558\\
32	1087.5808077558\\
33	1087.5808077558\\
34	1087.5808077558\\
35	1102.84041875516\\
36	1102.84041875516\\
37	1102.84041875516\\
38	1105.77960898215\\
39	1105.77960898215\\
40	1095.87119532589\\
41	1095.87119532589\\
42	1095.87119532589\\
43	1090.24071829408\\
44	1090.24071829408\\
45	1089.78040659101\\
46	1089.78040659101\\
47	1004.67625311707\\
48	1004.67625311707\\
49	1004.67625311707\\
50	988.088502715665\\
51	988.088502715665\\
52	988.088502715665\\
53	984.826716036288\\
54	984.826716036288\\
55	972.637201305519\\
56	977.181591121858\\
57	968.749190724494\\
58	967.366801072163\\
59	967.366801072163\\
60	967.366801072163\\
61	967.055518469755\\
62	972.235818403663\\
63	969.769356982082\\
64	940.917321746325\\
65	893.020967135211\\
66	899.206388312767\\
67	899.206388312767\\
68	899.206388312767\\
69	899.206388312767\\
70	894.312964287917\\
71	880.00682335816\\
72	880.00682335816\\
73	863.639120463252\\
74	863.639120463252\\
75	863.639120463252\\
76	863.639120463252\\
77	863.639120463252\\
78	843.991996197651\\
79	843.991996197651\\
80	841.200120192687\\
81	841.200120192687\\
82	841.487196506278\\
83	841.487196506278\\
84	841.487196506278\\
85	841.487196506278\\
86	841.487196506278\\
87	820.706698085173\\
88	820.706698085173\\
89	820.706698085173\\
90	820.706698085173\\
91	822.671530136847\\
92	789.441285574144\\
93	789.441285574144\\
94	742.62918814359\\
95	742.62918814359\\
96	744.466557519992\\
97	744.466557519992\\
98	744.466557519992\\
99	744.466557519992\\
100	744.466557519992\\
100	1262.13892785128\\
99	1262.13892785128\\
98	1262.13892785128\\
97	1262.13892785128\\
96	1262.13892785128\\
95	1269.70635544391\\
94	1269.70635544391\\
93	1264.72595094145\\
92	1264.72595094145\\
91	1262.91116366732\\
90	1270.35069591199\\
89	1270.35069591199\\
88	1270.35069591199\\
87	1270.35069591199\\
86	1270.31812513286\\
85	1270.31812513286\\
84	1270.31812513286\\
83	1270.31812513286\\
82	1270.31812513286\\
81	1271.39288989272\\
80	1271.39288989272\\
79	1306.02389488772\\
78	1306.02389488772\\
77	1308.38194118268\\
76	1308.38194118268\\
75	1308.38194118268\\
74	1308.38194118268\\
73	1308.38194118268\\
72	1314.85708538711\\
71	1314.85708538711\\
70	1324.71085299795\\
69	1324.73212386039\\
68	1324.73212386039\\
67	1324.73212386039\\
66	1324.73212386039\\
65	1347.92971073389\\
64	1360.78103567523\\
63	1357.87111834694\\
62	1358.68446303272\\
61	1378.93937038376\\
60	1379.03888480582\\
59	1379.03888480582\\
58	1379.03888480582\\
57	1379.48985947939\\
56	1379.13837271854\\
55	1396.70777886399\\
54	1396.04539941137\\
53	1396.04539941137\\
52	1396.84211366097\\
51	1396.84211366097\\
50	1396.84211366097\\
49	1402.05788668902\\
48	1402.05788668902\\
47	1402.05788668902\\
46	1401.0683457327\\
45	1401.0683457327\\
44	1401.0830175519\\
43	1401.0830175519\\
42	1401.81895112878\\
41	1401.81895112878\\
40	1401.81895112878\\
39	1403.59712014008\\
38	1403.59712014008\\
37	1414.75095300302\\
36	1414.75095300302\\
35	1414.75095300302\\
34	1472.43781470803\\
33	1472.43781470803\\
32	1472.43781470803\\
31	1472.43781470803\\
30	1520.75908141504\\
29	1520.75908141504\\
28	1520.75908141504\\
27	1520.75908141504\\
26	1526.06844108676\\
25	1526.06844108676\\
24	1526.06844108676\\
23	1538.38533029549\\
22	1538.38533029549\\
21	1537.79469969343\\
20	1537.79469969343\\
19	1537.79469969343\\
18	1537.79469969343\\
17	1537.79469969343\\
16	1538.36032657311\\
15	1540.64198562186\\
14	1540.64198562186\\
13	1540.64198562186\\
12	1540.64198562186\\
11	1540.64198562186\\
10	1540.64198562186\\
9	1540.64198562186\\
8	1540.64198562186\\
7	1540.64198562186\\
6	1540.64198562186\\
5	1540.64198562186\\
4	1590.25493197973\\
3	1626.52742740666\\
2	1626.52742740666\\
1	2025.16468665826\\
}--cycle;
\addplot [color=mycolor3]
  table[row sep=crcr]{%
1	1821\\
2	1505\\
3	1505\\
4	1486\\
5	1440\\
6	1440\\
7	1440\\
8	1440\\
9	1440\\
10	1440\\
11	1440\\
12	1440\\
13	1440\\
14	1440\\
15	1440\\
16	1433\\
17	1430\\
18	1430\\
19	1430\\
20	1430\\
21	1430\\
22	1410\\
23	1410\\
24	1329\\
25	1329\\
26	1329\\
27	1327\\
28	1327\\
29	1327\\
30	1327\\
31	1280\\
32	1280\\
33	1280\\
34	1280\\
35	1259\\
36	1259\\
37	1259\\
38	1255\\
39	1255\\
40	1249\\
41	1249\\
42	1249\\
43	1246\\
44	1246\\
45	1245\\
46	1245\\
47	1203\\
48	1203\\
49	1203\\
50	1192\\
51	1192\\
52	1192\\
53	1190\\
54	1190\\
55	1185\\
56	1178\\
57	1174\\
58	1173\\
59	1173\\
60	1173\\
61	1173\\
62	1165\\
63	1164\\
64	1151\\
65	1120\\
66	1112\\
67	1112\\
68	1112\\
69	1112\\
70	1110\\
71	1097\\
72	1097\\
73	1086\\
74	1086\\
75	1086\\
76	1086\\
77	1086\\
78	1075\\
79	1075\\
80	1056\\
81	1056\\
82	1056\\
83	1056\\
84	1056\\
85	1056\\
86	1056\\
87	1046\\
88	1046\\
89	1046\\
90	1046\\
91	1043\\
92	1027\\
93	1027\\
94	1006\\
95	1006\\
96	1003\\
97	1003\\
98	1003\\
99	1003\\
100	1003\\
};
\addlegendentry{no Fv}


\addplot[area legend, draw=none, fill=red!50!mycolor3, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	714.642165145053\\
2	577.664662386374\\
3	373.017962699277\\
4	312.141006539161\\
5	293.018698925139\\
6	236.648587837963\\
7	213.072965927348\\
8	214.938479074703\\
9	225.319358801184\\
10	224.094074102085\\
11	223.924135871563\\
12	224.55023381953\\
13	219.20410585992\\
14	221.682188234697\\
15	214.061924758005\\
16	212.056853132655\\
17	204.061504201661\\
18	205.777393026252\\
19	205.777393026252\\
20	205.777393026252\\
21	208.496078027618\\
22	208.496078027618\\
23	208.496078027618\\
24	208.496078027618\\
25	208.496078027618\\
26	207.908697883528\\
27	207.908697883528\\
28	206.749127250821\\
29	206.730121123396\\
30	206.200106157875\\
31	206.200106157875\\
32	206.200106157875\\
33	206.200106157875\\
34	206.200106157875\\
35	206.200106157875\\
36	205.707345753773\\
37	205.707345753773\\
38	205.542193635576\\
39	205.71106664158\\
40	201.00582399422\\
41	201.00582399422\\
42	201.00582399422\\
43	201.00582399422\\
44	201.00582399422\\
45	201.14657810679\\
46	201.718896282033\\
47	201.718896282033\\
48	201.718896282033\\
49	201.718896282033\\
50	201.718896282033\\
51	201.718896282033\\
52	201.718896282033\\
53	201.052298812961\\
54	201.052298812961\\
55	199.73556560286\\
56	199.73556560286\\
57	199.092454558158\\
58	199.092454558158\\
59	199.092461592103\\
60	198.745680190765\\
61	198.745680190765\\
62	198.745680190765\\
63	198.754991695966\\
64	198.754991695966\\
65	198.929539335919\\
66	198.853176880064\\
67	198.890146398793\\
68	198.890146398793\\
69	198.890146398793\\
70	198.01078153044\\
71	197.756214089891\\
72	197.756214089891\\
73	197.756214089891\\
74	197.862738058345\\
75	197.862738058345\\
76	197.862738058345\\
77	197.278292657537\\
78	195.565905229047\\
79	195.525273336009\\
80	195.525273336009\\
81	194.87933479985\\
82	194.87933479985\\
83	194.87933479985\\
84	194.87933479985\\
85	194.892891638289\\
86	194.892891638289\\
87	194.625228605794\\
88	194.625228605794\\
89	193.94927902338\\
90	193.94927902338\\
91	193.94927902338\\
92	193.94927902338\\
93	193.94927902338\\
94	193.94927902338\\
95	192.853879281778\\
96	192.853879281778\\
97	192.832240571083\\
98	192.832240571083\\
99	192.458244549961\\
100	192.458244549961\\
100	193.012457045282\\
99	193.012457045282\\
98	193.952156065403\\
97	193.952156065403\\
96	195.439719230671\\
95	195.439719230671\\
94	195.450561575406\\
93	195.450561575406\\
92	195.450561575406\\
91	195.450561575406\\
90	195.450561575406\\
89	195.450561575406\\
88	195.555866173997\\
87	195.555866173997\\
86	195.496614089061\\
85	195.496614089061\\
84	197.042716331576\\
83	197.042716331576\\
82	197.042716331576\\
81	197.042716331576\\
80	197.512670052923\\
79	197.512670052923\\
78	197.567251000864\\
77	198.328471324018\\
76	199.079006850673\\
75	199.079006850673\\
74	199.079006850673\\
73	199.486125362161\\
72	199.486125362161\\
71	199.486125362161\\
70	199.613331384718\\
69	199.839676343116\\
68	199.839676343116\\
67	199.839676343116\\
66	200.325721946334\\
65	200.505560494266\\
64	202.147084895947\\
63	202.147084895947\\
62	202.190085144994\\
61	202.190085144994\\
60	202.190085144994\\
59	202.834614534662\\
58	202.835027617205\\
57	202.835027617205\\
56	202.665316209626\\
55	202.665316209626\\
54	202.328634477843\\
53	202.328634477843\\
52	202.21620990137\\
51	202.21620990137\\
50	202.21620990137\\
49	202.21620990137\\
48	202.21620990137\\
47	202.21620990137\\
46	202.21620990137\\
45	205.327987968176\\
44	205.85760379763\\
43	205.85760379763\\
42	205.85760379763\\
41	205.85760379763\\
40	205.85760379763\\
39	208.847892009657\\
38	209.482535103879\\
37	209.487922298927\\
36	209.487922298927\\
35	215.126663745927\\
34	215.126663745927\\
33	215.126663745927\\
32	215.126663745927\\
31	215.126663745927\\
30	215.126663745927\\
29	215.665157897756\\
28	215.660859801846\\
27	215.409227561996\\
26	215.409227561996\\
25	218.833552932229\\
24	218.833552932229\\
23	218.833552932229\\
22	218.833552932229\\
21	218.833552932229\\
20	236.874638466688\\
19	236.874638466688\\
18	236.874638466688\\
17	243.777287000179\\
16	245.515914746835\\
15	246.077125825654\\
14	246.187176942319\\
13	255.543740604241\\
12	257.669185725598\\
11	260.487624132308\\
10	303.305052477892\\
9	303.079186630862\\
8	376.888085187709\\
7	384.455738974118\\
6	406.707396094151\\
5	521.017773276358\\
4	554.07537547378\\
3	684.479088761997\\
2	940.165408781266\\
1	1054.45336044889\\
}--cycle;
\addplot [color=red!50!mycolor3]
  table[row sep=crcr]{%
1	885\\
2	759\\
3	529\\
4	433\\
5	407\\
6	322\\
7	299\\
8	296\\
9	264\\
10	264\\
11	242\\
12	241\\
13	237\\
14	234\\
15	230\\
16	229\\
17	224\\
18	221\\
19	221\\
20	221\\
21	214\\
22	214\\
23	214\\
24	214\\
25	214\\
26	212\\
27	212\\
28	211\\
29	211\\
30	211\\
31	211\\
32	211\\
33	211\\
34	211\\
35	211\\
36	208\\
37	208\\
38	208\\
39	207\\
40	203\\
41	203\\
42	203\\
43	203\\
44	203\\
45	203\\
46	202\\
47	202\\
48	202\\
49	202\\
50	202\\
51	202\\
52	202\\
53	202\\
54	202\\
55	201\\
56	201\\
57	201\\
58	201\\
59	201\\
60	200\\
61	200\\
62	200\\
63	200\\
64	200\\
65	200\\
66	200\\
67	199\\
68	199\\
69	199\\
70	199\\
71	199\\
72	199\\
73	199\\
74	198\\
75	198\\
76	198\\
77	198\\
78	197\\
79	197\\
80	197\\
81	196\\
82	196\\
83	196\\
84	196\\
85	195\\
86	195\\
87	195\\
88	195\\
89	195\\
90	195\\
91	195\\
92	195\\
93	195\\
94	195\\
95	194\\
96	194\\
97	193\\
98	193\\
99	193\\
100	193\\
};
\addlegendentry{no actdyn}

\legend{}
\end{axis}


==> new_figures/dataefficiency_cost_pointreaching_pd.tex <==
\begin{axis}[%
name =ax1,
scaled y ticks=base 10:\Factor,
xlabel near ticks, ylabel near ticks,
every y tick scale label/.style={at={(yticklabel* cs:1.03,0cm)},anchor=near yticklabel},
title style={at={(0.5,0.93)}},
width=0.643\figW,
height=\figH,
scale only axis,
xmin=0,
xmax=100,
xtick={  0,  20,  40,  60,  80, 100},
xlabel style={font=\color{white!15!black}},
xlabel={generations},
ymin=0,
ymax=5000,
ylabel style={font=\color{white!15!black}},
ylabel={cost},
axis background/.style={fill=white},
title={smooth point-reaching (OC)},
legend style={at={(1.03,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]

\addplot[area legend, draw=none, fill=mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	5170.03227375288\\
2	3643.14937266689\\
3	3013.88527938524\\
4	2783.06302901892\\
5	2549.27558055067\\
6	2205.76574250587\\
7	1736.53564003158\\
8	2025.07266339973\\
9	1933.88406465493\\
10	1862.31313228524\\
11	1813.45295146484\\
12	1535.58352075129\\
13	1419.20393942324\\
14	1302.38076622633\\
15	1260.28962879832\\
16	1216.52422340768\\
17	1216.52422340768\\
18	1140.17085108422\\
19	1026.54299533562\\
20	1026.54299533562\\
21	989.444818262883\\
22	964.4433972427\\
23	1011.36789330552\\
24	1028.30328882717\\
25	995.364425543746\\
26	995.364425543746\\
27	861.221345909889\\
28	823.945474588184\\
29	782.86172469087\\
30	782.86172469087\\
31	672.346402142427\\
32	680.882151120109\\
33	668.05050271671\\
34	647.775849970312\\
35	661.863514329305\\
36	673.36497392303\\
37	650.899122928831\\
38	566.681462789805\\
39	565.824814884483\\
40	565.824814884483\\
41	581.248166400597\\
42	589.111342550479\\
43	568.737250729501\\
44	581.285834479515\\
45	624.045399513396\\
46	605.210537505279\\
47	605.210537505279\\
48	605.210537505279\\
49	575.082734050564\\
50	575.082734050564\\
51	522.021632429589\\
52	494.714663446711\\
53	492.470394688581\\
54	487.464935565014\\
55	450.039038431918\\
56	438.747085867178\\
57	433.1179991205\\
58	422.485130389727\\
59	417.929148202331\\
60	431.177789871439\\
61	458.839303277193\\
62	458.839303277193\\
63	460.71701090311\\
64	460.71701090311\\
65	463.58723210839\\
66	516.538182005144\\
67	475.511449975345\\
68	475.511449975345\\
69	475.511449975345\\
70	416.417408383608\\
71	403.575941395932\\
72	399.111668085704\\
73	384.812067099911\\
74	417.763251132279\\
75	408.163147211992\\
76	408.163147211992\\
77	393.830605810589\\
78	413.536109632479\\
79	413.536109632479\\
80	413.536109632479\\
81	408.284445260311\\
82	389.082529534418\\
83	388.288298937817\\
84	417.8818916726\\
85	417.8818916726\\
86	417.636749850663\\
87	397.310580403872\\
88	397.192368692042\\
89	393.936863880994\\
90	413.376581858168\\
91	413.376581858168\\
92	405.190150470063\\
93	433.503949282877\\
94	433.503949282877\\
95	430.256629385682\\
96	430.256629385682\\
97	430.247981309142\\
98	424.62876209212\\
99	416.460492542109\\
100	431.15899699201\\
100	1197.84165586544\\
99	1257.97137573982\\
98	1260.58849430647\\
97	1262.54808321891\\
96	1262.55085180562\\
95	1262.55085180562\\
94	1263.61816175387\\
93	1263.61816175387\\
92	1390.56130791087\\
91	1393.21489136149\\
90	1393.21489136149\\
89	1451.54191816615\\
88	1452.71548167627\\
87	1452.75223077959\\
86	1459.81164653627\\
85	1459.90206577437\\
84	1459.90206577437\\
83	1549.50567257604\\
82	1549.7937327662\\
81	1556.50279462597\\
80	1558.54644637074\\
79	1558.54644637074\\
78	1558.54644637074\\
77	1644.4319506761\\
76	1650.38071209823\\
75	1650.38071209823\\
74	1653.82364503072\\
73	1752.97187263258\\
72	1757.42776226991\\
71	1759.15794742782\\
70	1764.57193898686\\
69	1785.45032960566\\
68	1785.45032960566\\
67	1785.45032960566\\
66	1796.39057309957\\
65	1971.64672289783\\
64	1980.26674830263\\
63	1980.26674830263\\
62	1985.90591930752\\
61	1985.90591930752\\
60	2090.36077908667\\
59	2130.15679684688\\
58	2131.78529674959\\
57	2136.09402329121\\
56	2137.85312466122\\
55	2142.7685853537\\
54	2153.76840739466\\
53	2155.19037026667\\
52	2155.95160872277\\
51	2165.13087277362\\
50	2181.52532096602\\
49	2181.52532096602\\
48	2192.40522106257\\
47	2192.40522106257\\
46	2192.40522106257\\
45	2200.65619943934\\
44	2486.53412169753\\
43	2527.30643768789\\
42	2577.68449966283\\
41	2601.3313908603\\
40	2647.7088956018\\
39	2647.7088956018\\
38	2648.05186856348\\
37	2675.28029988324\\
36	2683.6543589496\\
35	2718.2407792816\\
34	2774.1504087651\\
33	2782.95884486911\\
32	2786.4183029955\\
31	2812.11423213712\\
30	2853.46061567132\\
29	2853.46061567132\\
28	2867.26835056141\\
27	2881.38937961344\\
26	2918.27442389441\\
25	2918.27442389441\\
24	2932.83070250423\\
23	2983.93259459486\\
22	3125.42726114772\\
21	3134.70195505357\\
20	3150.21711913398\\
19	3150.21711913398\\
18	3210.1664588243\\
17	3225.86509212053\\
16	3225.86509212053\\
15	3233.50488148559\\
14	3244.18632076094\\
13	3315.37838555635\\
12	3395.02896668288\\
11	3502.76422321806\\
10	3911.99422186422\\
9	3948.92765822696\\
8	3999.63463916276\\
7	4993.00451050724\\
6	5242.57856212147\\
5	5319.98328006031\\
4	5374.79535934662\\
3	5486.10505602762\\
2	5970.80733529359\\
1	7826.03005114544\\
}--cycle;
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	6498\\
2	4807\\
3	4250\\
4	4079\\
5	3935\\
6	3724\\
7	3365\\
8	3012\\
9	2941\\
10	2887\\
11	2658\\
12	2465\\
13	2367\\
14	2273\\
15	2247\\
16	2221\\
17	2221\\
18	2175\\
19	2088\\
20	2088\\
21	2062\\
22	2045\\
23	1998\\
24	1981\\
25	1957\\
26	1957\\
27	1871\\
28	1846\\
29	1818\\
30	1818\\
31	1742\\
32	1734\\
33	1726\\
34	1711\\
35	1690\\
36	1679\\
37	1663\\
38	1607\\
39	1607\\
40	1607\\
41	1591\\
42	1583\\
43	1548\\
44	1534\\
45	1412\\
46	1399\\
47	1399\\
48	1399\\
49	1378\\
50	1378\\
51	1344\\
52	1325\\
53	1324\\
54	1321\\
55	1296\\
56	1288\\
57	1285\\
58	1277\\
59	1274\\
60	1261\\
61	1222\\
62	1222\\
63	1220\\
64	1220\\
65	1218\\
66	1156\\
67	1130\\
68	1130\\
69	1130\\
70	1090\\
71	1081\\
72	1078\\
73	1069\\
74	1036\\
75	1029\\
76	1029\\
77	1019\\
78	986\\
79	986\\
80	986\\
81	982\\
82	969\\
83	969\\
84	939\\
85	939\\
86	939\\
87	925\\
88	925\\
89	923\\
90	903\\
91	903\\
92	898\\
93	849\\
94	849\\
95	846\\
96	846\\
97	846\\
98	843\\
99	837\\
100	815\\
};
\addlegendentry{torque, c = 0.05 s}


\addplot[area legend, draw=none, fill=blue!50!mycolor1, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	661.289616605163\\
2	977.246670931292\\
3	944.509069720273\\
4	797.088050841908\\
5	756.338211651292\\
6	756.338211651292\\
7	756.338211651292\\
8	713.338547394196\\
9	713.338547394196\\
10	732.614609950776\\
11	715.301703223654\\
12	715.301703223654\\
13	702.04431388911\\
14	684.770629381988\\
15	684.770629381988\\
16	685.317806528589\\
17	685.296116283732\\
18	662.233568320906\\
19	638.193654648692\\
20	633.014868592728\\
21	606.912306113397\\
22	584.742583739849\\
23	569.358785490491\\
24	566.87175227992\\
25	567.543842129013\\
26	567.543842129013\\
27	559.377762114584\\
28	554.973517325879\\
29	549.430901562195\\
30	545.424750257415\\
31	535.130794937847\\
32	528.045998842465\\
33	499.541660773917\\
34	489.238779114913\\
35	489.238779114913\\
36	493.922469729725\\
37	487.667479342535\\
38	486.397742459972\\
39	482.25104375025\\
40	479.047266542927\\
41	473.912832585759\\
42	489.806071925413\\
43	485.994712020022\\
44	469.405351037119\\
45	466.924573839571\\
46	461.895387821864\\
47	458.641032793744\\
48	452.323403061573\\
49	466.297711812363\\
50	450.639343158452\\
51	444.714664229167\\
52	439.839705700187\\
53	434.163446939647\\
54	389.77671703227\\
55	389.43363113756\\
56	389.744117920342\\
57	379.565692149799\\
58	342.279714205261\\
59	341.263581062384\\
60	329.105281336259\\
61	329.105281336259\\
62	324.465824693138\\
63	319.731088165226\\
64	321.711910102816\\
65	306.460308832485\\
66	304.988682722165\\
67	297.841720067647\\
68	298.091739237359\\
69	295.810940046274\\
70	295.964379056398\\
71	292.467723135313\\
72	291.961612840659\\
73	289.398128391543\\
74	288.918906132034\\
75	289.957864677694\\
76	287.262161123179\\
77	287.949082455263\\
78	288.004801819658\\
79	288.785248081413\\
80	287.699492653192\\
81	282.961945109615\\
82	281.889179708085\\
83	278.498393780664\\
84	278.57793028674\\
85	277.977567743912\\
86	275.1564070434\\
87	275.584023680347\\
88	273.586872250078\\
89	274.910214462076\\
90	274.910214462076\\
91	281.775586771367\\
92	279.425920195026\\
93	279.015757859746\\
94	278.635098154042\\
95	277.971443148872\\
96	277.969019823314\\
97	281.596297494516\\
98	284.819534000973\\
99	286.920146941799\\
100	286.580071340258\\
100	317.462913720376\\
99	317.556895364824\\
98	325.16357294226\\
97	348.676930738359\\
96	359.794350418751\\
95	359.795300566413\\
94	359.928093064211\\
93	360.067454042013\\
92	360.23173629622\\
91	369.587352887379\\
90	390.57323362271\\
89	390.57323362271\\
88	396.609671945447\\
87	397.406504780326\\
86	401.918404220232\\
85	403.077125648195\\
84	404.587142917951\\
83	404.830091701385\\
82	405.612187192105\\
81	406.030556139149\\
80	408.999185946104\\
79	417.602487608854\\
78	420.051272581233\\
77	420.225884117689\\
76	422.376279145479\\
75	423.226866337677\\
74	426.956258223376\\
73	427.02582965994\\
72	431.633091881714\\
71	431.988604231846\\
70	434.515388717464\\
69	436.130594478499\\
68	436.397404468093\\
67	437.183445970326\\
66	445.230281212171\\
65	445.91758916621\\
64	453.360502221058\\
63	469.048411168029\\
62	474.655871765328\\
61	481.322114569626\\
60	481.322114569626\\
59	503.941235621222\\
58	506.985183138122\\
57	534.127543197494\\
56	542.435333706015\\
55	546.133272723632\\
54	546.864736280153\\
53	553.79549207305\\
52	563.129994386468\\
51	568.262945993505\\
50	588.867367345949\\
49	588.071885361522\\
48	672.472730837903\\
47	682.582472158894\\
46	757.754189750951\\
45	759.435735920918\\
44	763.559698148652\\
43	765.370703547091\\
42	767.28504273211\\
41	820.234724090187\\
40	850.267694936585\\
39	850.415459155712\\
38	851.784669890548\\
37	856.111071147276\\
36	856.446090931515\\
35	871.217185250978\\
34	871.217185250978\\
33	873.995361148473\\
32	921.695713159492\\
31	921.763689415109\\
30	956.176790981338\\
29	966.964219813359\\
28	990.055513813827\\
27	990.368403938458\\
26	1003.38219992896\\
25	1003.38219992896\\
24	1005.76929383791\\
23	1006.05697110472\\
22	1010.57962817735\\
21	1010.65809201974\\
20	1022.35374868098\\
19	1022.91042944751\\
18	1026.62994856721\\
17	1034.13282897698\\
16	1034.15667088096\\
15	1075.64058534475\\
14	1075.64058534475\\
13	1075.75650922861\\
12	1094.62157339565\\
11	1094.62157339565\\
10	1322.2349201139\\
9	1505.05801564296\\
8	1505.05801564296\\
7	1596.18568083774\\
6	1596.18568083774\\
5	1596.18568083774\\
4	1615.70612566641\\
3	2324.15102345855\\
2	3680.9530728926\\
1	6491.36035484248\\
}--cycle;
\addplot [color=blue!50!mycolor1]
  table[row sep=crcr]{%
1	3576\\
2	2329\\
3	1634\\
4	1206\\
5	1176\\
6	1176\\
7	1176\\
8	1109\\
9	1109\\
10	1027\\
11	905\\
12	905\\
13	889\\
14	880\\
15	880\\
16	860\\
17	860\\
18	844\\
19	831\\
20	828\\
21	809\\
22	798\\
23	788\\
24	786\\
25	785\\
26	785\\
27	775\\
28	773\\
29	758\\
30	751\\
31	728\\
32	725\\
33	687\\
34	680\\
35	680\\
36	675\\
37	672\\
38	669\\
39	666\\
40	665\\
41	647\\
42	629\\
43	626\\
44	616\\
45	613\\
46	610\\
47	571\\
48	562\\
49	527\\
50	520\\
51	506\\
52	501\\
53	494\\
54	468\\
55	468\\
56	466\\
57	457\\
58	425\\
59	423\\
60	405\\
61	405\\
62	400\\
63	394\\
64	388\\
65	376\\
66	375\\
67	368\\
68	367\\
69	366\\
70	365\\
71	362\\
72	362\\
73	358\\
74	358\\
75	357\\
76	355\\
77	354\\
78	354\\
79	353\\
80	348\\
81	344\\
82	344\\
83	342\\
84	342\\
85	341\\
86	339\\
87	336\\
88	335\\
89	333\\
90	333\\
91	326\\
92	320\\
93	320\\
94	319\\
95	319\\
96	319\\
97	315\\
98	305\\
99	302\\
100	302\\
};
\addlegendentry{torque, c = 0.15 s}


\addplot[area legend, draw=none, fill=blue, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1083.94164841792\\
2	794.545435134731\\
3	704.192255409083\\
4	701.134326487207\\
5	694.808452919495\\
6	652.209499657079\\
7	648.888903551531\\
8	656.45155232808\\
9	656.920038632598\\
10	649.40664047447\\
11	649.40664047447\\
12	645.434130799015\\
13	645.434130799015\\
14	645.699902211598\\
15	645.542333450434\\
16	645.542333450434\\
17	636.415999106652\\
18	637.603189663503\\
19	637.778933691178\\
20	636.635836780502\\
21	614.495885603808\\
22	614.107635046692\\
23	572.580531743537\\
24	555.324258364133\\
25	536.071943719922\\
26	536.071943719922\\
27	535.336137312279\\
28	526.774258154144\\
29	514.285240413715\\
30	502.249790877919\\
31	502.249790877919\\
32	500.236038119568\\
33	479.344870023028\\
34	454.021923366868\\
35	455.237778680672\\
36	451.012544814158\\
37	450.710770075302\\
38	449.941725825424\\
39	450.413910826878\\
40	447.926388059455\\
41	434.272252263923\\
42	427.015894526178\\
43	426.387885160478\\
44	432.339144158234\\
45	432.029235590877\\
46	429.779197357935\\
47	424.231140827622\\
48	423.969410390353\\
49	423.969410390353\\
50	423.914239015292\\
51	421.37221510034\\
52	418.876497373984\\
53	416.192693428237\\
54	410.405103097919\\
55	409.966573650248\\
56	407.441313763792\\
57	402.385715395574\\
58	395.372603645508\\
59	394.961683309964\\
60	394.547491419885\\
61	394.336376450156\\
62	388.698095262638\\
63	388.50793500901\\
64	388.482677424752\\
65	388.478373721849\\
66	388.393843902907\\
67	388.318082207792\\
68	388.318082207792\\
69	388.231559875928\\
70	386.9228618396\\
71	385.966217080338\\
72	385.935400238512\\
73	385.895337634896\\
74	384.393837711543\\
75	381.68983822879\\
76	381.68743000909\\
77	381.575900482241\\
78	381.561644666656\\
79	381.519729874943\\
80	380.613914828196\\
81	380.02435361736\\
82	379.308840419949\\
83	379.011322748535\\
84	378.999782004617\\
85	378.999085191276\\
86	378.649916635589\\
87	378.581360010999\\
88	378.581360010999\\
89	378.484445050155\\
90	378.479237041359\\
91	378.478819593061\\
92	378.408931554198\\
93	378.391918974319\\
94	378.284118355776\\
95	378.186739329333\\
96	378.186739329333\\
97	378.178320436045\\
98	378.178320436045\\
99	378.172674021632\\
100	378.155784640731\\
100	466.869762461439\\
99	466.868974866717\\
98	466.902174999279\\
97	466.902174999279\\
96	466.931627562019\\
95	466.931627562019\\
94	466.921870728478\\
93	466.930828323438\\
92	466.936404268747\\
91	466.929550821431\\
90	466.929507280735\\
89	466.982290626576\\
88	467.023049044693\\
87	467.023049044693\\
86	467.016439061075\\
85	466.983549807674\\
84	466.990458006029\\
83	467.109115724308\\
82	467.252465621823\\
81	467.191270294799\\
80	467.145337579885\\
79	467.083068623541\\
78	467.077432366927\\
77	467.223219271684\\
76	467.320123743087\\
75	467.345179076365\\
74	467.428115916062\\
73	467.821871928179\\
72	467.87042884477\\
71	467.865112595187\\
70	468.378195083874\\
69	468.40740774632\\
68	468.488377925865\\
67	468.488377925865\\
66	469.182100103753\\
65	470.163152307302\\
64	470.189892572444\\
63	470.47930675546\\
62	473.47906893478\\
61	473.732402600548\\
60	476.420549491272\\
59	476.327097226378\\
58	476.489479051228\\
57	479.35959615439\\
56	483.19165356278\\
55	486.747300965976\\
54	490.473817954474\\
53	502.652926565333\\
52	502.582830860023\\
51	508.298520830002\\
50	507.748011685474\\
49	507.942358863781\\
48	507.942358863781\\
47	508.798787017036\\
46	516.896462757442\\
45	516.285607989744\\
44	516.202348079164\\
43	556.935876311467\\
42	557.649180713919\\
41	558.043721890984\\
40	565.202346335247\\
39	567.859633281839\\
38	570.436632407033\\
37	570.326255688148\\
36	570.771422077133\\
35	616.422455480104\\
34	627.572379348708\\
33	638.816652783296\\
32	646.677998694583\\
31	650.74489237834\\
30	650.74489237834\\
29	653.579133632443\\
28	650.968912436178\\
27	670.113057525592\\
26	669.954442762706\\
25	669.954442762706\\
24	678.720269805939\\
23	673.437200496022\\
22	663.06998283479\\
21	667.775571933131\\
20	678.25224407229\\
19	690.962253191531\\
18	692.343556652675\\
17	699.187313669683\\
16	702.860691206039\\
15	702.860691206039\\
14	709.895225790493\\
13	712.652724679152\\
12	712.652724679152\\
11	714.091371662041\\
10	714.091371662041\\
9	724.854655488439\\
8	741.628495624467\\
7	811.155073642865\\
6	820.179777899462\\
5	826.308457721423\\
4	1021.05984776962\\
3	1062.36690407385\\
2	1628.79830806761\\
1	2046.4385193762\\
}--cycle;
\addplot [color=blue]
  table[row sep=crcr]{%
1	1565\\
2	1212\\
3	883\\
4	861\\
5	761\\
6	736\\
7	730\\
8	699\\
9	691\\
10	682\\
11	682\\
12	679\\
13	679\\
14	678\\
15	674\\
16	674\\
17	668\\
18	665\\
19	664\\
20	657\\
21	641\\
22	639\\
23	623\\
24	617\\
25	603\\
26	603\\
27	603\\
28	589\\
29	584\\
30	576\\
31	576\\
32	573\\
33	559\\
34	541\\
35	536\\
36	511\\
37	511\\
38	510\\
39	509\\
40	507\\
41	496\\
42	492\\
43	492\\
44	474\\
45	474\\
46	473\\
47	467\\
48	466\\
49	466\\
50	466\\
51	465\\
52	461\\
53	459\\
54	450\\
55	448\\
56	445\\
57	441\\
58	436\\
59	436\\
60	435\\
61	434\\
62	431\\
63	429\\
64	429\\
65	429\\
66	429\\
67	428\\
68	428\\
69	428\\
70	428\\
71	427\\
72	427\\
73	427\\
74	426\\
75	425\\
76	425\\
77	424\\
78	424\\
79	424\\
80	424\\
81	424\\
82	423\\
83	423\\
84	423\\
85	423\\
86	423\\
87	423\\
88	423\\
89	423\\
90	423\\
91	423\\
92	423\\
93	423\\
94	423\\
95	423\\
96	423\\
97	423\\
98	423\\
99	423\\
100	423\\
};
\addlegendentry{torque, c = 0.3 s}


\addplot[area legend, draw=none, fill=orange, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	891.813524513513\\
2	819.409843551937\\
3	766.927512436109\\
4	681.790680263488\\
5	649.033795495181\\
6	592.132559512566\\
7	484.435877900163\\
8	472.088364883036\\
9	443.342397611295\\
10	426.391575269901\\
11	402.090747821125\\
12	385.924804431583\\
13	372.144984684559\\
14	359.458853051741\\
15	354.447215788007\\
16	347.479898170432\\
17	346.02794573735\\
18	336.158708629221\\
19	334.376507703783\\
20	329.870870084657\\
21	330.012487688409\\
22	329.471144850914\\
23	329.471144850914\\
24	328.405149708682\\
25	326.029065632327\\
26	323.784277314758\\
27	322.755013130461\\
28	321.875611921904\\
29	322.473074096898\\
30	321.665435072793\\
31	321.896634485784\\
32	321.621919715792\\
33	320.982561993955\\
34	320.982561993955\\
35	319.493867874908\\
36	318.652385910739\\
37	318.808018437192\\
38	318.808018437192\\
39	320.76094240268\\
40	319.860838462048\\
41	319.912091285084\\
42	320.07549917476\\
43	320.07549917476\\
44	320.07549917476\\
45	318.08163196237\\
46	318.08163196237\\
47	317.770448196243\\
48	317.291240761116\\
49	317.291240761116\\
50	316.171163054462\\
51	316.171163054462\\
52	316.171163054462\\
53	316.890828061565\\
54	315.960066347777\\
55	315.710672576696\\
56	315.710672576696\\
57	313.161472150081\\
58	312.509780109113\\
59	312.080489574408\\
60	311.585451287641\\
61	311.682414500046\\
62	311.682414500046\\
63	311.682414500046\\
64	310.544425483001\\
65	310.544425483001\\
66	310.246696193509\\
67	309.74268026204\\
68	309.74268026204\\
69	309.74268026204\\
70	309.739933175232\\
71	308.618275932413\\
72	308.618275932413\\
73	306.975277029445\\
74	306.975277029445\\
75	306.173589656686\\
76	306.562741648895\\
77	305.664372923498\\
78	305.664372923498\\
79	305.664372923498\\
80	305.640874469217\\
81	305.77782594072\\
82	305.77782594072\\
83	305.77782594072\\
84	305.880275684867\\
85	305.880275684867\\
86	305.579299824209\\
87	305.051837259119\\
88	304.551919087331\\
89	304.583425846264\\
90	304.583425846264\\
91	304.583425846264\\
92	304.583425846264\\
93	304.573778178\\
94	304.411291306328\\
95	304.411291306328\\
96	304.411291306328\\
97	304.411291306328\\
98	304.411291306328\\
99	304.411291306328\\
100	304.257610128137\\
100	309.523233804604\\
99	310.392556236287\\
98	310.392556236287\\
97	310.392556236287\\
96	310.392556236287\\
95	310.392556236287\\
94	310.392556236287\\
93	311.409361324253\\
92	311.578967880502\\
91	311.578967880502\\
90	311.578967880502\\
89	311.578967880502\\
88	312.35798113371\\
87	312.478676873282\\
86	312.807456768638\\
85	314.563128518639\\
84	314.563128518639\\
83	315.513123869668\\
82	315.513123869668\\
81	315.513123869668\\
80	316.308225496201\\
79	316.367888818264\\
78	316.367888818264\\
77	316.367888818264\\
76	316.177295979946\\
75	317.782385189032\\
74	318.633615309913\\
73	318.633615309913\\
72	321.168133906284\\
71	321.168133906284\\
70	321.714134862103\\
69	321.714234646203\\
68	321.714234646203\\
67	321.714234646203\\
66	322.348366315542\\
65	322.308677800564\\
64	322.308677800564\\
63	322.366906446803\\
62	322.366906446803\\
61	322.366906446803\\
60	323.3095213827\\
59	324.402983224711\\
58	329.43727699767\\
57	329.566591977709\\
56	329.539424948941\\
55	329.539424948941\\
54	329.555785881415\\
53	329.717094672125\\
52	332.929442762828\\
51	332.929442762828\\
50	332.929442762828\\
49	334.766872048467\\
48	334.766872048467\\
47	334.864782639788\\
46	334.953214384808\\
45	334.953214384808\\
44	339.141598778996\\
43	339.141598778996\\
42	339.141598778996\\
41	340.317282215621\\
40	340.486070378614\\
39	340.691905353095\\
38	346.90083866664\\
37	346.90083866664\\
36	347.386392996367\\
35	348.179239330056\\
34	351.944118040282\\
33	351.944118040282\\
32	353.560847305629\\
31	356.711858038168\\
30	360.366751381295\\
29	360.566123651921\\
28	366.714319688962\\
27	366.70049718591\\
26	366.845950420562\\
25	367.044018866555\\
24	369.097458938452\\
23	369.538389581555\\
22	369.538389581555\\
21	369.828437691072\\
20	372.882659133978\\
19	372.752109694634\\
18	381.884984204696\\
17	404.386836655814\\
16	414.595925807957\\
15	426.023966372821\\
14	441.544066109695\\
13	451.289982961733\\
12	462.47911059179\\
11	497.017208028262\\
10	535.203306088386\\
9	564.393761209783\\
8	570.317601196132\\
7	652.606919628772\\
6	673.567520911265\\
5	709.307959696982\\
4	798.762127891694\\
3	871.949668402133\\
2	957.603899121031\\
1	1021.93461883201\\
}--cycle;
\addplot [color=orange]
  table[row sep=crcr]{%
1	957\\
2	889\\
3	819\\
4	740\\
5	679\\
6	633\\
7	569\\
8	521\\
9	504\\
10	481\\
11	450\\
12	424\\
13	412\\
14	401\\
15	390\\
16	381\\
17	375\\
18	359\\
19	354\\
20	351\\
21	350\\
22	350\\
23	350\\
24	349\\
25	347\\
26	345\\
27	345\\
28	344\\
29	342\\
30	341\\
31	339\\
32	338\\
33	336\\
34	336\\
35	334\\
36	333\\
37	333\\
38	333\\
39	331\\
40	330\\
41	330\\
42	330\\
43	330\\
44	330\\
45	327\\
46	327\\
47	326\\
48	326\\
49	326\\
50	325\\
51	325\\
52	325\\
53	323\\
54	323\\
55	323\\
56	323\\
57	321\\
58	321\\
59	318\\
60	317\\
61	317\\
62	317\\
63	317\\
64	316\\
65	316\\
66	316\\
67	316\\
68	316\\
69	316\\
70	316\\
71	315\\
72	315\\
73	313\\
74	313\\
75	312\\
76	311\\
77	311\\
78	311\\
79	311\\
80	311\\
81	311\\
82	311\\
83	311\\
84	310\\
85	310\\
86	309\\
87	309\\
88	308\\
89	308\\
90	308\\
91	308\\
92	308\\
93	308\\
94	307\\
95	307\\
96	307\\
97	307\\
98	307\\
99	307\\
100	307\\
};
\addlegendentry{muscle, c = 0.05 s}


\addplot[area legend, draw=none, fill=red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	552.682241146824\\
2	532.195486728073\\
3	494.982852784691\\
4	458.861138435318\\
5	431.997275946587\\
6	408.396995591456\\
7	387.742175484299\\
8	370.309003353631\\
9	370.545132782615\\
10	362.592665080047\\
11	359.049052768056\\
12	340.88791327695\\
13	334.886017540123\\
14	332.314620106687\\
15	330.910297188282\\
16	330.910297188282\\
17	326.180634119869\\
18	321.805250128372\\
19	322.760608780375\\
20	317.313798359896\\
21	314.943710728092\\
22	314.435600535633\\
23	313.271744527597\\
24	312.58056132806\\
25	307.93361519106\\
26	307.892618440559\\
27	307.628295892923\\
28	307.628295892923\\
29	307.628295892923\\
30	305.829809290952\\
31	305.829809290952\\
32	306.427226186994\\
33	305.290178087892\\
34	302.86729123274\\
35	301.836009686807\\
36	301.358685655954\\
37	298.639750364164\\
38	297.088710303267\\
39	296.666613933378\\
40	296.666613933378\\
41	296.666613933378\\
42	296.666613933378\\
43	295.922884928342\\
44	295.922884928342\\
45	295.922884928342\\
46	298.904607297776\\
47	298.635085760101\\
48	298.635085760101\\
49	297.458750244978\\
50	297.409053523348\\
51	297.409053523348\\
52	297.274088662947\\
53	296.432088012206\\
54	295.895319641192\\
55	295.966679079473\\
56	295.82187808108\\
57	295.82187808108\\
58	295.82187808108\\
59	295.730491087913\\
60	295.930767620448\\
61	295.930767620448\\
62	295.021567464205\\
63	293.849212335177\\
64	293.849212335177\\
65	293.431147503788\\
66	293.431147503788\\
67	293.431147503788\\
68	292.870840882251\\
69	292.870840882251\\
70	292.870840882251\\
71	293.882471050094\\
72	293.762743690591\\
73	293.762743690591\\
74	293.614047478722\\
75	293.614047478722\\
76	293.614047478722\\
77	293.614047478722\\
78	293.583204800804\\
79	293.145118731767\\
80	293.0431027717\\
81	292.832716719971\\
82	293.03983837787\\
83	293.255007749399\\
84	293.255007749399\\
85	293.255007749399\\
86	292.908873796951\\
87	293.746636735984\\
88	293.399802072843\\
89	293.65941124007\\
90	293.65941124007\\
91	293.503528032247\\
92	293.521369224434\\
93	293.479526562105\\
94	293.479526562105\\
95	293.479526562105\\
96	293.378389847049\\
97	293.201098692096\\
98	293.201098692096\\
99	293.201098692096\\
100	293.208612584878\\
100	299.285750487676\\
99	299.343445420326\\
98	299.343445420326\\
97	299.343445420326\\
96	299.361803134541\\
95	299.431758787246\\
94	299.431758787246\\
93	299.431758787246\\
92	299.451103280379\\
91	299.506681995384\\
90	299.546107857017\\
89	299.546107857017\\
88	300.404192729822\\
87	300.601863677189\\
86	303.309530787653\\
85	303.449296759838\\
84	303.449296759838\\
83	303.449296759838\\
82	304.110987259452\\
81	304.975048644508\\
80	305.004153976787\\
79	305.026975227037\\
78	305.202122411977\\
77	305.206083655068\\
76	305.206083655068\\
75	305.206083655068\\
74	305.206083655068\\
73	305.255049799549\\
72	305.255049799549\\
71	305.301043688151\\
70	308.377474589691\\
69	308.377474589691\\
68	308.377474589691\\
67	308.656411476383\\
66	308.656411476383\\
65	308.656411476383\\
64	308.839302789658\\
63	308.839302789658\\
62	309.322895227011\\
61	309.792279942395\\
60	309.792279942395\\
59	311.9418471586\\
58	314.941545698064\\
57	314.941545698064\\
56	314.941545698064\\
55	315.000080653988\\
54	316.474834998047\\
53	316.809738331155\\
52	316.917644447434\\
51	317.016328129872\\
50	317.016328129872\\
49	317.022703541049\\
48	317.356134907148\\
47	317.356134907148\\
46	317.411298747907\\
45	328.602764805711\\
44	328.602764805711\\
43	328.602764805711\\
42	328.924306078856\\
41	328.924306078856\\
40	328.924306078856\\
39	328.924306078856\\
38	329.205093740657\\
37	329.71848713306\\
36	330.532495137564\\
35	330.741080513088\\
34	331.161791898278\\
33	331.855676971329\\
32	332.147620707169\\
31	337.038802431629\\
30	337.038802431629\\
29	337.885464925427\\
28	337.885464925427\\
27	337.885464925427\\
26	338.151817382729\\
25	338.196639034067\\
24	340.154745016621\\
23	340.538991652407\\
22	341.603028507782\\
21	341.537554335023\\
20	345.757949292655\\
19	345.255106311983\\
18	349.063446075038\\
17	351.276562073804\\
16	353.493318791377\\
15	353.493318791377\\
14	359.717515949388\\
13	362.380356689992\\
12	368.414944249113\\
11	374.885869760552\\
10	392.274111948794\\
9	399.382479588957\\
8	448.306287795917\\
7	494.469893338674\\
6	560.959781508393\\
5	628.047365255794\\
4	681.189497337559\\
3	760.867271863049\\
2	842.521082164984\\
1	927.149794195054\\
}--cycle;
\addplot [color=red]
  table[row sep=crcr]{%
1	740\\
2	687\\
3	628\\
4	570\\
5	530\\
6	485\\
7	441\\
8	409\\
9	385\\
10	377\\
11	367\\
12	355\\
13	349\\
14	346\\
15	342\\
16	342\\
17	339\\
18	335\\
19	334\\
20	332\\
21	328\\
22	328\\
23	327\\
24	326\\
25	323\\
26	323\\
27	323\\
28	323\\
29	323\\
30	321\\
31	321\\
32	319\\
33	319\\
34	317\\
35	316\\
36	316\\
37	314\\
38	313\\
39	313\\
40	313\\
41	313\\
42	313\\
43	312\\
44	312\\
45	312\\
46	308\\
47	308\\
48	308\\
49	307\\
50	307\\
51	307\\
52	307\\
53	307\\
54	306\\
55	305\\
56	305\\
57	305\\
58	305\\
59	304\\
60	303\\
61	303\\
62	302\\
63	301\\
64	301\\
65	301\\
66	301\\
67	301\\
68	301\\
69	301\\
70	301\\
71	300\\
72	300\\
73	300\\
74	299\\
75	299\\
76	299\\
77	299\\
78	299\\
79	299\\
80	299\\
81	299\\
82	299\\
83	298\\
84	298\\
85	298\\
86	298\\
87	297\\
88	297\\
89	297\\
90	297\\
91	297\\
92	296\\
93	296\\
94	296\\
95	296\\
96	296\\
97	296\\
98	296\\
99	296\\
100	296\\
};
\addlegendentry{muscle, c = 0.15 s}


\addplot[area legend, draw=none, fill=black!50!red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	478.784964605733\\
2	405.471064872286\\
3	371.293077597947\\
4	334.211355718086\\
5	307.72086890057\\
6	314.992386608893\\
7	309.494558607774\\
8	314.80792297688\\
9	316.945715123061\\
10	320.254359515838\\
11	320.254359515838\\
12	321.522045810314\\
13	321.522045810314\\
14	321.593397134307\\
15	315.080002510151\\
16	315.440630126395\\
17	315.052452168554\\
18	315.768254645231\\
19	314.982019815006\\
20	312.292325636975\\
21	311.250962132487\\
22	311.20627700475\\
23	309.546729077254\\
24	307.864576436952\\
25	307.733989558666\\
26	307.738727936513\\
27	306.968471738838\\
28	306.903692317399\\
29	306.903692317399\\
30	302.720290737671\\
31	302.049444733298\\
32	301.098596324628\\
33	300.86232388654\\
34	300.896349498827\\
35	301.2500477729\\
36	299.493512580349\\
37	299.493512580349\\
38	299.058271870041\\
39	299.971851466504\\
40	299.27014701626\\
41	298.7326150187\\
42	298.688094535372\\
43	298.688094535372\\
44	298.872348590486\\
45	298.818975230423\\
46	298.663696096775\\
47	298.632724864559\\
48	298.30039004882\\
49	298.263747831709\\
50	298.054445519377\\
51	297.769434461424\\
52	297.645645914504\\
53	297.645645914504\\
54	297.798436488542\\
55	297.441368811099\\
56	297.474038740806\\
57	297.463196541043\\
58	297.075002375787\\
59	297.075002375787\\
60	297.091501870633\\
61	297.14738620463\\
62	297.063581419628\\
63	297.063581419628\\
64	297.066901738977\\
65	296.96040675893\\
66	296.905477221653\\
67	296.73239123112\\
68	296.679288939549\\
69	296.38193836614\\
70	296.38193836614\\
71	296.258263077049\\
72	296.258263077049\\
73	296.096515432179\\
74	296.064794076049\\
75	295.878982979178\\
76	295.878982979178\\
77	295.874079302839\\
78	295.807449262563\\
79	295.807449262563\\
80	295.829974509044\\
81	295.80705517866\\
82	295.748636480224\\
83	295.690104573764\\
84	295.620965874913\\
85	295.531053499314\\
86	295.507753271011\\
87	295.503806281136\\
88	295.490050992914\\
89	295.471324035258\\
90	295.469055603906\\
91	295.466708822964\\
92	295.322785658597\\
93	295.322785658597\\
94	295.319357104251\\
95	295.213290065541\\
96	295.225047984934\\
97	295.218750949224\\
98	295.241732960207\\
99	295.185141706945\\
100	295.207515905097\\
100	296.586373624062\\
99	296.744789154563\\
98	296.758481322761\\
97	296.830223682989\\
96	296.84529919263\\
95	296.881890366744\\
94	296.926320742229\\
93	296.927465114184\\
92	296.927465114184\\
91	297.046559951219\\
90	297.046520721542\\
89	297.144622496289\\
88	297.271015503229\\
87	297.271253964249\\
86	297.272554508571\\
85	297.274976148588\\
84	297.31587165495\\
83	297.37105387912\\
82	297.534131463404\\
81	297.528366169792\\
80	297.52850887704\\
79	297.702675576991\\
78	297.702675576991\\
77	297.744711387975\\
76	297.808055619363\\
75	297.808055619363\\
74	297.824411043288\\
73	297.82029600616\\
72	298.112071739658\\
71	298.112071739658\\
70	298.127744495144\\
69	298.127744495144\\
68	298.444783258253\\
67	298.51816438613\\
66	298.791119361473\\
65	298.864810448537\\
64	299.448562220308\\
63	299.486941558375\\
62	299.486941558375\\
61	299.466518094596\\
60	299.822723559806\\
59	299.932578654324\\
58	299.932578654324\\
57	300.324016439382\\
56	300.473936213258\\
55	300.758478320026\\
54	300.957036842652\\
53	301.79806761209\\
52	301.79806761209\\
51	301.883617082383\\
50	301.938875423132\\
49	302.019544363849\\
48	302.090969132876\\
47	302.124407350267\\
46	302.155450503061\\
45	302.430556773513\\
44	303.155189568671\\
43	304.468835760873\\
42	304.468835760873\\
41	304.925579773449\\
40	306.661043106797\\
39	306.864639193877\\
38	309.949401243958\\
37	310.070071099272\\
36	310.070071099272\\
35	310.768267538967\\
34	311.925858288884\\
33	312.392857328035\\
32	312.415955980691\\
31	313.335379799198\\
30	313.493741306611\\
29	315.426303195577\\
28	315.426303195577\\
27	317.791511387295\\
26	318.864199388826\\
25	319.057883109539\\
24	319.347361658081\\
23	321.478311072659\\
22	321.941704326059\\
21	322.468406608785\\
20	327.116203869101\\
19	328.277876371554\\
18	329.64644410863\\
17	332.763691791231\\
16	333.545560136616\\
15	341.132416208063\\
14	349.101152806001\\
13	349.792668213235\\
12	349.792668213235\\
11	363.250716867875\\
10	363.250716867875\\
9	395.456901363967\\
8	402.427850686458\\
7	434.902433668952\\
6	463.030045055925\\
5	504.219555150483\\
4	581.319239144814\\
3	636.122637822107\\
2	724.181215955365\\
1	875.388880002082\\
}--cycle;
\addplot [color=black!50!red]
  table[row sep=crcr]{%
1	677\\
2	565\\
3	504\\
4	458\\
5	406\\
6	389\\
7	372\\
8	359\\
9	356\\
10	342\\
11	342\\
12	336\\
13	336\\
14	335\\
15	328\\
16	324\\
17	324\\
18	323\\
19	322\\
20	320\\
21	317\\
22	317\\
23	316\\
24	314\\
25	313\\
26	313\\
27	312\\
28	311\\
29	311\\
30	308\\
31	308\\
32	307\\
33	307\\
34	306\\
35	306\\
36	305\\
37	305\\
38	305\\
39	303\\
40	303\\
41	302\\
42	302\\
43	302\\
44	301\\
45	301\\
46	300\\
47	300\\
48	300\\
49	300\\
50	300\\
51	300\\
52	300\\
53	300\\
54	299\\
55	299\\
56	299\\
57	299\\
58	299\\
59	299\\
60	298\\
61	298\\
62	298\\
63	298\\
64	298\\
65	298\\
66	298\\
67	298\\
68	298\\
69	297\\
70	297\\
71	297\\
72	297\\
73	297\\
74	297\\
75	297\\
76	297\\
77	297\\
78	297\\
79	297\\
80	297\\
81	297\\
82	297\\
83	297\\
84	296\\
85	296\\
86	296\\
87	296\\
88	296\\
89	296\\
90	296\\
91	296\\
92	296\\
93	296\\
94	296\\
95	296\\
96	296\\
97	296\\
98	296\\
99	296\\
100	296\\
};
\addlegendentry{muscle, c = 0.3 s}


\addplot[area legend, draw=none, fill=black, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
1	1498.05094529742\\
2	1214.35009872221\\
3	1145.51915748188\\
4	1118.64337155315\\
5	874.71572301602\\
6	830.576879788365\\
7	766.038826156864\\
8	696.350458924902\\
9	696.350458924902\\
10	696.350458924902\\
11	623.557388428784\\
12	611.311255150693\\
13	611.311255150693\\
14	582.856230382506\\
15	547.512112726505\\
16	530.864362153688\\
17	530.864362153688\\
18	507.27889957147\\
19	526.219556409676\\
20	521.516055212499\\
21	529.461445720384\\
22	458.141731759516\\
23	458.141731759516\\
24	458.141731759516\\
25	449.886625389564\\
26	449.886625389564\\
27	449.886625389564\\
28	404.647497443819\\
29	386.787132384481\\
30	386.787132384481\\
31	377.923661677957\\
32	360.832179175351\\
33	360.832179175351\\
34	370.638960745341\\
35	353.433654685331\\
36	341.300187859\\
37	335.345895865153\\
38	335.345895865153\\
39	335.345895865153\\
40	335.135248222193\\
41	333.375132621378\\
42	333.739400114845\\
43	333.516817608427\\
44	329.560727879387\\
45	329.560727879387\\
46	329.560727879387\\
47	328.633568345932\\
48	328.866228343787\\
49	328.131674837868\\
50	325.684231955982\\
51	324.839372170797\\
52	320.731768368955\\
53	312.609564361849\\
54	311.334382687996\\
55	311.247880592564\\
56	309.358350692126\\
57	308.668902158726\\
58	308.668902158726\\
59	301.117143936196\\
60	302.180508729516\\
61	302.180508729516\\
62	298.625861668982\\
63	292.22533290062\\
64	291.313677576803\\
65	290.862178523449\\
66	289.292807881383\\
67	288.930884266898\\
68	288.32934003852\\
69	286.869467948533\\
70	286.869467948533\\
71	285.891094198332\\
72	282.992620322039\\
73	281.33648460868\\
74	280.728735008823\\
75	279.905456552405\\
76	279.905456552405\\
77	279.091757268986\\
78	278.901989173222\\
79	278.571574814409\\
80	278.176435713633\\
81	278.017380321934\\
82	277.779740926173\\
83	277.532913835529\\
84	277.532913835529\\
85	275.647222649881\\
86	275.583320540518\\
87	275.583320540518\\
88	275.098924711342\\
89	274.863814028613\\
90	271.828680778286\\
91	271.485639489282\\
92	271.333996922417\\
93	271.119915153225\\
94	270.996036428187\\
95	270.810254514992\\
96	270.381509270471\\
97	269.155610842265\\
98	268.938687070837\\
99	268.691922814389\\
100	268.509782751765\\
100	372.45837777393\\
99	372.526014377513\\
98	372.639067852759\\
97	372.691402149358\\
96	373.089514735505\\
95	373.284330416406\\
94	373.316786683258\\
93	373.338612079089\\
92	373.403104036463\\
91	373.436080045185\\
90	373.506485696184\\
89	374.707959009851\\
88	374.815733514635\\
87	375.010405330664\\
86	375.010405330664\\
85	375.03241709136\\
84	375.612577141572\\
83	375.612577141572\\
82	375.653908470556\\
81	375.739372483965\\
80	375.807981627215\\
79	375.876938847724\\
78	376.023912147237\\
77	376.0567952796\\
76	376.210069963413\\
75	376.210069963413\\
74	376.628654131276\\
73	376.78258387363\\
72	377.764224332313\\
71	379.385568592393\\
70	380.178170854396\\
69	380.178170854396\\
68	380.605878849402\\
67	380.734361212301\\
66	380.964449050384\\
65	381.248756040525\\
64	381.3061448209\\
63	381.633107417226\\
62	385.881506777823\\
61	390.25562044368\\
60	390.25562044368\\
59	394.063500188933\\
58	401.71794861804\\
57	401.71794861804\\
56	401.72165473308\\
55	402.268217779895\\
54	402.435296392506\\
53	404.497287000124\\
52	404.535062972796\\
51	410.060665403657\\
50	409.935144130293\\
49	413.539233305087\\
48	413.442853497217\\
47	430.128055525856\\
46	431.923611686079\\
45	431.923611686079\\
44	431.923611686079\\
43	458.723353273345\\
42	458.728131298335\\
41	494.921816304398\\
40	495.680793099078\\
39	495.69412751764\\
38	495.69412751764\\
37	495.69412751764\\
36	501.196070885682\\
35	502.633551828944\\
34	530.783756680897\\
33	590.60782930531\\
32	590.60782930531\\
31	590.030559368808\\
30	590.477670427861\\
29	590.477670427861\\
28	598.117221499888\\
27	597.430904688871\\
26	597.430904688871\\
25	597.430904688871\\
24	617.659792926435\\
23	617.659792926435\\
22	617.659792926435\\
21	632.306495621812\\
20	838.69253700014\\
19	838.461400716763\\
18	911.900228504086\\
17	919.050552911668\\
16	919.050552911668\\
15	918.813694483435\\
14	987.76819912001\\
13	987.196182813881\\
12	987.196182813881\\
11	990.306076542363\\
10	1014.35772899563\\
9	1014.35772899563\\
8	1014.35772899563\\
7	1067.92332719677\\
6	1052.26605174906\\
5	1518.81879077377\\
4	2241.96667635445\\
3	2267.3193322816\\
2	2311.16263355232\\
1	5162.89552734169\\
}--cycle;
\addplot [color=black]
  table[row sep=crcr]{%
1	3330\\
2	1763\\
3	1706\\
4	1680\\
5	1197\\
6	941\\
7	917\\
8	855\\
9	855\\
10	855\\
11	807\\
12	799\\
13	799\\
14	785\\
15	733\\
16	725\\
17	725\\
18	710\\
19	682\\
20	680\\
21	581\\
22	538\\
23	538\\
24	538\\
25	524\\
26	524\\
27	524\\
28	501\\
29	489\\
30	489\\
31	484\\
32	476\\
33	476\\
34	451\\
35	428\\
36	421\\
37	416\\
38	416\\
39	416\\
40	415\\
41	414\\
42	396\\
43	396\\
44	381\\
45	381\\
46	381\\
47	379\\
48	371\\
49	371\\
50	368\\
51	367\\
52	363\\
53	359\\
54	357\\
55	357\\
56	356\\
57	355\\
58	355\\
59	348\\
60	346\\
61	346\\
62	342\\
63	337\\
64	336\\
65	336\\
66	335\\
67	335\\
68	334\\
69	334\\
70	334\\
71	333\\
72	330\\
73	329\\
74	329\\
75	328\\
76	328\\
77	328\\
78	327\\
79	327\\
80	327\\
81	327\\
82	327\\
83	327\\
84	327\\
85	325\\
86	325\\
87	325\\
88	325\\
89	325\\
90	323\\
91	322\\
92	322\\
93	322\\
94	322\\
95	322\\
96	322\\
97	321\\
98	321\\
99	321\\
100	320\\
};
\addlegendentry{torque, pd}

\end{axis}

